Dissecting Chain-of-Thought: Compositionality through In-Context Filtering and Learning

Chain-of-thought (CoT) is a method that enables language models to handle complex reasoning tasks by decomposing them into simpler steps. Despite its success, the underlying mechanics of CoT are not yet fully understood. In an attempt to shed light on this, our study investigates the impact of CoT on the ability of transformers to in-context learn a simple to study, yet general family of compositional functions: multi-layer perceptrons (MLPs). In this setting, we find that the success of CoT can be attributed to breaking down in-context learning of a compositional function into two distinct phases: focusing on and filtering data related to each step of the composition and in-context learning the single-step composition function. Through both experimental and theoretical evidence, we demonstrate how CoT significantly reduces the sample complexity of in-context learning (ICL) and facilitates the learning of complex functions that non-CoT methods struggle with. Furthermore, we illustrate how transformers can transition from vanilla in-context learning to mastering a compositional function with CoT by simply incorporating additional layers that perform the necessary data-filtering for CoT via the attention mechanism. In addition to these test-time benefits, we show CoT helps accelerate pretraining by learning shortcuts to represent complex functions and filtering plays an important role in this process. These findings collectively provide insights into the mechanics of CoT, inviting further investigation of its role in complex reasoning tasks.

==> app/app_filter.tex <==
\section{Filtering lemma}
% \begin{lemma}
% Let $\X=[\x_1~\x_2~\dots~\x_n]^\top\in\R^{n\times d}$ be a prompt and assume inputs are embedded into $K$ orthogonal subspaces. Specifically, let $\bar\x:=\embd(\x,k)\in\R^p$ be the embedded vector corresponding to the subspace $k$, where $p$ is the embedding dimension. Assume the column vectors of $\W_K,\W_Q\in\R^{p\times m}$ lie in subspace $k$, then we have that $\attn(\X)=\sfm(\bar\X\W_Q\W_K^\top\bar\X^\top)\bar\X\V=\filter(\X,k)\bar\X\V$, where $\filter(\X,k)$

% Let $\bar\x:=\embd(\x)$ be the embedding vector corresponding to its specific space. Then if choosing $\W=\left[\begin{array}{cc}
%     \zero & \zero \\
%     \zero & \infty\cdot\Iden_k
% \end{array}\right]$, we have that $\attn(\x_n)=\sfm(\bar\x_n\W\bar\X^\top)\bar\X\V=\filter(\X,k)\bar\X\V$, where $\filter(\X,k)=\frac{\eb_n^\top\Eb}{\sum_{i=1}^n\eb_n^\top\eb_i}$.

% \end{lemma}
\begin{lemma}
Let $\X=[\x_1~\x_2~\dots~\x_n]^\top\in\R^{n\times d}$ be a prompt and assume inputs are embedded into $K$ orthogonal subspaces. Specifically, let $\eb^{(1)},\cdots,\eb^{(K)}\in\R^K$ be orthonormal vectors and assume $\x$ is assigned to subspace $k$, then $\embd(\x)=[\x~\eb^{(k)}]^\top$. Let $\bar\x:=\embd(\x)$ be the embedding vector corresponding to its specific space. Then if choosing $\W=\left[\begin{array}{cc}
    \zero & \zero \\
    \zero & \infty\cdot\red{\Iden_k}
\end{array}\right]$ (or any positive symmetric matrices), we have that $\attn(\x_n)=\sfm(\bar\x_n\W\bar\X^\top)\bar\X\V=\filter(\X,k)\bar\X\V$, where $\filter(\X,k)=\frac{\eb_n^\top\Eb}{\sum_{i=1}^n\eb_n^\top\eb_i}$.
% \[
% \filter(\X,k)=[\delta_1~\dots~\delta_n]~~\text{and}~~\delta_i=\begin{cases}
%     1, & \x_i~\text{is assigned to subspace $k$} \\
%     0, & \text{otherwise}.
% \end{cases}
% \]
% \[
% \filter(\X,k)=\frac{\eb_n^\top\Eb}{\sum_{i=1}^n\eb_n^\top\eb_i}
% \]

\end{lemma}
\AG{This lemma will give you a weighted average of the ones that have the same skill. I mean that assume that $k=5$, $n=6$ and we have $e_n = e^3$ and $E =[e^1,e^3, e^5, e^3,e^3, e^2]$. Then we have
\begin{align} \attn(\x_n)&=\sfm(\bar\x_n\W\bar\X^\top)\bar\X\V=\filter(\X,k)\bar\X\V\\
&= \sfm(C\begin{bmatrix}e^3e^{1,\top}\\
e^3e^{3,\top}\\
e^3e^{5,\top}\\
e^3e^{3,\top}\\
e^3e^{3,\top}\\
e^3e^{2,\top}
\end{bmatrix})\bar\X
\\
&= \begin{bmatrix}
    0\\
    1/3\\
    0\\
    1/3\\
    1/3\\
    0
\end{bmatrix}\bar\X
\end{align}
This will not perform filtering, this will give just a weighted average of the inputs with the same skill. }
\begin{proof}
                   
    Consider a scenario where inputs are embedded into different orthogonal subspaces. Specifically, let $\z=[\x~\eb]^\top$ be an embedding vector where $\eb\in\Ec:=\{\eb^1,\eb^2\dots,\eb^k:\eb^i~\text{are orthonormal vectors},\eb^i\in\R^k\}$. Let $\Zb=[\z_1~\z_2~\dots~\z_n]^\top\in\R^{n\times (d+k)}$, $\X=[\x_1~\x_2~\dots~\x_n]^\top\in\R^{n\times d}$ and $\Eb=[\eb_1~\eb_2~\dots~\eb_n]^\top\in\R^{n\times k}$. Then we have 
\begin{align*}
    \attn(\x,\eb)=\sfm(\z\W\Zb^\top)\X\V.
\end{align*}
where $\W\in\R^{(d+k)\times(d+k)}$. Consider a special case where 
\[
\W=\left[\begin{array}{cc}
    0 & 0 \\
    0 & C\cdot\Iden_{k}
\end{array}\right],
\]
then we have that 
\[
\attn(\x,\eb)=\sfm(C\cdot\eb\Eb^\top)\X\V.
\]
\end{proof}

\begin{lemma}[Informal, see Appendix X]
    Assume that the input to a transformer after the embedding layer is of the following form 
    \begin{equation}
        \X = \begin{bmatrix}
            \x_1&\x_2&\hdots &\x_{n-1}&\x_n\\
            \emb_{1}&\emb_{2}&\hdots &\emb_{{n-1}} &\emb_{n}\\
            \s_{f_1}&\s_{f_2}&\hdots &\s_{f_{n-1}} &{\s_{f_n}}
        \end{bmatrix}
    \end{equation}
    where $\x_i\in\R^{d'}$, $\emb_i\in\R^{d''}$, $i\in[n]$ are the input and position encodings and  $\s_{f_i}\in\{\s_1,\cdots,\s_K\}$ is the encoding of the skills. Define the ideal filtering
    \begin{align}
    \X^{\text{filter}}_k[t]=\begin{cases}\X[t]\quad\text{if}\quad \s_{f_t}=\s_k\\0\quad\text{else}\end{cases}.
    \end{align}
    Then for each skill $k$, there exists a single-head attention layer such that, the layer output $\attn(\X)$ satisfies 
    \begin{align}
        \tn{\attn(\X)[t]-\X^{\text{filter}}[t]} \leq\eps\quad\text{for all}\quad t\in[n].
        %&= \begin{bmatrix}\zero&\x_i&\hdots &\x_j&\eps\\\zero&\emb_{i}&\hdots &\emb_{j} &\eps\\\zero&\s_{k}&\hdots &\s_k &\eps
        %\end{bmatrix},
        \end{align}
    where $\eps=\frac{1}{n_k}$ and $n_k$ is the number of inputs assigned with $\s_k$ and $\sum_{k=1}^Kn_k=n$.
\end{lemma}
\begin{proof}
Notice that the dimension of the embedding is $d = d' + d''+ e $, where $e$ is the dimension of the positional encodings that the model has chosen. Let
    \begin{equation}
        \W_\key = \begin{bmatrix}
            \zero & \Iden_{d''} & \zero\\
            \zero & \zero & \s_k^\top
        \end{bmatrix},\W_\query = \begin{bmatrix}
            \zero & \Iden_{d''} & \zero\\
            \zero & \zero & \one_e^\top
        \end{bmatrix}
    \end{equation}
    we have that 
   \renewcommand{\arraystretch}{1.5}
    \begin{align}
    \arraycolsep=0.1pt
        \sfm((\W_\key\X)^\top(\W_\query\X)) &= \sfm\left(\begin{bmatrix}
            \emb_1^\top &\s_k^\top\s_{f_1}\\
            \vdots &\vdots \\
            \emb_n^\top &\s_k^\top\s_{f_n} \\
        \end{bmatrix}\begin{bmatrix}
            \emb_1 & \hdots &\emb_n\\
            1 & \hdots & 1 \\
        \end{bmatrix}\right)\\
        &= \sfm\left(\begin{bmatrix}
            \emb_1^\top\emb_1+\s_k^\top\s_{f_1}&\hdots &\emb_1^\top\emb_n+\s_k^\top\s_{f_1}\\
            \vdots &\hdots &\vdots \\
            \emb_n^\top\emb_1+\s_k^\top\s_{f_n}&\hdots &\emb_n^\top\emb_n+\s_k^\top\s_{f_n}
        \end{bmatrix}\right)\\
        &= \begin{bmatrix}
            \dfrac{ \exp(\emb_1^\top\emb_1+\s_k^\top\s_{f_1})} {\sum_{j=1}^n\exp( \emb_1^\top\emb_j+\s_k^\top\s_{f_1})}&\hdots &\dfrac{ \exp(\emb_1^\top\emb_n+\s_k^\top\s_{f_1})} {\sum_{j=1}^n\exp( \emb_1^\top\emb_j+\s_k^\top\s_{f_1})}\\
            \vdots &\hdots &\vdots \\
             \dfrac{ \exp(\emb_n^\top\emb_1+\s_k^\top\s_{f_n})} {\sum_{j=1}^n\exp( \emb_n^\top\emb_j+\s_k^\top\s_{f_n})}&\hdots &\dfrac{ \exp(\emb_n^\top\emb_n+\s_k^\top\s_{f_n})} {\sum_{j=1}^n\exp( \emb_n^\top\emb_j+\s_k^\top\s_{f_n})}
        \end{bmatrix}
    \end{align}
    Then letting $\emb_i^\top\emb_i=\s_k^\top\s_k\to\infty$ and $\W_\val=\Iden_d$, the output of the attention becomes
    \begin{align}
        \attn(\X) &= \begin{bmatrix}
            \eps&\x_i&\hdots &\x_j&\eps\\
            \eps&\emb_{i}&\hdots &\emb_{j} &\eps\\
            \eps&\s_{k}&\hdots &\s_k &\eps
        \end{bmatrix},
        \end{align}
    where $\eps=\frac{1}{n_k}$.
\end{proof}

==> app/app_hetero.tex <==
% \section{Unordered Deep Linear MLPs}
\section{Unordered CoT Prompt}
In Section~\ref{sec:deep nn} we presented experimental evidence illustrating that CoT can perform compositional learning and filtering. We also provided theoretical explanation in Section~\ref{sec:theory} and Appendix~\ref{ss:filtering}. In this section, we explore a more heterogeneous CoT setting where intermediate steps are not ordered provided. To start with, let us first introduce unordered CoT prompt. 

\subsection{Problem Setup}
\textbf{Unordered CoT prompt.} Recall from Section~\ref{subsec cot}, and we say that the CoT prompt defined in \eqref{cot pmt} is ordered (since step messages ($\tb^0,\tb^1,\cdots,\tb^{L}$) are given fully and ordered). Now let $\tb^0\to\tb^1\cdots\to\tb^{L}$ define a complete chain of an $L$-step problem. (Ordered) CoT prompt requires that the ordered and whole chain is provided as in-context examples in the prompts. 


.  However, in real world applications, examples contained in the prompt may not provide the whole and precise messages. Therefore we ask: \emph{can transformer learn to solve a complex problem without given the complete step message}. Specifically, the in-context example of unordered CoT prompt has the following form:
\begin{align}
\text{ordered: }(\tb^0,\tb^1,\cdots\tb^{L-1},\tb^L)\longrightarrow\text{unordered: }(\tb^{\ell_{\text{start}}}\cdots\tb^{\ell_{\text{end}}})\label{heter cot pmt}
\end{align}
where $0\leq\ell_{\text{start}}<\ell_{\text{end}}\leq L$. We emphasize that $\ell_{\text{start}}$ and $\ell_{\text{end}}$ are arbitrary for any example within any prompt, and then if given a new input $\x$, same $L$-step procedure is applied. 

the example contained in CoT prompt is no longer as \eqref{cot pmt} with contains $L+1$ tokens but can be any example from length $2$ to $L+1$, that is


are expecting that even the whole chain is not provided in the prompt, $\TF$ can still complete the chain automatically by identifying the token space. Recall that $\tb^0=\x$ and $\tb^L=\y$, then an heterogeneous CoT example is no longer as \eqref{cot pmt} with $L+1$ tokens but can be any example from length $2$ to $L+1$, that is
\begin{align}
\text{ordered: }(\tb^0,\tb^1,\cdots\tb^{L-1},\tb^L)\longrightarrow\text{unordered: }(\tb^{\ell_{\text{start}}}\cdots\tb^{\ell_{\text{end}}}).\label{heter cot pmt}
\end{align}
where $0\leq\ell_{\text{start}}<\ell_{\text{end}}\leq L$. We emphasize that $\ell_{\text{start}}$ and $\ell_{\text{end}}$ are arbitrary for any example within any prompt, and then if given a new input $\x$, same $L$-step procedure is applied. 

\textbf{Model training and evaluation.} 
\begin{align*}
\hat\bt=\arg\min_{\bt}\E_{(\x_n)_{n=1}^N,(f_\ell)_{\ell=1}^L}\left[\frac{1}{N}\sum_{n=1}^N\frac{1}{\elle[n]-\ells[n]}\sum_{\ell=\ells[n]}^{\elle[n]}\ell(\hat\tb_n^\ell,\tb_{n}^\ell)\right]\\
\text{where}~~\hat\tb_n^\ell=\TF(\pmt^{\text{u}}_n(f),\tb^{\ells}_n\cdots\tb_n^{\ell-1})\\
~~\pmt^{\text{u}}_n(f)=
\end{align*}


\subsection{Experimental Results}

\textbf{Dataset.} 

\textbf{Emergent ability of CoT. }

==> backup/app/app_add_exp.tex <==
\section{Additional Experimental Results}

\input{fig_sec/app_fig_one_layer}
\subsection{Filtering Evidence in 2-layer MLPs}\label{sec:2nn filter}
Section~\ref{sec:deep nn} has demonstrated the occurrence of filtering in the linear deep MLPs setting (black dotted curves in Fig.~\ref{fig:each layer 50k}). In this section, we present further empirical evidence based on the 2-layer MLPs setting discussed in Section~\ref{sec:2nn}.

Follow the same setting as Figure~\ref{fig:cot_d10_vs_d20} and choose $d=10$ and $k=8$. Assume we have a model pretrained using $\COT$ method. As described in Section~\ref{sec:2nn}, during training, the prompt consists of in-context samples in the form of $(\x,\tb,y)$ where $\tb=(\W\x)_+$ and $y=\vv^\top \tb$. To investigate filtering, we make three different predictions to evaluate the intermediate output, whose test prompts have in-context examples with the following forms:
\[
\text{CoT: }(\x,\tb,y),~~~~\text{CoT-zero: }(\x,\tb,0),~~~~\text{CoT-random: }(\x,\tb,z),
\]
where $z\sim\Nc(0,d)$. The results are displayed in Figure~\ref{fig:2nn filter} where blue, orange and green curves represent first layer prediction results using CoT, CoT-zero and CoT-random prompts, respectively. From this figure, we observe that the three curves are well aligned, indicating that when making a prediction for input $\x$, $\TF$ will attend only to $(\x,\tb)$ and ignore $y$. Therefore filling the positions of $y$ with any random values (or zero) will not change the performance of first layer prediction.  

\subsection{Comparison of Filtered CoT with ICL}
Until now, many experimental results have shown that $\COT$ provides benefits in terms of sample complexity and model expressivity compared to $\ICL$. As an interpretation, we state that CoT can be decoupled into two phases: \emph{Filtering} and \emph{ICL}, and theoretical results have been provided to prove this statement. As for the empirical evidence, Sections~\ref{sec:deep nn} and \ref{sec:2nn filter} precisely show that filtering does occur in practice. In this section, we provide additional experiments to demonstrate that, after filtering, CoT performs similarly to ICL.

For convenience and easier comparison, we repeat the same results as Fig.~\ref{fig:cot_d10_vs_d20} in Fig.~\ref{fig:cot composed}, where $d\in\{10,20\}$, $k\in\{4,8,16\}$, and train with a small GPT-2. We again recap the data setting for the 2-layer MLP, where the in-context examples of CoT prompt are in the form of $(\x,\tb,y)$. Given that filtering happens, we make first and second layer predictions following Section~\ref{sec:emp} and results are presented in Fig.~\ref{fig:cot first} and Fig.~\ref{fig:cot second}, respectively. These results show the performances of the filtered CoT prompts. Next, we need to compare the performance with separate ICL training. To achieve this goal, we train a small GPT-2 model using $\ICL$ method with prompt containing $(\x,\tb)$ pairs (first layer). The test results are shown in Fig.~\ref{fig:icl first}. Additionally, in Fig.~\ref{fig:icl second}, we train another small GPT-2 model using ICL but with prompts containing $(\tb,y)$ pairs (second layer). By comparing Fig.~\ref{fig:cot first} and \ref{fig:icl first}, as well as Fig.~\ref{fig:cot second} and \ref{fig:icl second}, we observe that after filtering, $\COT$ achieves similar performance as individually training a single-step problem through the ICL phase. 

\input{fig_sec/app_fig_diff_gpt}
\subsection{CoT across Different Sizes of GPT-2}
In Figure~\ref{fig:diff gpt}, we have demonstrated that larger models help in improving performance due to their ability of solving more complex function sets. However, since tiny, small and standard GPT-2 models scale the layer number, head number and embedding dimension simultaneously, it is difficult to determine which component has the greatest impact on performance. Therefore in this section, we  investigate how different components of transformer model affect the resulting performance by run $\COT$ on various GPT-2 architectures.

We maintain the same setting as in Section~\ref{sec:2nn}, fix $d=10$ and $k=8$, and consider a base GPT-2 model (small GPT-2) with $6$ attention layers, $4$ heads in each layer and $128$-dimensional embeddings. In Fig.~\ref{fig:diff layer}, we fix the number of heads at $4$ and the embedding dimension at $128$, while varying the number of layers in $\{3,6,12\}$. Similarly, we explore different models with different numbers of heads and embedding dimensions, and the results are respectively presented in Fig.~\ref{fig:diff head} and \ref{fig:diff embed}. Comparing them, we can observe the following: 1) once the problem is sufficiently solved, increasing the model size does not significantly improve the prediction performance (see Fig.~\ref{fig:diff head}\&\ref{fig:diff embed}); 2) the number of layers influences model expressivity, particularly for small GPT-2 architecture (see Fig.~\ref{fig:diff layer}).  


\input{fig_sec/app_fig_regression}
\subsection{Comparison of Transformer Prediction and Linear Regression}
We also provide experimental findings to verify Assumption~\ref{assume oracle} in this section. Previous work \citep{giannou2023looped,akyurek2022learning} has theoretically proven that $\TF$ can perform similar to gradient descent, and empirical evidence from \citep{dai2022can, garg2022can, li2023transformers} suggests that $\TF$ can even be competitive with Bayes optimizer in certain scenario. To this end, we first repeat the same first/layer predictions from Figure~\ref{fig:largek} in Figure~\ref{fig:linear regression}, where $d=10$ and blue, orange and green solid curves represent the performances of $k=4,16,64$ using pretrained small GPT-2 models. We also display the evaluations of gradient descent/least square solutions in dashed curves. Specifically, in Fig.~\ref{fig:relu gd} , we solve problem 
\[
\hat\w_n=\arg\min_{\w}\frac{1}{n}\sum_{i=1}^n\|(\w^\top\x_i)_+-y_i\|^2~~\text{where}~~\x_i\sim\Nc(0,\Iden_d),~y_i=({\w^\st}^\top\x_i)_+
\]
for some $\w^\st\sim\Nc(0,2\Iden_d)$ and $n$ is the training sample size. Then the normalized test risks are computed by $\Lc(n)=\E_{\w^\st,\x}[\|(\hat\w_n^\top\x)_+-y\|^2]/d$, and we show point-to-point results for $n\in[N]$ in black dashed curve in Fig.~\ref{fig:relu gd}\footnote{To mitigate the bias introduced by ReLU activation, we subtract the mean value during prediction, \ie $\Lc(n)=\E_{\w^\st,\x}[\|(\hat\w_n^\top\x)_+-y-(\E_{\x}[(\hat\w_n^\top\x)_+-y])\|^2]/d$. }. As for the second layer, we solve least squares problems as follows
\[
\hat\vv_n=\Sb^\dagger\y~~\text{where}~~\Sb\in\R^{n\times k},~\Sb[i]=(\W^\st\x_i)_+,~ \y[i]={\vv^\st}^\top\Sb[i],~\x_i\in\Nc(0,\Iden_d)
\]
for some $\W^\st\in\R^{k\times d}\sim\Nc(0,2/k)$ and $\vv^\st\sim\Nc(0,\Iden_k)$. Here, $^\dagger$ represents the pseudo-inverse operator. Then we calculate the normalized test risk of least square solution (given $n$ training samples) as $\Lc(n)=\E_{\W^\st,\vv^\st,\x}[\|\hat\vv_n^\top\tb-y\|^2]/d$ where $\tb=(\W^\st\x)_+$ and $y={\vv^\st}^\top\tb$. The results are presented in Fig.~\ref{fig:linear ls} where blue, orange and green dashed curves correspond to solving the problem using different values of $k\in\{4,16,64\}$. In this figure, the curves for $k=4,16$ are aligned with GPT-2 risk curves, which indicates that $\TF$ can efficiently solve linear regression as a least squares optimizer. However, the curve for $k=64$ does not align, which can be attributed to the increased complexity of the function set with higher dimensionality ($k=64$). Learning such complex functions requires a larger $\TF$ model. 

==> backup/app/app_filter.tex <==
\section{Filtering lemma}
% \begin{lemma}
% Let $\X=[\x_1~\x_2~\dots~\x_n]^\top\in\R^{n\times d}$ be a prompt and assume inputs are embedded into $K$ orthogonal subspaces. Specifically, let $\bar\x:=\embd(\x,k)\in\R^p$ be the embedded vector corresponding to the subspace $k$, where $p$ is the embedding dimension. Assume the column vectors of $\W_K,\W_Q\in\R^{p\times m}$ lie in subspace $k$, then we have that $\attn(\X)=\sfm(\bar\X\W_Q\W_K^\top\bar\X^\top)\bar\X\V=\filter(\X,k)\bar\X\V$, where $\filter(\X,k)$

% Let $\bar\x:=\embd(\x)$ be the embedding vector corresponding to its specific space. Then if choosing $\W=\left[\begin{array}{cc}
%     \zero & \zero \\
%     \zero & \infty\cdot\Iden_k
% \end{array}\right]$, we have that $\attn(\x_n)=\sfm(\bar\x_n\W\bar\X^\top)\bar\X\V=\filter(\X,k)\bar\X\V$, where $\filter(\X,k)=\frac{\eb_n^\top\Eb}{\sum_{i=1}^n\eb_n^\top\eb_i}$.

% \end{lemma}
\begin{lemma}
Let $\X=[\x_1~\x_2~\dots~\x_n]^\top\in\R^{n\times d}$ be a prompt and assume inputs are embedded into $K$ orthogonal subspaces. Specifically, let $\eb^{(1)},\cdots,\eb^{(K)}\in\R^K$ be orthonormal vectors and assume $\x$ is assigned to subspace $k$, then $\embd(\x)=[\x~\eb^{(k)}]^\top$. Let $\bar\x:=\embd(\x)$ be the embedding vector corresponding to its specific space. Then if choosing $\W=\left[\begin{array}{cc}
    \zero & \zero \\
    \zero & \infty\cdot\red{\Iden_k}
\end{array}\right]$ (or any positive symmetric matrices), we have that $\attn(\x_n)=\sfm(\bar\x_n\W\bar\X^\top)\bar\X\V=\filter(\X,k)\bar\X\V$, where $\filter(\X,k)=\frac{\eb_n^\top\Eb}{\sum_{i=1}^n\eb_n^\top\eb_i}$.
% \[
% \filter(\X,k)=[\delta_1~\dots~\delta_n]~~\text{and}~~\delta_i=\begin{cases}
%     1, & \x_i~\text{is assigned to subspace $k$} \\
%     0, & \text{otherwise}.
% \end{cases}
% \]
% \[
% \filter(\X,k)=\frac{\eb_n^\top\Eb}{\sum_{i=1}^n\eb_n^\top\eb_i}
% \]

\end{lemma}
\AG{This lemma will give you a weighted average of the ones that have the same skill. I mean that assume that $k=5$, $n=6$ and we have $e_n = e^3$ and $E =[e^1,e^3, e^5, e^3,e^3, e^2]$. Then we have
\begin{align} \attn(\x_n)&=\sfm(\bar\x_n\W\bar\X^\top)\bar\X\V=\filter(\X,k)\bar\X\V\\
&= \sfm(C\begin{bmatrix}e^3e^{1,\top}\\
e^3e^{3,\top}\\
e^3e^{5,\top}\\
e^3e^{3,\top}\\
e^3e^{3,\top}\\
e^3e^{2,\top}
\end{bmatrix})\bar\X
\\
&= \begin{bmatrix}
    0\\
    1/3\\
    0\\
    1/3\\
    1/3\\
    0
\end{bmatrix}\bar\X
\end{align}
This will not perform filtering, this will give just a weighted average of the inputs with the same skill. }
\begin{proof}
                   
    Consider a scenario where inputs are embedded into different orthogonal subspaces. Specifically, let $\z=[\x~\eb]^\top$ be an embedding vector where $\eb\in\Ec:=\{\eb^1,\eb^2\dots,\eb^k:\eb^i~\text{are orthonormal vectors},\eb^i\in\R^k\}$. Let $\Zb=[\z_1~\z_2~\dots~\z_n]^\top\in\R^{n\times (d+k)}$, $\X=[\x_1~\x_2~\dots~\x_n]^\top\in\R^{n\times d}$ and $\Eb=[\eb_1~\eb_2~\dots~\eb_n]^\top\in\R^{n\times k}$. Then we have 
\begin{align*}
    \attn(\x,\eb)=\sfm(\z\W\Zb^\top)\X\V.
\end{align*}
where $\W\in\R^{(d+k)\times(d+k)}$. Consider a special case where 
\[
\W=\left[\begin{array}{cc}
    0 & 0 \\
    0 & C\cdot\Iden_{k}
\end{array}\right],
\]
then we have that 
\[
\attn(\x,\eb)=\sfm(C\cdot\eb\Eb^\top)\X\V.
\]
\end{proof}

\begin{lemma}[Informal, see Appendix X]
    Assume that the input to a transformer after the embedding layer is of the following form 
    \begin{equation}
        \X = \begin{bmatrix}
            \x_1&\x_2&\hdots &\x_{n-1}&\x_n\\
            \emb_{1}&\emb_{2}&\hdots &\emb_{{n-1}} &\emb_{n}\\
            \s_{f_1}&\s_{f_2}&\hdots &\s_{f_{n-1}} &{\s_{f_n}}
        \end{bmatrix}
    \end{equation}
    where $\x_i\in\R^{d'}$, $\emb_i\in\R^{d''}$, $i\in[n]$ are the input and position encodings and  $\s_{f_i}\in\{\s_1,\cdots,\s_K\}$ is the encoding of the skills. Define the ideal filtering
    \begin{align}
    \X^{\text{filter}}_k[t]=\begin{cases}\X[t]\quad\text{if}\quad \s_{f_t}=\s_k\\0\quad\text{else}\end{cases}.
    \end{align}
    Then for each skill $k$, there exists a single-head attention layer such that, the layer output $\attn(\X)$ satisfies 
    \begin{align}
        \tn{\attn(\X)[t]-\X^{\text{filter}}[t]} \leq\eps\quad\text{for all}\quad t\in[n].
        %&= \begin{bmatrix}\zero&\x_i&\hdots &\x_j&\eps\\\zero&\emb_{i}&\hdots &\emb_{j} &\eps\\\zero&\s_{k}&\hdots &\s_k &\eps
        %\end{bmatrix},
        \end{align}
    where $\eps=\frac{1}{n_k}$ and $n_k$ is the number of inputs assigned with $\s_k$ and $\sum_{k=1}^Kn_k=n$.
\end{lemma}
\begin{proof}
Notice that the dimension of the embedding is $d = d' + d''+ e $, where $e$ is the dimension of the positional encodings that the model has chosen. Let
    \begin{equation}
        \W_\key = \begin{bmatrix}
            \zero & \Iden_{d''} & \zero\\
            \zero & \zero & \s_k^\top
        \end{bmatrix},\W_\query = \begin{bmatrix}
            \zero & \Iden_{d''} & \zero\\
            \zero & \zero & \one_e^\top
        \end{bmatrix}
    \end{equation}
    we have that 
   \renewcommand{\arraystretch}{1.5}
    \begin{align}
    \arraycolsep=0.1pt
        \sfm((\W_\key\X)^\top(\W_\query\X)) &= \sfm\left(\begin{bmatrix}
            \emb_1^\top &\s_k^\top\s_{f_1}\\
            \vdots &\vdots \\
            \emb_n^\top &\s_k^\top\s_{f_n} \\
        \end{bmatrix}\begin{bmatrix}
            \emb_1 & \hdots &\emb_n\\
            1 & \hdots & 1 \\
        \end{bmatrix}\right)\\
        &= \sfm\left(\begin{bmatrix}
            \emb_1^\top\emb_1+\s_k^\top\s_{f_1}&\hdots &\emb_1^\top\emb_n+\s_k^\top\s_{f_1}\\
            \vdots &\hdots &\vdots \\
            \emb_n^\top\emb_1+\s_k^\top\s_{f_n}&\hdots &\emb_n^\top\emb_n+\s_k^\top\s_{f_n}
        \end{bmatrix}\right)\\
        &= \begin{bmatrix}
            \dfrac{ \exp(\emb_1^\top\emb_1+\s_k^\top\s_{f_1})} {\sum_{j=1}^n\exp( \emb_1^\top\emb_j+\s_k^\top\s_{f_1})}&\hdots &\dfrac{ \exp(\emb_1^\top\emb_n+\s_k^\top\s_{f_1})} {\sum_{j=1}^n\exp( \emb_1^\top\emb_j+\s_k^\top\s_{f_1})}\\
            \vdots &\hdots &\vdots \\
             \dfrac{ \exp(\emb_n^\top\emb_1+\s_k^\top\s_{f_n})} {\sum_{j=1}^n\exp( \emb_n^\top\emb_j+\s_k^\top\s_{f_n})}&\hdots &\dfrac{ \exp(\emb_n^\top\emb_n+\s_k^\top\s_{f_n})} {\sum_{j=1}^n\exp( \emb_n^\top\emb_j+\s_k^\top\s_{f_n})}
        \end{bmatrix}
    \end{align}
    Then letting $\emb_i^\top\emb_i=\s_k^\top\s_k\to\infty$ and $\W_\val=\Iden_d$, the output of the attention becomes
    \begin{align}
        \attn(\X) &= \begin{bmatrix}
            \eps&\x_i&\hdots &\x_j&\eps\\
            \eps&\emb_{i}&\hdots &\emb_{j} &\eps\\
            \eps&\s_{k}&\hdots &\s_k &\eps
        \end{bmatrix},
        \end{align}
    where $\eps=\frac{1}{n_k}$.
\end{proof}

==> backup/app/app_hetero.tex <==
% \section{Unordered Deep Linear MLPs}
\section{Unordered CoT Prompt}
In Section~\ref{sec:deep nn} we presented experimental evidence illustrating that CoT can perform compositional learning and filtering. We also provided theoretical explanation in Section~\ref{sec:theory} and Appendix~\ref{ss:filtering}. In this section, we explore a more heterogeneous CoT setting where intermediate steps are not ordered provided. To start with, let us first introduce unordered CoT prompt. 

\subsection{Problem Setup}
\textbf{Unordered CoT prompt.} Recall from Section~\ref{subsec cot}, and we say that the CoT prompt defined in \eqref{cot pmt} is ordered (since step messages ($\tb^0,\tb^1,\cdots,\tb^{L}$) are given fully and ordered). Now let $\tb^0\to\tb^1\cdots\to\tb^{L}$ define a complete chain of an $L$-step problem. (Ordered) CoT prompt requires that the ordered and whole chain is provided as in-context examples in the prompts. 


.  However, in real world applications, examples contained in the prompt may not provide the whole and precise messages. Therefore we ask: \emph{can transformer learn to solve a complex problem without given the complete step message}. Specifically, the in-context example of unordered CoT prompt has the following form:
\begin{align}
\text{ordered: }(\tb^0,\tb^1,\cdots\tb^{L-1},\tb^L)\longrightarrow\text{unordered: }(\tb^{\ell_{\text{start}}}\cdots\tb^{\ell_{\text{end}}})\label{heter cot pmt}
\end{align}
where $0\leq\ell_{\text{start}}<\ell_{\text{end}}\leq L$. We emphasize that $\ell_{\text{start}}$ and $\ell_{\text{end}}$ are arbitrary for any example within any prompt, and then if given a new input $\x$, same $L$-step procedure is applied. 

the example contained in CoT prompt is no longer as \eqref{cot pmt} with contains $L+1$ tokens but can be any example from length $2$ to $L+1$, that is


are expecting that even the whole chain is not provided in the prompt, $\TF$ can still complete the chain automatically by identifying the token space. Recall that $\tb^0=\x$ and $\tb^L=\y$, then an heterogeneous CoT example is no longer as \eqref{cot pmt} with $L+1$ tokens but can be any example from length $2$ to $L+1$, that is
\begin{align}
\text{ordered: }(\tb^0,\tb^1,\cdots\tb^{L-1},\tb^L)\longrightarrow\text{unordered: }(\tb^{\ell_{\text{start}}}\cdots\tb^{\ell_{\text{end}}}).\label{heter cot pmt}
\end{align}
where $0\leq\ell_{\text{start}}<\ell_{\text{end}}\leq L$. We emphasize that $\ell_{\text{start}}$ and $\ell_{\text{end}}$ are arbitrary for any example within any prompt, and then if given a new input $\x$, same $L$-step procedure is applied. 

\textbf{Model training and evaluation.} 
\begin{align*}
\hat\bt=\arg\min_{\bt}\E_{(\x_n)_{n=1}^N,(f_\ell)_{\ell=1}^L}\left[\frac{1}{N}\sum_{n=1}^N\frac{1}{\elle[n]-\ells[n]}\sum_{\ell=\ells[n]}^{\elle[n]}\ell(\hat\tb_n^\ell,\tb_{n}^\ell)\right]\\
\text{where}~~\hat\tb_n^\ell=\TF(\pmt^{\text{u}}_n(f),\tb^{\ells}_n\cdots\tb_n^{\ell-1})\\
~~\pmt^{\text{u}}_n(f)=
\end{align*}


\subsection{Experimental Results}

\textbf{Dataset.} 

\textbf{Emergent ability of CoT. }

==> backup/app/app_implement.tex <==
\section{Experimental Details}
In this section, we provide the implementation details of our experiments. 

\subsection{Model Evaluation} Recap the same setting as in Section~\ref{sec:train} and assume we have pretrained models with parameters $\hat\bt^{\EXP}$ and $\hat\bt^{\COT}$. Next we make predictions following Section~\ref{subsec cot}. Letting $\ell(\cdot,\cdot):\Yc\times\Yc\to\R$ be loss function, we can define test risks as follows.
\begin{align*}
    \Lc^{\EXP}(n)=\E_{(\x_i)_{i=1}^n,(f_\ell)_{\ell=1}^L}\left[\ell(\hat\y_n,f(\x_n))\right]~~\text{where}~~\hat\y_n=\TF(\pmt_n(f),\x_n;\hat\bt^{\EXP})
\end{align*}
and
\begin{align*}
    \Lc^{\COT}(n)=\E_{(\x_i)_{i=1}^n,(f_\ell)_{\ell=1}^L}\left[\ell(\hat\y_n,f(\x_n))\right]~~\text{where}~~\hat\y_n=\TF(\pmt_n(f),\x_n,\hat\tb^1\cdots,\hat\tb^{L-1};\hat\bt^{\COT}).
\end{align*}
Here, we use $\Lc(n)$ to define the test risk when given prompt with $n$ in-context samples. Then, results shown in Figures~\ref{fig:smallk}\&\ref{fig:largek}\&\ref{fig:diff gpt}\&\ref{fig:diff k}\&\ref{fig:d5} are test risks $\Lc(n)$ given $n\in[N]$. Following model training and evaluation, we can see that once loss function is the same for both training and predicting, $\EXP$ (as well as $\ICL$) accepts training risk $\Lc_{\text{\tiny train}}^{\EXP}=\frac{1}{N}\sum_{n=1}^N\Lc^{\EXP}(n)$. 

\subsection{Implementation} All the transformer experiments use the GPT-2 model \citep{radford2019language} and our codebase is based on prior works~\citep{garg2022can,wolf2019huggingface}. Specifically, the model is trained using the \texttt{Adam} optimizer with learning rate $0.0001$ and batch size $64$, and we train $500$k iterations in total for all $\ICL$, $\EXP$ and $\COT$ methods. Each iteration randomly samples inputs $\x$s and functions $f$s. We also apply curriculum learning over the prompt $n$ as \cite{garg2022can} did for 2-layer random MLPs (Sec.~\ref{sec:2nn}). For both training and testing, we use the squared error as the loss function, \ie $\ell(\hat\y,\y)=\|\hat\y-\y\|^2$ (or $\ell(\hat y,y)=(\hat y-y)^2$ for scalar).
% \begin{align*}
% \hat\bt^{\EXP}=\arg\min_{\bt}\E_{(\x_n)_{n=1}^N,(f_\ell)_{\ell=1}^L}\left[\frac{1}{N}\sum_{n=1}^N\ell(\hat\y_n,f(\x))\right]~~\text{where}~~\hat\y_n=\TF(\pmt_n(f),\x_n)%\label{erm cot i}
% \end{align*}
% and
% \begin{align*}
% \hat\bt^{\COT}=\arg\min_{\bt}\E_{(\x_n)_{n=1}^N,(f_\ell)_{\ell=1}^L}\left[\frac{1}{NL}\sum_{n=1}^N\sum_{\ell=1}^L\ell(\hat\tb_n^\ell,\tb_{n}^\ell)\right]~~\text{where}~~\hat\tb_n^\ell=\TF(\pmt_n(f),\x_n\cdots\tb_n^{\ell-1}). %\label{erm cot io}
% \end{align*}

==> backup/fig_sec/app_fig_diff_gpt.tex <==
\begin{figure}[!t]
\centering
\subfigure[Varying GPT-2 layers]{
    \includegraphics[height=.25\columnwidth]{fig_sec/figs/diff_layer.pdf}
    \label{fig:diff layer}
    \hspace{-1mm}
}
\subfigure[Varying GPT-2 heads]{
    \includegraphics[height=.25\columnwidth,trim={1.5cm 0 0 0},clip]{fig_sec/figs/diff_head.pdf}
    \label{fig:diff head}
    \hspace{-1mm}
}
\subfigure[Varying embedding dimensions]{
    \includegraphics[height=.25\columnwidth,trim={1.5cm 0 0 0},clip]{fig_sec/figs/diff_embed.pdf}
    \label{fig:diff embed}
    \hspace{-1mm}
}
\caption{To further investigate how model architectures impact the prediction performance, we fix the number of heads and embedding dimension in Fig.~\ref{fig:diff layer} and change the layer number in $\{3,6,12\}$. Similarly for Fig.~\ref{fig:diff head}\&\ref{fig:diff embed} but instead, change number of heads (in $\{2,4,8\}$) and embedding dimensions (in $\{64,128,256\}$). }
\label{fig:diff gpt comp}
\end{figure}

==> backup/fig_sec/app_fig_one_layer.tex <==
\begin{figure}[!t]
\centering
\subfigure[Test filtering on first layer prediction]{
    \includegraphics[height=.25\columnwidth]{fig_sec/figs/2nn_filter.pdf}
    \label{fig:2nn filter}
    \hspace{10mm}
}
\subfigure[$\COT$: composed risk (same as Fig.~\ref{fig:cot_d10_vs_d20}) ]{
    \includegraphics[height=.25\columnwidth]{fig_sec/figs/cot_composed.pdf}
    \label{fig:cot composed}
    \hspace{15mm}
}
\caption{Fig.~\ref{fig:2nn filter} presents a filtering evidence of 2-layer MLPs. Given a 2-layer MLP in-context example $(\x,\tb,y)$, CoT admits $(\x,\tb,y)$ as test sample; while test samples of CoT-zero and CoT-random are formed by $(\x,\tb,0)$ and $(\x,\tb,z)$ where $z\sim\Nc(0,d)$. Fig.~\ref{fig:cot composed} is directly cloned form Fig.~\ref{fig:cot_d10_vs_d20} with error bar for better comparison with results in Fig.~\ref{fig:cot vs icl}.}
% \label{fig:diff gpt comp}
\end{figure}

\begin{figure}[!t]
\centering
\subfigure[$\COT$: 1st layer prediction]{
    \includegraphics[height=.25\columnwidth]{fig_sec/figs/cot_first.pdf}
    \label{fig:cot first}
    \hspace{10mm}
}
\subfigure[Train $\ICL$ with $(\x,\tb)$ pairs]{
    \includegraphics[height=.25\columnwidth]{fig_sec/figs/icl_first.pdf}
    \label{fig:icl first}
    \hspace{10mm}
}
\subfigure[$\COT$: 2nd layer prediction]{
    \includegraphics[height=.25\columnwidth]{fig_sec/figs/cot_second.pdf}
    \label{fig:cot second}
    \hspace{10mm}
}
\subfigure[Train $\ICL$ with $(\tb,y)$ pairs]{
    \includegraphics[height=.25\columnwidth]{fig_sec/figs/icl_second.pdf}
    \label{fig:icl second}
    \hspace{10mm}
}
\caption{We compare the performance of filtered CoT and ICL. In Fig.~\ref{fig:cot first}\&\ref{fig:cot second}, we decouple the composed risk of predicting 2-layer MLPs into risks of individual layers (following Section~\ref{sec:emp}), which shows the filtered CoT results. In Fig.~\ref{fig:icl first}\&\ref{fig:icl second}, we train two additional models using ICL method taking $(\x,\tb)$ and $(\tb,y)$ as inputs.}
\label{fig:cot vs icl}
\end{figure}


==> backup/fig_sec/app_fig_regression.tex <==
\begin{figure}[!t]
\centering
\subfigure[1st layer: compare with GD solving ReLU]{
    \includegraphics[height=.25\columnwidth]{fig_sec/figs/regression_first.pdf}
    \label{fig:relu gd}
    \hspace{10mm}
}
\subfigure[2nd layer: compare with least squares]{
    \includegraphics[height=.25\columnwidth]{fig_sec/figs/regression_second.pdf}
    \label{fig:linear ls}
    \hspace{10mm}
}
\caption{Fig.~\ref{fig:relu gd}: compare transformer results (solid) with gradient descent optimizer (dashed) when solving first layer of 2-layer MLPs; Fig.~\ref{fig:linear ls}: compare transformer result (solid) with least squares optimizer (dashed) when solving the second layer of 2-layer MLPs.}
\label{fig:linear regression}
\end{figure}

==> backup/fig_sec/fig_50k_it.tex <==
\begin{figure}[!t]
\vspace{-15pt}
\centering
    \hspace{-3mm}
\subfigure[Composed risk]{
    \includegraphics[height=.25\columnwidth]{fig_sec/figs/composed_50k.pdf}
    \label{fig:composed 50k}
    \hspace{-3mm}
}
\subfigure[Risk of each layer output]{
    \includegraphics[height=.25\columnwidth]{fig_sec/figs/each_layer_50k_filter.pdf}
    \label{fig:each layer 50k}
    \hspace{-3mm}
}
\vspace{-2mm}
\caption{Fig.~\ref{fig:composed 50k} is generated by magnifying the initial 50k iterations of Fig.~\ref{fig:one shot}, and we decouple the composed risks from predicting $6$-layer linear MLPs into predictions for each layer, and the results are depicted in Fig.~\ref{fig:each layer 50k}. Additional implementation details can be found in Section~\ref{sec:deep nn}.}
\label{fig:long chain 50k}
\vspace{-10pt}
\end{figure}

==> backup/fig_sec/fig_cot.tex <==
\begin{figure}[!t]
\vspace{-20pt}
\centering
% \subfigure[$\ICL~vs~\EXP~vs~\COT$]{
%     \includegraphics[height=.25\columnwidth]{fig_sec/figs/k=16.pdf}
%     \label{fig:k16}
%     \hspace{-1mm}
% }
\subfigure[$\COT$: $d=10~vs~20$]{
    \includegraphics[height=.25\columnwidth,trim={1.5cm 0 0 0},clip]{fig_sec/figs/cot_d10_vs_d20.pdf}
    \label{fig:cot_d10_vs_d20}
    % \hspace{-1mm}
}
\subfigure[Alignment in Fig.~\ref{fig:cot_d10_vs_d20}]{
    \includegraphics[height=.25\columnwidth,trim={1.5cm 0 0 0},clip]{fig_sec/figs/cotk16_d10_vs_d20.pdf}
    \label{fig:cot_d10_vs_d20_align}
    % \hspace{-2mm}
}
\vspace{-2mm}
\caption{Solving 2-layer MLPs with varying input dimension $d$ and hidden neuron size $k$. }\label{fig:smallk}

\centering
\subfigure[$\COT$: composed risk ($d=10$)]{
    \includegraphics[height=.25\columnwidth]{fig_sec/figs/cot_d10_largek.pdf}
    \label{fig:largek compose}
    \hspace{-1mm}
}
\subfigure[Risk of first layer]{
    \includegraphics[height=.25\columnwidth,trim={1.5cm 0 0 0},clip]{fig_sec/figs/cot_d10_largek_first_layer.pdf}
    \label{fig:largek first}
    \hspace{-1mm}
}
\subfigure[Risk of second layer]{
    \includegraphics[height=.25\columnwidth,trim={1.5cm 0 0 0},clip]{fig_sec/figs/cot_d10_largek_second_layer.pdf}
    \label{fig:largek second}
    \hspace{-1mm}
}
\vspace{-2mm}
\caption{We decouple the composed risk of predicting 2-layer MLPs into risks of individual layers. }
\label{fig:largek}
\vspace{-10pt}
\end{figure}

==> backup/fig_sec/fig_diff_gpt.tex <==
\begin{figure}[!t]
\centering
\hspace{-20pt}
\subfigure[Averaged risk]{
    \includegraphics[height=.2\columnwidth]{fig_sec/figs/avg_risk_k8.pdf}
    \label{fig:avg risk model}
    \hspace{-3mm}
}
\subfigure[Standard GPT-2]{
    \includegraphics[height=.2\columnwidth]{fig_sec/figs/standard.pdf}
    \label{fig:gpt standard}
    \hspace{-3mm}
}
\subfigure[Small GPT-2]{
    \includegraphics[height=.2\columnwidth,trim={1.5cm 0 0 0},clip]{fig_sec/figs/small.pdf}
    \label{fig:gpt small}
    \hspace{-3mm}
}
\subfigure[Tiny GPT-2]{
    \includegraphics[height=.2\columnwidth,trim={1.5cm 0 0 0},clip]{fig_sec/figs/tiny.pdf}
    \label{fig:gpt tiny}
    \hspace{-3mm}
}
\vspace{-2mm}
\caption{Comparison of the three methods for solving $2$-layer MLPs using different GPT-2 models.}
\label{fig:diff gpt}
\vspace{-10pt}
\end{figure}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{fig_sec/figs/diff_gpt}
%     \caption{Compare the three methods with training $2$-layer neural nets with different GPT-2 models.}
%     \label{fig:diff gpt}
% \end{figure}

==> backup/fig_sec/fig_diff_k.tex <==
\begin{figure}[!t]
\centering
\hspace{-10mm}
\subfigure[Averaged risk]{
    \includegraphics[height=.2\columnwidth]{fig_sec/figs/avg_risk_small.pdf}
    \label{fig:avg risk k}
    \hspace{-3mm}
}
\subfigure[$k=4$]{
    \includegraphics[height=.2\columnwidth]{fig_sec/figs/k=4.pdf}
    \label{fig:k4}
    \hspace{-3mm}
}
\subfigure[$k=8$]{
    \includegraphics[height=.2\columnwidth,trim={1.5cm 0 0 0},clip]{fig_sec/figs/k=8.pdf}
    \label{fig:k8}
    \hspace{-3mm}
}
\subfigure[$k=16$]{
    \includegraphics[height=.2\columnwidth,trim={1.5cm 0 0 0},clip]{fig_sec/figs/k=16.pdf}
    \label{fig:k16}
    \hspace{-3mm}
}

\vspace{-2mm}
\caption{Comparison of the three methods for solving $2$-layer MLPs with different hidden sizes.}
\label{fig:diff k}
\vspace{-10pt}
\end{figure}

% \begin{figure}
%     \centering    \includegraphics[width=\linewidth]{fig_sec/figs/diff_k}
%     \caption{Compare the three methods when training $2$-layer neural nets with different hidden sizes.}
%     \label{fig:diff k}
% \end{figure}

==> backup/fig_sec/fig_intro.tex <==
% \begin{figure}[!t]
% \hspace{-10pt}
% \begin{minipage}[b]{0.5\textwidth}
% \centering
%     \includegraphics[width=\columnwidth]{fig_sec/figs/CoT_intro.png}
% \caption{$\COT$ mechanics.\red{[TO DO]}
% }\label{fig:intro}
% \end{minipage}
% \begin{minipage}[b]{0.5\textwidth}
% \centering
% % \setlength{\arrayrulewidth}{0.5mm}
% % \setlength{\tabcolsep}{2pt}
% \renewcommand{\arraystretch}{1.2}
% {\small{
%     \begin{tabular}{|l|ccc|}
%         \hline
%         Methods & $\ICL$ & $\EXP$ & $\COT$ \\
%         \hline
%         Step-by-step prompt & \ding{55} & \ding{51} & \ding{51}\\
%         Step-by-step prediction & \ding{55} & \ding{55} & \ding{51} \\
%         \hline
%     \end{tabular}}}
%     \captionof{table}{Data structure of $\ICL$, $\EXP$ and $\COT$.}
%     \label{tab:intro}
% \end{minipage}
% \end{figure}
\begin{figure}[!t]
\vspace{-20pt}
\centering
\begin{tikzpicture}
    % \centering
    \node at (0.15,-0.15){\includegraphics[width=0.9\columnwidth]{fig_sec/figs/CoT_intro.pdf}};

    % \node at (-3.8,2.45) {\textbf{\small Target 3-layer MLPs}};
    \node at (-5.9,2) {{\tiny Input: $\x$}};
    \node at (-5.9,1.4) {{\tiny 1st hidden: $\tb^1$}};
    \node at (-5.9,0.75) {{\tiny 2nd hidden: $\tb^2$}};
    \node at (-5.9,0.1) {{\tiny Output: $\y$}};

    % \node at (-3.8,-0.5) {\textbf{\small Performance curves}};

    \node at (-0.2,2.) {\textbf{\small $\ICL$}};
    \node at (-0.9,1.5) {{\tiny $\x_1$}};
    \node at (-0.6,1.5) {{\tiny $\y_1$}};
    \node at (-0.3,1.5) {{\tiny $\x_2$}};
    \node at (0.,1.5) {{\tiny $\y_2$}};
    \node at (0.3,1.5) {{\tiny \dots}};
    \node at (0.6,1.5) {{\tiny $\xtest$}};
    \node at (0.55,0.55) {{\tiny $\hat\y$}};

    \node at (-0.2,-0.9) {\textbf{\small $\EXP$}};
    \node at (-1.4,-1.4) {{\tiny $\x_1$}};
    \node at (-1.1,-1.39) {{\tiny $\tb^1_1$}};
    \node at (-0.8,-1.39) {{\tiny $\tb^2_1$}};
    \node at (-0.5,-1.4) {{\tiny $\y_1$}};
    \node at (-0.2,-1.4) {{\tiny $\x_2$}};
    \node at (0.1,-1.39) {{\tiny $\tb_2^1$}};
    \node at (0.6,-1.4) {{\tiny\dots}};
    \node at (1.1,-1.4) {{\tiny$\xtest$}};
    \node at (1,-2.35) {{\tiny $\hat\y$}};


    \node at (4,2.) {\textbf{\small $\COT$}};
    \node at (2.7,1.5) {{\tiny $\x_1$}};
    \node at (3,1.55) {{\tiny $\tb^1_1$}};
    \node at (3.3,1.55) {{\tiny $\tb^2_1$}};
    \node at (3.6,1.5) {{\tiny $\y_1$}};
    \node at (3.9,1.5) {{\tiny $\x_2$}};
    \node at (4.35,1.5) {{\tiny\dots}};
    \node at (4.8,1.5) {{\tiny$\xtest$}};
    \node at (4.8,0.55) {{\tiny $\hat\tb^1$}};

    \node at (4.35,0.1) {{\tiny\dots}};
    \node at (4.75,0.1) {{\tiny$\xtest$}};
    \node at (5.15,0.15) {{\tiny$\hat\tb^1$}};
    \node at (5.1,-0.9) {{\tiny$\hat\tb^2$}};

    \node at (4.35,-1.35) {{\tiny\dots}};
    \node at (4.75,-1.35) {{\tiny$\xtest$}};
    \node at (5.15,-1.3) {{\tiny$\hat\tb^1$}};
    \node at (5.5,-1.3) {{\tiny$\hat\tb^2$}};
    \node at (5.4,-2.35) {{\tiny$\hat\y$}};

    \node at (-4.5,-1.7) {\includegraphics[height=.2\columnwidth]{fig_sec/figs/k=16.pdf}};
\end{tikzpicture}
\vspace{-5pt}
\caption{An illustration of $\ICL$, $\EXP$ and $\COT$ methods, using a 3-layer MLP as an example (top left, where $\x$, $\y$, $\tb^1$, $\tb^2$ denote input, output and hidden features respectivaly). The $\ICL$ method utilizes in-context examples in the form of $(\x,\y)$ and makes predictions directly based on the provided $\xtest$. Both $\EXP$ and $\COT$ methods admit prompts with samples formed by $(\x,\tb^1,\tb^2,\y)$. However, $\COT$ uniquely makes recurrent predictions by re-inputting the intermediate output (as shown on the right). The performance of these methods is shown on the bottom left, with a more detailed discussion available in Sections~\ref{sec prelim} and \ref{sec:2nn}.}\label{fig:intro}
\vspace{-10pt}
\end{figure}

==> backup/fig_sec/fig_intro_backup_.tex <==
\setlength{\arrayrulewidth}{.5pt}
\begin{equation}
% \arraycolsep=0pt
\def\arraystretch{1.5}
\begin{array}{cc|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
\cline{3-13}
&&\cellcolg\tikzmark{111}\x_1 & \tikzmark{112}\tb_1 &\tikzmark{113}\y_1 & \cellcolg\tikzmark{121}\x_2 & \tikzmark{122}\tb_2 &\tikzmark{123}\y_2 & \cellcolg\tikzmark{131}\x_3 & \tikzmark{132}\tb_3 &\tikzmark{133}\y_3 & \cdots & \cellcolg\tikzmark{141}\x_{\text{new}} \\
\cline{3-13}\\\\
\cline{3-14}
&&\x_1 & \cellcolr\tb_1 &\y_1 & \x_2 & \cellcolr\tb_2 &\y_2 & \x_3 & \cellcolr\tb_3 & \y_3 & \cdots & \x_{\text{new}} & \cellcolr\hat\tb\\
\cline{3-14}\\\\
\cline{3-15}
&&\x_1 & \tb_1 &\y_1 & \x_2 & \tb_2 &\y_2 & \x_3 & \tb_3 & \y_3 & \cdots & \x_{\text{new}} & \hat\tb & \hat\y\\
\cline{3-15}
\end{array}
\end{equation}


\begin{tikzpicture}[remember picture,overlay,rounded corners]
\draw[->] ([yshift=12pt, xshift=6pt]{pic cs:111}) [out=90,in=90,looseness=1.5] to node [midway, above]{$f$}([yshift=12pt, xshift=6pt]{pic cs:112}) ;
\draw[->] ([yshift=12pt, xshift=6pt]{pic cs:121}) [out=90,in=90,looseness=1.5] to node [midway, above]{$f$}([yshift=12pt, xshift=6pt]{pic cs:122}) ;
\draw[->] ([yshift=12pt, xshift=6pt]{pic cs:131}) [out=90,in=90,looseness=1.5] to node [midway, above]{$f$}([yshift=12pt, xshift=6pt]{pic cs:132}) ;
% \draw[<-] (com2)|- (com) coordinate (comm);
% \draw[<-] (com3)|- (comm);
% \draw[<-] (ceof)
%     |- +(0.5,0.6)% short up and long right% remember position for other arrow and other label
%     node[right]{EOF};
%      \draw[<-,color=teal] (mem)
%     -- +(-0.4,0)% short line to the left
%     |- +(+0.2,+0.8)% up one and long left% remember position for other arrow and other label
%     node[right]{Block of memory};
%      \draw[<-,color = violet] (scr)
%      -- +(-0.6,0) %short line to the left
%     |- +(+0,+1.4)% short up and left% remember position for other arrow and other label
%     node[right]{Scratchpad};
%     \draw[<-,color=olive] (point)
%      -- +(-0.5,0) %short line to the left
%     |- +(+0.8,+2.3)% short up and left% remember position for other arrow and other label
%     node[right]{Program Counter};
%     \draw[<-,color=gray] (ee)
%      -- +(-0.4,0) %short line to the left
%     % --(+0,-0.3)
%     |- +(0.1,-1.5)% short up and left% remember position for other arrow and other label
%     %coordinate (ee2)
%     node[right]{Encodings};
%      \draw[<-,color=gray] (ee1)
%     % -- +(-1,0)
%     |- +(0.1,-0.7)
%    % |- +(1,0.2)
%      node[right]{Indicator of the scratchpad};
%      %short line to the left
%  %   |- (ee2);
\end{tikzpicture}

==> backup/fig_sec/fig_largek.tex <==
\begin{figure}[!t]
\centering
\subfigure[Composed risk]{
    \includegraphics[width=.315\columnwidth]{fig_sec/figs/cot_d10_largek.pdf}
    \label{fig:largek compose}
    % \hspace{-1mm}
}
\subfigure[Risk of first layer]{
    \includegraphics[width=.315\columnwidth]{fig_sec/figs/cot_d10_largek_first_layer.pdf}
    \label{fig:largek first}
    % \hspace{1mm}
}
\subfigure[Risk of second layer]{
    \includegraphics[width=.315\columnwidth]{fig_sec/figs/cot_d10_largek_second_layer.pdf}
    \label{fig:largek second}
    % \hspace{1mm}
}
\vspace{-2mm}
\caption{Decouple the composed risk into risks of first and second layers. }

\label{fig:largek}
\end{figure}

==> backup/fig_sec/fig_long_chain.tex <==
\begin{figure}[!t]
\vspace{-0pt}
\centering
\subfigure[Point-to-point meta prediction]{
    \includegraphics[height=.25\columnwidth]{fig_sec/figs/cot_d5_f4c6.pdf}
    \label{fig:d5}
    \hspace{5mm}
}
\subfigure[One-shot prediction over time]{
    \includegraphics[height=.25\columnwidth,trim={1.5cm 0 0 0},clip]{fig_sec/figs/training_1-shot.pdf}
    \label{fig:one shot}
    % \hspace{-3mm}
}
% \subfigure[Attentions of last layer]{
%     \includegraphics[height=.3\columnwidth,trim={1.5cm 0 0 0},clip]{fig_sec/figs/attention.pdf}
%     \label{fig:attn}
%     % \hspace{-3mm}
% }
\vspace{-2mm}
\caption{Evaluations over deep linear MLPs using $\COT$ and $\ICL$ where CoT-$X$ represents the $X$-step $\COT$. Fig.~\ref{fig:d5} illustrates point-to-point meta results where the model is trained with substantial number of samples. In contrast, Fig.~\ref{fig:one shot} displays the one-shot performance (with only one in-context sample provided) when making predictions during training. See Section~\ref{sec:deep nn} for further implementation details.}
\label{fig:long chain}
\vspace{-10pt}
\end{figure}

==> backup/fig_sec/fig_main.tex <==
% \begin{figure}
% \centering
% \begin{minipage}{0.325\textwidth}
% 	\centering
% 	\includegraphics[scale=0.22]{fig_sec/figs/k16.pdf}
% % \caption{}
% \end{minipage}
% \begin{minipage}{0.325\textwidth}
% 	\centering
% 	\includegraphics[scale=0.22]{fig_sec/figs/cot_d10_vs_d20.pdf}
% % \caption{}
% \end{minipage}
% \begin{minipage}{0.325\textwidth}
% 	\centering
% 	\includegraphics[scale=0.22]{fig_sec/figs/cotk16_d10_vs_d20.pdf}
% % \caption{}
% \end{minipage}
% \caption{Comparing the }
% \end{figure}

\begin{figure}[!t]
\centering
\subfigure[$\COT~vs~\EXP~vs~\ICL$]{
    \includegraphics[width=.315\columnwidth]{fig_sec/figs/k16.pdf}
    \label{fig:k16}
    % \hspace{-1mm}
}
\subfigure[$\COT$: $d=10~vs~20$]{
    \includegraphics[width=.315\columnwidth]{fig_sec/figs/cot_d10_vs_d20.pdf}
    \label{fig:cot_d10_vs_d20}
    % \hspace{1mm}
}
\subfigure[Alignment in Fig.~\ref{fig:cot_d10_vs_d20}]{
    \includegraphics[width=.315\columnwidth]{fig_sec/figs/cotk16_d10_vs_d20.pdf}
    \label{fig:cot_d10_vs_d20_align}
    % \hspace{1mm}
}
\vspace{-2mm}
\caption{(a) Comparing the performance of the three algorithms CoT-I/O, CoT-I and ICL. \ks{I think all the plots should be CoT vs ICL vs CoT-I. So fig1: algo comparison with fixed model, fixed d, varying k. fig2: algo comparison with varying model, fixed d, fixed k and so on.. Like our older plots? What do you think @yc?}}

\label{fig:main_fig1}
\end{figure}

==> backup/fig_sec/fig_method.tex <==
% \setlength{\arrayrulewidth}{.5pt}
% \begin{equation}
% \arraycolsep=2pt
% \def\arraystretch{1}
% \begin{array}{lc|ccccccccccc|ccc}
% \cline{3-13}
% \ICL&&\cellcolg\x_1 &\cellcolg&\cellcolg\y_1 & \cellcolr\x_2 &\cellcolr&\cellcolr\y_2 & \cellcolb\x_3 &\cellcolb&\cellcolb\y_3 & \cdots & \x_n \\
% \cline{3-13}
% \\
% \cline{3-13}
% \EXP&&\cellcolg\x_1 &\cellcolg\tb_1 &\cellcolg\y_1 & \cellcolr\x_2 & \cellcolr\tb_2 &\cellcolr\y_2 & \cellcolb\x_3 & \cellcolb\tb_3 & \cellcolb\y_3 & \cdots & \x_n & \hat\tb\\
% \cline{3-13}\\
% \cline{3-13}
% \COT&&\cellcolg\x_1 & \cellcolg\tb_1 &\cellcolg\y_1 & \cellcolr\x_2 & \cellcolr\tb_2 &\cellcolr\y_2 & \cellcolb\x_3 & \cellcolb\tb_3 & \cellcolb\y_3 & \cdots & \x_n & \hat\tb & \hat\y\\
% \cline{3-13}
% \end{array}
% \end{equation}


\setlength{\arrayrulewidth}{.5pt}
\begin{equation}
\arraycolsep=2pt
\def\arraystretch{1}
\begin{array}{ccc}
    \begin{array}{l}
    \begin{array}{ccccccccccccc|ccc}
    % \cline{3-13}
    \cellcolg\hat\y_1 && \cellcolr\hat\y_2 && \cellcolb\hat\y_3 && \cdots & \x_n \\
    % \cline{3-13}
    \\
    % \cline{3-13}
    \end{array}\\
    \begin{array}{ccccccccccccc|ccc}
    \cellcolg\x_1 &\cellcolg\y_1 & \cellcolr\x_2 &\cellcolr\y_2 & \cellcolb\x_3 & \cellcolb\y_3 & \cdots & \x_n & \hat\tb\\
    \end{array}\\
    \begin{array}{ccccccccccccc|ccc}
    \cellcolg\x_1 &\cellcolg\y_1 & \cellcolr\x_2 &\cellcolr\y_2 & \cellcolb\x_3 & \cellcolb\y_3 & \cdots & \x_n & \hat\tb & \hat\y    \end{array}
    \end{array}
    &
    \begin{array}{cc}
         &  \\
         & 
    \end{array}
    &
    \begin{array}{cc}
         &  \\
         & 
    \end{array}\\
    \ICL & \EXP & \COT
\end{array}
\end{equation}

==> backup/fig_sec/fig_skill.tex <==
\begin{figure}[t]
\centering
\begin{minipage}[t]{0.45\linewidth}
    \centering
    \includegraphics[width=\linewidth]{fig_sec/figs/diff_clen}
    \caption{}
    \label{fig:diff_clen}
\end{minipage}
\hspace{30pt}
\begin{minipage}[t]{0.45\linewidth}
    \centering
    \includegraphics[width=\linewidth]{fig_sec/figs/diff_nfunc.pdf}
    \caption{}
    \label{fig:diff_func}
\end{minipage}
\end{figure}

% \begin{minipage}[b]{0.5\textwidth}
% \centering
% \setlength{\arrayrulewidth}{0.5mm}
% \setlength{\tabcolsep}{2pt}
\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.2}
{\small{
    \begin{tabular}{|c|cccc|c|}
        \hline
        Chain length & $3$ & $5$ & $7$ & $9$ & Unique\\
        \hline
         Zero-shot risk ($\times10^{-4}$)  & - & - & - & - & $9.7$\\
         One-shot risk ($\times10^{-4}$)  & $0.21$ & $0.57$ & $0.95$ & $1.29$ & $0.16$\\
        \hline
    \end{tabular}}}
    \captionof{table}{Your caption here}
    \label{tab:skill}
\end{table}
% \end{minipage}

==> backup/fig_sec/graph.tex <==
\begin{tikzpicture}[node distance={1mm}, thick, main/.style = {draw, circle}, fill/.style = {red,draw,circle}] 
\node[main] (0) at (-1,1) {$\s_0$}; 
\node[fill] (1) at (0,0) {$\s_1$}; 
\node[main] (2) at (1.5,2) {$\s_2$}; 
\node[fill] (3) at (4,0) {$\s_3$}; 
\node[fill] (4) at (2,-1) {$\s_4$}; 
\node[fill] (5) at (3,2.5) {$\s_5$}; 
\node[fill] (6) at (6,0) {$\s_6$}; 
\node[fill] (7) at (5,2) {$\s_7$}; 
\node[main] (8) at (8,0) {$\s_8$}; 
\node[main] (9) at (7,-1) {$\s_9$}; 
\draw (0) -- (1);
\draw (0) -- (2); 
\draw (1) -- (2); 
% \draw (1) -- (3); 
% \draw (1) -- (4); 
\draw (2) -- (3); 
\draw (2) -- (5); 
\draw (2) -- (4); 
\draw (3) -- (7); 
\draw (3) -- (4); 
% \draw (3) -- (5); 
\draw (3) -- (6); 
\draw (3) -- (9); 
\draw (4) -- (9); 
\draw (5) -- (6); 
% \draw (5) -- (7); 
% \draw (6) -- (7); 
\draw (6) -- (8); 
\draw (6) -- (9); 
\draw (7) -- (8); 
\draw (8) -- (9); 
\draw[red,very thick, ->] (6) -- (7);
\draw[red,very thick, ->] (7) -- (5);
\draw[red,very thick, ->] (5) -- (3);
\draw[red,very thick, ->] (3) -- (1);
\draw[red,very thick, ->] (1) -- (4);
% \draw (1) -- (2); 
% \draw[->] (1) -- (3); 
% \draw (1) to [out=135,in=90,looseness=1.5] (5); 
% \draw (1) to [out=180,in=270,looseness=5] (1); 
% \draw (2) -- (4); 
% \draw (3) -- (4); 
% \draw (5) -- (4); 
% \draw[->] (5) to [out=315, in=315, looseness=2.5] (3); 
% \draw[->] (6) -- node[midway, above right, sloped, pos=1] {+1} (4); 
\end{tikzpicture} 
% \begin{tikzpicture}[node distance={15mm}, thick, main/.style = {draw, circle}] 
% \node[main] (1) {$\s_1$}; 
% \node[main] (2) [above right of=1] {$\s_2$}; 
% \node[main] (3) [below right of=1] {$\s_3$}; 
% \node[main] (4) [above right of=3] {$\s_4$}; 
% \node[main] (5) [above right of=4] {$\s_5$}; 
% \node[main] (6) [below right of=4] {$\s_6$}; 
% % \draw[->] (1) -- (2); 
% % \draw[->] (1) -- (3); 
% % \draw (1) to [out=135,in=90,looseness=1.5] (5); 
% % \draw (1) to [out=180,in=270,looseness=5] (1); 

% \draw (1) -- (2); 
% \draw (2) -- (4); 
% \draw (3) -- (4); 
% \draw (5) -- (4); 
% % \draw[->] (5) to [out=315, in=315, looseness=2.5] (3); 
% % \draw[->] (6) -- node[midway, above right, sloped, pos=1] {+1} (4); 
% \end{tikzpicture} 

==> backup/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

%\usepackage{amsmath,amsfonts,bm}
\usepackage{bm}
\usepackage{bbm}
\usepackage[mathscr]{eucal}

\newcommand{\dmu}{\textnormal{d}\mu}
\newcommand{\dnu}{\textnormal{d}\nu}
\newcommand{\ds}{\textnormal{d}s}
\newcommand{\dt}{\textnormal{d}t}
\newcommand{\du}{\textnormal{d}u}
\newcommand{\dv}{\textnormal{d}v}
\newcommand{\dx}{\textnormal{d}x}
\newcommand{\dy}{\textnormal{d}y}
\newcommand{\dz}{\textnormal{d}z}




% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}

%\newcommand{\newterm}[1]{\mathbf{ #1}}


% % Figure reference, lower-case.
% \def\figref#1{figure~\ref{#1}}
% % Figure reference, capital. For start of sentence
% \def\Figref#1{Figure~\ref{#1}}
% \def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
% \def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% % Section reference, lower-case.
% \def\secref#1{section~\ref{#1}}
% % Section reference, capital.
% \def\Secref#1{Section~\ref{#1}}
% % Reference to two sections.
% \def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% % Reference to three sections.
% \def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% % Reference to an equation, lower-case.
% \def\eqref#1{equation~\ref{#1}}
% % Reference to an equation, upper case
% \def\Eqref#1{Equation~\ref{#1}}
% % A raw reference to an equation---avoid using if possible
% \def\plaineqref#1{\ref{#1}}
% % Reference to a chapter, lower-case.
% \def\chapref#1{chapter~\ref{#1}}
% % Reference to an equation, upper case.
% \def\Chapref#1{Chapter~\ref{#1}}
% % Reference to a range of chapters
% \def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% % Reference to an algorithm, lower-case.
% \def\algref#1{algorithm~\ref{#1}}
% % Reference to an algorithm, upper case.
% \def\Algref#1{Algorithm~\ref{#1}}
% \def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
% \def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% % Reference to a part, lower case
% \def\partref#1{part~\ref{#1}}
% % Reference to a part, upper case
% \def\Partref#1{Part~\ref{#1}}
% \def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
% \newcommand{\train}{\mathcal{D}}
% \newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
% \newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}
\def\rvbeta{{\mathbf{\beta}}}
% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}
\def\rmZero{{\mathbf{0}}}
\def\rmGamma{{\mathbf{\Gamma}}}
% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vZero{{\bm{0}}}
\def\vOne{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mZero{{\bm{0}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% calligraphic
\def\cA{{\mathcal{A}}}
\def\cB{{\mathcal{B}}}
\def\cC{{\mathcal{C}}}
\def\cD{{\mathcal{D}}}
\def\cE{{\mathcal{E}}}
\def\cF{{\mathcal{F}}}
\def\cG{{\mathcal{G}}}
\def\cH{{\mathcal{H}}}
\def\cI{{\mathcal{I}}}
\def\cJ{{\mathcal{J}}}
\def\cK{{\mathcal{K}}}
\def\cL{{\mathcal{L}}}
\def\cM{{\mathcal{M}}}
\def\cN{{\mathcal{N}}}
\def\cO{{\mathcal{O}}}
\def\cP{{\mathcal{P}}}
\def\cQ{{\mathcal{Q}}}
\def\cR{{\mathcal{R}}}
\def\cS{{\mathcal{S}}}
\def\cT{{\mathcal{T}}}
\def\cU{{\mathcal{U}}}
\def\cV{{\mathcal{V}}}
\def\cW{{\mathcal{W}}}
\def\cX{{\mathcal{X}}}
\def\cY{{\mathcal{Y}}}
\def\cZ{{\mathcal{Z}}}

% blackboard
\def\bOne{{\mathbbm{1}}}
\def\bA{{\mathbb{A}}}
\def\bB{{\mathbb{B}}}
\def\bC{{\mathbb{C}}}
\def\bD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\bE{{\mathbb{E}}}
\def\bF{{\mathbb{F}}}
\def\bG{{\mathbb{G}}}
\def\bH{{\mathbb{H}}}
\def\bI{{\mathbb{I}}}
\def\bJ{{\mathbb{J}}}
\def\bK{{\mathbb{K}}}
\def\bL{{\mathbb{L}}}
\def\bM{{\mathbb{M}}}
\def\bN{{\mathbb{N}}}
\def\bO{{\mathbb{O}}}
\def\bP{{\mathbb{P}}}
\def\bQ{{\mathbb{Q}}}
\def\bR{{\mathbb{R}}}
\def\bS{{\mathbb{S}}}
\def\bT{{\mathbb{T}}}
\def\bU{{\mathbb{U}}}
\def\bV{{\mathbb{V}}}
\def\bW{{\mathbb{W}}}
\def\bX{{\mathbb{X}}}
\def\bY{{\mathbb{Y}}}
\def\bZ{{\mathbb{Z}}}

% script
\def\sA{{\mathscr{A}}}
\def\sB{{\mathscr{B}}}
\def\sC{{\mathscr{C}}}
\def\sD{{\mathscr{D}}}
\def\sE{{\mathscr{E}}}
\def\sF{{\mathscr{F}}}
\def\sG{{\mathscr{G}}}
\def\sH{{\mathscr{H}}}
\def\sI{{\mathscr{I}}}
\def\sJ{{\mathscr{J}}}
\def\sK{{\mathscr{K}}}
\def\sL{{\mathscr{L}}}
\def\sM{{\mathscr{M}}}
\def\sN{{\mathscr{N}}}
\def\sO{{\mathscr{O}}}
\def\sP{{\mathscr{P}}}
\def\sQ{{\mathscr{Q}}}
\def\sR{{\mathscr{R}}}
\def\sS{{\mathscr{S}}}
\def\sT{{\mathscr{T}}}
\def\sU{{\mathscr{U}}}
\def\sV{{\mathscr{V}}}
\def\sW{{\mathscr{W}}}
\def\sX{{\mathscr{X}}}
\def\sY{{\mathscr{Y}}}
\def\sZ{{\mathscr{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

%\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
%\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\sigma_{\text{S}}}
%\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
%\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

%\DeclareMathOperator*{\argmax}{arg\,max}
%\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{\mathrm{sign}}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> backup/notation.tex <==
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{xcolor}         % colors
\usepackage{xcolor,colortbl}
% \usepackage{floatrow}
\usepackage{caption}
\usepackage{amssymb}% http://ctan.org/pkg/amssymb
\usepackage{pifont}% http://ctan.org/pkg/pifont

\newcommand{\RSIS}{RSI$+$Smooth}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{wrapfig,amsmath,amssymb,bm,comment,color,mathbbol}
\usepackage{breakurl,epsfig,epsf,fmtcount,semtrans,multirow,boldline}
\usepackage{tcolorbox}
\tcbuselibrary{skins}
\usepackage{tikz}
\usetikzlibrary{tikzmark}
\usepackage{mathtools}

\definecolor{darkred}{RGB}{150,0,0}
\definecolor{darkgreen}{RGB}{0,150,0}
\definecolor{darkblue}{RGB}{0,0,200}
\hypersetup{colorlinks=true, linkcolor=darkred, citecolor=darkgreen, urlcolor=darkblue}

\setcounter{secnumdepth}{3}
\newtheorem{theorem}{Theorem}%[section]
\newtheorem{result}{Result}
\newtheorem{fact}{Fact}
\newtheorem{problem}{Problem}
\newtheorem{claim}{Claim}
\newtheorem{assumption}{Assumption}
\newtheorem{question}{Question}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\newtheorem{definition}{Definition}
\newtheorem{condition}{Condition}
\newtheorem{conjecture}{Conjecture}
\newtheorem{remark}{Remark}
\newtheorem{remarks}{Remarks}
\newtheorem{example}{Example}
\numberwithin{equation}{section} 

\newenvironment{assbis}[1]
  {\renewcommand{\theassumption}{\ref{#1}$'$}%
   \addtocounter{assumption}{-1}%
   \begin{assumption}}
  {\end{assumption}}
  
\def \endprf{\hfill {\vrule height6pt width6pt depth0pt}\medskip}

 \newenvironment{proof}{\noindent {\bf Proof.} }{\endprf\par}
\newenvironment{proofsk}{\noindent {\bf Proof sketch.} }{\endprf\par}

% \newcommand{\qed}{{\unskip\nobreak\hfil\penalty50\hskip2em\vadjust{}
%            \nobreak\hfil$\Box$\parfillskip=0pt\finalhyphendemerits=0\par}}

\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}
\newcommand{\tsn}[1]{{\left\vert\kern-0.25ex\left\vert\kern-0.25ex\left\vert #1 
    \right\vert\kern-0.25ex\right\vert\kern-0.25ex\right\vert}}
    
    
\newcommand{\red}{\textcolor{red}}
\newcommand{\so}[1]{\textcolor{darkblue}{#1}}
\newcommand{\SO}[1]{\textcolor{blue}{SO: #1}}
\newcommand{\dat}[1]{\textcolor{darkgreen}{#1}}
\newcommand{\DAT}[1]{\textcolor{green}{DAT: #1}}
\newcommand{\yl}[1]{\textcolor{orange}{#1}}
\newcommand{\YL}[1]{\textcolor{orange}{YL: #1}}
% \newcommand{\todo}[1]{\textcolor{darkred}{TODO: #1}}
\newcommand{\clr}[1]{\red{#1}}
\newcommand{\cln}[1]{\red{}}
\newcommand{\som}[1]{\marginpar{\color{darkblue}\tiny\ttfamily SO: #1}}
\newenvironment{myitemize}{\begin{list}{$\bullet$}
		{\setlength{\topsep}{1mm}
			\setlength{\itemsep}{0.25mm}
			\setlength{\parsep}{0.25mm}
			\setlength{\itemindent}{0mm}
			\setlength{\partopsep}{0mm}
			\setlength{\labelwidth}{15mm}
			\setlength{\leftmargin}{4mm}}}{\end{list}}

%% TT's definitions
\newcommand\tr{{{\operatorname{trace}}}}
\newcommand{\noi}{\noindent}
% \newcommand{\pmt}{\texttt{pmt}}
\newcommand{\pmt}{{\p}}
\newcommand{\pmtid}[1]{\pmt^{#1}}
\newcommand{\ins}{\texttt{ist}}
\newcommand{\flt}{\texttt{flt}}
\newcommand{\new}{\text{new}}
\newcommand{\prm}{\text{prompt}}
\newcommand{\TF}{{\texttt{TF}}\xspace}
\newcommand{\TFLR}{{\texttt{TF}_{\texttt{LR}}}\xspace}
\newcommand{\TFBE}{{\texttt{TF}_{\texttt{BE}}}}
\newcommand{\hTF}{{\widehat{\texttt{TF}}}}
\newcommand{\tTF}{{\tilde{\texttt{TF}}}}
\newcommand{\outr}[1]{\text{outer\_update}(#1)}
\newcommand{\eps}{\varepsilon}
\newcommand{\beps}{\boldsymbol{\eps}}
\newcommand{\ept}{\eps_{\TF}}
\newcommand{\cz}{c_0}
\newcommand{\cc}[1]{\Cc(#1)}%textbf{d}
\newcommand{\kz}{\nu}
\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\vs}{\vspace}
\newcommand{\fnn}{f_{\text{nn}}}
\newcommand{\ff}{f_{\text{nn}}}
\newcommand{\wi}{k_\st}
\newcommand{\fF}[1]{f_{\text{nn},#1}}
\newcommand{\vc}{\text{vec}}
\newcommand{\flin}{f_{\text{lin}}}
\newcommand{\fln}[1]{f_{\text{lin},#1}}
\newcommand{\rest}{\text{rest}}
\newcommand{\exc}[1]{\mathcal{R}_{\text{gap}}(#1)}
\newcommand{\Mb}{\bar{\M}}
\newcommand{\Nb}{\bar{N}}
\newcommand{\epsr}{\varepsilon_R}
\newcommand{\mur}{\mu_R}
\newcommand{\bp}{\bar{p}}
\newcommand{\zig}{\nu}
\newcommand{\bh}{\bar{h}}
\newcommand{\hb}{\vct{h}}
\newcommand{\al}{\alpha}
\newcommand{\als}{\alpha}
\newcommand{\fs}{f^{\Dc}}
\newcommand{\Ncov}{\mathcal{N}_\eps(\Bal)}
\newcommand{\ft}{h}
\newcommand{\ftv}{f^{\Tc\cup\Vc}}
\newcommand{\deff}{h_{\text{eff}}}
\newcommand{\defz}{\bar{h}_{\text{eff}}}
\newcommand{\deft}{\tilde{h}_{\text{eff}}}
\newcommand{\defg}{\bar{h}^{\nabla}_{\text{eff}}}
\newcommand{\defF}{\bar{h}^{\FB}_{\text{eff}}}
\newcommand{\bC}{\bar{C}}
\newcommand{\st}{\star}
\newcommand{\nt}{n_\mathcal{T}}
\newcommand{\h}{h}
\usepackage{xspace}
\newcommand{\nv}{n_\mathcal{V}}
\newcommand{\distas}{\overset{\text{i.i.d.}}{\sim}}
\newcommand{\pleq}{\overset{{P}}{\leq}}
\newcommand{\np}{{n\wedge p}}
\newcommand{\KB}{\bar{K}}
\newcommand{\bG}{\boldsymbol{\Gamma}}
\newcommand{\rP}{\stackrel{{P}}{\longrightarrow}}
\newcommand{\xw}{\x_{\w}}
\newcommand{\xv}{\x_{\vb}}
\newcommand{\xu}{\x_{\ub}}
\newcommand{\xvt}[1]{\x_{\vb_{#1}}}
\newcommand{\xvtt}[1]{\x_{\vb,#1}}
\newcommand{\xwt}[1]{\x_{#1,\w}}
\newcommand{\xws}[1]{\x_{#1,\ws}}
\newcommand{\xs}{\x_{\ws}}
\newcommand{\xtest}{\x_{\text{\tiny test}}}
\newcommand{\yst}{\hat{\y}}
\newcommand{\yb}{\bar{\y}}
\newcommand{\eig}{\text{eigvec}}
\newcommand{\hu}{h}
\newcommand{\ru}{r}
\newcommand{\pbar}{{{\bar{p}}}}
\newcommand{\pbd}{p}
\newcommand{\lay}[1]{{\vct{k}}^{(#1)}}
\newcommand{\lah}[1]{{\vct{\hat{k}}}^{(#1)}}
\newcommand{\lan}{\vct{k}}
\newcommand{\cmp}{P_{\text{nn}}}
%\newcommand{\rest}{{\bf{r}}}
\newcommand{\dcp}{\vct{d}^{\text{cnn}}}
\newcommand{\fcp}{\vct{g}^{\text{CNN}}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\ba}{\begin{align}}
\newcommand{\ea}{\end{align}}
\newcommand{\bea}[1]{\begin{align}#1\end{align}}
\newcommand{\nrest}{\bar{n}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\prox}{{{\text{\bf{prox}}}}}
\newcommand{\cov}{{{\text{\bf{cov}}}}}
\newcommand{\ex}{{{\text{\bf{ex}}}}}
\newcommand{\modu}{{{\text{{mod}}}}}
\newcommand{\map}{{{\text{\bf{map}}}}}
\newcommand{\var}[1]{{{\text{\bf{var}}}}[#1]}
\newcommand{\vrn}{\sigma}
\newcommand{\sgt}[1]{\tilde{\sigma}^{(#1)}}
\newcommand{\tsig}{\tilde{\sigma}}
\newcommand{\func}[1]{{f_{\text{CNN}}}(#1)}
\newcommand{\funh}[1]{{{\hat{f}}_{\text{CNN}}}(#1)}
\newcommand{\funcp}[1]{{f'_{\text{cnn}}}(#1)}
\newcommand{\funcw}[1]{{{{f}}'_{\text{cnn}}}(#1)}
\newcommand{\dev}{{{\text{\bf{dev}}}}}
\newcommand{\meas}{{{\text{\bf{mean}}(\sigma)}}}
\newcommand{\nn}{\nonumber}
\newcommand{\la}{\lambda}
\newcommand{\laz}{\la_0}
\newcommand{\blaz}{\bar{\la}_0}
\newcommand{\caz}{\la_C}
\newcommand{\saz}{L_\sigma}
\newcommand{\Lat}{\tilde{\Lambda}}
\newcommand{\K}{{K}}
\newcommand{\A}{{\mtx{A}}}
\newcommand{\Aa}{{\mtx{A}}}
\newcommand{\Bb}{{\mtx{B}}}
\newcommand{\N}{{\mtx{N}}}
\newcommand{\amp}{\alpha_{\text{cnn}}}
\newcommand{\btm}{\bigotimes}
\newcommand{\robt}[1]{\bigotimes_{\ell=1}^D{#1}_{\ell}}
\newcommand{\robtu}[1]{\bigotimes_{\ell=1}^D{#1}^{(\ell)}}
\newcommand{\bd}{\bigodot}
\newcommand{\kal}{\prod_{i=1}^{D-1}\tn{\lay{i}}}
%\newcommand{\kall}[1]{\prod_{i=1}^{#1}\tn{\lay{i}}}
\newcommand{\kall}[1]{1_{\lan #1}}
\newcommand{\lall}[1]{{\order{\lip_{\lan #1}}}}%{L^{#1}\prod_{i=1}^{#1}\tn{\lay{i}}}
\newcommand{\lell}[1]{{\lip}_{\lan #1}}
\newcommand{\bell}[1]{{{{\beta}}}_{\lan #1}}
\newcommand{\Ub}{{\mtx{U}}}
\newcommand{\Ubb}{{\mtx{U}}}
\newcommand{\V}{{\mtx{V}}}
\newcommand{\ten}{(\{\vb_\ell\}_{\ell=1}^D)}
\newcommand{\uten}{(\{\ub_\ell\}_{\ell=1}^D)}
\newcommand{\ken}{(\{\lay{i}\}_{i=1}^D)}
\newcommand{\B}{{{\mtx{B}}}}
\newcommand{\alx}{{{\alpha_\X}}}
\newcommand{\aly}[1]{{{\alpha_{\X_{#1}}}}}
\newcommand{\Ib}{{{\mtx{I}}}}
\newcommand{\fp}{F}
\newcommand{\Xbin}{{{\mtx{B}}}}
\newcommand{\Gbin}{{{\mtx{S}}}}
\newcommand{\xbin}{{{\mtx{b}}}}
\newcommand{\Sb}{{{\mtx{S}}}}
\newcommand{\Gb}{{\mtx{G}}}
\newcommand{\ymean}{{\bar{\y}(\w;\text{avg})}}
\newcommand{\yavg}{{{y}_{\text{avg}}}}
\newcommand{\ravg}[1]{{{r}_{{\text{avg}}}(#1)}}
\newcommand{\fmean}{{\funcw{\w;\text{avg}}}}
\newcommand{\diag}[1]{\text{diag}(#1)}
\newcommand{\out}{\text{out}}
\newcommand{\linest}{\text{lin}}
\newcommand{\inp}{\text{in}}
\newcommand{\inh}{\hat{\text{in}}}
\newcommand{\sexp}{subexponential }
\newcommand{\Lc}{{\cal{L}}}
\newcommand{\Hc}{{\cal{H}}}
\newcommand{\Lcz}{{\cal{L}}^{0-1}}
\newcommand{\Lczh}{{\hat{\cal{L}}}^{0-1}}
\newcommand{\Lch}{{\widehat{\cal{L}}}}
\newcommand{\Lcv}[1]{{\cal{L}}^{#1}_{\text{up}}}
\newcommand{\Lct}{{\tilde{\cal{L}}}}%[1]{{\cal{L}}^{#1}_{\text{low}}}
\newcommand{\Lcb}{{\bar{\cal{L}}}}
\newcommand{\Nc}{{\cal{N}}}
\newcommand{\Jc}{{\cal{J}}}
\newcommand{\Dc}{{\cal{D}}}
\newcommand{\Dci}{{\cal{D}}_{\text{init}}}
%\newcommand{\smn}{\s_{\min}}
\newcommand{\Ro}{{\cal{RO}}}
\newcommand{\PC}{{\cal{PC}}}
\newcommand{\Pb}{{\mtx{P}}}
\newcommand{\Tb}{{\mtx{T}}}
\newcommand{\Tn}{{T_0}}
\newcommand{\Kba}{{\vct{k}}_{\text{all}}}
\newcommand{\Qb}{{\mtx{Q}}}
\newcommand{\rng}{\gamma}
\newcommand{\Cb}{{\mtx{C}}}
\newcommand{\BC}{{\bar{C}}}
\newcommand{\Eb}{{\mtx{E}}}
\newcommand{\Hb}{{\mtx{H}}}
\newcommand{\Gc}{{\cal{G}}}
\newcommand{\Zc}{{\cal{Z}}}
\newcommand{\Zcid}[1]{{{\cal{Z}}^{#1}}}
\newcommand{\F}{{\mtx{F}}}
\newcommand{\diff}{{\text{diff}}}
\newcommand{\La}{{\boldsymbol{{\Lambda}}}}
\newcommand{\noresamp}[1]{{\textcolor{red}{#1}}}
\newcommand{\sigmap}{\phi'}
\newcommand{\relu}[1]{\phi(#1)}
\newcommand{\one}{{\bm{1}}}
\newcommand{\sigmal}[1]{\sigma^{(#1)}}
\newcommand{\sigmalp}[1]{\sigma'^{(#1)}}
\newcommand{\sigmaa}{\sigma'_{\text{all}}}
\newcommand{\sigmai}[1]{\sigma'_{\text{all},#1}}
\newcommand{\bSi}{{\boldsymbol{{\Sigma}}}}
\newcommand{\bSii}{{\boldsymbol{{\Sigma}}}_{i,i}}
\newcommand{\bSib}{\bar{{\boldsymbol{{\Sigma}}}}}
\newcommand{\bSit}{{\boldsymbol{{\tilde{\Sigma}}}}}
\newcommand{\bSih}{{\boldsymbol{{\hat{\Sigma}}}}}
\newcommand{\bmu}{{\boldsymbol{{\mu}}}}
\newcommand{\Db}{{\mtx{D}}}
\newcommand{\bB}{{\bar{B}}}
\newcommand{\tB}{{\tilde{B}}}
\newcommand{\db}{{\vct{d}}}
\newcommand{\oneb}{{\mathbb{1}}}
\newcommand{\onebb}{{\mathbf{1}}}
\newcommand{\Iden}{{\mtx{I}}}
\newcommand{\M}{{\mtx{M}}}
\newcommand{\gm}{\gamma_m}
\newcommand{\order}[1]{{\cal{O}}(#1)}
\newcommand{\OR}{\text{OR}}
\newcommand{\ordet}[1]{{\widetilde{\cal{O}}}(#1)}
\newcommand{\rmax}[1]{{\bf{r}_{\max}(#1)}}
\newcommand{\rbmax}[1]{{\bf{\bar{r}}_{\max}(#1)}}
\newcommand{\rmin}[1]{{\bf{r}_{\min}(#1)}}
\newcommand{\smn}[1]{{s_{\min}(#1)}}
\newcommand{\smx}[1]{{s_{\max}(#1)}}
\newcommand{\z}{{\vct{z}}}
\newcommand{\zid}[1]{{\z}^{#1}}
\newcommand{\hzid}[1]{{\hat\z}^{#1}}
\newcommand{\zt}{{\tilde{\vct{z}}}}
\newcommand{\fab}{f^\bal_\bt}
\newcommand{\zb}{{\bar{\z}}}
\newcommand{\el}{{\ell}}
\newcommand{\sft}[1]{\text{shift}(#1)}
\newcommand{\tht}{\hat{\tb}}
\newcommand{\tbt}{\tb_{\text{\tiny test}}}
\newcommand{\tn}[1]{\|{#1}\|}%_{\ell_2}
\newcommand{\tl}[1]{\|{#1}\|_{L_2}}
\newcommand{\ts}[1]{\|{#1}\|_{\Sc}}
\newcommand{\ti}[1]{\|{#1}\|_{\infty}}
\newcommand{\nrm}[1]{\|{#1}\|}%_{#2}}
\newcommand{\inr}[1]{\left<#1\right>}
\newcommand{\tone}[1]{\|{#1}\|_{\ell_1}}
\newcommand{\lix}[1]{\|{#1}\|_{\Xc}}
\newcommand{\lif}[1]{\text{dist}_{\FB}({#1})}
\newcommand{\lit}[1]{\text{max}(#1)}%_{\Ttc}
\newcommand{\lia}[1]{\text{avg}(#1)}%
\newcommand{\lin}[1]{\|{#1}\|_{L_\infty}}
\newcommand{\tff}[1]{\|{#1}\|_{\ell_4}}
\newcommand{\tin}[1]{\|{#1}\|_{\ell_\infty}}
\newcommand{\trow}[1]{\|{#1}\|_{2,\infty}}
\newcommand{\bad}{{\bar{d}}}
\newcommand{\Lcg}{\tilde{\Lc}}
\newcommand{\Dp}{{D^+}}
\newcommand{\tf}[1]{\|{#1}\|_{F}}
\newcommand{\te}[1]{\|{#1}\|_{\psi_1}}
\newcommand{\tsub}[1]{\|{#1}\|_{\psi_2}}
\newcommand{\tsut}[1]{\|{#1}\|_{\psi_{2/3}}}
\newcommand{\tsup}[1]{\|{#1}\|_{\psi_a}}
\newcommand{\dist}[1]{\text{dist}(#1)}
\newcommand{\upp}{{\cal{B}}_{\alpha,\Gamma}}
\newcommand{\upz}{{\cal{B}}_{\alpha_0,\Gamma}}
\newcommand{\dpz}{{\cal{D}}_{\alpha_0,\Gamma}}
\newcommand{\dpp}{{\cal{D}}_{\alpha,\Gamma}}
\newcommand{\mpp}{M_{\alpha,\Gamma}}
%\newcommand{\supp}[1]{\text{supp}(#1)}
\newcommand{\cone}[1]{{\text{cone}(#1)}}
\newcommand{\paf}{\partial f(\x)}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\Ac}{\mathcal{A}}
\newcommand{\Al}[1]{\Ac(#1)}
\newcommand{\Alg}[1]{\Ac_g(#1)}
\newcommand{\Acg}{\Ac_g}
\newcommand{\At}{\mathcal{A}}
%\newcommand{\Pc}{\mathcal{P}}
\newcommand{\Acr}{\mathcal{A_\text{ridge}}}
\newcommand{\Bal}{{\boldsymbol{\Delta}}}
\newcommand{\del}{\delta}
\newcommand{\bdel}{\boldsymbol{\delta}}
\newcommand{\Ccb}{\bar{\mathcal{C}}}
\newcommand{\Rc}{\mathcal{R}}
\newcommand{\Rcp}{\mathcal{\bar{R}}'}
\newcommand{\Rcb}{\mathcal{N}}
\newcommand{\btrue}{\bbeta_{true}}
\newcommand{\bt}{{\boldsymbol{\theta}}}
\newcommand{\bT}{{\boldsymbol{\Theta}}}
\newcommand{\bts}{{\boldsymbol{\beta}_\st}}
\newcommand{\btb}{\bar{\boldsymbol{\theta}}}
\newcommand{\btid}{\boldsymbol{\theta}^\text{ideal}}
\newcommand{\btt}{\tilde{\boldsymbol{\theta}}}
\newcommand{\bal}{\texttt{Alg}}%{{\boldsymbol{\alpha}}}
\newcommand{\bgam}{{\boldsymbol{\gamma}}}
\newcommand{\bab}{{\boldsymbol{\bar{\alpha}}}}
\newcommand{\sbl}[1]{\sigma_{\boldsymbol{\alpha^{(#1)}}}}
\newcommand{\bl}[1]{{\boldsymbol{\alpha}}^{(#1)}}
\newcommand{\blb}[1]{\bar{\boldsymbol{\alpha}}^{(#1)}}
\newcommand{\bah}{{\widehat{\bal}}}
\newcommand{\berm}{\bal^{\texttt{ERM}}}
\newcommand{\bas}{{\boldsymbol{\alpha}_\st}}
\newcommand{\bth}{{\boldsymbol{\hat{\beta}}}}
\newcommand{\bPhi}{{\boldsymbol{\Phi}}}
\newcommand{\bbteta}{\widetilde{\boldsymbol{\theta}}}
\newcommand{\bbeta}{{\boldsymbol{\beta}}}
\newcommand{\ddelta}{{\boldsymbol{\delta}}}
\newcommand{\DD}{{D}}
\newcommand{\babeta}{{\bar{\beta}}}
\newcommand{\balpha}{{\bar{\alpha}}}
\newcommand{\bgamma}{{\bar{\gamma}}}
\newcommand{\No}{N}
\newcommand{\Bc}{\mathcal{B}}
\newcommand{\Sc}{\mathcal{S}}
\newcommand{\Sca}{\mathcal{S}_{\text{all}}}
\newcommand{\Dca}{\mathcal{D}_{\text{all}}}
\newcommand{\Scn}{\mathcal{S}_{\new}}
\newcommand{\Dcn}{\mathcal{D}_{new}}
\newcommand{\Scb}{\bar{\mathcal{S}}}
\newcommand{\Sci}{\mathcal{S}_{\text{in}}}
\newcommand{\Sco}{\mathcal{S}_{\text{out}}}
\newcommand{\Ec}{{\mathcal{E}}}
\newcommand{\Ect}{\mathcal{S}_{\text{top}}}
\newcommand{\Mc}{\mathcal{M}}
\newcommand{\pa}{{\partial}}
\newcommand{\Nn}{\mathcal{N}}
\newcommand{\pol}{^\circ}
\newcommand{\vb}{\vct{v}}
\newcommand{\Jb}{\mtx{J}}
\newcommand{\Jt}{\mtx{\tilde{J}}}
\newcommand{\vbl}{\vct{v}^{\text{lin}}}
\newcommand{\fb}{\vct{f}}
\newcommand{\f}{\vct{f}}
\newcommand{\fid}[1]{f^{#1}}
\newcommand{\Fb}{\vct{F}}
\newcommand{\FB}{\mathbb{F}}
\newcommand{\Ft}{\tilde{\vct{F}}}
\newcommand{\fa}{\tilde{\vct{f}}}
\newcommand{\ib}{{\bf{i}}}
\newcommand{\hib}{{\bf{\hat{i}}}}
\newcommand{\Ic}{{\mathcal{I}}}
\newcommand{\all}{{\text{all}}}
\newcommand{\vh}{\vct{\hat{v}}}
\newcommand{\vbb}{\vct{\bar{v}}}
\newcommand{\Xb}{\mtx{\bar{X}}}
\newcommand{\xb}{\vct{\bar{x}}}
\newcommand{\abb}{\mtx{\bar{a}}}
\newcommand{\cb}{\mtx{c}}
\newcommand{\bbb}{\mtx{\bar{b}}}
\newcommand{\w}{\vct{w}}
\newcommand{\ist}{i_\st}
\newcommand{\err}[1]{\text{Err}_{\Dc}(#1)}
\newcommand{\Wp}{\mtx{W}^\dagger}
\newcommand{\tilW}{\widetilde{\mtx{W}}}
\newcommand{\tilw}{\widetilde{\vct{w}}}
\newcommand{\ob}{\mtx{o}}
\newcommand{\obh}{\mtx{\hat{o}}}
\newcommand{\wh}{{\hat{\mtx{w}}}}
\newcommand{\li}{\left<}
\newcommand{\ri}{\right>}
\newcommand{\s}{\vct{s}}
\newcommand{\ab}{\vct{a}}
\newcommand{\bb}{\vct{b}}
\newcommand{\ub}{{\vct{u}}}
\newcommand{\ubb}{\bar{\vct{u}}}
%\newcommand{\h}{\vct{h}}
\newcommand{\hh}{{\vct{h}}}
\newcommand{\g}{{\vct{g}}}
\newcommand{\ii}{{\vct{i}}}
\newcommand{\zm}[1]{{\texttt{{{zm}}}[#1]}}
\newcommand{\dd}{{\vct{d}}}
\newcommand{\ddt}{{\vct{d}}_\tau}
\newcommand{\Zb}{\mtx{Z}}
\newcommand{\hf}{\hat{f}}
\newcommand{\corrCA}{\rho_\Cc(\M)}
\newcommand{\corr}[1]{{\bf{cor}}(#1)}
\newcommand{\Tc}{\mathcal{T}}
\newcommand{\TVc}{\Tc\cup\Vc}
\newcommand{\Ttc}{\mathcal{T}_{\text{test}}}
\newcommand{\Fc}{\mathcal{F}}
\newcommand{\Fcid}[1]{{\mathcal{F}^{#1}}}
\newcommand{\bFc}{\boldsymbol{\mathcal{F}}}
\newcommand{\Fcl}{\mathcal{F}^{\text{lin}}}
\newcommand{\Xc}{\mathcal{X}}
\newcommand{\Xcid}[1]{\mathcal{X}^{#1}}
\newcommand{\Yc}{\mathcal{Y}}


%%YP's macros
\newcommand{\qqq}[1]{{\textcolor{red}{?{#1}?}}}
\newcommand{\ihere}{{\textcolor{red}{I AM HERE! }}}
\newcommand{\mat}[1]{{\text{mat}{#1}}}
\newcommand{\gb}{\bar{\g}}
\newcommand{\bs}{\bar{s}}
\newcommand{\cgain}{\alpha_{\text{CNN}}}
\newcommand{\cgainp}{\tn{\E_{\x\sim\Nn(0,\Iden)}[\gcnn{}]}}
\newcommand{\gcnn}[1]{{\vct{g}}_{\text{cnn}#1}}
\newcommand{\ccorr}{\rho_{\text{cnn}}}
\newcommand{\kb}{\vct{k}}
\newcommand{\xh}{\hat{\x}}
%\newcommand{\yh}{\hat{\y}}
\newcommand{\xbr}{\bar{\h}}
\newcommand{\xdr}{\tilde{\x}}
\newcommand{\xp}[1]{\x^{(#1)}_\prm}
\newcommand{\Sn}[1]{\Sc^{(#1)}}
\newcommand{\Dn}[1]{\Dc^{(#1)}}
\newcommand{\m}{\vct{m}}
\newcommand{\xt}[1]{\x^{(#1)}}
\newcommand{\yt}[1]{y^{(#1)}}
\newcommand{\ybt}{\tilde{\y}}
\newcommand{\Xt}{\tilde{\X}}
\newcommand{\gh}{\hat{\g}}
\newcommand{\gt}{\tilde{\g}}
\newcommand{\wb}{\bar{\w}}
%\newcommand{\lip}{L}
\newcommand{\mipp}{L_{\max}}
\newcommand{\mupp}{\bar{\mu}_{\max}}
\newcommand{\mapp}{\mu}
\newcommand{\tcnn}{{\mtx{T}}_{\text{cnn}}}
\newcommand{\lcnn}{{\mtx{L}}_{\text{CNN}}}
\newcommand{\smo}{S}
\newcommand{\SM}{{{\bf{S}}}_{L,\kb}}
\newcommand{\SMB}{{{\bf{\bar{S}}}}_{L,\kb}}
\newcommand{\Ws}{\W^\star}
\newcommand{\ws}{{\w^\star}}
\newcommand{\wss}{{\w^\star}}
\newcommand{\yp}[1]{\textcolor{red}{ #1}}
% \newcommand{\zero}{{\boldsymbol{0}}}
\newcommand{\zeronorm}[1]{\left\|#1 \right\|_0}
\newcommand{\unorm}[1]{\left\|#1 \right\|_u}
\newcommand{\ynorm}[1]{\left\|#1 \right\|_{\bar{y}}}
\newcommand{\onetwonorm}[1]{\left\|#1\right\|_{1,2}}
\newcommand{\opnorm}[1]{\left\|#1\right\|}
\newcommand{\fronorm}[1]{\left\|#1\right\|_{F}}
\newcommand{\onenorm}[1]{\left\|#1\right\|_{\ell_1}}
\newcommand{\twonorm}[1]{\left\|#1\right\|_{\ell_2}}
\newcommand{\wnorm}[2]{\left\|#1\right\|_{#2}}
\newcommand{\Dnorm}[1]{\left\|#1\right\|_{D}}
\newcommand{\oneinfnorm}[1]{\left\|#1\right\|_{1,\infty}}
\newcommand{\infnorm}[1]{\left\|#1\right\|_{\ell_\infty}}
\newcommand{\nucnorm}[1]{\left\|#1\right\|_*}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\lab}{\bar{\la}}
\newcommand{\avg}[1]{\left< #1 \right>}


\newcommand{\mult}{B^D\bar{M}N}
\newcommand{\liptwo}{20R^3B\nt^2\laz^{-2}(B\nt+1)}
\newcommand{\lipp}{5R^2\sqrt{B^3\nt^3\h}\laz^{-2}\tn{\yT}}
\newcommand{\lips}{6R^3B^2\sqrt{\nt^3\h}\laz^{-2}\tn{\yT}}
\newcommand{\lipl}{5(RB\nt\sqrt{\h}+1)RB\nt\laz^{-2}}
\newcommand{\lip}{\frac{5B^2\tn{\yT}}{\laz^2}}
\newcommand{\lipt}{6R^3B^2\Gamma\sqrt{\nt^3\h}\laz^{-2} \tn{\yT}}
\newcommand{\lipf}{{20R^4B^2\laz^{-2}\Gamma\nt^2\tn{\yT}}}
%\newcommand{\lipv}{{30R^4B^4\laz^{-2}\Gamma\sqrt{\nt^3\nv^2d} \tn{\y}}}
\newcommand{\lipsum}{30R^4B^2\laz^{-2}\Gamma(\nt^2+\nv^2) \tn{\yT}}
%\newcommand{\lipnn}{120c_0^4B^4\laz^{-2}\Gamma(\nt^2+\nv^2) \tn{\yT}}
\newcommand{\lipnn}{120B^4\blaz^{-2}\Gamma(\nt^2+\nv^2) \tn{\yT}}
\newcommand{\bL}{\bar{L}}
\newcommand{\scl}{M}
\renewcommand{\d}{\mathrm{d}}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\x}{\vct{x}}
\newcommand{\xx}[1]{\vct{x}^{(#1)}}
\newcommand{\rb}{\vct{r}}
\newcommand{\rbb}{\vct{\widetilde{r}}}
\newcommand{\y}{\vct{y}}
\newcommand{\yT}{\vct{y}}
\newcommand{\yh}{\hat{y}}
\newcommand{\ybh}{\vct{\hat{y}}}
\newcommand{\W}{\mtx{W}}
\newcommand{\Ww}[1]{\mtx{W}^{(#1)}}
\newcommand{\Wt}{\tilde{\mtx{W}}}
\newcommand{\Wc}{{\cal{W}}}
\newcommand{\Vc}{{\cal{V}}}
\newcommand{\bgl}{{~\big |~}}

%--------------

% EJC's macros

\definecolor{emmanuel}{RGB}{255,127,0}
\newcommand{\ejc}[1]{\textcolor{emmanuel}{EJC: #1}}

\newcommand{\p}{{\vct{p}}}
\newcommand{\Kb}{{\mtx{K}}}
\newcommand{\Kbb}{{\mtx{\bar{K}}}}
\newcommand{\Kbh}{{\widehat{\mtx{K}}}}
\newcommand{\somelog}{16\Kb\log (\Kb)}
\newcommand{\somelg}{\Kb\log (\Kb)}
\newcommand{\pb}{{\vct{p}}}
\newcommand{\pbf}{{\vct{p}}^{\text{filter}}}
\newcommand{\qb}{{\vct{q}}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Pro}{\mathbb{P}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
\newcommand{\Var}{\textrm{Var}}
\newcommand{\sgn}[1]{\textrm{sgn}(#1)}
\renewcommand{\P}{\operatorname{\mathbb{P}}}
\newcommand{\E}{\operatorname{\mathbb{E}}}
\newcommand{\Eh}{\operatorname{\mathbb{\hat{E}}}}
%\newcommand{\var}{\operatorname{\mathbf{var}}}

%\newcommand{\todo}[1]{{\bf TODO: #1}}
\newcommand{\grad}[1]{{\nabla\Lc(#1)}}
\newcommand{\gradf}[1]{{\nabla f(#1)}}
\newcommand{\hessf}[1]{{\nabla^2f(#1)}}
\newcommand{\gradw}[1]{{\nabla{\Lc}(#1)}}
\newcommand{\grd}[2]{{\nabla\Lc_{#1}(#2)}}
\newcommand{\e}{\mathrm{e}}
\newcommand{\eb}{\vct{e}}
\newcommand{\n}[1]{^{(#1)}}
\newcommand{\tb}{\vct{s}}
\newcommand{\ct}{\text{CoT}\xspace}
\newcommand{\icl}{\text{ICL}\xspace}
\newcommand{\FF}{F}


\newcommand{\vct}[1]{\bm{#1}}
\newcommand{\mtx}[1]{\bm{#1}}

% MS's macros

\newcommand{\rank}{\operatorname{rank}}
\newcommand{\supp}[1]{\operatorname{supp}(#1)}
\newcommand{\restrict}[1]{\big\vert_{#1}}
\newcommand{\Id}{\text{\em I}}
\newcommand{\bPi}{\boldsymbol{\Pi}}
\newcommand{\OpId}{\mathcal{I}}

\newcommand{\Real}{\operatorname{Re}}
\newcommand{\Imag}{\operatorname{Im}}

\newcommand{\piyp}{\pi'_1(\vct{y})}
\newcommand{\piy}{\pi_1(\vct{y})}
\newcommand{\piar}{\pi_1(\vct{a}_r)}
\newcommand{\piarp}{\pi'_1(\vct{a}_r)}
\newcommand{\set}{{\cal{F}}}
\newcommand{\des}{{\x_0}}

\newcommand{\Pc}{{\cal{P}}}
\newcommand{\X}{{\mtx{X}}}
\newcommand{\Y}{{\mtx{Y}}}
\newcommand{\Vb}{{\mtx{V}}}
\newcommand{\Vh}{\hat{{\mtx{V}}}}
\newcommand{\Vbd}{{\mtx{V}^\dagger}}
\newcommand{\Rb}{{\mtx{R}}}
\newcommand{\bR}{{\bar{R}}}

\newcommand{\calF}{\mathcal{I}}
\newcommand{\calS}{\mathcal{N}}


\newcommand{\note}[1]{{\bf [{\em Note:} #1]}}

\newcommand{\iprod}[2]{\left\langle #1 , #2 \right\rangle}
\newcommand{\gi}{\ab_{\gamma_i}}
\newcommand{\ang}{\text{ang}}
\newcommand{\ham}[2]{{\|#1,#2\|_H}}

\newcommand{\attn}{\textit{attn}}
\newcommand{\sfm}{\textit{softmax}}
\newcommand{\filter}{\textit{filtered}}
\newcommand{\embd}{\textit{embd}}

\newcommand{\ells}{\ell_{\text{\tiny start}}}
\newcommand{\elle}{\ell_{\text{\tiny end}}}

\newcommand{\COT}{\text{CoT-I/O}\xspace}
\newcommand{\EXP}{\text{CoT-I}\xspace}
\newcommand{\ICL}{\text{ICL}\xspace}

\newcommand{\cellcolg}{\cellcolor{green!20}}
\newcommand{\cellcolr}{\cellcolor{red!20}}
\newcommand{\cellcolb}{\cellcolor{blue!20}}

% @KS: adding notations for vectors and matrices from ICML math_commands.tex
% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

==> backup/rebuttal/fig_filter.tex <==
\begin{figure}[H]
% \vspace{-20pt}
\centering
\begin{tikzpicture}
    \node at (0,0){\includegraphics[scale=0.35]{figs/filter_v2.pdf}};


    \node at (-4.2,.0) {\textbf{\small CoT}};
    \node at (4.5,1.5) {\textbf{\small Step-1 ICL}};
    \node at (4.5,.0) {\textbf{\small Step-2 ICL}};
    \node at (4.5,-1.55) {\textbf{\small Step-3 ICL}};
    
    \node at (0,.5) {\textbf{\small Filtering}};
    \node at (2.3,2.7) {{\small 1st sample}};
    \node at (4.2,2.7) {{\small 2nd sample}};
    \node at (6.3,2.7) {{\small Test sample}};
    \node at (6.6,-2.7) {{\small Prediction}};
    \node at (4.2,3.3) {\textbf{{ICL with Filtered Prompts}}};
    \node at (4.2,2) {{}};
    
    % \node at (-5.05,0.5) {{\small $\x$}};
    % \node at (-4.7,0.5) {{\small $\s_1$}};
    % \node at (-4.35,0.5) {{\small $\s_2$}};
    % \node at (-4.,0.5) {{\small $\y$}};
    % \node at (-3.65,0.5) {{\small $\x$}};
    % \node at (-3.3,0.5) {{\small $\s_1$}};
    % \node at (-2.95,0.5) {{\small $\s_2$}};
    % \node at (-2.6,0.5) {{\small $\y$}};
    % \node at (-2.3,0.5) {{\small ...}};
    % \node at (-2.3,0.5) {{\small ...}};

    % \node at (-0.2,-0.9) {\textbf{\small $\EXP$}};
    % \node at (-1.4,-1.4) {{\tiny $\x_1$}};
    % \node at (-1.1,-1.39) {{\tiny $\tb^1_1$}};
    % \node at (-0.8,-1.39) {{\tiny $\tb^2_1$}};
    % \node at (-0.5,-1.4) {{\tiny $\y_1$}};
    % \node at (-0.2,-1.4) {{\tiny $\x_2$}};
    % \node at (0.1,-1.39) {{\tiny $\tb_2^1$}};
    % \node at (0.6,-1.4) {{\tiny\dots}};
    % \node at (1.1,-1.4) {{\tiny$\xtest$}};
    % \node at (1,-2.35) {{\tiny $\hat\y$}};


    % \node at (4,2.) {\textbf{\small $\COT$}};
    % \node at (2.7,1.5) {{\tiny $\x_1$}};
    % \node at (3,1.55) {{\tiny $\tb^1_1$}};
    % \node at (3.3,1.55) {{\tiny $\tb^2_1$}};
    % \node at (3.6,1.5) {{\tiny $\y_1$}};
    % \node at (3.9,1.5) {{\tiny $\x_2$}};
    % \node at (4.35,1.5) {{\tiny\dots}};
    % \node at (4.8,1.5) {{\tiny$\xtest$}};
    % \node at (4.8,0.55) {{\tiny $\hat\tb^1$}};

    % \node at (4.35,0.1) {{\tiny\dots}};
    % \node at (4.75,0.1) {{\tiny$\xtest$}};
    % \node at (5.15,0.15) {{\tiny$\hat\tb^1$}};
    % \node at (5.1,-0.9) {{\tiny$\hat\tb^2$}};

    % \node at (4.35,-1.35) {{\tiny\dots}};
    % \node at (4.75,-1.35) {{\tiny$\xtest$}};
    % \node at (5.15,-1.3) {{\tiny$\hat\tb^1$}};
    % \node at (5.5,-1.3) {{\tiny$\hat\tb^2$}};
    % \node at (5.4,-2.35) {{\tiny$\hat\y$}};

\end{tikzpicture}
\vspace{-5pt}
\caption{\textbf{An illustration of our theory: $\text{CoT}=\text{filtering}+\ICL$.} Here, (Yellow, Green, Orange, Blue) circles represent in-context sample ($\x,\s^1,\s^2,\y$). }
\vspace{-10pt}
\end{figure}

==> backup/rebuttal/icl_padding.tex <==
\begin{figure}[H]
\centering
% \begin{minipage}{12cm}
% \begin{minipage}{6cm}
%  % \vspace{-.5cm} 
%     \centering
%    % \subfigure[small GPT-2, $d=10$, $k=4$]{
%         \begin{tikzpicture}
%         \node at (0,0) {\includegraphics[scale=.3]{figs/noise_rebuttal.pdf}};
%         \node at (0.4, -2.5) {(a) Test with noisy data};
%         \end{tikzpicture}
% \end{minipage}
% \begin{minipage}{6cm}
%  % \vspace{-.5cm}
%     % \centering
%    % \subfigure[small GPT-2, $d=10$, $k=4$]{
%         \begin{tikzpicture}
%         \node at (0,0) {\includegraphics[scale=.3]{figs/diff_k_rebuttal.pdf}};
%         \node at (0.4, -2.5) {(b) Test with different $k$};
%         \end{tikzpicture}
% \end{minipage}
% \caption{}
% \end{minipage}
\begin{minipage}{8cm}
 % \vspace{-.5cm} 
    \centering
   % \subfigure[small GPT-2, $d=10$, $k=4$]{
        \begin{tikzpicture}
        \node at (0,0) {\includegraphics[scale=.3]{figs/5-layer_MLP_rebuttal.pdf}};
        % \node at (0.4, -2.5) {(a) Train ICL with sample formed by $(\x,[?],\y)$};
        \end{tikzpicture}
        \caption{\textbf{Investigation of deep MLPs.}}
\end{minipage}
\hspace{10pt}
\begin{minipage}{8cm}
 % \vspace{-.5cm} 
    \centering
   % \subfigure[small GPT-2, $d=10$, $k=4$]{
        \begin{tikzpicture}
        % \node at (0,0) {\includegraphics[scale=.3]{figs/icl_random_rebuttal.pdf}};
        \node at (0,0) {\includegraphics[scale=.3]{figs/icl_random_-1_rebuttal.pdf}};
        % \node at (0.4, -2.5) {(a) Train ICL with sample formed by $(\x,[?],\y)$};
        \end{tikzpicture}
        \caption{\textbf{Train ICL with input $(\x,[?],\y)$.}}
\end{minipage}

\end{figure}

==> backup/rebuttal/n200.tex <==
\begin{figure}[H]
\centering
%\begin{minipage}{15cm}
 \vspace{-.5cm} 
    \centering
   % \subfigure[small GPT-2, $d=10$, $k=4$]{
        \begin{tikzpicture}
        \node at (0,0) {\includegraphics[scale=.3]{figs/small_d10k4_n200_rebuttal.pdf}};
        \node at (0.4, -2.5) {(a) Small GPT-2, $d=10$, $k=4$};
        \end{tikzpicture}
   % }
    \hspace{10pt}
   % \subfigure[standard GPT-2, $d=10$, $k=4$]{
        \begin{tikzpicture}
        \node at (0,0) {\includegraphics[scale=.3]{figs/standard_d10k4_n200_rebuttal.pdf}};
        \node at (0.4, -2.5) {(b) Standard GPT-2, $d=10$, $k=4$};
        \end{tikzpicture}
   % }
    % \vspace{-10pt}
    \caption{\textbf{Train ICL with more in-context samples.} }
   % \end{minipage}
\end{figure}

==> backup/rebuttal/robust.tex <==

\begin{figure}[H]
\centering
\begin{minipage}{19cm}
% \begin{minipage}{6cm}
 % \vspace{-.5cm} 
    \centering
   % \subfigure[small GPT-2, $d=10$, $k=4$]{
 \hspace{-.5cm}
        \begin{tikzpicture}
        \node at (0,0) {\includegraphics[scale=.3]{figs/noise_rebuttal.pdf}};
        \node at (0.4, -2.5) {(a) Test with noisy data};
        \end{tikzpicture}
% \end{minipage}
% \begin{minipage}{6cm}
 \hspace{-.5cm}
    % \centering
   % \subfigure[small GPT-2, $d=10$, $k=4$]{
        \begin{tikzpicture}
        \node at (0,0) {\includegraphics[scale=.3]{figs/diff_k_rebuttal.pdf}};
        \node at (0.4, -2.5) {(b) Test with different $k$};
        \end{tikzpicture}
% \end{minipage}
% \caption{}
% \end{minipage}
% \begin{minipage}{6cm}
 \hspace{-.5cm} 
    \centering
   % \subfigure[small GPT-2, $d=10$, $k=4$]{
        \begin{tikzpicture}
        \node at (0,0) {\includegraphics[scale=.3]{figs/diff_d_rebuttal.pdf}};
        \node at (0.4, -2.5) {(c) Test with different $d$};
        \end{tikzpicture}
        \caption{\textbf{Out-of-distribution experiments.}}
\end{minipage}

\end{figure}



==> backup/sec/2nn.tex <==
\section{Experimental Results}\label{sec:exp}
\subsection{Model Training}\label{sec:train}
In Figure~\ref{fig:intro} and Section~\ref{sec prelim}, we have discussed vanilla $\ICL$, $\EXP$ and $\COT$ methods. 
% , whose inputs structure %data structures are 
% is shown in Table~\ref{tab:intro}. 
Intuitively, $\ICL$ can be viewed as a special case of $\EXP$ (or $\COT$) if we assume only one step is performed. Consequently, we will focus on implementing  $\EXP$ and $\COT$ for model training in the following. %, while $\ICL$ will be a special case of that implementation.%we will introduce the implementation of $\EXP$ and $\COT$ model training in the following and $\ICL$ can be easily applied by setting $L=1$. 

Consider the CoT prompt as in  %same CoT prompt setting as in 
\eqref{cot pmt}, and assume that $\x\sim\Dc_{\Xc}$,  %and training functions obey 
and $f_\ell\sim\Dc_{\ell},\ell\in[L]$, where $L$ denotes the number of compositions/steps, such that the final prediction should approximate $f(\x)=f_L(f_{L-1}\dots f_1(\x)):=\y\in\Yc$. We define $\ell(\hat\y,\y):\Yc\times\Yc\to\R$ as a loss function. For simplicity, we assume $f_\ell(\dots f_1(\x))\in\Yc$, $\ell\in[L]$. Let $N$ represent the in-context window of $\TF$, which implies that $\TF$ can only admit a prompt containing up to $N$ in-context samples. Generally, our goal is to ensure high prediction performance given any length-$n$ prompt, where $n\in[N]$. To this end, we train the model using prompts with length from $1$ to $N$ equally and aim to minimize the averaged risk over different prompt size. 
Assuming the model $\TF$ is parameterized by $\bt$ and considering meta learning problem, the objective functions for $\EXP$ and $\COT$ are defined as follows. 
% and CoT prompt structures (see \eqref{icl pmt} and \eqref{cot pmt}), and also one-shot and multi-step prediction. 
% and intuitively, ICL prompting is a special case of CoT prompting. Therefore, next, we introduce our training and evaluating process that admit CoT prompts as datasets, which is directly applied to the ICL setting.
% Consider meta learning problems where input $\x_i\in\Dc_{\x},i\in[N]$ and functions $\f\sim\Dc_{\f}$. Let $\ell(\hat\y,\y):\Yc\times\Yc\to\R$ be a loss function, and assume model $\TF$ is parameterized by $\bt$. Then the objective functions for $\EXP$ and $\COT$ are as follows. 
\begin{align*}
\hat\bt^{\EXP}=\arg\min_{\bt}\E_{(\x_n)_{n=1}^N,(f_\ell)_{\ell=1}^L}\left[\frac{1}{N}\sum_{n=1}^N\ell(\hat\y_n,f(\x_n))\right]~~\text{where}~~\hat\y_n=\TF(\pmt_n(f),\x_n)%\label{erm cot i}
\end{align*}
and
\begin{align*}
\hat\bt^{\COT}=\arg\min_{\bt}\E_{(\x_n)_{n=1}^N,(f_\ell)_{\ell=1}^L}\left[\frac{1}{NL}\sum_{n=1}^N\sum_{\ell=1}^L\ell(\hat\tb_n^\ell,\tb_{n}^\ell)\right]~~\text{where}~~\hat\tb_n^\ell=\TF(\pmt_n(f),\x_n\cdots\tb_n^{\ell-1}). %\label{erm cot io}
\end{align*}
Here $\pmt_n(f)$ is given by \eqref{cot pmt}, and as mentioned previously,  $\tb^0=\x$ and $\tb^L=\y$. All $\x$ and $f_\ell$ are independent, and we take the expectation of the risk over their respective distributions. 
\input{fig_sec/fig_diff_gpt}
\input{fig_sec/fig_diff_k}
\subsection{2-layer Random MLPs}\label{sec:2nn}
% Our first evaluation concerns the statistical benefit of \AG{add text here}. For a clear exposition we focus on the case of two layer MLPs and compare \AG{text here}. 
For a clear exposition, we first focus on the case of two layer MLPs which are 2-step tasks, and compare three different methods: $\ICL$, $\EXP$ and $\COT$. 
% , whose prompt and prediction data structures have been discussed in Section~\ref{sec prelim}. 
Comparison results are shown in Figures~\ref{fig:diff gpt} and \ref{fig:diff k}.
% \red{Additionally, we also investigate the exact in-context samples needed for $\COT$ to learn the 2-layer MLPs by varying the input dimension ($d$) and hidden neuron number ($k$). The phenomenon is shown in Figures~\ref{fig:smallk} and \ref{fig:largek}, which empirically verifies Theorem~\ref{}.
% }
% experiments by comparing three different methods: $\ICL$, $\EXP$ and $\COT$. Here $\ICL$ follows the same setting as in \cite{garg2022can}, where prompts are given by input-output pairs (also see \eqref{icl pmt}). While $\EXP$ and $\COT$ admit chain-of-thought prompting and $\COT$ does chain-of-thought predictions as well (see \eqref{exp pmt} for $\EXP$ and \eqref{cot pmt} for $\COT$). 


% While the difference between  and Vanilla is that, Explanation has prompt formed by input-instruction-output. Therefore, Transformer can learn more by following the step-by-step messages. In addition to taking all step-messages as input, CoT also trains to predict each step so that the model performs as expected. 

\textbf{Dataset.} Consider 2-layer MLPs with input $\x\in\R^d$, hidden feature (step-1 output) $\tb\in\R^k$, and output $y\in\R$. Here,  $\tb=f_1(\x):=(\W\x)_+$ and $y=f_2(\tb):=\vv^\top\tb$, with $\W\in\R^{k\times d}$ and $\vv\in\R^{k}$ being the parameters of the first and second layer/sub-function, and $(x)_+=\max(x,0)$ being {ReLU} activation. The function is composed as $y=\vv^\top(\W\x)_+$. We define the function distributions as follows: each entry of $\W$ is sampled via $\W_{ij}\sim\Nc(0,\frac{2}{k})$, and $\vv\sim\Nc(0,\Iden_k)$, with inputs being randomly sampled through $\x\sim\Nc(0,\Iden_d)$\footnote{Following this strategy for data generation, the expected norms of $\x$, $\tb$ and $y$ are equivalent, and the risk curves displayed in the figures are normalized for comparison.}. We apply the quadratic loss in our experiments. To avoid the implicit bias due to distribution shift, both training and test datasets are generated following the same strategy. 

% and $\W$ and $\vv$ can also been seen as the 

% where $\W$, $\vv$ are the respective function parameters following i.i.d. Gaussian distribution, specifically, each entry of $\W$ is sampled via $\W_{ij}\sim\Nc(0,\frac{2}{k})$, and $\vv\sim\Nc(0,\Iden_k)$. 

% $\bullet$ \textbf{$\mathbf{\ICL~vs~\EXP~vs~\COT}$ (Figures~\ref{fig:diff gpt}\&\ref{fig:diff k}).} 
\textbf{Varying model sizes (Figure~\ref{fig:diff gpt}).} We initially assess the benefits of $\COT$ over $\ICL$ and $\EXP$ across different $\TF$ models. With $d=10$ and $k=8$ fixed, we train three different GPT-2 models: standard, small and tiny GPT-2. The small GPT-2 has $6$ layers, $4$ attention heads per layer and $128$ dimensional embeddings. The standard GPT-2 consists of twice the number of layers, attention heads and embedding dimensionality compared to the small GPT-2, and tiny GPT-2, on the other hand, possesses only half of these hyperparameters compared to the small GPT-2. We evaluate the performance using prompts containing $n$ in-context samples, where $n$ ranges from $1$ to $N$ ($N=100$). The associated test risks are displayed in Figs.~\ref{fig:gpt standard},~\ref{fig:gpt small} and \ref{fig:gpt tiny}. The blue, orange and green curves correspond to $\COT$, $\EXP$ and $\ICL$, respectively. In Fig.~\ref{fig:avg risk model}, we present the averaged risks. The results show that using $\COT$, the small GPT-2 can solve 2-layer MLPs with approximately $60$ samples, while $\EXP$ requires the standard GPT-2. Conversely, $\ICL$ is unable to achieve zero test risk even with the standard GPT-2 model and up to $100$ samples. This indicates that to learn 2-layer MLPs in a single shot, $\ICL$ requires at least ${\cal{O}}(dk+d)$ samples to restore all function parameters. Conversely, $\EXP$ and $\COT$ can leverage implicit samples contained in the CoT prompt. Let $f_1\in\Fc_1$ (first layer) and $f_2\in\Fc_2$ (second layer). By comparing the performance of $\EXP$ and $\COT$, it becomes evident that the standard GPT-2 is capable of learning the composed function $f=f_2\circ f_1\in\Fc$, which the small GPT-2 cannot express. 
% However, it can express the union of the function sets $\Fc_1\bigcup\Fc_2$. 

% The results show that $\COT$ achieves the best performance and larger model learns to solve 2-layer MLPs better. 

% Results show that small model is enough to solve the problem for $\COT$ (Fig.~\ref{fig:diff gpt cot}), while $\EXP$ requires standard GPT-2 model (Fig.~\ref{fig:diff gpt exp}), and $\ICL$ is not able to learn the model recovering the neural networks. It is because that to learn the problem in one shot, the model should be enough to represent all possible 2-layer neural networks and additionally, needs at least $O(dk+d)$ samples.

\textbf{Varying MLP widths (Figure~\ref{fig:diff k}). } Next, we explore how different MLP widths impact the performance (by varying the hidden neuron size $k\in\{4,8,16\}$). The corresponding results are depicted in Figure~\ref{fig:diff k}. The blue, orange and green curves in Fig.~\ref{fig:k4}, \ref{fig:k8} and \ref{fig:k16} correspond to hidden layer sizes of $k=4$, $8$, and $16$, respectively. Fig.~\ref{fig:avg risk k} displays the averaged risks. We keep $d=10,~N=100$ fixed and train with the small GPT-2 model. As discussed in Section~\ref{sec:main}, $\COT$ can learn a 2-layer MLP using around $60$ samples for all $k=4,8,16$ due to its capability to deconstruct composed functions. However, $\EXP$ can only learn the narrow MLPs with $k=4$, and $\ICL$ is unable to learn any of them. Moreover, we observe a substantial difference in the performance of $\ICL$ and $\EXP$ with varying $k$ (e.g., see averaged risks in Fig.~\ref{fig:avg risk k}). This can be explained by the fact that enlarging $k$ results in more complex $\Fc_1$ and $\Fc_2$, thus making the learning of  $\Fc=\Fc_2\times\Fc_1$ more challenging for $\ICL$ and $\EXP$. 
% What's more, in Fig.~\ref{fig:avg risk k}, we observe that the average risks of $\COT$ do not significantly change with hidden size $k$. To further analyze the reason, we introduce the following $\COT$ experiments.

% Following the same setting, Figure~\ref{fig:k16} shows the result when $k=16$. This validates the approximation benefits of CoT prompts and predictions. 



% varying $d$ will  Therefore, solving the problem requires $O(\max{(k,d)})$ samples. 

% , which is parameterized by $\vv\in\R^k$. 

% which verifies out statement that in the previous setting, $d$ dominates the test performance. 

% We also observe that there exist alignments in Figure~\ref{fig:diff k cot}, which means $\COT$ needs the same number of sample to learn the given three neural width. The interpretation is that, $\COT$ treats the problem as $k$ $d$-dimensional and $1$ $k$-dimensional linear regression problems and solves them in parallel. Therefore, solving the problem requires $O(\max{(k,d)})$ samples. The evidence in Fig.~\ref{fig:diff k cot} dues from the fact that the data dimension $d$ dominates the problem. To further verify our explanation, in Figure~\ref{fig:cot_d10_vs_d20}, we repeat the $\COT$ experiments but with $d=20$. Dashed curves are showing $d=20$ results with the same $k$ choices. Fig.~\ref{fig:cot_d10_vs_d20_align} shows the alignment in Fig.~\ref{fig:cot_d10_vs_d20}, where $x$-axis is valued by $n/d$ where $n$ is the sample size, which shows that for $d=20$, $\COT$ needs exact two times more samples to learn the neural network compared to $d=10$. What's more in Fig.~\ref{fig:largek}, we tried with larger $k$ so that hidden dimension size $k$ turns to dominate the problem. Fig.~\ref{fig:largek compose} shows the composed CoT risk where $\TF$ first generates \emph{thought} prediction $\hat\tb$, and feeding it back to the model results in the final prediction $\hat y$. While in Fig.~\ref{fig:largek first}, losses are calculated by $\|\tb-\hat\tb\|^2$, and to get the second layer risk in Fig.~\ref{fig:largek second}, we feed toe model with the oracle \emph{thought} $\tb$ and the model only needs to learn the last linear function. To clearer compare their performance, we plot the first risks of $k=4,16$ (dotted) and second layer risk of $k=64$ (dashed) in Fig.~\ref{fig:largek second}. The alignments again verifies our statement that to learn a 2-layer neural network with $d$ input dimension and $k$ neurons, CoT needs exact $O(\max(k,d))$ samples. 

% \red{MORE EXPERIMENTS TO DISCUSS:
% \begin{itemize}
%     \item feed the output of second with zeros/random, and test the filtering observation of first-layer prediction
%     \item separately first/second layer predictions are aligned with linear regression problem
% \end{itemize}
% }

==> backup/sec/backup/main.tex <==
\section{How can Transformer Deal with the CoT Prompts?}\label{sec main theory}
\YL{Show the main results: filtering+composition}
\begin{theorem}[Filtering]

\end{theorem}

\begin{theorem}[Composition]

\end{theorem}

\begin{assumption}
    Assume the model $\TF$ is $\Gamma$-Lipschitz with respect to the last input, that is
    \[
    \|\TF(\pmt,\x)-\TF(\pmt,\x')\|\leq\Gamma\|\x-\x'\|.
    \]
\end{assumption}

\begin{assumption}[Approximation to ERM]
Assume there exists model $\tTF$ such that for any $f\in\Fc_\ell$,
\[
\E_{(\x_i)_{i=1}^n,\x}\left[\|\tTF(\pmt_n,\x)- \hat f_n(\x)\|\right]\leq\eps
\]
\[
\text{where}~~~~\pmt_n=(\x_i,f(\x_i))_{i=1}^n,~~\text{and}~~
\hat f_n =\arg\min_{f_n\in\Fc_\ell}\frac{1}{n}\sum_{i=1}^n\ell(f_n(\x_i),f(\x_i))
\]
and $\x\sim\Dc_{\Fc_{\ell-1}}\times\dots\Dc_{\Fc_1}\times\Dc_{\x}$. 
% Here $r(n)$ is a non-increasing function capturing the ability of transformer of learning function $f\in\Fc_\ell$ with randomly distributed $n$ samples.
\end{assumption}

% Here, if treating $\TF$ as a learning algorithm that admits a dataset as input, $r(n)$ can be treated as the approximation error $\TF$ achieves

\begin{theorem}
\begin{align}
    \lesssim\sum_{\ell=1}^L\Gamma^{\ell+1}(\eps+\Rc_n(\Fc_\ell))
\end{align}    
\end{theorem}

\input{sec/nn}


==> backup/sec/backup/nn.tex <==
\subsection{Deep Neural Networks as Compositional Functions}
\YL{Introduce the results when functions are linear}\\
% \YL{Also introduce neural nets experiments}


==> backup/sec/backup/setup__backup_v2_.tex <==
\section{Problem Setup}
\noindent\textbf{Notation:} Let $[n]=\{1,2,\cdots,n\}$. Let $\Xc$ denote token/input space, $\Yc$ denote output space and $\Zcid{k}$, $k\in[K]$ denote the intermediate feature space, where $\x\in\Xc,\y\in\Yc$ and $\zid{k}\in\Zcid{k}$. We can define an ICL example of CoT by 
\[
\p=(\x,\zid{1},\zid{2},\cdots,\zid{K},\y).
\]
Then ICL admits length-$t$ prompt as form $\pmt=(\p_1,\p_2,\cdots,\p_t,\x)$.

Consider an in-context-learning (ICL) problem, and assume we are given $n$ training sequences, and each contains $T$ samples. Specifically, define training dataset $\Sc=((\p_{it})_{t=1}^T)_{i=1}^n$ where $\p_{it}=(\x_{it},\zid{1}_{it},\cdots\zid{K}_{it},\y_{it})$, and assume the input-output pairs follow the distribution $\y_{it}=f_{it}(\x_{it})$ where $f_{it}=\fid{K}_{it}\circ\cdots\fid{1}_{it}\circ\fid{0}_{it}$ where $f_{it}\in\Fc:\Xc\to\Yc$, $\fid{k}_{it}\in\Fcid{k} (0\leq k\leq K)$, and $\Fc=\Fcid{K}\times\cdots\Fcid{0}$. Let $\TF$ denote any auto-regressive model (e.g., Transformer) which admits sequences of data as inputs, and $\ell_0:\Yc\times\Yc\to\R$, $\ell_k:\Zcid{k}\times\Zcid{k}\to\R$ be loss functions. Then ICL aims to solve the empirical risk minimization problem over training dataset $\Sc$ as follows.
\begin{align}
% \hat\bt=&\arg\min_{\bt}\frac{1}{nT}\sum_{i=1}^n\sum_{t=1}^T\ell(\TF(\pmtid{K}_{it}),\y_{it})\label{erm}\\
\hat\bt=\arg\min_{\bt}\frac{1}{nT}&\sum_{i=1}^n\sum_{t=1}^T\left(\ell_0(\TF(\pmtid{K}_{it}),\y_{it})+\sum_{k=1}^K\ell_k(\TF(\pmtid{k-1}_{it}),\zid{k}_{it})\right)\label{erm}\\
\text{where}~~~~&\pmtid{0}_{it}=(\p_{i1},\p_{i2},\cdot,\p_{i,t-1},\x_{it})\nn\\
&\pmtid{k}_{it}=(\p_{i1},\p_{i2},\cdot,\p_{i,t-1},\x_{it},\zid{1}_{it},\cdots,\zid{k}_{it}).\nn
\end{align}
where model $\TF$ is parameterized by $\bt$ and let $\widehat\TF$ be the trained model weighted by $\hat\bt$ from \eqref{erm}. Then the CoT test risk can be defined as 
\begin{align}
    \Lc(\hat\bt)=&\E\left[\frac{1}{T}\sum_{t=1}^T\ell_0(\widehat\TF(\pmtid{K}_t),\y)\right]\\
    \text{where}~~~~&\pmtid{0}_t=(\p_1,\cdots,\p_{t-1},\x),\nn\\
    &\pmtid{k}_t=(\p_1,\cdots,\p_{t-1},\x,\hzid{1}_t,\cdots,\hzid{k}_t),\nn\\
    &\hzid{k}_t=\widehat\TF(\pmtid{k-1}_t).\nn
\end{align}


\section{Problem Setup}
\noindent\textbf{Notation:} Let $\Xc$ denote token/input space and $\Yc$ denote output space where $\x\in\Xc$ and $\y\in\Yc$. Assume there are $K$ types of tokens and  denote the set of $k$th type as $\Xcid{k}$, then we have $\Xc=\bigcup_{k=1}^K\Xcid{k}$. For an example, in natural language processing, words can be categorized into verbs, nouns, adjectives etc. Denote $\Xc^{\otimes t}$ as $t$-times Cartesian product of $\Xc$. 

Consider an in-context-learning (ICL) problem, and assume we are given $n$ training sequences, and each contains $T$ samples. Specifically, define training dataset $\Sc=((\X_{it},\y_{it})_{t=1}^T)_{i=1}^n$ where $\X_{it}=(\x_{i1},\x_{i2},\cdots\x_{it})\in\Xc^{\otimes t}$ and $\y_{it}\in\Yc$, and assume the input-output pairs follow the distribution $\y_{it}=f_{it}(\x_{it})$ where $f_{it}\in\Fc=\bigcup_{k=1}^K\Fc^k$. We say that $\x_{it}\in\Xcid{k}$ if $f_{it}\in\Fc^k$. Let $\TF$ denote any auto-regressive model (e.g., Transformer) which admits sequences of data as inputs, and $\ell:\Yc\times\Yc\to\R$ be loss function. Then ICL aims to solve the empirical risk minimization problem over $\Sc$ as follows.
\begin{align}
\hat\bt=\arg\min_{\bt}\frac{1}{nT}\sum_{i=1}^n\sum_{t=1}^T\ell(\TF(\X_{ti}),\y_{it})\label{erm}
\end{align}
where model $\TF$ is parameterized by $\bt$ and let $\widehat\TF$ be the trained model weighted by $\hat\bt$ from \eqref{erm}.

Consider any input sequence $\X=(\x_1,\x_2,\cdots,\x_t)$, and its corresponding output $\Y=(f_!(\x_1),f_2(\x_2),\cdots,f_t(\x_t))$. Then we say that $\x_\tau$ is relevant to $\x_t$ if they are from the same token space. Without loss of generality, let us assume $\x_t\in\Xcid{1}$, and then we can build relevant set of $\x_t$ by $\X_R=\{\x_\tau:\tau\leq t,\x_\tau\in\Xcid{1}\}$.

\noindent $\bullet$ \textbf{Transformer can handle heterogeneous prompts.} Given a prompt containing tokens from multiple feature spaces, the $\TF$ is able to filter out irrelevant tokens and focus on the relevant ones. That is 
\[
\TF(\X)\approx\TF(\X_R).
\]
Here, $\X_R$ is defined by the sequence $\X$ and the feature space its last token belongs to. Then instead of taking $T$-length sequence as input, the $\TF$ performs almost the same as treating $\X_R$ as input with $|\X_R|<T$. It implies that the irrelevant tokens are helpless in predicting the input at hand. This allows the model to effectively handle prompts with heterogeneous features, and the resulting performance is almost as good as if the prompt was constructed using only the relevant tokens.

\noindent $\bullet$ \textbf{Implicit chain-of-thought property.} The property arises from the Transformer's ability to focus on different relevant sets of tokens. Generally, we have $\Yc\subseteq\Xc$. When the Transformer generates an output based on a given input, the relevant set of tokens for the output is different from the relevant set for the input. Let $\hat\y_t=\TF(\X)$ and without loss of generality, assume $\y_t\in\Xcid{2}$. Feeding $\hat\y$ back to the model as the next token results in different relevant set, that is $\X'_R=\{\x_\tau:\tau\leq t+1,\x_\tau\in\Xcid{2}\}$ where $\X'=(\X,\hat\y)$ and $\x_{t+1}=\hat\y$. By repeating this process, the Transformer generates a sequence of outputs that reflect a "chain-of-thought" behavior, where each output is generated based on a different set of relevant tokens.
% \noindent\textbf{Notation:} Let $\Xc$ denote the token/feature space where $\x\in\Xc$, and assume there are $D$ types of tokens. Denote the $i$th type as $\Xcid{i}$, then we have $\Xc=\bigcup_{i=1}^D\Xcid{i}$. For an example, in natural language processing, words can be categorized into verbs, nouns, adjectives etc.

% Now define the input sequence (as prompt) by 
% \[
% \pmt=(\x_1,f_1(\x_1),\x_2,f_2(\x_2),\cdots,\x_t,f_t(\x_t);\x_\new).
% \]
% The goal of ICL is to predict current input $\x_\new$ based on the given prefix and the training stage. Let $\TF$ define any auto-regressive model admits the prompt as input and outputs $\hat f(\x_\new)=\TF(\pmt)$. 
% % For cleaner notations, let $\y_{i}=f_i(\x_i)$ and $\hat\y=\hat f(\x_\new)$. 
% Assume we are given training dataset $\Sc=((\x_{it},f_{it})_{t=1}^T)_{i=1}^n$ where $\pmt_{it}:=(\x_{i1},f_{i1}(\x_{i1}),\cdots,\x_{i,t-1},f_{i,t-1}(\x_{i,t-1});\x_t)$. What's more, assume for each $(\x,f)$ pair, if $\x\in\Xc^1$ then $f\in\Fc^1$, and within a sequence, function is fixed for $\x$ from the same feature space. Then the objective function is written by
% \[
% \arg\min_{\bt}\frac{1}{nT}\sum_{i=1}^n\sum_{t=1}^T\ell(\TF(\pmt_{it}),f_{it}(\x_{it}))
% \]
% where model $\TF$ is parameterized by $\bt$.
% There are two main observations contributing this work.

% \noindent $\bullet$ \textbf{Transformer can handle heterogeneous prompts.} Without loss of generality, let us assume $\x_\new\in\Xcid{1}$ and define $\pmtid{1}=(\texttt{FILTERED},\x_i,f_i(\x_i)\cdots;\x_\new)$ where $\pmtid{1}$ filters out the irrelevant tokens and the relevant ones remain, that is $\x_i\in\Xc^1$. Then instead $\pmt^1$ turns to be a homogeneous prompt. We observe that  $\TF(\pmt)\approx\TF(\pmt^1)$. In a nutshell, transformers can filter the prompt and automatically pick the most relevant tokens (from the same feature space in our case) as inference. 

% \noindent $\bullet$ \textbf{ICL as a function learning.} Consider a filtered homogeneous prompt $\pmt^1=(\x'_1,f(\x'_1),\cdots,\x'_\tau,f(\x'_\tau);\x_\new)$, and we observe that ICL outputs $\hat f(\x_\new)$ where 

% Combining both properties results in the chain-of-thought behavior of transformers, that is, given a few in-context examples, the model can automatically generate the next prediction sequentially, and the generation is based on 1) Which feature follows the input more frequently; and 2) How generating function is learned based on the given identified examples.



==> backup/sec/construction.tex <==
\section{Construction}
\subsection{The Transformer Architecture }\label{ss:transformer}
For the purpose of this proof, we consider encoder-based transformer architectures and assume that the positional encodings are appended to the input\footnote{We note here that in terms of our construction adding the encodings or appending them to the input can be viewed in a similar manner. Specifically, we can consider that the up-projection step projects the input to  zero padded vectors, while the encodings are orthogonal to that projection in the sense that the have zero in the non-zero coordinates of the input. In that case adding the positional encodings  corresponds to appending them to the input. }. We also consider that the heads are added and each one has each own key, query and value weight matrices. Formally, we have 
\begin{align}\label{eq:transformer}
    \attn(\X) &= \X + \sum_{h=1}^H\weights^h_\val\X\sfm((\weights^h_\key\X)^\top\weights^h_\query\X)\\
    \TF(\X) &= \attn(\X) + \weights_2(\weights_1\attn(\X) +\vb_1\one_n)_{+} +\vb_2\one_n
\end{align}
where $\X\in\R^{d\times n}$, $H$ is the number of heads used and $f(x) = (x)_{+}$ is the ReLU activation. We also make use of the temperature $\lambda$, which is a parameter of the softmax. Specifically, $\sfm(\x) = \{\e^{\lambda x_i}/\sum_j\e^{\lambda x_j}\}_{i}$. Notice that as $\lambda\to\infty$ we have $\sfm(\x)\to \max_i x_i$. We also assume that the inputs are bounded; we denote with $N_{max}$ the maximum sequence length of the model.
\begin{assumption}\label{asm:bounded}Each entry is bounded by some constant $c$, which implies that  $\|\X\|\leq c'$, for some large $c'$ that depends on the maximum sequence length and the width of the transformer.
\end{assumption}
\subsection{Positional Encodings}\label{ss:pencodings}  In the constructions below we use a combination of the binary representation of each position, as well as some additional information (e.g. 0-1 bits) as described in the following sections. The binary representations and in general encodings we construct, require only logarithmic space with respect to the sequence length. Notice that binary representation of the positions satisfy the following two conditions:
\begin{enumerate}
    \item Let $\emb_i$ be the binary representation of the $i$-th position, then there exists $\varepsilon > 0$ such that $\emb_i^\top\emb_i > \emb_i^\top\emb_j +\varepsilon$ for all $j\neq i$.
    \item There exists a one layer transformer that can implement the addition of two pointers (see Lemma \ref{lem:addition} ).
\end{enumerate}
%We note here that any choice of encodings could be made that satisfy the following two conditions: 
% \begin{assumption}\label{asm:distinct}
%     Let $\emb_i$ be the encoding of the $i$-th position, then there exists $\varepsilon > 0$ such that $\emb_i^\top\emb_i > \emb_i^\top\emb_j +\varepsilon$ for all $j\neq i$. 
% \end{assumption} 
% \begin{assumption}\label{asm:increasing}
%     There exists an operator $*$ that the transformer can implement in one layer (or constant layers) such that $\emb_i *\emb_j  =\emb_{i+j}$.
% \end{assumption}
% We note here that multiple choices of positional encodings satisfy these two assumptions. For example, \cite{..} have used binary positional encodings

%One useful fact about the encodings is that as 
\subsection{Constructing Some Useful ``Black-box'' Functions}
We follow the construction of previous work \citep{giannou2023looped}  and use the following individual implementations as they do. We repeat the statements here for convenience. The first lemma is also similar to \cite{akyurek2022learning}, we however follow a slightly different proof. 
\begin{lemma}\label{lem:copy}
A transformer with one layer, two heads, and embedding dimension of ${\cal{O}}(\log n +d)$, where $d$ is the input dimension and $n$ is the sequence length, can copy any block of the input to any other block of the input with error $\varepsilon$ arbitrarily small.
\end{lemma}
\begin{proof}
 Consider an input of the following form 
 \begin{equation}
     \X = \begin{bmatrix}
         \x_1 & \x_2 &\hdots &\x_n\\
         \y_1 &\y_2 &\hdots &\y_n\\
         \emb_1 &\emb_2 &\hdots &\emb_n\\
         \emb_k &\emb_2 &\hdots &\emb_n
     \end{bmatrix}
 \end{equation}
 where $\x_i,\y_i\in\R^d$ are column vectors for all $i=1,\hdots, n$.
We present how we can move a block of data from the $(d+1:2d,k)$ position block to the $(1:d,1)$ position block, meaning to move the point $\y_k$ to the position of the point $\x_1$.   It is straightforward to generalize the proof that follows to move blocks from $(i:i+k, j)$ to $(i':i'+k,j')$ for arbitrary $i,i',j,j',k$. 

Let in Eq. \ref{eq:transformer} $\weights^1_\key =\begin{bmatrix}\zero &\zero &\Iden& \zero \end{bmatrix}$ and $\weights^1_\query = \begin{bmatrix}\zero &\zero & \zero &\Iden\end{bmatrix}$ and   $\weights^2_\key =\begin{bmatrix}\zero &\zero& \zero  &\Iden\end{bmatrix}$ and $\weights^2_\query = \begin{bmatrix}\zero &\zero & \zero &\Iden\end{bmatrix}$ then we have
\begin{equation}
(\weights^1_\key\X)^\top(\weights^1_\query\X) = \begin{bmatrix}
    \emb_1^\top\emb_k & \emb_1^\top\emb_2 &\hdots &\emb_1^\top\emb_k &\hdots &\emb_1^\top\emb_n\\
    \emb_2^\top\emb_k & \emb_2^\top\emb_2 &\hdots &\emb_2^\top\emb_k &\hdots &\emb_2^\top\emb_n\\
    \vdots &\vdots &\ddots &\vdots &\ddots & \vdots\\
    \emb_k^\top\emb_k & \emb_k^\top\emb_2 &\hdots &\emb_k^\top\emb_k &\hdots &\emb_k^\top\emb_n\\
    \vdots &\vdots &\ddots &\vdots &\ddots & \vdots\\
    \emb_n^\top\emb_k & \emb_n^\top\emb_2 &\hdots &\emb_n^\top\emb_k &\hdots &\emb_n^\top\emb_n\\
\end{bmatrix}
\end{equation}
As $\lambda\to \infty$ and after the application of the softmax operator the above matrix becomes equal to 
$\begin{bmatrix}
    \e_k & \e_2 &\hdots &\e_k &\hdots \e_n
\end{bmatrix} + \eps\rmM$, where $\e_i$ is the one-hot vector with $1$ in the $k$-th position, $\|M\|\leq 1$ and $\eps$ is controllable by the temperature parameter and can be arbitrary small. Let finally $\weights^1_\val = \begin{bmatrix}
    \zero &\Iden &\zero &\zero \\
    \zero &\zero &\zero &\zero
\end{bmatrix}$ we get that 
\begin{equation}
    \weights^1_\val\X\sfm((\weights^1_\key\X)^\top(\weights^1_\query\X)) = \begin{bmatrix}
        \y_k &\x_2 &\hdots &\x_n\\
        \zero &\zero &\hdots &\zero 
    \end{bmatrix} + \eps\rmM
\end{equation}By repeating the exact same steps for the second head and letting $\weights_\val^2 = \begin{bmatrix}
    -\Iden &\zero &\zero &\zero\\
    \zero &\zero &\zero &\zero 
\end{bmatrix}$ and adding back the residual we get the desired result.
\end{proof}
A slightly different implementation can be found in \cite{giannou2023looped}, in which the ReLU layers are also used, together with indicator vectors that define whether a position should be updated or not.
% This is the move operation in \cite{akyurek2022learning}. Notice that since \cite{akyurek2022learning} use decoder only models they can only move things only from $(i,j)$ to $(i',j')$ such that $i'>i$ and $j'>j$. However, since we consider encoder models by repeating their proof we can get the result for arbitrary positions. We also consider the positional encodings of \cite{giannou2023looped} which leads to the $\varepsilon$ error.

% \begin{remark} For the idea on how this is possible we illustrate a simple example. Assume that $\seqlen=5$ and we want to copy and element from position (1,2) where the first element signifies the row and the second the column to position (3,5). The first step is to copy the second column to the fifth one; to do so we force the softmax matrix to acts as a permutation matrix, \emph{i.e.,} $[\ve_1\;\ve_2\;\ve_3\;\ve_4\;\ve_2]$ where $\ve_i$ is the one hot vector for the $i$-th row. This is achieved by the bianary representations by using as $\weights_\key\X = [\emb_1\;\hdots\;\emb_5]$, $\weights_\query\X = [\emb_1\;\hdots\;\emb_2]$ and by using $\lambda$ large enough the result follows. Then, we use a value matrix that only keeps the row $1$ and permutes it to the row 3. Finally, to account for the residual, we use an extra head, which softmax is approximately the identity and the value weight matrix is zero expect for the first row which is again permuted to the third one. This description follows the construction of \cite{akyurek2022learning}.
% \end{remark}
\begin{lemma}\label{lem:addition}
   There exists a 1-hidden layer feedforward, ReLU network, with $8d$ activations in the hidden layer and $d$ neurons in the output layer that when given two $d$-dimensional binary vectors representing two non-negative integers, can output the binary vector representation of their sum, as long as the sum is less than $2^{d+1}$. 
   % Further, there is a special bit indicator that is 1 for the scratchpad and 0 for the rest of the input. If this bit is 1 then the operation above is performed, otherwise 0 is returned.
\end{lemma}
% \begin{lemma}\label{lem:transpose}
% Fix $\epsilon >0$ and consider an input of the following form
% \begin{equation}
%     \X = \left[\begin{array}{c|c|c|cc}
%         \rmA  &\zero&\zero &\dots & \zero \\
%  \zero&      \zero&\zero &\dots & \zero\\
%          \emb_{1:d}&\emb_{1:d}&\emb_{1:d}& \dots  &\emb_{1:d}\\
%          \embed_1'&\embed_{2}'&\embed_{3}'& \dots  &\embed_{d}'
%     \end{array}\right]. \nonumber
% \end{equation}
% where $\rmA\in\R^{d\times d}$; then there exists transformer-based function block with 4 layers, 1 head and dimensionality $r = 2d+2\log d = O(d)$ that outputs the following matrix
% \begin{equation}
%     \X = \left[\begin{array}{c|c|c|cc}
% \rmA' &\rmA'&\rmA'&\dots &\rmA' \\
%         \zero&\zero&\zero &\dots &\zero \\
%          \emb_{1:d}& \emb_{1:d}& \emb_{1:d}& \dots &\emb_{1:d} \\
%         \embed_1'&\embed_{2}'&\embed_{3}'& \dots  &\embed_{d}'
%     \end{array}\right]. \nonumber
% \end{equation}
% where $\rmA' = \rmA^\top +\epsilon\rmM$, for some $\|\rmM\|\leq 1$. The error $\epsilon$ depends on the choice of the temperature $\lambda$, as it is  a consequence of the \texttt{read/write} operations.
% \end{lemma}
\begin{lemma}\label{lem:matrixmul_app}
Let $\rmA\in \R^{d\times m}$ and $\rmB \in \R^{d\times n}$. Then for any $\epsilon >0$ there exists a transformer-based function block with  2 layers, 1 head and width  $r = O(d)$ that  outputs the multiplication $\rmA^\top\rmB +\eps\rmM$, for some $\|\rmM\|\leq 1$ .
\end{lemma}
% \begin{lemma}[Lemma 7 in \cite{giannou2023looped}]\label{lem:matrixmul_app} 
% Let $\rmA\in \R^{k\times m}$ and $\rmB \in \R^{k\times n}$. Then for any $\epsilon >0$ there exists a transformer-based function block with  2 layers, 1 head and \red{dimensionality $r = O(d)$} that  outputs the multiplication $\rmA^\top\rmB +\eps\rmM$, for some $\|\rmM\|\leq 1$ .\YL{What do the $r$ and $d$ stand for here?}
% \end{lemma}
\begin{remark}
    Notice that based on the proof of this lemma, the matrices/scalars/vectors need to be in the same rows, \emph{i.e.},
$\rmQ =\begin{bmatrix}
            \rmA &\rmB 
        \end{bmatrix}
$. By also appending the appropriate binary encodings we can move the output at any specific place we choose as in Lemma \ref{lem:copy}. Also, following the proof of the paper the input matrix is
\begin{equation*}
    \X = \begin{bmatrix}
        \rmQ& \zero &\zero \\
        \zero & \one\one^{\top} &\zero\\
        \Iden&\zero &\zero\\ 
        &\emb^{(1)}&\\
        &\emb^{(2)}&\\
        %\zero &\one^{\top} &\zero 
    \end{bmatrix}  
\end{equation*} 
where $\emb^{(1)}, \emb^{(2)}$ are chosen as to specify the position of the result.
\end{remark}
\subsection{Results on Filtering}\label{ss:filtering}
\begin{lemma}\label{lem:binary-app}
    Assume that the input to a transformer layer is of the following form
    \begin{equation}
        \X = \begin{bmatrix}
            \x_1 &\x_2 &\hdots&\x_{n-1} &\x_n\\
            \zero &\zero &\hdots &\zero &\zero\\
        b_1 & b_2 & \hdots &b_{n-1} &b_n\\
        b_1' &b_2' &\hdots &b_{n-1}' &b_n
        \end{bmatrix}
    \end{equation}
    where $b_i,b_i'\in\{0,1\}$, with zero indicating that the corresponding point should be ignored. Then there exists a transformer $\TF$ consisting only of a ReLU layer that performs this filtering, \textit{i.e.}, 
    \begin{equation}
        \TF(\X) = \begin{bmatrix}
           \one\{b_1\neq 0\}\x_1&\one\{b_2\neq 0\}\x_2 &\hdots &\one\{b_{n-1}\neq 0\}\x_{n-1} &\one\{b_n\neq 0\}\x_n\\
            \one\{b_1'\neq 0\}\x_1&\one\{b_2'\neq 0\}\x_2 &\hdots &\one\{b_{n-1}'\neq 0\}\x_{n-1} &\one\{b_n'\neq 0\}\x_n\\
            b_1 & b_2 & \hdots &b_{n-1} &b_n\\
            b_1' &b_2' &\hdots &b_{n-1}' &b_n
        \end{bmatrix}
    \end{equation}
\end{lemma}
\begin{proof}
    The layer is the following:
    \begin{equation}
       \TF(\x_i) = x_i + (-Cb_i - \x_i)_+ - (-Cb_i + \x_i)_+
    \end{equation}
    for some large constant $C$. Notice that if $b_i =1$ the output is just $\x_i$. But if $b_i = 0$ then the output is zero. For the second set instead of using the bits $b_i$,  we use the $b_i'$.
\end{proof}
\begin{remark}\label{rem:error-app} Notice that if some $b_i$ is instead of $1$, $1\pm \varepsilon$, $\varepsilon < c/C$. Then the output of the above layer would be \begin{align}
\TF(\x_i) &= \x_i + (-C \pm C\varepsilon - \x_i) -( -C \pm C\varepsilon +\x_i)\\
& = \x_i
\end{align}
while if some $b_i =\pm \varepsilon$ instead of zero, and assuming that $\x_i > c>0$ or $\x_i < -c< 0$ the output would be 
\begin{align}
    \TF(\x_i) &= \x_i  +(-C\varepsilon - \x_i)_+ - (-Cb_i +\x_i)_+\\
    &= \x_i \pm C\varepsilon - \x_i \\
    &\leq c
\end{align}
If $\abs{\x_i} \leq c$, again the output would be less than or equal to $c$, where $c$ can be arbitrarily small.
\end{remark}
Our target is to create these binary tokens, as to perform the filtering. 
  We now describe for clarity how next word prediction is performed. An $d\times N$-dimensional input is given to the transformer architecture, which is up-projected using the embedding layer;  the positional encodings are also added/appended to the input. At the last layer, the last token predicted is appended to the initial input to the transformer architecture.  The only difference of the new input including the positional encodings ( the input for the next iteration ) is the $n+1$-th token. This is a property that our construction maintains, \emph{i.e.,} the positional encodings used are oblivious to the prediction step performed and are always the same for each individual token. We consider encoder-based architectures in all of our lemmas below. 

In the subsequent lemma we  construct an automated process that works along those guidelines.
To do so we assume that the input to the transformer contains the following information:
\begin{enumerate}
    \item An enumeration of the tokens from $1$ to $N$. 
    \item The $\ln$ of the above enumeration.
    \item Zeros for the tokens that correspond to the data points, $1$ for each token that is the $\x_{\text{test}}$ or it is a prediction based on it.
    \item An enumeration $1$ to $L$ for each one of the data points provided. For example, if we are given three sets of data we would have : $1\hdots L \; 1\hdots L\; 1\hdots L$.
    \item Some extra information that is needed to implement a multiplication step as described in Lemma \ref{lem:matrixmul_app} and to move things to the correct place.
\end{enumerate}
The above information can be viewed as part of the encodings that are appended to the input of the transformer. Formally, we have
\begin{lemma}\label{lem:filtering-app}
Consider that a prompt with $n$ in-context samples is given and 
the $\ell-1$-th prediction has been made, and the transformer is to  predict the $\ell$-th one. Assume the input to the transformer is:
\renewcommand{\arraystretch}{1.5}

\begin{equation*}{\small
\arraycolsep=1.5pt
\X = \left[\begin{array}{*{12}c}
    \x_1 & \hdots &\s_1^{\ell-1}& \s_1^{\ell}&\hdots & \s_2^{\ell-1} &\s_2^{\ell} &\hdots & \s_{n}^{L} &\xtest &\hdots &\hat\tb^{\ell-1}\\
    \zero &\hdots &\zero  &\zero &\hdots &\zero &\zero &\hdots &\zero &\zero &\hdots &\zero\\
        \hline
     1 & \hdots & \ell & \ell+1& \hdots &\ell &\ell+1 &\hdots &L+1 &1&\hdots & \ell\\
     1 & \hdots & \ell &\ell+1 &\hdots &\ell &\ell+1&\hdots &L+1 &1&\hdots & \ell\\
     \hline
     1 & \hdots & \ell &\ell+1 &\hdots &L+\ell+1 &L+\ell+2 &\hdots &n(L+1) &n(L+1)+1 &\hdots & \seqlen\\
    \ln(1) & \hdots & \ln(\ell) &\ln(\ell+1) &\hdots &\ln(L+\ell+1) &\ln(L+\ell+2) &\hdots &\ln(n(L+1)) &\ln(n(L+1)+1) &\hdots & \ln(\seqlen)\\
 0 & \hdots & 0 &0&\hdots &0  &0 &\hdots &0 &1 &\hdots & 1\\
1 & \hdots & 1 &1 &\hdots &1&1 &\hdots &1 &1 &\hdots & 1\\ 
\m_1 & \hdots & \m_\ell &\m_{\ell+1} &\hdots &\m_{L+\ell+1} &\m_{L+\ell+2} &\hdots &\m_{n(L+1)} &\m_{n(L+1)+1} &\hdots & \m_{\seqlen}\\
 \end{array}\right]}
\end{equation*}
where $(\hat\tb^i)_{i=1}^{\ell-1}$ denote the first $\ell-1$ recurrent outputs of $\TF$ and for simplicity, let $\seqlen:=n(L+1)+\ell$ denote the total number of tokens. 
Then there exists a transformer $\TF$ consisting of 7 layers that has as output
\renewcommand{\arraystretch}{1.3}
\begin{equation*}
{\small
\arraycolsep=1.2pt
  \TF(\X)  =  \left[\begin{array}{*{12}c}
      \zero  & \hdots &\s_1^{\ell-1}& \zero&\hdots & \s_2^{\ell-1} &\zero &\hdots & \zero &\zero &\hdots &\hat\tb^{\ell-1}\\
      \zero & \hdots &\zero& \s_1^{\ell}&\hdots & \zero &\s_2^{\ell} &\hdots & \zero &\zero &\hdots &\zero\\
      \hline
     0 & \hdots & 1 &0 &\hdots &1 &0 &\hdots &0&0 &\hdots & 1\\
     0 & \hdots & 0 &1 &\hdots &0 &1 &\hdots &0 &0 &\hdots &0 \\
     \hline
     1 & \hdots & \ell &\ell+1 &\hdots &L+\ell+1 &L+\ell+2 &\hdots &n(L+1) &n(L+1)+1 &\hdots & N\\
       \ln(1) & \hdots & \ln(\ell) &\ln(\ell+1) &\hdots &\ln(L+\ell+1) &\ln(L+\ell+2) &\hdots &\ln(n(L+1)) &\ln(n(L+1)+1) &\hdots & \ln(\seqlen)\\
 0 & \hdots & 0 &0&\hdots &0  &0 &\hdots &0 &1 &\hdots & 1\\
1 & \hdots & 1 &1 &\hdots &1&1 &\hdots &1 &1 &\hdots & 1\\ 
\m_1 & \hdots & \m_\ell &\m_{\ell+1} &\hdots &\m_{L+\ell+1} &\m_{L+\ell+2} &\hdots &\m_{n(L+1)} &\m_{n(L+1)+1} &\hdots & \m_{\seqlen}\\
  \end{array}\right] }
\end{equation*}
with error up to $\delta\rmM$, where $\|{\rmM}\|\leq 1$ and $\delta>0$ is a constant that is controlled and can be arbitrarily small.
\end{lemma}
\begin{proof}
%Since the error of each step we use is controlled and can be arbitrarily small, we can omit it  in the sequence to make the proof simpler. Each one of the seven layers will induce an error of the form $\varepsilon_i \rmM_i$ with $\|\rmM_i\|\leq 1$; at the end the error is aggregated and we have a total error of $\sum_{i=1}^7\varepsilon_i \rmM_i $ with $\|\sum_{i=1}^7\varepsilon_i \rmM_i\| \leq \sum_{i=1}^7\varepsilon_i$. By setting $\varepsilon_i = \delta/7$ we get the desired error bound.

\noindent\textbf{Step 1: Extract the sequence length (1 layer).} Let 
\begin{align}
\weights_{\key}= \begin{bmatrix}
    \zero &\zero &0 &0 &0&1 &0 &0 &\zero
\end{bmatrix} 
 \;\;\; \weights_{\query} =  \begin{bmatrix}
    \zero &\zero &0 &0 &0 &0 &0 &0 &1 &\zero 
\end{bmatrix}
\end{align}
and thus 
\begin{equation}
    (\weights_{\key}\X)^\top(\weights_{\query}\X) = \begin{bmatrix}
        \ln(1) &\ln(1) &\hdots &\ln(1)\\
        \ln(2) &\ln(2) &\hdots &\ln(2)\\
        \vdots &\vdots &\ddots &\vdots\\
        \ln(\seqlen) &\ln(\seqlen) &\hdots &\ln(\seqlen)\\
    \end{bmatrix}.
\end{equation}
So after the softmax is applied we have
\begin{equation} \sfm((\weights_{\key}\X)^\top(\weights_{\query}\X)) = \begin{bmatrix}
        \dfrac{1}{\sum_{i=1}^\seqlen i} &\dfrac{1}{\sum_{i=1}^\seqlen i}&\hdots &\dfrac{1}{\sum_{i=1}^\seqlen i}\\
        \dfrac{2}{\sum_{i=1}^\seqlen i} &\dfrac{2}{\sum_{i=1}^\seqlen i} &\hdots &\dfrac{2}{\sum_{i=1}^\seqlen i}\\
        \vdots &\vdots &\ddots &\vdots\\
        \dfrac{\seqlen}{\sum_{i=1}^\seqlen i} &\dfrac{\seqlen}{\sum_{i=1}^\seqlen i}  &\hdots &\dfrac{\seqlen}{\sum_{i=1}^\seqlen i} \\
    \end{bmatrix}.
\end{equation}
We then set the weight value matrix as to zero-out all lines except for one line as follows
\begin{equation}
   \weights_{\val}\X =\begin{bmatrix}
   \zero &\zero & \hdots &\zero \\
    1 & 2 &\hdots &\seqlen\\
 \zero &\zero &\hdots &\zero 
   \end{bmatrix}.
\end{equation}
% \begin{equation}
%    \weights_{\val}\rmI =\begin{bmatrix}
%    \zero &\zero & \hdots &\zero \\
%   \zero &\zero & \hdots &\zero \\
%     \zero &\zero & \hdots &\zero \\
%     \zero &\zero & \hdots &\zero \\
%     1 & 2 &\hdots &\seqlen\\
%     0 &0 &\hdots &0\\
%      0 &0 &\hdots &0\\
%        0 &0 &\hdots &0
%    \end{bmatrix}
% \end{equation}
After adding the residual and using an extra head where the softmax returns identity matrix and the value weight matrix is minus the identity, we get attenton output
\renewcommand{\arraystretch}{1.5}
\begin{equation*}
{\small
\arraycolsep = 1.5pt
    \left[\begin{array}{*{12}c}
    \x_1 & \hdots &\s_1^{\ell-1}& \s_1^{\ell}&\hdots & \s_2^{\ell-1} &\s_2^{\ell} &\hdots & \s_{n}^{L} &\xtest &\hdots &\hat\tb^{\ell-1}\\
    \zero &\hdots &\zero  &\zero &\hdots &\zero &\zero &\hdots &\zero &\zero &\hdots &\zero\\
        \hline
     1 & \hdots & \ell & \ell+1& \hdots &\ell &\ell+1 &\hdots &L+1 &1&\hdots & \ell\\
     1 & \hdots & \ell &\ell+1 &\hdots &\ell &\ell+1&\hdots &L+1 &1&\hdots & \ell\\
     \hline
     \dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i} & \hdots & \dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i} &\dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i} &\hdots &\dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i}&\dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i} &\hdots &\dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i} &\dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i} &\hdots & \dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i}\\
    \ln(1) & \hdots & \ln(\ell) &\ln(\ell+1) &\hdots &\ln(L+\ell+1) &\ln(L+\ell+2) &\hdots &\ln(n(L+1)) &\ln(n(L+1)+1) &\hdots & \ln(\seqlen)\\
 0 & \hdots & 0 &0&\hdots &0  &0 &\hdots &0 &1 &\hdots & 1\\
1 & \hdots & 1 &1 &\hdots &1&1 &\hdots &1 &1 &\hdots & 1\\ 
\m_1 & \hdots & \m_\ell &\m_{\ell+1} &\hdots &\m_{L+\ell+1} &\m_{L+\ell+2} &\hdots &\m_{n(L+1)} &\m_{n(L+1)+1} &\hdots & \m_{\seqlen}\\
 \end{array}\right].}
\end{equation*}
Notice that $\dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i} = \dfrac{2\seqlen(\seqlen+1)(2\seqlen+1)}{6\seqlen(\seqlen+1)} = \dfrac{2\seqlen+1}{3}$. We then use the ReLU layer as to multiply with $3/2$ and subtract $1$ from this column. This results to attention output
\begin{equation*}
{\small
\arraycolsep = 1.5pt
    \left[\begin{array}{*{12}c}
    \x_1 & \hdots &\s_1^{\ell-1}& \s_1^{\ell}&\hdots & \s_2^{\ell-1} &\s_2^{\ell} &\hdots & \s_{n}^{L} &\xtest &\hdots &\hat\tb^{\ell-1}\\
    \zero &\hdots &\zero  &\zero &\hdots &\zero &\zero &\hdots &\zero &\zero &\hdots &\zero\\
        \hline
     1 & \hdots & \ell & \ell+1& \hdots &\ell &\ell+1 &\hdots &L+1 &1&\hdots & \ell\\
     1 & \hdots & \ell &\ell+1 &\hdots &\ell &\ell+1&\hdots &L+1 &1&\hdots & \ell\\
     \hline
     \seqlen & \hdots & \seqlen &\seqlen&\hdots &\seqlen&\seqlen &\hdots &\seqlen&\seqlen&\hdots & \seqlen\\
    \ln(1) & \hdots & \ln(\ell) &\ln(\ell+1) &\hdots &\ln(L+\ell+1) &\ln(L+\ell+2) &\hdots &\ln(n(L+1)) &\ln(n(L+1)+1) &\hdots & \ln(\seqlen)\\
 0 & \hdots & 0 &0&\hdots &0  &0 &\hdots &0 &1 &\hdots & 1\\
1 & \hdots & 1 &1 &\hdots &1&1 &\hdots &1 &1 &\hdots & 1\\ 
\m_1 & \hdots & \m_\ell &\m_{\ell+1} &\hdots &\m_{L+\ell+1} &\m_{L+\ell+2} &\hdots &\m_{n(L+1)} &\m_{n(L+1)+1} &\hdots & \m_{\seqlen}\\
 \end{array}\right]}
\end{equation*}
Notice that this step does not involve any error.

\textbf{Step 2: Extract the identifier of the prediction to be made $\ell$ (3 layers). }Now, by setting the key and query weight matrices of the attention as  to just keep the all ones row, we get a matrix that attends equally  to all tokens. Then the value weight matrix keeps the row that contains $\ell$ ones and thus we get the number $\dfrac{\ell}{\seqlen}$, propagated in all the sequence length. Then the attention output is as follows:
\begin{equation}
    \arraycolsep = 1.5pt
    \left[\begin{array}{*{12}c}
    \x_1 & \hdots &\s_1^{\ell-1}& \s_1^{\ell}&\hdots & \s_2^{\ell-1} &\s_2^{\ell} &\hdots & \s_{n}^{L} &\xtest &\hdots &\hat\tb^{\ell-1}\\
    \zero &\hdots &\zero  &\zero &\hdots &\zero &\zero &\hdots &\zero &\zero &\hdots &\zero\\
        \hline
     1 & \hdots & \ell & \ell+1& \hdots &\ell &\ell+1 &\hdots &L+1 &1&\hdots & \ell\\
     1 & \hdots & \ell &\ell+1 &\hdots &\ell &\ell+1&\hdots &L+1 &1&\hdots & \ell\\
     \hline
     \seqlen & \hdots & \seqlen &\seqlen&\hdots &\seqlen&\seqlen &\hdots &\seqlen&\seqlen&\hdots & \seqlen\\
    \dfrac{\ell}{\seqlen} & \hdots & \dfrac{\ell}{\seqlen} &\dfrac{\ell}{\seqlen} &\hdots &\dfrac{\ell}{\seqlen} &\dfrac{\ell}{\seqlen} &\hdots &\dfrac{\ell}{\seqlen} &\dfrac{\ell}{\seqlen} &\hdots &\dfrac{\ell}{\seqlen}\\
 0 & \hdots & 0 &0&\hdots &0  &0 &\hdots &0 &1 &\hdots & 1\\
1 & \hdots & 1 &1 &\hdots &1&1 &\hdots &1 &1 &\hdots & 1\\ 
\m_1 & \hdots & \m_\ell &\m_{\ell+1} &\hdots &\m_{L+\ell+1} &\m_{L+\ell+2} &\hdots &\m_{n(L+1)} &\m_{n(L+1)+1} &\hdots & \m_{\seqlen}\\
 \end{array}\right].
\end{equation}
So far this step does not involve any error.
% \YL{Can we do something like this:
% \renewcommand{\arraystretch}{1.5}
% \begin{equation*}{\small
% \arraycolsep=1.5pt
% \X = \left[\begin{array}{*{12}c}
%     \x_1 & \hdots &\s_1^{\ell-1}& \s_1^{\ell}&\hdots & \s_2^{\ell-1} &\s_2^{\ell} &\hdots & \s_{n}^{L} &\xtest &\hdots &\hat\tb^{\ell-1}\\
%     \zero &\hdots &\zero  &\zero &\hdots &\zero &\zero &\hdots &\zero &\zero &\hdots &\zero\\
%         \hline
%      1 & \hdots & \ell & \ell+1& \hdots &\ell &\ell+1 &\hdots &L+1 &1&\hdots & \ell\\
%      1 & \hdots & \ell &\ell+1 &\hdots &\ell &\ell+1&\hdots &L+1 &1&\hdots & \ell\\
%      \hline
%      0 & \hdots & 0 & 0 &\hdots &0 &0 &\hdots &0 &0 &\hdots & 0\\
%      0 & \hdots & 0 & 0 &\hdots &0 &0 &\hdots &0 &0 &\hdots & 0\\
%  0 & \hdots & 0 &0&\hdots &0  &0 &\hdots &0 &0 &\hdots & 1\\
% 1 & \hdots & 1 &1 &\hdots &1&1 &\hdots &1 &1 &\hdots & 1\\ 
% \m_1 & \hdots & \m_\ell &\m_{\ell+1} &\hdots &\m_{L+\ell+1} &\m_{L+\ell+2} &\hdots &\m_{n(L+1)} &\m_{n(L+1)+1} &\hdots & \m_{\seqlen}\\
%  \end{array}\right]}.
% \end{equation*}
% Then by setting 
% \begin{align*}
% \weights_{\key}= \begin{bmatrix}
%     \zero &\zero &0 &0 &0&0 &1 &0 &\zero
% \end{bmatrix} 
%  \;\;\; \weights_{\query} =  \begin{bmatrix}
%     \zero &\zero &0 &0 &0 &0 &0 &0 &1 &\zero 
% \end{bmatrix},
% \end{align*}
% we can get 
% \[
% \sfm((\W_\key\X)^\top\W_\query\X)=\begin{bmatrix}
%         0 & 0 &\hdots &0 \\
%         0 & 0 &\hdots &0\\
%         \vdots &\vdots &\hdots &\vdots\\
%         1 & 1 &\hdots & 1
%     \end{bmatrix}.
% \]
% Let $\W_\val\X$ returns (copy the row contains $[1~2~\dots\ell~\dots~\ell]$ to the all-zero row)
% \begin{equation*}
%    \weights_{\val}\X =\begin{bmatrix}
%    \zero &\zero & \hdots &\zero \\
%     1 & 2 &\hdots &\ell\\
%  \zero &\zero &\hdots &\zero 
%    \end{bmatrix}, 
% \end{equation*}
% then by applying ..., the attention output results in
% \renewcommand{\arraystretch}{1.5}
% \begin{equation*}{\small
% \arraycolsep=1.5pt
% \left[\begin{array}{*{12}c}
%     \x_1 & \hdots &\s_1^{\ell-1}& \s_1^{\ell}&\hdots & \s_2^{\ell-1} &\s_2^{\ell} &\hdots & \s_{n}^{L} &\xtest &\hdots &\hat\tb^{\ell-1}\\
%     \zero &\hdots &\zero  &\zero &\hdots &\zero &\zero &\hdots &\zero &\zero &\hdots &\zero\\
%         \hline
%      1 & \hdots & \ell & \ell+1& \hdots &\ell &\ell+1 &\hdots &L+1 &1&\hdots & \ell\\
%      1 & \hdots & \ell &\ell+1 &\hdots &\ell &\ell+1&\hdots &L+1 &1&\hdots & \ell\\
%      \hline
%      \ell & \hdots & \ell & \ell &\hdots &\ell &\ell &\hdots &\ell &\ell &\hdots & \ell\\
%      0 & \hdots & 0 & 0 &\hdots &0 &0 &\hdots &0 &0 &\hdots & 0\\
%  0 & \hdots & 0 &0&\hdots &0  &0 &\hdots &0 &0 &\hdots & 1\\
% 1 & \hdots & 1 &1 &\hdots &1&1 &\hdots &1 &1 &\hdots & 1\\ 
% \m_1 & \hdots & \m_\ell &\m_{\ell+1} &\hdots &\m_{L+\ell+1} &\m_{L+\ell+2} &\hdots &\m_{n(L+1)} &\m_{n(L+1)+1} &\hdots & \m_{\seqlen}\\
%  \end{array}\right]}.
% \end{equation*}
% }
As described in Lemma \ref{lem:matrixmul_app} to implement multiplication of two values up to any error $\eps$, we need 1) have the two numbers to be multiplied next to each other and an extra structure (some constants, which we consider that are encoded in the last rows of the matrix $\m_i$) and 2) the corresponding structure presented in Lemma \ref{lem:matrixmul_app} . So we need to make the following transformation in the rows containing $\seqlen$ and $\dfrac{\ell}{\seqlen}$
\begin{align}
    \begin{bmatrix}
        \seqlen & \seqlen &\hdots &\seqlen\\
        \dfrac{\ell}{\seqlen} &\dfrac{\ell}{\seqlen} &\hdots &\dfrac{\ell}{\seqlen}
    \end{bmatrix} &\to \begin{bmatrix}
        \seqlen & \dfrac{\ell}{\seqlen} &\hdots &\seqlen\\
        \dfrac{\ell}{\seqlen} &\dfrac{\ell}{\seqlen} &\hdots &\dfrac{\ell}{\seqlen}
    \end{bmatrix}\\
    &\to 
    \begin{bmatrix}
         \ell& *&\hdots &*\\
        * &* &\hdots &*
    \end{bmatrix}\\
    &\to \begin{bmatrix}
        \ell& \ell&\hdots &\ell\\
         * &* &\hdots &*
    \end{bmatrix}
\end{align}
where $*$ denotes inconsequential values.
For the first step we assume that we have the necessary binary representations \footnote{the size that we need will be $2\log \seqlen_{\text{max}}+1$, where $\seqlen_{\text{max}}$ is the maximum sequence length} and then we use Lemma \ref{lem:copy} which shows how we can perform the operation of copy/paste. This step involves an error and the current output would be $\tilde{\X}_1 = \X^* +\varepsilon_1\M_1$, where $\varepsilon_1$ is controlled and we will determine it in the sequence, $\|\M_1\|\leq 1$ and $\X_1^*$ is the desired output. For the second step now we use Lemma \ref{lem:matrixmul_app} to perform the multiplication, this will affect some of the other values. 
To analyze the error of this step, we know that given $\X^*_1$ we will get the desired output $\X_2^*+ \varepsilon_2\M_2$, where $\|\M_2\|\leq 1$ and $\varepsilon_2$ is to be determined. However, are given $\tilde{X}_1$ in the multiplication procedure\footnote{Note that the true error is even smaller since the operation performed only affects one row.} which results in the following output $\tilde{\X}_2 = (\tilde{\X}_1)^\top \tilde{\X}_1 +\varepsilon_2\M_2 = {\X^*_1}^\top\X_1^* + \varepsilon_1\M_1^\top\X^*_1 + \varepsilon_1\M_1^\top\M_1 + \varepsilon_2\M_2$. 
Thus by choosing $\varepsilon_1, \varepsilon_2$ to be of order $\mathcal{O}(\delta)$we get that $\tilde{\X}_2 = \X^*_2 + \frac{\delta}{C}\|M\|$ for some $C$ chosen to be large enough.
Then for the last step consider the follow (sub-)rows of the matrix $\X$
\begin{equation}
    \begin{bmatrix}
        \ell & * &* &\hdots &*\\
        \emb_1 &\emb_1 &\emb_1 &\hdots &\emb_1\\
        \emb_1 &\emb_2 &\emb_3 &\hdots &\emb_\seqlen
    \end{bmatrix}
\end{equation}
where $\emb_i$ is the binary representation of position $i$. By choosing $\weights_\key,\weights_\query$ as to
\begin{equation}
    \weights_\key\X = \begin{bmatrix}
        \emb_1 &\emb_2 &\hdots &\emb_\seqlen
    \end{bmatrix}, \;\;\;\weights_\query\X = \begin{bmatrix}
        \emb_1 &\emb_1 &\hdots &\emb_1 
    \end{bmatrix} 
\end{equation}
and consider $\weights_\val\X = \begin{bmatrix}
        \ell & * & \hdots &*\\
        \zero &\zero &\hdots &\zero 
    \end{bmatrix}$ we have that 
    \begin{align*}
       \attn(\X) &= \X+ \weights_\val\X \sfm((\weights_\key\X)^\top\weights_\query\X)\\
       &= \X + \begin{bmatrix}
        \ell & * & \hdots &*\\
        \zero &\zero &\hdots &\zero 
    \end{bmatrix} \sfm\left(\begin{bmatrix}
        \emb_1^\top\emb_1 &\emb_1^\top\emb_1 &\hdots &\emb_1^\top\emb_1\\
         \emb_1^\top\emb_2 &\emb_1^\top\emb_2 & \hdots &\emb_1^\top\emb_2 \\
         \vdots &\vdots &\ddots &\vdots\\
         \emb_1^\top\emb_\seqlen &\emb_1^\top\emb_\seqlen &\hdots &\emb_1^\top\emb_\seqlen
    \end{bmatrix}\right)\\
    &= \X+ \begin{bmatrix}
        \ell & * & \hdots &*\\
        \zero &\zero &\hdots &\zero 
    \end{bmatrix}   \begin{bmatrix}
        1 & 1 &\hdots &1 \\
        0 & 0 &\hdots &0\\
        \vdots &\vdots &\hdots &\vdots\\
        0 & 0 &\hdots & 0
    \end{bmatrix} +\varepsilon_3 \rmM_3
    \end{align*}
    By subtracting one identity head for the first that we focus on as described in Lemma \ref{lem:copy} we have that $\attn(\X)$ results in the desired matrix. We output this result and overwrite $\ell/\seqlen$, thus we have
    \begin{equation}
    \arraycolsep = 1.5pt
    \left[\begin{array}{*{12}c}
    \x_1 & \hdots &\s_1^{\ell-1}& \s_1^{\ell}&\hdots & \s_2^{\ell-1} &\s_2^{\ell} &\hdots & \s_{n}^{L} &\xtest &\hdots &\hat\tb^{\ell-1}\\
    \zero &\hdots &\zero  &\zero &\hdots &\zero &\zero &\hdots &\zero &\zero &\hdots &\zero\\
        \hline
     1 & \hdots & \ell & \ell+1& \hdots &\ell &\ell+1 &\hdots &L+1 &1&\hdots & \ell\\
     1 & \hdots & \ell &\ell+1 &\hdots &\ell &\ell+1&\hdots &L+1 &1&\hdots & \ell\\
     \hline
     \seqlen & \hdots & \seqlen &\seqlen&\hdots &\seqlen&\seqlen &\hdots &\seqlen&\seqlen&\hdots & \seqlen\\
   \ell & \hdots & \ell &\ell &\hdots &\ell &\ell &\hdots &\ell &\ell &\hdots &\ell\\
 0 & \hdots & 0 &0&\hdots &0  &0 &\hdots &0 &1 &\hdots & 1\\
1 & \hdots & 1 &1 &\hdots &1&1 &\hdots &1 &1 &\hdots & 1\\ 
\m_1 & \hdots & \m_\ell &\m_{\ell+1} &\hdots &\m_{L+\ell+1} &\m_{L+\ell+2} &\hdots &\m_{n(L+1)} &\m_{n(L+1)+1} &\hdots & \m_{\seqlen}\\
 \end{array}\right]
\end{equation}

The new error introduced by this operation is again controlled as to be $\varepsilon_3\M_3 = \dfrac{\delta}{C}$, with $\|\M_3\|\leq 1$.
    \paragraph{Step 3: Create $\ell+1$ (0 layer). } We first copy the row with $\ell$ to the row with $N$, this can trivially be done with a ReLU layer that outputs zero everywhere else except for the row of $N$s that output $(\ell)_{+} - (N)_{+}$ to account also for the residual. We now use one of the bias terms (notice that $\ell$ is always positive) and set to one in one of the two rows that contain the $\ell$, again we account for the residual as before; everything else remains unchanged. Thus, we have
    \begin{equation}
    \arraycolsep = 1.5pt
    \left[\begin{array}{*{12}c}
    \x_1 & \hdots &\s_1^{\ell-1}& \s_1^{\ell}&\hdots & \s_2^{\ell-1} &\s_2^{\ell} &\hdots & \s_{n}^{L} &\xtest &\hdots &\hat\tb^{\ell-1}\\
    \zero &\hdots &\zero  &\zero &\hdots &\zero &\zero &\hdots &\zero &\zero &\hdots &\zero\\
        \hline
     1 & \hdots & \ell & \ell+1& \hdots &\ell &\ell+1 &\hdots &L+1 &1&\hdots & \ell\\
     1 & \hdots & \ell &\ell+1 &\hdots &\ell &\ell+1&\hdots &L+1 &1&\hdots & \ell\\
     \hline
     \ell+1 & \hdots & \ell+1 &\ell+1&\hdots &\ell+1 &\ell+1 &\hdots &\ell+1 &\ell+1 &\hdots &\ell+1\\
    \ell & \hdots & \ell &\ell &\hdots &\ell &\ell &\hdots &\ell &\ell &\hdots &\ell\\
 0 & \hdots & 0 &0&\hdots &0  &0 &\hdots &0 &1 &\hdots & 1\\
1 & \hdots & 1 &1 &\hdots &1&1 &\hdots &1 &1 &\hdots & 1\\ 
\m_1 & \hdots & \m_\ell &\m_{\ell+1} &\hdots &\m_{L+\ell+1} &\m_{L+\ell+2} &\hdots &\m_{n(L+1)} &\m_{n(L+1)+1} &\hdots & \m_{\seqlen}\\
 \end{array}\right]
\end{equation}
This operation can collectively be implemented (add the bias + copy the row) in the ReLU layer of the previous transformer layer that was not used in the previous step.
    \paragraph{Step 4: Create the binary bits (2 layers). }We will now use the information extracted in the previous steps, to create the binary indicators/bit to identify which tokens we want to filter. This can be easily implemented with one layer of transformer and especially the  ReLU part of it. Notice that if we subtract the row that contains the tokens that have already been predicted, \emph{i.e.,} $[\ell~\ell\hdots~\ell]$ from the row that contains $[1~2\hdots L~1~2\hdots L \hdots L]$ we will get zero only in the positions that we want to filter out and some non-zero quantity in the rest. This is trivially implemented with one ReLU layer. So, we need to implement an if..then type of operation. Basically, if the quantity at hand is zero we want to set the bit to one, while if it non-zero to set it to be zero. This can be implemented with the following ReLU part of a transformer layer 
    \begin{equation}
     \TF(x_i) = 1 - (x_i)_{+}-(-x_i)_{+} + (x_i -1 )_{+} +(-x_i -1)_{+} - ((x_i)_{+} - (-x_i)_{+})
    \end{equation}
    the last two terms are to account for the residual. Again the rest of the rows do not change and are zeroed-out. 
    
    \textbf{Step 5: Implement the filtering (1 layer).}  We now apply Lemma \ref{lem:binary-app} and our proof is completed. In this step as in Lemma \ref{lem:binary-app}, the error remains of the order of the error of the previous step. Thus, by fine-tuning the constants appropriately, depending on 1) the bound on the input as of Assumption \ref{asm:bounded}, the targeted error $\delta$ and the constant used in Lemma \ref{lem:binary-app} we achieve that the error has the target upped bound.
\end{proof}

\begin{theorem}[Theorem~\ref{thm:MLP} restated] Consider a prompt $\pmt_n(f)$ generated from an $L$-layer MLP $f(\cdot)$ as described in Definition \ref{MLP assump}, and assume given test example $(\xtest,\tb^1_{\text{\tiny test}}, \dots\tb^L_{\text{\tiny test}})$. 
% , containing $n$ examples and ends with $\x^{\texttt{test}}$. 
For any resolution $\eps>0$, there exists $\delta=\delta(\eps)$, iteration choice $T={\cal{O}}(\kappa_{\max}^2\log(1/\eps))$, and a backend transformer construction $\TFBE$ such that the concatenated transformer $\TF=\TFLR \circ \TFBE$ implements the following: Let $(\tht^{i})_{i=1}^{\ell-1}$ denote the first $\ell-1$ $\COT$ outputs of $\TF$ and set $\pb[\ell]=(\pb_n(f),\xtest,\tht^{1}\dots\tht^{\ell-1})$. At step $\ell$, $\TF$ implements
\begin{enumerate}
\item \textbf{Filtering.} Define the filtered prompt with input/output features of layer $\ell$,
\[
\arraycolsep = 1pt
\pbf_n=\left(\begin{array}{*{10}c}
\hdots \zero,&\tb^{\ell-1}_{1},&\zero&\hdots&\zero,&\tb^{\ell-1}_n, &\zero&\hdots&\zero,&\tht^{\ell-1}\\
\hdots\zero,&\zero,& \tb^{\ell}_{1}&\dots&\zero,&\zero,& \tb^{\ell}_n&\dots&\zero,&\zero\end{array}\right).
\]
There exists a fixed projection matrix $\bPi$ that applies individually on tokens such that the backend output obeys $\tn{\bPi(\TFBE(\pb[\ell]))-\pbf_n}\leq \delta$. %The more precise statement is provided in Lemma \ref{lem:filtering}. % up to $\eps$ accuracy via a fixed linear projection. 
\item \textbf{Gradient descent.} The combined model obeys $\tn{\TF(\pb[\ell])-\tb_{\text{\tiny test}}^{\ell}}\leq {\ell\cdot \eps}/{L}$.
\end{enumerate}
$\TFBE$ has constant number of layers independent of $T$ and $n$. Consequently, after $L$ rounds of $\COT$, \TF outputs $f(\xtest)$ up to $\eps$ accuracy.
\end{theorem}
\begin{proof}
    We apply Lemma \ref{lem:filtering-app} from which it is clear that there exists a projection such that the result stated in (1. Filtering) holds, and it is independent to $T$, $n$ and $\ell$. Next we turn to prove (2. Gradient descent). 
    In Definition~\ref{MLP assump}, we assume that the network's activation function is leaky-ReLU, \emph{i.e.,} 
\begin{equation}
     \phi(x) =   \left\{\begin{matrix}
 x,& \text{ if }x\geq 0 \\ 
 \alpha x,& \text{ otherwise.} 
\end{matrix}\right.
    \end{equation}
    Thus, as a first step we construct the inverse of leaky-ReLU and apply it in the second row of $\p_n^{\text{filter}}$ where the inverse of leaky-ReLU is 
    \begin{equation}
         \phi^{-1}(y) =   \left\{\begin{matrix}
 y,& \text{ if }y\geq 0 \\ 
y/\alpha,& \text{ otherwise.} 
\end{matrix}\right.
    \end{equation}
    This can be implemented with the following activation function (denoted by $\sigma(\cdot)$) using ReLUs:
    \begin{equation}
        \sigma(x) = (x)_+ - 1/\alpha (-x)_+.
    \end{equation}
    After it, it remains $\TFLR$ to solve linear regression problems. Taking $\ell$th layer, first neuron prediction as an example, and letting $\x'_i:=\tb_i^{\ell-1}$, $y'_i:=\phi^{-1}(\tb_i^{\ell}[0])$ and $\w=\W_\ell[0]$, linear regression has form of $y'_i=\w^\top\x'_i$ for $i\in[n]$. Notice that the extra zeros do not contribute in the update performed by gradient descent, and after gradient descent has been performed, we apply back the leaky ReLU. Then 
    following  Assumption~\ref{assume oracle}, since we assume $\TFLR$ performs the same as gradient descent optimizer, given matrix condition as described in Definition~\ref{MLP assump}, after running $T$ iterations of gradient descend on the linear regression problem and considering each layer prediction with resolution $\eps/L$, we can get that $\|\TFLR(\pmt[\ell])-\bar\tb^\ell\|\leq\eps/L$, where $\bar\tb^\ell=\phi(\W_\ell\hat\tb^{\ell-1})$ is the correct prediction if taking $\hat\tb^{\ell-1}$ as input. Then we have 
    \[
    \|\TFLR(\pmt[\ell]-\tbt^\ell)\|\leq\|\TFLR(\pmt[\ell])-\bar\tb^\ell\|+\|\W_\ell(\hat\tb^{\ell-1}-\tbt^{\ell-1})\|\lesssim\eps/L+\|\TFLR(\pmt[\ell-1]-\tbt^{\ell-1})\|.
    \]
    Let $\TFLR(\pmt[0])$ returns $\xtest$ and therefore $\|\TFLR(\pmt[0])-\xtest\|=0$. Combing results in that  $\|\TFLR(\pmt[\ell]-\tbt^\ell)\|\lesssim\ell\cdot\eps/L$. 
    Since from Lemma \ref{lem:filtering-app} we have that we can choose $\delta$ to be arbitrary. Let $\delta = \eps/L$, where $L$ is the total predictions we will make. Then it will result in $\|\TF(\pmt[\ell]-\tbt^\ell)\|\lesssim\ell\cdot\eps/L$, which completes the proof.
    
    % ; then from Assumption \ref{assume oracle} we run gradient descend on the input. 
    
    % We then apply this layer  to the labels as already mentioned. As a final step we add the two rows and use Assumption \ref{assume oracle} to run gradient descent. Notice that the extra zeros do not contribute in the update performed by gradient descent. After gradient descent has been performed, we apply back the leaky ReLU.  For the error bound, fix $\eps > 0$, from Lemma \ref{lem:filtering-app} we have that we can choose $\delta$ to be arbitrary. Let $\delta = \eps/L$, where $L$ is the total predictions we will make. Since from Assumption \ref{assume oracle} we do not induce any extra error, the error after $\ell$ predictions will be $\ell \delta = \ell\eps/L$.
\end{proof}



% \begin{lemma}[Filtering]\label{lem:filtering-app}
    
% \end{lemma}
% \begin{lemma}[Skills] Consider an input of the form
% \begin{equation}
%     \X = \begin{bmatrix}
%         \x_1 &\x_2 &\hdots &\x_n &\x\\
%         \s_{f_1} &\s_{f_2} &\hdots &\s_{f_n} &\s_k\\
%         \emb_1 &\emb_2 &\hdots &\emb_n &\emb_{n+1}
%     \end{bmatrix}
% \end{equation}
%  Then there exists a transformer $\TF$ with  five layers with output
%  \begin{equation}
%      \TF(\X) = \begin{bmatrix}
%          \one_{\{\s_{f_1} = \s_k\}}\x_1 &\one_{\{\s_{f_2} = \s_k\}}\x_2 &\hdots &\one_{\{\s_{f_n} = \s_k\}}\x_n &\x\\
%         \s_{f_1} &\s_{f_2} &\hdots &\s_{f_n} &\s_k\\
%         \emb_1 &\emb_2 &\hdots &\emb_n &\emb_{n+1}
%      \end{bmatrix}
%  \end{equation}
% \end{lemma}
% \begin{proof}
%     \begin{enumerate}
%         \item Use $\emb_i$ create one line that has everywhere $n+1$ like in lemma 1. 
%         \item Create the $\emb_{n+1}$ everywhere. 
%         \item Use this and the classic embeddings and copy everyehre the skill $\s_k$. 
%         \item Subtract the skill 
%     \end{enumerate}
%\end{proof}
% Our implementation of filtering is divided in two parts. In the first part we show how the filtering can be performed, given the appropriate encodings. In the second part we will show how we can perform some preprocessing to generalize this operation to any iteration, given always encodings of a specific form. The second part is to demonstrate that as it holds in practice we don't require to change the encodings to perform the filtering at each one of the iterations \AG{I will rephrase this}. 

% For the first lemma, we consider the more general setting in which the data are given in a possibly random order attached with an indicator vector that defines which is their actual position as explained in \AG{Mention the section in which we explain this setting.}
% \begin{lemma}
%     Assume that the input to a transformer after the embedding layer is of the following form 
%     \begin{equation}
%         \X = \begin{bmatrix}
%             \x_1&\x_2&\hdots &\x_{n-1}&\x_n\\
%             \emb_1 &\emb_2 &\hdots&\emb_{n-1} &\emb_n\\
%             \emb_{f_1}&\emb_{f_2}&\hdots &\zero &\zero\\
%             1 & 1 &\hdots & 0 & 0\\
%             \zero &\zero &\hdots &\zero &\zero\\
%             \zero &\zero &\hdots &\zero &\zero
%         \end{bmatrix}
%     \end{equation}
%     where $\x_i\in\R^{d'}$ $\emb_i$, $i=1,\hdots,n$ is the positional encoding as described in subsection \ref{sub:pencodings} for the $i$-th position and $\emb_{f_i}$, $i=1,\hdots, k$ is the encoding of the position we want to filter. If $k\leq n$ then we are given zeroes afterwards. Then there exists one layer of transformer $\TF$ such that 
%     \begin{equation}
%         \TF(\X) = \begin{bmatrix}
%             \x_1&\x_2&\hdots &\x_{n-1}&\x_n\\
%             \emb_1 &\emb_2 &\hdots&\emb_{n-1} &\emb_n\\
%             \emb_{f_1}&\emb_{f_2}&\hdots &\zero &\zero\\
%                         1 & 1 &\hdots & 0 & 0\\
%                         \zero &\zero &\hdots &\zero &\zero\\
%             \x_{f_1}&\x_{f_2}&\hdots &\zero &\zero
%         \end{bmatrix}
%     \end{equation}
% \end{lemma}
% \begin{proof}
% Notice that the dimension of the input is $d = 3d' + 2e $, where $e$ is the dimension of the positional encodings that the model has chosen. Let
%     \begin{equation}
%         \W_\key = \begin{bmatrix}
%             \zero_{d'} &
%             \Iden_{e} & \zero_{2d'+e}            
%         \end{bmatrix}, \W_\query = \begin{bmatrix}
%             \zero_{d'+e} &
%             \Iden_{e} & \zero_{2d'}            
%         \end{bmatrix}
%     \end{equation}
%     we have that 
%    \renewcommand{\arraystretch}{1.5}
%     \begin{align}
%     \arraycolsep=0.1pt
%         \sfm((\W_\key\X)^\top(\W_\query\X)) &= \sfm(\begin{bmatrix}
%             \emb_1^\top\emb_{f_1} &\emb_1^\top\emb_{f_2}&\hdots &\zero\\
%            \emb_2^\top\emb_{f_1} &\emb_2^\top\emb_{f_2}&\hdots &\zero\\
%            \vdots &\vdots &\ddots &\vdots\\
%            \emb_n^\top\emb_{f_1} &\emb_n^\top\emb_{f_2}&\hdots &\zero\\
%         \end{bmatrix})\\
%         &= \begin{bmatrix}
%             \dfrac{ \exp(\lambda\emb_1^\top\emb_{f_1})} {\sum_{i=1}^n\exp( \lambda\emb_i^\top\emb_{f_1})}&\hdots &\dfrac{1}{n}\\
%             \vdots &\hdots &\vdots \\
%              \dfrac{ \exp(\lambda\emb_n^\top\emb_{f_1})} {\sum_{i=1}^n\exp(\lambda \emb_i^\top\emb_{f_1})}&\hdots &\dfrac{1}{n}
%         \end{bmatrix}
%     \end{align}
%     Notice that for the columns that we had non-zeros the above matrix becomes a permutation matrix (as $\lambda\to\infty$ ) with $1$ at the $f_i$-th position of each column $i$. For example, for the first column we will have one in the $f_1$-th row. After this permutation of the identity matrix ( plus some error matrix, which can have arbitrarily small norm by tuning the temperature) is multiplied with $\X$ and by letting 
%     \begin{equation}
%         \W_\val = \begin{bmatrix}
%         \zero & \zero &\zero &\zero &\zero \\
%         \zero & \zero &\zero &\zero &\zero \\
%         \zero & \zero &\zero &\zero &\zero \\
%        \zero & \zero &\zero &\zero &\zero \\
%         \Iden_{d'} & \zero &\zero &\zero &\zero\\
%         \zero & \zero &\zero &\zero &\zero 
%     \end{bmatrix}
%     \end{equation}
%    Thus, the output of the attention becomes
%     \begin{align}
%         \attn(\X) &=  \begin{bmatrix}
%             \x_1&\x_2&\hdots &\x_{n-1}&\x_n\\
%             \emb_1 &\emb_2 &\hdots&\emb_{n-1} &\emb_n\\
%             \emb_{f_1}&\emb_{f_2}&\hdots &\zero &\zero\\
%                         1 & 1 &\hdots & 0 & 0\\
%             \x_{f_1}&\x_{f_2}&\hdots &* &*\\
%             \zero &\zero &\hdots &\zero &\zero 
%         \end{bmatrix}
%         \end{align}
%     where * denotes inconsequential values. We then use the ReLU layers to move the result in the last rows and substitute * with zeros. To do so we follow the construction of \cite{}; specifically we use the fourth row of ones and zeros, which indicates which columns should be updated and which not. For this we have that 
%     \begin{equation}
%         \TF(\X) = \X + \W_2\relu{\W_1\X}
%     \end{equation}
%     Then we set $\W_1, \W_2$ as to output zero in the first four set of rows. For the last set of rows we have \AG{Will add here the relu construction. But this proof is completed}... Thus,
%     \begin{equation}
%         \TF(\X) = \begin{bmatrix}
%             \x_1&\x_2&\hdots &\x_{n-1}&\x_n\\
%             \emb_1 &\emb_2 &\hdots&\emb_{n-1} &\emb_n\\
%             \emb_{f_1}&\emb_{f_2}&\hdots &\zero &\zero\\
%                         1 & 1 &\hdots & 0 & 0\\
%                         \zero &\zero &\hdots &\zero &\zero\\
%             \x_{f_1}&\x_{f_2}&\hdots &\zero &\zero
%         \end{bmatrix}
%     \end{equation}
%     and the proof is completed.
% \end{proof}







% We now continue to show how a transformer can predict 
% The following lemma states that transformers can implement the step of filtering. For simplicity we consider that we have just two intermediate steps and that  the model will predict the second step. It would be easy then to see that this construction can be generalized to multiple intermediate steps and implement a specific step each time depending on the given input.
% \begin{lemma} 

% \end{lemma}
% \begin{proof}
% We consider the following set-up: 
% The user gives an input of the form $\rmI = \begin{bmatrix}
%         \dpoint_1 &\prompt{1}{1} &\prompt{1}{2} \hdots &  \prompt{1}{\layer} &\hdots &\dpoint_n &\prompt{n}{1} &\hdots &\prompt{n}{\layer} &\dpoint_{\text{test}}
% \end{bmatrix}$.

% After the embedding layer the input is transformed as follows: 
%  \renewcommand{\arraystretch}{1.7}
% \begin{equation*}
% \arraycolsep=1.5pt
%    \rmI = \left[\begin{array}{*{11}c}
%     \dpoint_1 &\prompt{1}{1} &\prompt{1}{2}& \hdots &  \prompt{1}{\layer} &\hdots &\dpoint_n &\prompt{n}{1} &\hdots &\prompt{n}{\layer} &\dpoint_{\text{test}}\\
%     \zero &\zero &\zero&\hdots &\zero &\hdots &\zero &\zero &\hdots &\zero &\zero \\
%     \emb_0 &\emb_{L+1} &\emb_2 &\hdots &\emb_{\layer} &\hdots& \emb_{(n-1)(\layer + 1)+1} &\emb_{(n-1)(\layer+1)+ 2} &\hdots &\emb_{\seqlen-2}&\emb_{\seqlen-1}\\
%     \emb_0 & \emb_{\layer+1} &\emb_{2\layer+1} &\hdots & \emb_{f(\layer)}&\hdots& \emb_{f((n-1)(\layer + 1)+1)} & \emb_{f((n-1)(\layer+1)+ 2)}&\hdots &\emb_{f(\seqlen-1)}&\emb_{f(\seqlen)}\\
%      \text{!!!!} & \emb_{\layer+1} &\emb_{2\layer+1} &\hdots & \emb_{f(\layer)}&\hdots& \emb_{f((n-1)(\layer + 1)+1)} & \emb_{f((n-1)(\layer+1)+ 2)}&\hdots &\emb_{f(\seqlen-1)}&\emb_{f(\seqlen)}\\
%     1 & 2 &3&\hdots &\layer+1 &\hdots& (n-1)\layer + n &(n-1)\layer + n+1 &\hdots &\seqlen-1 &\seqlen\\ 
%      \ln(1) & \ln(2) & \ln(3)&\hdots &\ln(\layer+1) &\hdots& \ln((n-1)\layer + n) &\ln((n-1)\layer + n+1 )&\hdots &\ln(\seqlen-1) &\ln(\seqlen)\\ 
%      1 & 1 &1 &\hdots &1 &\hdots &1 &1 &\hdots &1 &1 \\ 
%      0 & 0&0&\hdots &0 &\hdots &0 &0 &\hdots &0 &0
%     \end{array} 
%     \right]
% \end{equation*}
% where $\seqlen$ is the sequence length, (write the function***)$f(x) =...$. Also, the second row is a block of rows set to zero, which will be used for storing necessary intermediate results.

% \noindent\textbf{Step 1: Extract the number of tokens.} Let 
% \begin{align}
% \weights_{\key}= \begin{bmatrix}
%     \zero &\zero &\zero &\zero &\zero &0 &1 &0 &0 
% \end{bmatrix} 
%  \;\;\; \weights_{\query} =  \begin{bmatrix}
%     \zero &\zero &\zero &\zero &\zero &0 &0 &1 &0 
% \end{bmatrix}
% \end{align}
% and thus 
% \begin{equation}
%     (\weights_{\key}\rmI)^\top(\weights_{\query}\rmI) = \begin{bmatrix}
%         \ln(1) &\ln(1) &\hdots &\ln(1)\\
%         \ln(2) &\ln(2) &\hdots &\ln(2)\\
%         \vdots &\vdots &\ddots &\vdots\\
%         \ln(\seqlen) &\ln(\seqlen) &\hdots &\ln(\seqlen)\\
%     \end{bmatrix}
% \end{equation}
% So after the softmax is applied we have
% \begin{equation}
%     \softmax((\weights_{\key}\rmI)^\top(\weights_{\query}\rmI)) = \begin{bmatrix}
%         \dfrac{1}{\sum_{i=1}^\seqlen i} &\dfrac{1}{\sum_{i=1}^\seqlen i}&\hdots &\dfrac{1}{\sum_{i=1}^\seqlen i}\\
%         \dfrac{2}{\sum_{i=1}^\seqlen i} &\dfrac{2}{\sum_{i=1}^\seqlen i} &\hdots &\dfrac{2}{\sum_{i=1}^\seqlen i}\\
%         \vdots &\vdots &\ddots &\vdots\\
%         \dfrac{\seqlen}{\sum_{i=1}^\seqlen i} &\dfrac{\seqlen}{\sum_{i=1}^\seqlen i}  &\hdots &\dfrac{\seqlen}{\sum_{i=1}^\seqlen i} \\
%     \end{bmatrix}
% \end{equation}
% We then set the weight value matrix as to zero-out all lines except for one line as follows
% \begin{equation}
%    \weights_{\val}\rmI =\begin{bmatrix}
%    \zero &\zero & \hdots &\zero \\
%     1 & 2 &\hdots &\seqlen\\
%  \zero &\zero &\hdots &\zero 
%    \end{bmatrix}
% \end{equation}
% % \begin{equation}
% %    \weights_{\val}\rmI =\begin{bmatrix}
% %    \zero &\zero & \hdots &\zero \\
% %   \zero &\zero & \hdots &\zero \\
% %     \zero &\zero & \hdots &\zero \\
% %     \zero &\zero & \hdots &\zero \\
% %     1 & 2 &\hdots &\seqlen\\
% %     0 &0 &\hdots &0\\
% %      0 &0 &\hdots &0\\
% %        0 &0 &\hdots &0
% %    \end{bmatrix}
% % \end{equation}
% After adding the residual this results to 
% \begin{equation*}
%     \arraycolsep=1.5pt
%    \rmI = \left[\begin{array}{*{11}c}
%     \dpoint_1 &\prompt{1}{1} &\prompt{1}{2}& \hdots &  \prompt{1}{\layer} &\hdots &\dpoint_n &\prompt{n}{1} &\hdots &\prompt{n}{\layer} &\dpoint_{\text{test}}\\
%     \zero &\zero &\zero&\hdots &\zero &\hdots &\zero &\zero &\hdots &\zero &\zero \\
%     \emb_0 &\emb_{1} &\emb_2 &\hdots &\emb_{\layer} &\hdots& \emb_{(n-1)(\layer + 1)+1} &\emb_{(n-1)(\layer+1)+ 2} &\hdots &\emb_{\seqlen-2}&\emb_{\seqlen-1}\\
%     \emb_0 & \emb_{\layer+1} &\emb_{2\layer+1} &\hdots & \emb_{f(\layer)}&\hdots& \emb_{f((n-1)(\layer + 1)+1)} & \emb_{f((n-1)(\layer+1)+ 2)}&\hdots &\emb_{f(\seqlen-1)}&\emb_{f(\seqlen)}\\
%      \text{!!!!} & \emb_{\layer+1} &\emb_{2\layer+1} &\hdots & \emb_{f(\layer)}&\hdots& \emb_{f((n-1)(\layer + 1)+1)} & \emb_{f((n-1)(\layer+1)+ 2)}&\hdots &\emb_{f(\seqlen-1)}&\emb_{f(\seqlen)}\\
%     \dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i} & \dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i} &\dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i}&\hdots &\dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i}&\hdots& \dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i}&\dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i} &\hdots &\dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i} &\dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i}\\ 
%      \ln(1) & \ln(2) & \ln(3)&\hdots &\ln(\layer+1) &\hdots& \ln((n-1)\layer + n) &\ln((n-1)\layer + n+1 )&\hdots &\ln(\seqlen-1) &\ln(\seqlen)\\ 
%      1 & 1 &1 &\hdots &1 &\hdots &1 &1 &\hdots &1 &1 \\ 
%      0 & 0&0&\hdots &0 &\hdots &0 &0 &\hdots &0 &0
%     \end{array} 
%     \right]
% \end{equation*}
% However, notice that $\dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i} = \dfrac{2\seqlen(\seqlen+1)(2\seqlen+1)}{6\seqlen(\seqlen+1)} = \dfrac{2\seqlen+1}{3}$. We then use the ReLU layer as to multiply with $3/2$ and subtract $1/3$ from this column. This results to 
% \begin{equation*}
%     \arraycolsep=1.5pt
%    \rmI = \left[\begin{array}{*{11}c}
%     \dpoint_1 &\prompt{1}{1} &\prompt{1}{2}& \hdots &  \prompt{1}{\layer} &\hdots &\dpoint_n &\prompt{n}{1} &\hdots &\prompt{n}{\layer} &\dpoint_{\text{test}}\\
%     \zero &\zero &\zero&\hdots &\zero &\hdots &\zero &\zero &\hdots &\zero &\zero \\
%     \emb_0 &\emb_{1} &\emb_2 &\hdots &\emb_{\layer} &\hdots& \emb_{(n-1)(\layer + 1)+1} &\emb_{(n-1)(\layer+1)+ 2} &\hdots &\emb_{\seqlen-2}&\emb_{\seqlen-1}\\
%     \emb_0 & \emb_{\layer+1} &\emb_{2\layer+1} &\hdots & \emb_{f(\layer)}&\hdots& \emb_{f((n-1)(\layer + 1)+1)} & \emb_{f((n-1)(\layer+1)+ 2)}&\hdots &\emb_{f(\seqlen-1)}&\emb_{f(\seqlen)}\\
%      \text{!!!!} & \emb_{\layer+1} &\emb_{2\layer+1} &\hdots & \emb_{f(\layer)}&\hdots& \emb_{f((n-1)(\layer + 1)+1)} & \emb_{f((n-1)(\layer+1)+ 2)}&\hdots &\emb_{f(\seqlen-1)}&\emb_{f(\seqlen)}\\
%     \seqlen&  \seqlen& \seqlen&\hdots & \seqlen&\hdots&  \seqlen& \seqlen &\hdots & \seqlen & \seqlen\\ 
%      \ln(1) & \ln(2) & \ln(3)&\hdots &\ln(\layer+1) &\hdots& \ln((n-1)\layer + n) &\ln((n-1)\layer + n+1 )&\hdots &\ln(\seqlen-1) &\ln(\seqlen)\\ 
%      1 & 1 &1 &\hdots &1 &\hdots &1 &1 &\hdots &1 &1 \\ 
%      0 & 0&0&\hdots &0 &\hdots &0 &0 &\hdots &0 &0
%     \end{array} 
%     \right]
% \end{equation*}
% \noindent\textbf{Step 2: Create the positional encodings for $\seqlen$.}
% This step is implemented by \textcolor{orange}{Lemma}. Now output is
% \begin{equation*}
%     \arraycolsep=1.5pt
%    \rmI = \left[\begin{array}{*{11}c}
%     \dpoint_1 &\prompt{1}{1} &\prompt{1}{2}& \hdots &  \prompt{1}{\layer} &\hdots &\dpoint_n &\prompt{n}{1} &\hdots &\prompt{n}{\layer} &\dpoint_{\text{test}}\\
%     \zero &\zero &\zero&\hdots &\zero &\hdots &\zero &\zero &\hdots &\zero &\zero \\
%     \emb_{\seqlen} &\emb_{\seqlen} &\emb_{\seqlen}&\hdots &\emb_{\seqlen} &\hdots &\emb_{\seqlen} &\emb_{\seqlen} &\hdots &\emb_{\seqlen} &\emb_{\seqlen} \\
%     \emb_0 &\emb_{1} &\emb_2 &\hdots &\emb_{\layer} &\hdots& \emb_{(n-1)(\layer + 1)+1} &\emb_{(n-1)(\layer+1)+ 2} &\hdots &\emb_{\seqlen-2}&\emb_{\seqlen-1}\\
%     \emb_0 & \emb_{\layer+1} &\emb_{2\layer+1} &\hdots & \emb_{f(\layer)}&\hdots& \emb_{f((n-1)(\layer + 1)+1)} & \emb_{f((n-1)(\layer+1)+ 2)}&\hdots &\emb_{f(\seqlen-1)}&\emb_{f(\seqlen)}\\
%      \text{!!!!} & \emb_{\layer+1} &\emb_{2\layer+1} &\hdots & \emb_{f(\layer)}&\hdots& \emb_{f((n-1)(\layer + 1)+1)} & \emb_{f((n-1)(\layer+1)+ 2)}&\hdots &\emb_{f(\seqlen-1)}&\emb_{f(\seqlen)}\\
%     \seqlen&  \seqlen& \seqlen&\hdots & \seqlen&\hdots&  \seqlen& \seqlen &\hdots & \seqlen & \seqlen\\ 
%      \ln(1) & \ln(2) & \ln(3)&\hdots &\ln(\layer+1) &\hdots& \ln((n-1)\layer + n) &\ln((n-1)\layer + n+1 )&\hdots &\ln(\seqlen-1) &\ln(\seqlen)\\ 
%      1 & 1 &1 &\hdots &1 &\hdots &1 &1 &\hdots &1 &1 \\ 
%      0 & 0&0&\hdots &0 &\hdots &0 &0 &\hdots &0 &0
%     \end{array} 
%     \right]
% \end{equation*}
% \textcolor{orange}{We need to create the encodings of max length.}
% \end{proof}

==> backup/sec/construction_v2.tex <==
\section{Construction}
\subsection{The transformer architecture. }\label{ss:transformer}
For the purpose of this proof, we consider encoder-based transformer architectures; we assume that the positional encodings are appended to the input\footnote{We note here that in terms of our construction adding the encodings or appending them to the input can be viewed in a similar manner. Specifically, we can consider that the up-projection step projects the input to  zero padded vectors, while the encodings are orthogonal to that projection in the sense that the have zero in the non-zero coordinates of the input. In that case adding the positional encodings  corresponds to appending them to the input. }. We also consider that the heds are added and each one has each own key, query and value weight matrices. Formally, we have 
\begin{align}\label{eq:transformer}
    \attn(\X) &= \X + \sum_{h=1}^H\weights^h_\val\X\sfm((\weights^h_\key\X)^\top\weights^h_\query\X)\\
    \TF(\X) &= \attn(\X) + \weights_2(\weights_1\attn(\X) +\vb_1\one_n)_{+} +\vb_2\one_n
\end{align}
where $\X\in\R^{d\times n}$, $H$ is the number of heads used and $f(x) = (x)_{+}$ is the ReLU function. We also make use of the temperature $\lambda$, which is a parameter of the softmax. Specifically, $\sfm(\x) = \{\e^{\lambda x_i}/\sum_j\e^{\lambda x_j}\}_{i}$. Notice that as $\lambda\to\infty$ we have $\sfm(\x)\to \max_i x_i$. We also assume that the inputs are bounded; we denote with $N_{max}$ the maximum sequence length of the model.
\begin{assumption}Each entry is bounded by some constant $c$, which implies that  $\|\X\|\leq c'$, for some large $c'$ that depends on the maximum sequence length and the width of the transformer.
\end{assumption}
\subsection{The positional encodings}\label{ss:pencodings} In the constructions below we use a combination of the binary representation of each position as well as some more information mentioned in the sections to follow. The binary representations, as well the encodings we construct,  require only logarithmic space with respect to the sequence length. Notice that binary representation of the positions satisfy the following two conditions:
\begin{enumerate}
    \item Let $\emb_i$ be the binary representation of the $i$-th position, then there exists $\varepsilon > 0$ such that $\emb_i^\top\emb_i > \emb_i^\top\emb_j +\varepsilon$ for all $j\neq i$.
    \item There exists a one layer transformer that can implement the addition of two pointers (see Lemma \ref{lem:addition} ).
\end{enumerate}%We note here that any choice of encodings could be made that satisfy the following two conditions: 
% \begin{assumption}\label{asm:distinct}
%     Let $\emb_i$ be the encoding of the $i$-th position, then there exists $\varepsilon > 0$ such that $\emb_i^\top\emb_i > \emb_i^\top\emb_j +\varepsilon$ for all $j\neq i$. 
% \end{assumption} 
% \begin{assumption}\label{asm:increasing}
%     There exists an operator $*$ that the transformer can implement in one layer (or constant layers) such that $\emb_i *\emb_j  =\emb_{i+j}$.
% \end{assumption}
% We note here that multiple choices of positional encodings satisfy these two assumptions. For example, \cite{..} have used binary positional encodings

One useful fact about the encodings is that as 
\subsection{``Black-box'' functions}
We follow the construction of \cite{giannou2023looped}  and we use the following individual implementations as they are. We repeat the statements here for convenience.
\begin{lemma}\label{lem:copy}
A transformer with one layer, one head, and width of $O(\log n +d)$, where $d$ is the dimension of the data vectors and $n$ is the length of the input, can read data/command vectors from the input to the scratchpad from the location pointed to by the position embedding vector in the scratchpad.
\end{lemma}
\begin{remark} For the idea on how this is possible we illustrate a simple example. Assume that $\seqlen=5$ and we want to copy and element from position (1,2) where the first element signifies the row and the second the column to position (3,5). The first step is to copy the second column to the fifth one; to do so we force the softmax matrix to acts as a permutation matrix, \emph{i.e.,} $[\ve_1\;\ve_2\;\ve_3\;\ve_4\;\ve_2]$ where $\ve_i$ is the one hot vector for the $i$-th row. This is achieved by the bianary representations by using as $\weights_\key\X = [\emb_1\;\hdots\;\emb_5]$, $\weights_\query\X = [\emb_1\;\hdots\;\emb_2]$ and by using $\lambda$ large enough the result follows. Then, we use a value matrix that only keeps the row $1$ and permutes it to the row 3. Finally, to account for the residual, we use an extra head, which softmax is approximately the identity and the value weight matrix is zero expect for the first row which is again permuted to the third one. This description follows the construction of \cite{akyurek2022learning}.
\end{remark}
\begin{lemma}\label{lem:addition}
   There exists a 1-hidden layer feedforward, ReLU network, with $8d$ activations in the hidden layer and $d$ neurons in the output layer that when given two $d$-dimensional binary vectors representing two non-negative integers, can output the binary vector representation of their sum, as long as the sum is less than $2^{d+1}$. 
   % Further, there is a special bit indicator that is 1 for the scratchpad and 0 for the rest of the input. If this bit is 1 then the operation above is performed, otherwise 0 is returned.
\end{lemma}
\begin{lemma}\label{lem:transpose}
Fix $\epsilon >0$ and consider an input of the following form
\begin{equation}
    \X = \left[\begin{array}{c|c|c|cc}
        \rmA  &\zero&\zero &\dots & \zero \\
 \zero&      \zero&\zero &\dots & \zero\\
         \emb_{1:d}&\emb_{1:d}&\emb_{1:d}& \dots  &\emb_{1:d}\\
         \rmP_1'&\rmP_{2}'&\rmP_{3}'& \dots  &\rmP_{d}'
    \end{array}\right]. \nonumber
\end{equation}
where $\rmA\in\R^{d\times d}$; then there exists transformer-based function block with 4 layers, 1 head and dimensionality $r = 2d+2\log d = O(d)$ that outputs the following matrix
\begin{equation}
    \X = \left[\begin{array}{c|c|c|cc}
\rmA' &\rmA'&\rmA'&\dots &\rmA' \\
        \zero&\zero&\zero &\dots &\zero \\
         \emb_{1:d}& \emb_{1:d}& \emb_{1:d}& \dots &\emb_{1:d} \\
        \rmP_1'&\rmP_{2}'&\rmP_{3}'& \dots  &\rmP_{d}'
    \end{array}\right]. \nonumber
\end{equation}
where $\rmA' = \rmA^\top +\epsilon\rmM$, for some $\|\rmM\|\leq 1$. The error $\epsilon$ depends on the choice of the temperature $\lambda$, as it is  a consequence of the \texttt{read/write} operations.
\end{lemma}
\begin{lemma}\label{lem:matrixmul_app}
Let $\rmA\in \R^{k\times m}$ and $\rmB \in \R^{k\times n}$; then for any $\epsilon >0$ there exists a transformer-based function block with  2 layers, 1 head and dimensionality $r = O(d)$ that  outputs the multiplication $\rmA^T\rmB^T +\eps\rmM$, for some $\|\rmM\|\leq 1$ .
\end{lemma}
\begin{remark}
    Notice that based on the proof of this lemma, the matrices/scalars/vectors need to be in the same rows, \emph{i.e.},
$\begin{bmatrix}
          \rmQ =  \rmA &\rmB 
        \end{bmatrix}
$. By also appending the appropriate binary encodings we can move the output in any specific place we choose as in Lemma \ref{lem:copy}. Also, following the proof of the paper the input matrix is actually 
\begin{equation*}
    \X = \begin{bmatrix}
        \rmQ& \zero &\zero \\
        \zero & \one\one^{\top} &\zero\\
        \Iden&\zero &\zero\\ 
        &\emb^{(1)}&\\
        &\emb^{(2)}&\\
        %\zero &\one^{\top} &\zero 
    \end{bmatrix}  
\end{equation*} 
where $\emb^{(1)}, \emb^{(2)}$ are chosen as in Lemma \ref{lem:copy} to specify the position of the result.
\end{remark}
\subsection{Filtering}\label{ss filtering}
\begin{lemma}\label{lem:zeroout-app}
    Assume that the input to a transformer layer is of the following form
    \begin{equation}
        \X = \begin{bmatrix}
            \x_1 &\x_2 &\hdots&\x_{n-1} &\x_n\\
            \zero &\zero &\hdots &\zero &\zero\\
        b_1 & b_2 & \hdots &b_{n-1} &b_n\\
        b_1' &b_2' &\hdots &b_{n-1}' &b_n
        \end{bmatrix}
    \end{equation}
    where $b_i,b_i'\in\{0,1\}$, with zero indicating that the corresponding point should be ignored. Then there exists a transformer $\TF$ consisting only of a ReLU layer that performs this filtering, \textit{i.e.}, 
    \begin{equation}
        \TF(\X) = \begin{bmatrix}
           \one\{b_1\neq 0\}\x_1&\one\{b_2\neq 0\}\x_2 &\hdots &\one\{b_{n-1}\neq 0\}\x_{n-1} &\one\{b_n\neq 0\}\x_n\\
            \one\{b_1'\neq 0\}\x_1&\one\{b_2'\neq 0\}\x_2 &\hdots &\one\{b_{n-1}'\neq 0\}\x_{n-1} &\one\{b_n'\neq 0\}\x_n\\
            b_1 & b_2 & \hdots &b_{n-1} &b_n\\
            b_1' &b_2' &\hdots &b_{n-1}' &b_n
        \end{bmatrix}
    \end{equation}
\end{lemma}
\begin{proof}
    The layer is the following:
    \begin{equation}
       \TF(\x_i) = x_i + (-Cb_i - \x_i)_+ - (-Cb_i + \x_i)_+
    \end{equation}
    for some large constant $C$. Notice that if $b_i =1$ the output is just $\x_i$. But if $b_i = 0$ then the output is zero. For the second set instead of using the bits $b_i$,  we use the $b_i'$.
\end{proof}
\begin{remark}\label{rem:error-app} Notice that if some $b_i$ is instead of $1$, $1\pm \varepsilon$, $\varepsilon < c/C$. Then the output of the above layer would be \begin{align}
\TF(\x_i) &= \x_i + (-C \pm C\varepsilon - \x_i) -( -C \pm C\varepsilon +\x_i)\\
& = \x_i
\end{align}
while if some $b_i =\pm \varepsilon$ instead of zero, and assuming that $\x_i > c>0$ or $\x_i < -c< 0$ the output would be 
\begin{align}
    \TF(\x_i) &= \x_i  +(-C\varepsilon - \x_i)_+ - (-Cb_i +\x_i)_+\\
    &= \x_i \pm C\varepsilon - \x_i \\
    &\leq c
\end{align}
If $\abs{\x_i} \leq c$ again the output would be less or equal than $c$, where $c$ can be arbitrarily small.
\end{remark}
But how we can create these bits for each different token we want to produce?  We now describe for clarity how next word prediction is performed. An $d\times N$-dimensional input is given to the transformer architecture, which is up-projected using the embedding layer; afterwards the positional encodings are added/appended to the it. At the last layer, the last token predicted is appended to the input, while the rest of the tokens remain unchanged. The same holds for the actual input to the transformer after appending the encodings. The only difference of the new input is the $n+1$-th token. We consider encoder-based architectures in all of our lemmas below. 

In the subsequent lemma we will try to construct and automated process that works along those guidelines.
To do so we assume that the input to the transformer contains the following information:
\begin{enumerate}
    \item An enumeration of the tokens from $1$ to $N$. 
    \item The $\ln$ of the above enumeration.
    \item Zeros for the tokens that correspond to the data points, $1$ for each token that is the $\x_{\text{test}}$ or it is a prediction based on this.
    \item An enumeration $1$ to $L$ for each one of the data points provided. For example, if we are given three sets of data we would have : $1\hdots L \; 1\hdots L\; 1\hdots L$.
    \item Some extra information that is needed to implement a multiplication step as described in Lemma \ref{lem:matrixmul_app} and to move things to the correct place.
\end{enumerate}
The above information can be viewed as part of the encodings that are appended to the transformer. Formally, we have
\begin{lemma}\label{lem:binary-app}
Consider that the $\ell-1$-th prediction has been made and the transformer is to  make the $\ell$-th one. The input to the transformer is:
\renewcommand{\arraystretch}{1.5}
\begin{equation*}
\arraycolsep=1.5pt
\X = \left[\begin{array}{*{12}c}
    \x_1 & \hdots &\x_{\ell}& \x_{\ell+1}&\hdots & \x_{L+\ell+1} &\x_{L+\ell+2} &\hdots & \x_{n} &\x &\hdots &f_{\ell-1}(\x)\\
    \zero &\hdots &\zero  &\zero &\hdots &\zero &\zero &\hdots &\zero &\zero &\hdots &\zero\\
        \hline
     1 & \hdots & \ell & \ell+1& \hdots &\ell &\ell+1 &\hdots &L &1&\hdots & \ell\\
     1 & \hdots & \ell &\ell+1 &\hdots &\ell &\ell+1&\hdots &L &1&\hdots & \ell\\
     \hline
     1 & \hdots & \ell &\ell+1 &\hdots &L+\ell+1 &L+\ell+2 &\hdots &n &n+1 &\hdots & N\\
    \ln(1) & \hdots & \ln(\ell) &\ln(\ell+1) &\hdots &\ln(L+\ell+1) &\ln(L+\ell+2) &\hdots &\ln(n) &\ln(n+1) &\hdots & \ln(N)\\
 0 & \hdots & 0 &0&\hdots &0  &0 &\hdots &0 &1 &\hdots & 1\\
1 & \hdots & 1 &1 &\hdots &1&1 &\hdots &1 &1 &\hdots & 1\\ 
\m_1 & \hdots & \m_\ell &\m_{\ell+1} &\hdots &\m_{L+\ell+1} &\m_{L+\ell+2} &\hdots &\m_{n} &\m_{n+1} &\hdots & \m_{N}\\
 \end{array}\right]
\end{equation*}
Then there exists a transformer $\TF$ consisting of 4 layers that has as output
\renewcommand{\arraystretch}{1.3}
\begin{equation*}
\arraycolsep=1.2pt
  \TF(\X)  =  \left[\begin{array}{*{12}c}
      \x_1  &\hdots &\x_{\ell}& \x_{\ell+1}&\hdots & \x_{L+\ell+1} &\x_{L+\ell+2} &\hdots & \x_{n} &\x &\hdots &f_{\ell-1}(\x)\\
      \x_1  &\hdots &\x_{\ell}& \x_{\ell+1}&\hdots  & \x_{L+\ell+1} &\x_{L+\ell+2} &\hdots & \x_{n} &\x &\hdots &f_{\ell-1}(\x)\\
      \hline
     0 & \hdots & 1 &0 &\hdots &1 &0 &\hdots &0&0 &\hdots & 1\\
     0 & \hdots & 0 &1 &\hdots &0 &1 &\hdots &0 &0 &\hdots &0 \\
     \hline
     1 & \hdots & \ell &\ell+1 &\hdots &L+\ell+1 &L+\ell+2 &\hdots &n &n+1 &\hdots & N\\
       \ln(1) & \hdots & \ln(\ell) &\ln(\ell+1) &\hdots &\ln(L+\ell+1) &\ln(L+\ell+2) &\hdots &\ln(n) &\ln(n+1) &\hdots & \ln(N)\\
 0 & \hdots & 0 &0&\hdots &0  &0 &\hdots &0 &1 &\hdots & 1\\
1 & \hdots & 1 &1 &\hdots &1&1 &\hdots &1 &1 &\hdots & 1\\ 
\m_1 & \hdots & \m_\ell &\m_{\ell+1} &\hdots &\m_{L+\ell+1} &\m_{L+\ell+2} &\hdots &\m_{n} &\m_{n+1} &\hdots & \m_{N}\\
  \end{array}\right] 
\end{equation*}
with error up to $\varepsilon\rmM$, where $\|{\rmM}\|\leq 1$ and $\varepsilon$ is a constant that is controlled and can be arbitrarily small.
\end{lemma}
\begin{proof}
\noindent\textbf{Step 1: Extract the sequence length (1 layer).} Let 
\begin{align}
\weights_{\query} =  \begin{bmatrix}
    \zero &\zero &0 &0 &0 &0 &0 &0 &1 &\zero 
\end{bmatrix}
 \;\;\; 
\weights_{\key}= \begin{bmatrix}
    \zero &\zero &0 &0 &0&1 &0 &0 &\zero
\end{bmatrix} 
\end{align}
and thus 
\begin{equation}
    (\weights_{\query}\X)^\top(\weights_{\key}\X) = \begin{bmatrix}
        \ln(1) &\ln(2) &\hdots &\ln(\seqlen)\\
        \ln(1) &\ln(2) &\hdots &\ln(\seqlen)\\
        \vdots &\vdots &\ddots &\vdots\\
        \ln(1) &\ln(2) &\hdots &\ln(\seqlen)\\
    \end{bmatrix}.
\end{equation}
So after the softmax is applied we have
\begin{equation} \sfm((\weights_{\query}\X)^\top(\weights_{\key}\X)) = \begin{bmatrix}
        \dfrac{1}{\sum_{i=1}^\seqlen i} &\dfrac{2}{\sum_{i=1}^\seqlen i}&\hdots &\dfrac{\seqlen}{\sum_{i=1}^\seqlen i}\\
        \dfrac{1}{\sum_{i=1}^\seqlen i} &\dfrac{2}{\sum_{i=1}^\seqlen i}&\hdots &\dfrac{\seqlen}{\sum_{i=1}^\seqlen i}\\
        \vdots &\vdots &\ddots &\vdots\\
        \dfrac{1}{\sum_{i=1}^\seqlen i} &\dfrac{2}{\sum_{i=1}^\seqlen i}&\hdots &\dfrac{\seqlen}{\sum_{i=1}^\seqlen i}\\
    \end{bmatrix}.
\end{equation}
We then set the weight value matrix as to zero-out all lines except for one line as follows
\begin{equation}
   \weights_{\val}\X =\begin{bmatrix}
   \zero &\zero & \hdots &\zero \\
    1 & 2 &\hdots &\seqlen\\
 \zero &\zero &\hdots &\zero 
   \end{bmatrix}
\end{equation}
% \begin{equation}
%    \weights_{\val}\rmI =\begin{bmatrix}
%    \zero &\zero & \hdots &\zero \\
%   \zero &\zero & \hdots &\zero \\
%     \zero &\zero & \hdots &\zero \\
%     \zero &\zero & \hdots &\zero \\
%     1 & 2 &\hdots &\seqlen\\
%     0 &0 &\hdots &0\\
%      0 &0 &\hdots &0\\
%        0 &0 &\hdots &0
%    \end{bmatrix}
% \end{equation}
After adding the residual and using an extra head whose softmax returns identity matrix and the value weight matrix is minus the identity, we get 
\renewcommand{\arraystretch}{1.5}
\begin{equation*}
\arraycolsep = 1.5pt
    \X = \left[\begin{array}{*{12}c}
    \x_1 & \hdots &\x_{\ell}& \x_{\ell+1}&\hdots & \x_{L+\ell+1} &\x_{L+\ell+2} &\hdots & \x_{n} &\x &\hdots &f_{\ell-1}(\x)\\
    \zero &\hdots &\zero  &\zero &\hdots &\zero &\zero &\hdots &\zero &\zero &\hdots &\zero\\
        \hline
     1 & \hdots & \ell & \ell+1& \hdots &\ell &\ell+1 &\hdots &L &1&\hdots & \ell\\
     1 & \hdots & \ell &\ell+1 &\hdots &\ell &\ell+1&\hdots &L &1&\hdots & \ell\\
     \hline
     \dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i} & \hdots & \dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i} &\dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i} &\hdots &\dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i}&\dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i} &\hdots &\dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i} &\dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i} &\hdots & \dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i}\\
    \ln(1) & \hdots & \ln(\ell) &\ln(\ell+1) &\hdots &\ln(L+\ell+1) &\ln(L+\ell+2) &\hdots &\ln(n) &\ln(n+1) &\hdots & \ln(N)\\
 0 & \hdots & 0 &0&\hdots &0  &0 &\hdots &0 &1 &\hdots & 1\\
1 & \hdots & 1 &1 &\hdots &1&1 &\hdots &1 &1 &\hdots & 1\\ 
\m_1 & \hdots & \m_\ell &\m_{\ell+1} &\hdots &\m_{L+\ell+1} &\m_{L+\ell+2} &\hdots &\m_{n} &\m_{n+1} &\hdots & \m_{N}\\
 \end{array}\right]
\end{equation*}
Notice that $\dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i} = \dfrac{2\seqlen(\seqlen+1)(2\seqlen+1)}{6\seqlen(\seqlen+1)} = \dfrac{2\seqlen+1}{3}$. We then use the ReLU layer as to multiply with $3/2$ and subtract $1/3$ from this column. This results to 
\begin{equation*}
\arraycolsep = 1.5pt
    \X = \left[\begin{array}{*{12}c}
    \x_1 & \hdots &\x_{\ell}& \x_{\ell+1}&\hdots & \x_{L+\ell+1} &\x_{L+\ell+2} &\hdots & \x_{n} &\x &\hdots &f_{\ell-1}(\x)\\
    \zero &\hdots &\zero  &\zero &\hdots &\zero &\zero &\hdots &\zero &\zero &\hdots &\zero\\
        \hline
     1 & \hdots & \ell & \ell+1& \hdots &\ell &\ell+1 &\hdots &L &1&\hdots & \ell\\
     1 & \hdots & \ell &\ell+1 &\hdots &\ell &\ell+1&\hdots &L &1&\hdots & \ell\\
     \hline
     N & \hdots & N &N&\hdots &N&N &\hdots &N&N&\hdots & N\\
    \ln(1) & \hdots & \ln(\ell) &\ln(\ell+1) &\hdots &\ln(L+\ell+1) &\ln(L+\ell+2) &\hdots &\ln(n) &\ln(n+1) &\hdots & \ln(N)\\
 0 & \hdots & 0 &0&\hdots &0  &0 &\hdots &0 &1 &\hdots & 1\\
1 & \hdots & 1 &1 &\hdots &1&1 &\hdots &1 &1 &\hdots & 1\\ 
\m_1 & \hdots & \m_\ell &\m_{\ell+1} &\hdots &\m_{L+\ell+1} &\m_{L+\ell+2} &\hdots &\m_{n} &\m_{n+1} &\hdots & \m_{N}\\
 \end{array}\right]
\end{equation*}

\textbf{Step 2: Extract the number of the prediction to be made $\ell$ (3 layers). }Now, by setting the key and query weight matrices of the attention as  to just keep the all ones row, we get a matrix that attends equally  to all tokens. Then the value weight matrix keeps the row that contains $\ell$ ones and thus we get the number $\dfrac{\ell}{N}$, propagated in all the sequence length. 
\begin{equation}
    \arraycolsep = 1.5pt
    \X = \left[\begin{array}{*{12}c}
    \x_1 & \hdots &\x_{\ell}& \x_{\ell+1}&\hdots & \x_{L+\ell+1} &\x_{L+\ell+2} &\hdots & \x_{n} &\x &\hdots &f_{\ell-1}(\x)\\
    \zero &\hdots &\zero  &\zero &\hdots &\zero &\zero &\hdots &\zero &\zero &\hdots &\zero\\
        \hline
     1 & \hdots & \ell & \ell+1& \hdots &\ell &\ell+1 &\hdots &L &1&\hdots & \ell\\
     1 & \hdots & \ell &\ell+1 &\hdots &\ell &\ell+1&\hdots &L &1&\hdots & \ell\\
     \hline
     N & \hdots & N &N&\hdots &N&N &\hdots &N&N&\hdots & N\\
    \dfrac{\ell}{N} & \hdots & \dfrac{\ell}{N} &\dfrac{\ell}{N} &\hdots &\dfrac{\ell}{N} &\dfrac{\ell}{N} &\hdots &\dfrac{\ell}{N} &\dfrac{\ell}{N} &\hdots &\dfrac{\ell}{N}\\
 0 & \hdots & 0 &0&\hdots &0  &0 &\hdots &0 &1 &\hdots & 1\\
1 & \hdots & 1 &1 &\hdots &1&1 &\hdots &1 &1 &\hdots & 1\\ 
\m_1 & \hdots & \m_\ell &\m_{\ell+1} &\hdots &\m_{L+\ell+1} &\m_{L+\ell+2} &\hdots &\m_{n} &\m_{n+1} &\hdots & \m_{N}\\
 \end{array}\right]
\end{equation}
As described in Lemma \ref{lem:matrixmul_app} to implement multiplication of two values up to any error $\eps$, we need 1) have the two numbers to be multiplied next to each other and an extra structure (some constants, which we consider that are encoded in the last rows of the matrix $\m_i$) and 2) the corresponding structure presented in Lemma \ref{lem:matrixmul_app} . So we need to make the following transformation in the rows containing $N$ and $\dfrac{\ell}{N}$
\begin{align}
    \begin{bmatrix}
        N & N &\hdots &N\\
        \dfrac{\ell}{N} &\dfrac{\ell}{N} &\hdots &\dfrac{\ell}{N}
    \end{bmatrix} &\to \begin{bmatrix}
        N & \dfrac{\ell}{N} &\hdots &N\\
        \dfrac{\ell}{N} &\dfrac{\ell}{N} &\hdots &\dfrac{\ell}{N}
    \end{bmatrix}\\
    &\to 
    \begin{bmatrix}
         \ell& *&\hdots &*\\
        * &* &\hdots &*
    \end{bmatrix}\\
    &\to \begin{bmatrix}
        \ell& \ell&\hdots &\ell\\
         * &* &\hdots &*
    \end{bmatrix}
\end{align}
where $*$ denotes inconsequential values.
For the first step we assume that we have the necessary binary representations \footnote{the size that we need will be $2\log N_{\text{max}}+1$, where $N_{\text{max}}$ is the maximum sequence length} and then we use Lemma \ref{lem:copy} which shows how we can perform the operation of copy/paste. For the second step now we use Lemma \ref{lem:matrixmul_app} to perform the multiplication, this will affect some of the other values. Then for the last step consider the follow (sub-)rows of the matrix $\X$
\begin{equation}
    \begin{bmatrix}
        \ell & * &* &\hdots &*\\
        \emb_1 &\emb_1 &\emb_1 &\hdots &\emb_1\\
        \emb_1 &\emb_2 &\emb_3 &\hdots &\emb_N
    \end{bmatrix}
\end{equation}
where $\emb_i$ is the binary representation of position $i$. By choosing $\weights_\key,\weights_\query$ as to
\begin{equation}
    \weights_\key\X = \begin{bmatrix}
        \emb_1 &\emb_2 &\hdots &\emb_N
    \end{bmatrix}, \;\;\;\weights_\query\X = \begin{bmatrix}
        \emb_1 &\emb_1 &\hdots &\emb_1 
    \end{bmatrix} 
\end{equation}
and consider $\weights_\val\X = \begin{bmatrix}
        \ell & * & \hdots &*\\
        \zero &\zero &\hdots &\zero 
    \end{bmatrix}$ we have that 
    \begin{align*}
       \attn(\X) &= \X+ \weights_\val\X \sfm((\weights_\key\X)^\top\weights_\query)\\
       &= \X + \begin{bmatrix}
        \ell & * & \hdots &*\\
        \zero &\zero &\hdots &\zero 
    \end{bmatrix} \sfm(\begin{bmatrix}
        \emb_1^\top\emb_1 &\emb_1^\top\emb_1 &\hdots &\emb_1^\top\emb_1\\
         \emb_1^\top\emb_2 &\emb_1^\top\emb_2 & \hdots &\emb_1^\top\emb_2 \\
         \vdots &\vdots &\ddots &\vdots\\
         \emb_1^\top\emb_N &\emb_1^\top\emb_N &\hdots &\emb_1^\top\emb_N
    \end{bmatrix})\\
    &= \X+ \begin{bmatrix}
        \ell & * & \hdots &*\\
        \zero &\zero &\hdots &\zero 
    \end{bmatrix}   \begin{bmatrix}
        1 & 1 &\hdots &1 \\
        0 & 0 &\hdots &0\\
        \vdots &\vdots &\hdots &\vdots\\
        0 & 0 &\hdots & 0
    \end{bmatrix} +\varepsilon \rmM
    \end{align*}
    By subtracting one identity head for the first that we focus on as described in Lemma \ref{lem:copy} we have that $\attn(\X)$ results in the desired matrix. We output this result and overwrite $\ell/N$, thus we have
    \begin{equation}
    \arraycolsep = 1.5pt
    \X = \left[\begin{array}{*{12}c}
    \x_1 & \hdots &\x_{\ell}& \x_{\ell+1}&\hdots & \x_{L+\ell+1} &\x_{L+\ell+2} &\hdots & \x_{n} &\x &\hdots &f_{\ell-1}(\x)\\
    \zero &\hdots &\zero  &\zero &\hdots &\zero &\zero &\hdots &\zero &\zero &\hdots &\zero\\
        \hline
     1 & \hdots & \ell & \ell+1& \hdots &\ell &\ell+1 &\hdots &L &1&\hdots & \ell\\
     1 & \hdots & \ell &\ell+1 &\hdots &\ell &\ell+1&\hdots &L &1&\hdots & \ell\\
     \hline
     N & \hdots & N &N&\hdots &N&N &\hdots &N&N&\hdots & N\\
   \ell & \hdots & \ell &\ell &\hdots &\ell &\ell &\hdots &\ell &\ell &\hdots &\ell\\
 0 & \hdots & 0 &0&\hdots &0  &0 &\hdots &0 &1 &\hdots & 1\\
1 & \hdots & 1 &1 &\hdots &1&1 &\hdots &1 &1 &\hdots & 1\\ 
\m_1 & \hdots & \m_\ell &\m_{\ell+1} &\hdots &\m_{L+\ell+1} &\m_{L+\ell+2} &\hdots &\m_{n} &\m_{n+1} &\hdots & \m_{N}\\
 \end{array}\right]
\end{equation}
    \paragraph{Step 3: Create $\ell+1$ (0 layer). } We first copy the row with $\ell$ to the row with $N$, this can trivially be done with a ReLU layer that outputs zero everywhere else except for the row of $N$s that output $(\ell)_{+} - (N)_{+}$ to account also for the residual. We now use one of the bias terms (notice that $\ell$ is always positive) and set to one in one of the two rows that contain the $\ell$, again we account for the residual as before; everything else remains unchanged. Thus, we have
    \begin{equation}
    \arraycolsep = 1.5pt
    \X = \left[\begin{array}{*{12}c}
    \x_1 & \hdots &\x_{\ell}& \x_{\ell+1}&\hdots & \x_{L+\ell+1} &\x_{L+\ell+2} &\hdots & \x_{n} &\x &\hdots &f_{\ell-1}(\x)\\
    \zero &\hdots &\zero  &\zero &\hdots &\zero &\zero &\hdots &\zero &\zero &\hdots &\zero\\
        \hline
     1 & \hdots & \ell & \ell+1& \hdots &\ell &\ell+1 &\hdots &L &1&\hdots & \ell\\
     1 & \hdots & \ell &\ell+1 &\hdots &\ell &\ell+1&\hdots &L &1&\hdots & \ell\\
     \hline
     \ell+1 & \hdots & \ell+1 &\ell+1&\hdots &\ell+1 &\ell+1 &\hdots &\ell+1 &\ell+1 &\hdots &\ell+1\\
    \ell & \hdots & \ell &\ell &\hdots &\ell &\ell &\hdots &\ell &\ell &\hdots &\ell\\
 0 & \hdots & 0 &0&\hdots &0  &0 &\hdots &0 &1 &\hdots & 1\\
1 & \hdots & 1 &1 &\hdots &1&1 &\hdots &1 &1 &\hdots & 1\\ 
\m_1 & \hdots & \m_\ell &\m_{\ell+1} &\hdots &\m_{L+\ell+1} &\m_{L+\ell+2} &\hdots &\m_{n} &\m_{n+1} &\hdots & \m_{N}\\
 \end{array}\right]
\end{equation}
This operation can collectively be implemented (add the bias + copy the row) in the ReLU layer of the previous transformer layer that was not used in the previous step.
    \paragraph{Step 4: Create the binary bits (1 layer). }We will now use the information extracted in the previous steps, to create the binary indicators/bit to identify which tokens we want to filter. This can be easily implemented with one layer of transformer and especially the  ReLU part of it. Notice that if we subtract the row that contains the tokens that have already been predicted, \emph{i.e.,} $[\ell\ell\hdots \ell]$ from the row that contains $[12\hdots L  12\hdots L \hdots L]$ we will get zero only in the positions that we want to filter out and some non-zero quantity in the rest. So, we need to implement an if..then type of operation. Basically, if the quantity at hand is zero we want to set the bit to one, while if it non-zero to set it to be zero. This can be implemented with the following ReLU layer
    \AG{Add the expression}

    \textbf{Step 5: Implement the filtering (1 layer).}  We now apply Lemma \ref{lem:binary-app} and our proof is completed.
\end{proof}

\begin{theorem}[Decoupling CoT]\label{thm:MLP} Consider a prompt $\pmt_n(f)$ generated from an $L$-layer MLP $f(\cdot)$ as described in Definition \ref{MLP assump}, and assume given test example $(\xtest,\tb^1_{\text{\tiny test}}, \dots\tb^L_{\text{\tiny test}})$. 
% , containing $n$ examples and ends with $\x^{\texttt{test}}$. 
For any resolution $\eps>0$, there exists $\delta=\delta(\eps)$, iteration choice $T={\cal{O}}(\kappa_{\max}^2\log(1/\eps))$, and a backend transformer construction $\TFBE$ such that the concatenated transformer $\TF=\TFLR \circ \TFBE$ implements the following: Let $(\tht^{i})_{i=1}^{\ell-1}$ denote the first $\ell-1$ $\COT$ outputs of $\TF$ and set $\pb[\ell]=(\pb_n(f),\xtest,\tht^{1}\dots\tht^{\ell-1})$. At step $\ell$, $\TF$ implements
\begin{enumerate}
\item \textbf{Filtering.} Define the filtered prompt with input/output features of layer $\ell$,
\[
\arraycolsep = 1pt
\pbf_n=\left(\begin{array}{*{10}c}
\hdots \zero,&\tb^{\ell-1}_{1},&\zero&\hdots&\zero,&\tb^{\ell-1}_n, &\zero&\hdots&\zero,&\tht^{\ell-1}\\
\hdots\zero,&\zero,& \tb^{\ell}_{1}&\dots&\zero,&\zero,& \tb^{\ell}_n&\dots&\zero,&\zero\end{array}\right).
\]
There exists a fixed projection matrix $\bPi$ that applies individually on tokens such that the backend output obeys $\tn{\bPi(\TFBE(\pb[\ell]))-\pbf_n}\leq \delta$. %The more precise statement is provided in Lemma \ref{lem:filtering}. % up to $\eps$ accuracy via a fixed linear projection. 
\item \textbf{Gradient descent.} The combined model obeys $\tn{\TF(\pb[\ell])-\tb_{\text{\tiny test}}^{\ell}}\leq {\ell\cdot \eps}/{L}$.
\end{enumerate}
$\TFBE$ has constant number of layers independent of $T$ and $n$. Consequently, after $L$ rounds of $\COT$, \TF outputs $f(\xtest)$ up to $\eps$ accuracy.
\end{theorem}
% \begin{lemma}[Filtering]\label{lem:filtering-app}
    
% \end{lemma}
% \begin{lemma}[Skills] Consider an input of the form
% \begin{equation}
%     \X = \begin{bmatrix}
%         \x_1 &\x_2 &\hdots &\x_n &\x\\
%         \s_{f_1} &\s_{f_2} &\hdots &\s_{f_n} &\s_k\\
%         \emb_1 &\emb_2 &\hdots &\emb_n &\emb_{n+1}
%     \end{bmatrix}
% \end{equation}
%  Then there exists a transformer $\TF$ with  five layers with output
%  \begin{equation}
%      \TF(\X) = \begin{bmatrix}
%          \one_{\{\s_{f_1} = \s_k\}}\x_1 &\one_{\{\s_{f_2} = \s_k\}}\x_2 &\hdots &\one_{\{\s_{f_n} = \s_k\}}\x_n &\x\\
%         \s_{f_1} &\s_{f_2} &\hdots &\s_{f_n} &\s_k\\
%         \emb_1 &\emb_2 &\hdots &\emb_n &\emb_{n+1}
%      \end{bmatrix}
%  \end{equation}
% \end{lemma}
% \begin{proof}
%     \begin{enumerate}
%         \item Use $\emb_i$ create one line that has everywhere $n+1$ like in lemma 1. 
%         \item Create the $\emb_{n+1}$ everywhere. 
%         \item Use this and the classic embeddings and copy everyehre the skill $\s_k$. 
%         \item Subtract the skill 
%     \end{enumerate}
%\end{proof}
% Our implementation of filtering is divided in two parts. In the first part we show how the filtering can be performed, given the appropriate encodings. In the second part we will show how we can perform some preprocessing to generalize this operation to any iteration, given always encodings of a specific form. The second part is to demonstrate that as it holds in practice we don't require to change the encodings to perform the filtering at each one of the iterations \AG{I will rephrase this}. 

% For the first lemma, we consider the more general setting in which the data are given in a possibly random order attached with an indicator vector that defines which is their actual position as explained in \AG{Mention the section in which we explain this setting.}
% \begin{lemma}
%     Assume that the input to a transformer after the embedding layer is of the following form 
%     \begin{equation}
%         \X = \begin{bmatrix}
%             \x_1&\x_2&\hdots &\x_{n-1}&\x_n\\
%             \emb_1 &\emb_2 &\hdots&\emb_{n-1} &\emb_n\\
%             \emb_{f_1}&\emb_{f_2}&\hdots &\zero &\zero\\
%             1 & 1 &\hdots & 0 & 0\\
%             \zero &\zero &\hdots &\zero &\zero\\
%             \zero &\zero &\hdots &\zero &\zero
%         \end{bmatrix}
%     \end{equation}
%     where $\x_i\in\R^{d'}$ $\emb_i$, $i=1,\hdots,n$ is the positional encoding as described in subsection \ref{sub:pencodings} for the $i$-th position and $\emb_{f_i}$, $i=1,\hdots, k$ is the encoding of the position we want to filter. If $k\leq n$ then we are given zeroes afterwards. Then there exists one layer of transformer $\TF$ such that 
%     \begin{equation}
%         \TF(\X) = \begin{bmatrix}
%             \x_1&\x_2&\hdots &\x_{n-1}&\x_n\\
%             \emb_1 &\emb_2 &\hdots&\emb_{n-1} &\emb_n\\
%             \emb_{f_1}&\emb_{f_2}&\hdots &\zero &\zero\\
%                         1 & 1 &\hdots & 0 & 0\\
%                         \zero &\zero &\hdots &\zero &\zero\\
%             \x_{f_1}&\x_{f_2}&\hdots &\zero &\zero
%         \end{bmatrix}
%     \end{equation}
% \end{lemma}
% \begin{proof}
% Notice that the dimension of the input is $d = 3d' + 2e $, where $e$ is the dimension of the positional encodings that the model has chosen. Let
%     \begin{equation}
%         \W_\key = \begin{bmatrix}
%             \zero_{d'} &
%             \Iden_{e} & \zero_{2d'+e}            
%         \end{bmatrix}, \W_\query = \begin{bmatrix}
%             \zero_{d'+e} &
%             \Iden_{e} & \zero_{2d'}            
%         \end{bmatrix}
%     \end{equation}
%     we have that 
%    \renewcommand{\arraystretch}{1.5}
%     \begin{align}
%     \arraycolsep=0.1pt
%         \sfm((\W_\key\X)^\top(\W_\query\X)) &= \sfm(\begin{bmatrix}
%             \emb_1^\top\emb_{f_1} &\emb_1^\top\emb_{f_2}&\hdots &\zero\\
%            \emb_2^\top\emb_{f_1} &\emb_2^\top\emb_{f_2}&\hdots &\zero\\
%            \vdots &\vdots &\ddots &\vdots\\
%            \emb_n^\top\emb_{f_1} &\emb_n^\top\emb_{f_2}&\hdots &\zero\\
%         \end{bmatrix})\\
%         &= \begin{bmatrix}
%             \dfrac{ \exp(\lambda\emb_1^\top\emb_{f_1})} {\sum_{i=1}^n\exp( \lambda\emb_i^\top\emb_{f_1})}&\hdots &\dfrac{1}{n}\\
%             \vdots &\hdots &\vdots \\
%              \dfrac{ \exp(\lambda\emb_n^\top\emb_{f_1})} {\sum_{i=1}^n\exp(\lambda \emb_i^\top\emb_{f_1})}&\hdots &\dfrac{1}{n}
%         \end{bmatrix}
%     \end{align}
%     Notice that for the columns that we had non-zeros the above matrix becomes a permutation matrix (as $\lambda\to\infty$ ) with $1$ at the $f_i$-th position of each column $i$. For example, for the first column we will have one in the $f_1$-th row. After this permutation of the identity matrix ( plus some error matrix, which can have arbitrarily small norm by tuning the temperature) is multiplied with $\X$ and by letting 
%     \begin{equation}
%         \W_\val = \begin{bmatrix}
%         \zero & \zero &\zero &\zero &\zero \\
%         \zero & \zero &\zero &\zero &\zero \\
%         \zero & \zero &\zero &\zero &\zero \\
%        \zero & \zero &\zero &\zero &\zero \\
%         \Iden_{d'} & \zero &\zero &\zero &\zero\\
%         \zero & \zero &\zero &\zero &\zero 
%     \end{bmatrix}
%     \end{equation}
%    Thus, the output of the attention becomes
%     \begin{align}
%         \attn(\X) &=  \begin{bmatrix}
%             \x_1&\x_2&\hdots &\x_{n-1}&\x_n\\
%             \emb_1 &\emb_2 &\hdots&\emb_{n-1} &\emb_n\\
%             \emb_{f_1}&\emb_{f_2}&\hdots &\zero &\zero\\
%                         1 & 1 &\hdots & 0 & 0\\
%             \x_{f_1}&\x_{f_2}&\hdots &* &*\\
%             \zero &\zero &\hdots &\zero &\zero 
%         \end{bmatrix}
%         \end{align}
%     where * denotes inconsequential values. We then use the ReLU layers to move the result in the last rows and substitute * with zeros. To do so we follow the construction of \cite{}; specifically we use the fourth row of ones and zeros, which indicates which columns should be updated and which not. For this we have that 
%     \begin{equation}
%         \TF(\X) = \X + \W_2\relu{\W_1\X}
%     \end{equation}
%     Then we set $\W_1, \W_2$ as to output zero in the first four set of rows. For the last set of rows we have \AG{Will add here the relu construction. But this proof is completed}... Thus,
%     \begin{equation}
%         \TF(\X) = \begin{bmatrix}
%             \x_1&\x_2&\hdots &\x_{n-1}&\x_n\\
%             \emb_1 &\emb_2 &\hdots&\emb_{n-1} &\emb_n\\
%             \emb_{f_1}&\emb_{f_2}&\hdots &\zero &\zero\\
%                         1 & 1 &\hdots & 0 & 0\\
%                         \zero &\zero &\hdots &\zero &\zero\\
%             \x_{f_1}&\x_{f_2}&\hdots &\zero &\zero
%         \end{bmatrix}
%     \end{equation}
%     and the proof is completed.
% \end{proof}







% We now continue to show how a transformer can predict 
% The following lemma states that transformers can implement the step of filtering. For simplicity we consider that we have just two intermediate steps and that  the model will predict the second step. It would be easy then to see that this construction can be generalized to multiple intermediate steps and implement a specific step each time depending on the given input.
% \begin{lemma} 

% \end{lemma}
% \begin{proof}
% We consider the following set-up: 
% The user gives an input of the form $\rmI = \begin{bmatrix}
%         \dpoint_1 &\prompt{1}{1} &\prompt{1}{2} \hdots &  \prompt{1}{\layer} &\hdots &\dpoint_n &\prompt{n}{1} &\hdots &\prompt{n}{\layer} &\dpoint_{\text{test}}
% \end{bmatrix}$.

% After the embedding layer the input is transformed as follows: 
%  \renewcommand{\arraystretch}{1.7}
% \begin{equation*}
% \arraycolsep=1.5pt
%    \rmI = \left[\begin{array}{*{11}c}
%     \dpoint_1 &\prompt{1}{1} &\prompt{1}{2}& \hdots &  \prompt{1}{\layer} &\hdots &\dpoint_n &\prompt{n}{1} &\hdots &\prompt{n}{\layer} &\dpoint_{\text{test}}\\
%     \zero &\zero &\zero&\hdots &\zero &\hdots &\zero &\zero &\hdots &\zero &\zero \\
%     \emb_0 &\emb_{L+1} &\emb_2 &\hdots &\emb_{\layer} &\hdots& \emb_{(n-1)(\layer + 1)+1} &\emb_{(n-1)(\layer+1)+ 2} &\hdots &\emb_{\seqlen-2}&\emb_{\seqlen-1}\\
%     \emb_0 & \emb_{\layer+1} &\emb_{2\layer+1} &\hdots & \emb_{f(\layer)}&\hdots& \emb_{f((n-1)(\layer + 1)+1)} & \emb_{f((n-1)(\layer+1)+ 2)}&\hdots &\emb_{f(\seqlen-1)}&\emb_{f(\seqlen)}\\
%      \text{!!!!} & \emb_{\layer+1} &\emb_{2\layer+1} &\hdots & \emb_{f(\layer)}&\hdots& \emb_{f((n-1)(\layer + 1)+1)} & \emb_{f((n-1)(\layer+1)+ 2)}&\hdots &\emb_{f(\seqlen-1)}&\emb_{f(\seqlen)}\\
%     1 & 2 &3&\hdots &\layer+1 &\hdots& (n-1)\layer + n &(n-1)\layer + n+1 &\hdots &\seqlen-1 &\seqlen\\ 
%      \ln(1) & \ln(2) & \ln(3)&\hdots &\ln(\layer+1) &\hdots& \ln((n-1)\layer + n) &\ln((n-1)\layer + n+1 )&\hdots &\ln(\seqlen-1) &\ln(\seqlen)\\ 
%      1 & 1 &1 &\hdots &1 &\hdots &1 &1 &\hdots &1 &1 \\ 
%      0 & 0&0&\hdots &0 &\hdots &0 &0 &\hdots &0 &0
%     \end{array} 
%     \right]
% \end{equation*}
% where $\seqlen$ is the sequence length, (write the function***)$f(x) =...$. Also, the second row is a block of rows set to zero, which will be used for storing necessary intermediate results.

% \noindent\textbf{Step 1: Extract the number of tokens.} Let 
% \begin{align}
% \weights_{\key}= \begin{bmatrix}
%     \zero &\zero &\zero &\zero &\zero &0 &1 &0 &0 
% \end{bmatrix} 
%  \;\;\; \weights_{\query} =  \begin{bmatrix}
%     \zero &\zero &\zero &\zero &\zero &0 &0 &1 &0 
% \end{bmatrix}
% \end{align}
% and thus 
% \begin{equation}
%     (\weights_{\key}\rmI)^\top(\weights_{\query}\rmI) = \begin{bmatrix}
%         \ln(1) &\ln(1) &\hdots &\ln(1)\\
%         \ln(2) &\ln(2) &\hdots &\ln(2)\\
%         \vdots &\vdots &\ddots &\vdots\\
%         \ln(\seqlen) &\ln(\seqlen) &\hdots &\ln(\seqlen)\\
%     \end{bmatrix}
% \end{equation}
% So after the softmax is applied we have
% \begin{equation}
%     \softmax((\weights_{\key}\rmI)^\top(\weights_{\query}\rmI)) = \begin{bmatrix}
%         \dfrac{1}{\sum_{i=1}^\seqlen i} &\dfrac{1}{\sum_{i=1}^\seqlen i}&\hdots &\dfrac{1}{\sum_{i=1}^\seqlen i}\\
%         \dfrac{2}{\sum_{i=1}^\seqlen i} &\dfrac{2}{\sum_{i=1}^\seqlen i} &\hdots &\dfrac{2}{\sum_{i=1}^\seqlen i}\\
%         \vdots &\vdots &\ddots &\vdots\\
%         \dfrac{\seqlen}{\sum_{i=1}^\seqlen i} &\dfrac{\seqlen}{\sum_{i=1}^\seqlen i}  &\hdots &\dfrac{\seqlen}{\sum_{i=1}^\seqlen i} \\
%     \end{bmatrix}
% \end{equation}
% We then set the weight value matrix as to zero-out all lines except for one line as follows
% \begin{equation}
%    \weights_{\val}\rmI =\begin{bmatrix}
%    \zero &\zero & \hdots &\zero \\
%     1 & 2 &\hdots &\seqlen\\
%  \zero &\zero &\hdots &\zero 
%    \end{bmatrix}
% \end{equation}
% % \begin{equation}
% %    \weights_{\val}\rmI =\begin{bmatrix}
% %    \zero &\zero & \hdots &\zero \\
% %   \zero &\zero & \hdots &\zero \\
% %     \zero &\zero & \hdots &\zero \\
% %     \zero &\zero & \hdots &\zero \\
% %     1 & 2 &\hdots &\seqlen\\
% %     0 &0 &\hdots &0\\
% %      0 &0 &\hdots &0\\
% %        0 &0 &\hdots &0
% %    \end{bmatrix}
% % \end{equation}
% After adding the residual this results to 
% \begin{equation*}
%     \arraycolsep=1.5pt
%    \rmI = \left[\begin{array}{*{11}c}
%     \dpoint_1 &\prompt{1}{1} &\prompt{1}{2}& \hdots &  \prompt{1}{\layer} &\hdots &\dpoint_n &\prompt{n}{1} &\hdots &\prompt{n}{\layer} &\dpoint_{\text{test}}\\
%     \zero &\zero &\zero&\hdots &\zero &\hdots &\zero &\zero &\hdots &\zero &\zero \\
%     \emb_0 &\emb_{1} &\emb_2 &\hdots &\emb_{\layer} &\hdots& \emb_{(n-1)(\layer + 1)+1} &\emb_{(n-1)(\layer+1)+ 2} &\hdots &\emb_{\seqlen-2}&\emb_{\seqlen-1}\\
%     \emb_0 & \emb_{\layer+1} &\emb_{2\layer+1} &\hdots & \emb_{f(\layer)}&\hdots& \emb_{f((n-1)(\layer + 1)+1)} & \emb_{f((n-1)(\layer+1)+ 2)}&\hdots &\emb_{f(\seqlen-1)}&\emb_{f(\seqlen)}\\
%      \text{!!!!} & \emb_{\layer+1} &\emb_{2\layer+1} &\hdots & \emb_{f(\layer)}&\hdots& \emb_{f((n-1)(\layer + 1)+1)} & \emb_{f((n-1)(\layer+1)+ 2)}&\hdots &\emb_{f(\seqlen-1)}&\emb_{f(\seqlen)}\\
%     \dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i} & \dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i} &\dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i}&\hdots &\dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i}&\hdots& \dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i}&\dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i} &\hdots &\dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i} &\dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i}\\ 
%      \ln(1) & \ln(2) & \ln(3)&\hdots &\ln(\layer+1) &\hdots& \ln((n-1)\layer + n) &\ln((n-1)\layer + n+1 )&\hdots &\ln(\seqlen-1) &\ln(\seqlen)\\ 
%      1 & 1 &1 &\hdots &1 &\hdots &1 &1 &\hdots &1 &1 \\ 
%      0 & 0&0&\hdots &0 &\hdots &0 &0 &\hdots &0 &0
%     \end{array} 
%     \right]
% \end{equation*}
% However, notice that $\dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i} = \dfrac{2\seqlen(\seqlen+1)(2\seqlen+1)}{6\seqlen(\seqlen+1)} = \dfrac{2\seqlen+1}{3}$. We then use the ReLU layer as to multiply with $3/2$ and subtract $1/3$ from this column. This results to 
% \begin{equation*}
%     \arraycolsep=1.5pt
%    \rmI = \left[\begin{array}{*{11}c}
%     \dpoint_1 &\prompt{1}{1} &\prompt{1}{2}& \hdots &  \prompt{1}{\layer} &\hdots &\dpoint_n &\prompt{n}{1} &\hdots &\prompt{n}{\layer} &\dpoint_{\text{test}}\\
%     \zero &\zero &\zero&\hdots &\zero &\hdots &\zero &\zero &\hdots &\zero &\zero \\
%     \emb_0 &\emb_{1} &\emb_2 &\hdots &\emb_{\layer} &\hdots& \emb_{(n-1)(\layer + 1)+1} &\emb_{(n-1)(\layer+1)+ 2} &\hdots &\emb_{\seqlen-2}&\emb_{\seqlen-1}\\
%     \emb_0 & \emb_{\layer+1} &\emb_{2\layer+1} &\hdots & \emb_{f(\layer)}&\hdots& \emb_{f((n-1)(\layer + 1)+1)} & \emb_{f((n-1)(\layer+1)+ 2)}&\hdots &\emb_{f(\seqlen-1)}&\emb_{f(\seqlen)}\\
%      \text{!!!!} & \emb_{\layer+1} &\emb_{2\layer+1} &\hdots & \emb_{f(\layer)}&\hdots& \emb_{f((n-1)(\layer + 1)+1)} & \emb_{f((n-1)(\layer+1)+ 2)}&\hdots &\emb_{f(\seqlen-1)}&\emb_{f(\seqlen)}\\
%     \seqlen&  \seqlen& \seqlen&\hdots & \seqlen&\hdots&  \seqlen& \seqlen &\hdots & \seqlen & \seqlen\\ 
%      \ln(1) & \ln(2) & \ln(3)&\hdots &\ln(\layer+1) &\hdots& \ln((n-1)\layer + n) &\ln((n-1)\layer + n+1 )&\hdots &\ln(\seqlen-1) &\ln(\seqlen)\\ 
%      1 & 1 &1 &\hdots &1 &\hdots &1 &1 &\hdots &1 &1 \\ 
%      0 & 0&0&\hdots &0 &\hdots &0 &0 &\hdots &0 &0
%     \end{array} 
%     \right]
% \end{equation*}
% \noindent\textbf{Step 2: Create the positional encodings for $\seqlen$.}
% This step is implemented by \textcolor{orange}{Lemma}. Now output is
% \begin{equation*}
%     \arraycolsep=1.5pt
%    \rmI = \left[\begin{array}{*{11}c}
%     \dpoint_1 &\prompt{1}{1} &\prompt{1}{2}& \hdots &  \prompt{1}{\layer} &\hdots &\dpoint_n &\prompt{n}{1} &\hdots &\prompt{n}{\layer} &\dpoint_{\text{test}}\\
%     \zero &\zero &\zero&\hdots &\zero &\hdots &\zero &\zero &\hdots &\zero &\zero \\
%     \emb_{\seqlen} &\emb_{\seqlen} &\emb_{\seqlen}&\hdots &\emb_{\seqlen} &\hdots &\emb_{\seqlen} &\emb_{\seqlen} &\hdots &\emb_{\seqlen} &\emb_{\seqlen} \\
%     \emb_0 &\emb_{1} &\emb_2 &\hdots &\emb_{\layer} &\hdots& \emb_{(n-1)(\layer + 1)+1} &\emb_{(n-1)(\layer+1)+ 2} &\hdots &\emb_{\seqlen-2}&\emb_{\seqlen-1}\\
%     \emb_0 & \emb_{\layer+1} &\emb_{2\layer+1} &\hdots & \emb_{f(\layer)}&\hdots& \emb_{f((n-1)(\layer + 1)+1)} & \emb_{f((n-1)(\layer+1)+ 2)}&\hdots &\emb_{f(\seqlen-1)}&\emb_{f(\seqlen)}\\
%      \text{!!!!} & \emb_{\layer+1} &\emb_{2\layer+1} &\hdots & \emb_{f(\layer)}&\hdots& \emb_{f((n-1)(\layer + 1)+1)} & \emb_{f((n-1)(\layer+1)+ 2)}&\hdots &\emb_{f(\seqlen-1)}&\emb_{f(\seqlen)}\\
%     \seqlen&  \seqlen& \seqlen&\hdots & \seqlen&\hdots&  \seqlen& \seqlen &\hdots & \seqlen & \seqlen\\ 
%      \ln(1) & \ln(2) & \ln(3)&\hdots &\ln(\layer+1) &\hdots& \ln((n-1)\layer + n) &\ln((n-1)\layer + n+1 )&\hdots &\ln(\seqlen-1) &\ln(\seqlen)\\ 
%      1 & 1 &1 &\hdots &1 &\hdots &1 &1 &\hdots &1 &1 \\ 
%      0 & 0&0&\hdots &0 &\hdots &0 &0 &\hdots &0 &0
%     \end{array} 
%     \right]
% \end{equation*}
% \textcolor{orange}{We need to create the encodings of max length.}
% \end{proof}

==> backup/sec/discuss.tex <==
\section{Conclusion and Discussion}\label{sec:discuss}
In this work, we investigate chain-of-thought prompting and shed light on how it enables compositional learning of multilayer perceptrons step-by-step. Specially, we have explored and contrasted three methods: $\ICL$, $\EXP$ and $\COT$, and found that $\COT$ facilitates better approximation and faster convergence through looping and sample efficiency. Additionally, we empirically and theoretically demonstrated that to learn a 2-layer MLP with $d$-dimensional input and $k$ neurons, $\COT$ requires ${\cal{O}}(\max(d,k))$ in-context samples whereas $\ICL$ runs into approximation error bottlenecks. 

%potential questions regarding our findings
There are several interesting avenues for future research building on our findings. To what extent our decoupling of CoT (filtering followed by ICL) align with the empirical evidence in practical problems such as code generation and mathematical reasoning? We have shown that $\COT$ can rely on linear regression oracle to learn an MLP. To what extent transformers can approximate MLPs without $\COT$ (e.g.~with $\EXP$), what are lower/upper bounds?

%Since $\EXP$ and $\COT$ provide intermediate messages in the prefix, is there proper algorithm using input-output only but can get competitive performance as CoT. 


%How can we evidence filtering if training with real/complex dataset? 2) 
% assume correct data in the prefix, can we do better ICL so that $\TF$ will improved itself by looping 

% In a nutshell, $\TF$ can 

==> backup/sec/exp.tex <==
\section{Experiments}
% \subsection{Experimental Setup}
In this section, we present our experiments to evaluate the expressiveness and effectiveness of ICL as compositional learning. Our main results are trained with GPT-2 models.

%Our main results are trained with GPT-2 models with different model sizes.: Small GPT-2, consisting of $6$ layers, $4$ attention heads, and $128$-dimensional embeddings; Tiny GPT-2, with half the layer, attention head, and embedding size; and Standard GPT-2, with double the number of those components. 

% \input{fig_sec/fig_largek}

\subsection{Compositional Learning of 2-layer ReLU Neural Networks}\label{sec:2nn}
To first evaluate the statistical benefit of ICL, we introduce 2-layer neural network experiments by comparing three different methods: $\ICL$, $\EXP$ and $\COT$. Here $\ICL$ follows the same setting as in \cite{garg2022can}, where prompts are given by input-output pairs (also see \eqref{icl pmt}). While $\EXP$ and $\COT$ admit chain-of-thought prompting and $\COT$ does chain-of-thought predictions as well (see \eqref{exp pmt} for $\EXP$ and \eqref{cot pmt} for $\COT$). 


% While the difference between  and Vanilla is that, Explanation has prompt formed by input-instruction-output. Therefore, Transformer can learn more by following the step-by-step messages. In addition to taking all step-messages as input, CoT also trains to predict each step so that the model performs as expected. 

\textbf{Dataset.} Consider 2-layer neural nets with input $\x\in\R^d$, hidden feature (1-step thought) $\tb\in\R^k$, and output $y\in\R$, where $\tb=(\W\x)_+$ and $y=\vv^\top\tb$. Here $\W\in\R^{k\times d}$, $\vv\in\R^{k}$, and $(\cdot)_+$ is the \texttt{ReLU} activation. Hence, the function is composed as $y=\vv^\top(\W\x)_+$ where $\W$, $\vv$ are the respective function parameters following i.i.d. Gaussian distribution, specifically, each entry of $\W$ is sampled via $\W_{ij}\sim\Nc(0,\frac{2}{k})$, and $\vv\sim\Nc(0,\Iden_k)$. Within each prompt, we also randomly sample inputs through $\x\sim\Nc(0,\Iden_d)$. To avoid the implicit bias due to distribution shift, both training and test datasets are generated following the same strategy.

In Figure~\ref{fig:diff gpt}, we train the same dataset with $d=10$ and $k=8$ over three different GPT-2 models: standard, small and tiny GPT-2. The small GPT-2 has $6$ layers, $4$ attention heads per layer and $128$ dimensional embeddings. While, standard GPT-2 contains twice of the layer number, attention heads and embedding dimension of small GPT-2 and tiny only contains half of each. Results show that small model is enough to solve the problem for $\COT$ (Fig.~\ref{fig:diff gpt cot}), while $\EXP$ requires standard GPT-2 model (Fig.~\ref{fig:diff gpt exp}), and $\ICL$ is not able to learn the model recovering the neural networks. It is because that to learn the problem in one shot, the model should be enough to represent all possible 2-layer neural networks and additionally, needs at least $O(dk+d)$ samples.

We then evaluate the three methods based on different neural net architectures (by varying neuron size $k$) and results are shown in Figure~\ref{fig:diff k}. All experiments are trained using small GPT-2, which contains $6$ layers, $4$ attention heads per layer and $128$ dimensional embedding, and blue, orange and green curves correspond to the hidden layer size $4$, $8$, and $16$ respectively. Fix $d=10$ and change neuron number $k\in\{4,8,16\}$. Results show that $\COT$ can learn the neural net using around $60$ samples for $k$ up to $16$ (Fig.~\ref{fig:diff k cot}), $\EXP$ can only learn the narrow neural network with $k=4$ (Fig.~\ref{fig:diff k exp}), and $\ICL$ is not able to learn the networks given $100$ samples (Fig.~\ref{fig:diff k icl}). Following the same setting, Figure~\ref{fig:k16} shows the result when $k=16$. This validates the approximation benefits of CoT prompts and predictions. 

We also observe that there exist alignments in Figure~\ref{fig:diff k cot}, which means $\COT$ needs the same number of sample to learn the given three neural width. The interpretation is that, $\COT$ treats the problem as $k$ $d$-dimensional and $1$ $k$-dimensional linear regression problems and solves them in parallel. Therefore, solving the problem requires $O(\max{(k,d)})$ samples. The evidence in Fig.~\ref{fig:diff k cot} dues from the fact that the data dimension $d$ dominates the problem. To further verify our explanation, in Figure~\ref{fig:cot_d10_vs_d20}, we repeat the $\COT$ experiments but with $d=20$. Dashed curves are showing $d=20$ results with the same $k$ choices. Fig.~\ref{fig:cot_d10_vs_d20_align} shows the alignment in Fig.~\ref{fig:cot_d10_vs_d20}, where $x$-axis is valued by $n/d$ where $n$ is the sample size, which shows that for $d=20$, $\COT$ needs exact two times more samples to learn the neural network compared to $d=10$. What's more in Fig.~\ref{fig:largek}, we tried with larger $k$ so that hidden dimension size $k$ turns to dominate the problem. Fig.~\ref{fig:largek compose} shows the composed CoT risk where $\TF$ first generates \emph{thought} prediction $\hat\tb$, and feeding it back to the model results in the final prediction $\hat y$. While in Fig.~\ref{fig:largek first}, losses are calculated by $\|\tb-\hat\tb\|^2$, and to get the second layer risk in Fig.~\ref{fig:largek second}, we feed toe model with the oracle \emph{thought} $\tb$ and the model only needs to learn the last linear function. To clearer compare their performance, we plot the first risks of $k=4,16$ (dotted) and second layer risk of $k=64$ (dashed) in Fig.~\ref{fig:largek second}. The alignments again verifies our statement that to learn a 2-layer neural network with $d$ input dimension and $k$ neurons, CoT needs exact $O(\max(k,d))$ samples. 

\red{MORE EXPERIMENTS TO DISCUSS:
\begin{itemize}
    \item feed the output of second with zeros/random, and test the filtering observation of first-layer prediction
    \item separately first/second layer predictions are aligned with linear regression problem
\end{itemize}
}

% ----------------------------------

% Comparing $\EXP$ with $\ICL$ shows that, CoT prompt helps in reducing sample size needed in learning the neural network, and $\COT$ achieves the best performance verifies the benefit of step-by-step predictions.


% We evaluate our results based on different neural net architectures (by varying neuron size $k$) and transformer models. 
% ---------------------------

% $\bullet$ \textbf{Vanilla:} $\X_{it}=(\x_{i1},y_{i1},\x_{i2},y_{i2},\cdots,\x_{it})$ and $\y_{it}=y_{it}$.\\
% $\bullet$ \textbf{Explanation: }$\X_{it}=(\x_{i1},\eb_{i1},y_{i1},\x_{i2},\eb_{i2},y_{i2},\cdots,\x_{it},\eb_{it})$ and $\y_{it}=y_{it}$.\\
% $\bullet$ \textbf{CoT: }Different to Vanilla and Explanation, CoT needs to predict both $\eb$ and $y$. Therefore its dataset has two forms: $\X_{it}=(\x_{i1},\eb_{i1},y_{i1},\x_{i2},\eb_{i2},y_{i2},\cdots,\x_{it})$ and $\y_{it}=\eb_{it}$; while $\X'_{it}= (\X_{it},\eb_{it})$ and $\y'_{it}=y_{it}$.

% Treat each sequence as a task, that it, $\W_1,\W_2$ are the same within a sequence, and we randomly sample $n$ tasks as $\W_1,\W_2\sim\Nc(0,1)$.



% the raw input and final prediction in prompt contains all the step message (in neural network, the step messages are the intermediate features). Comparing Explanation with Vanilla shows that ...

% What's more, as for CoT, in addition to feeding all the step messages as prompt, the model also outputs each step following the instruction. The comparison of the three methods are given in Figure~\ref{}.

% % \input{fig_sec/fig_skill}

\subsection{Deep Linear Neural Networks}
In Section~\ref{sec:2nn}, we have discussed the approximation benefit of CoT and how it in-context learns 2-layer ReLU neural network as compositional learns two linear regression problems. In the section, we investigate the ability of CoT in compositional learning long novel chains. In the following, for cleaner notation, we use CoT to refer to $\COT$. 

\textbf{Dataset. } Consider a $L$-layer linear neural nets with input $\x\in\R^d\sim\Nc(0,\Iden_d)$, and output is generated by $\y=\W_L(\W_{L-1}\cdots\W_1(\x))$, where $\W_\ell\in\R^{d\times d}$, $\ell\in[L]$. In this work, we assume each layer is parameterized from the same function set $\Wc=\{\bar\W_k:\bar\W_k^\top\bar\W_k=\Iden,k\in[K]\}$. Therefore to learn the $L$-layer neural net, CoT only needs to learn $\Wc$ whereas $\ICL$ needs to learn function set $\Wc^{L}$, which contains $K^L$ random matrices. 



\subsection{Heterogeneous CoT Prompting}


----------------------------------------------

 and let $\widehat\TF$ be the trained model weighted by $\hat\bt$ from \eqref{erm}. Then the CoT test risk can be defined as 
\begin{align}
    \Lc^{\text{CoT-I}}(\hat\bt,n)=&\E_{\{\x_i\}_{i=1}^n,\f}\left[\ell(\hat\y_n,\y_n)\right]~~~~\text{where}~~~~\hat\y_n=\widehat\TF(\pmt_n(\f),\x_n)
\end{align}
\begin{align}
    \Lc^{\text{CoT-I/O}}(\hat\bt,n)=&\E_{\{\x_i\}_{i=1}^n,\f}\left[\ell(\hat\y_n,\y_n)\right]\\
    \text{where}~~~~&\hat\tb_n^1=\widehat\TF(\pmt_n(\f),\x_n)\\
    &\hat\tb_n^\ell=\widehat\TF(\pmt_n(\f),\x_n,\hat\tb_n^1\cdots,\hat\tb_n^{\ell-1}),~\ell\in[L]
\end{align}

==> backup/sec/experiment_setup.tex <==
\subsection{Experimental setting}


% (we might want to call this a \emph{session} instead?)
\noindent\textbf{Prompt structure:} Each prompt pmt is obtained by concatenating chains i.e.~$pmt=(chn1~chn2~\dots)$. Each chain $chn$ has the following form:
\[
chn=(x_1,s_1,x_2,s_2,\dots,x_{n+1},s_{\text{stop}}).
\]
Here $x_i$ are the features and $s_i$ are the skills. The only requirement is that a chain has to end with $s_{\text{stop}}$.

%distribution $D_i$ over a 
\noindent\textbf{What skills do:} Each skill $s_i$ is associated to a function class $F_i$: Skill $s_i$ means we will apply some $f\in F_i$ on the input. Thus, during training, all triples $(x_i,s_i,x_{i+1})$ satisfy $x_{i+1}=f(x_i)$ where $f\in F_i$. We can call these functions \emph{skill repertoire} (or subskill?). We will later learn these functions in-context because, given $s_i$, it is not clear which function to apply. So training chains have the form
\[
chn=(x,s_1,f^{s_1}(x),f^{s_{1:2}}(x),\dots,f^{s_{1:n}}(x),s_{\text{stop}}).
\]

\noindent\textbf{Example skills to kickstart experiments:} I think each skill $s_i$ can do a matrix multiplication and ReLU nonlinearity (honestly we can even avoid ReLU initially). So imagine for each $F_i$, we generate $1\leq k\leq 10$ random matrices $(W_{ij})_{j=1}^k$ of size $d\times d$ (with $d\leq 5$?) with proper normalization. Then $f_i=(W_{ij}x)_+$.

Important thing here is that each skill has access to their own unique matrices. So it is not simply learning matmul. It is learning exact weights so skill ID matters. Also for skills with $k=1$, skill ID uniquely determines the function so no function learning is needed during ICL time.\footnote{On the other hand, when $k=\infty$, then we have to select from a rich set of functions by learning a continuous ERM algorithm.}
%linear regression (or more generally 

Training involves two datasets. The main goal is to make it so that training process only involves basic learning elements but that basic stuff should suffice to do complex compositional learning.\\

\noindent\textbf{Dataset 1: Learning skills:} Consider all $(i,j)$ pairs where $i$ is the skill ID and $j$ is the subskill ID. We create many prompts with the following rules:
\begin{itemize}
\item All $(i,j)$ pairs should appear in the training data (e.g.~equally likely).
\item Throughout the same prompt, skill $i$ always uses the same subskill/function $f_j^i$. This way transformer will learn $f_j^i$ functions and get to call them in-context.
\item \textbf{Input distribution:} We want to train skill $i$ always with the same input distribution we will use in CoT. This is not difficult for the neural net model above because with He-initialization all other layers except the input should have the same distribution. So we can as well train the skill for both distributions?
\item \textbf{(To discuss)} $(x,i,f_j^i(x))$ tuples should ideally be randomly located throughout the prompt. This way transformer will be less likely to get confused during test-time CoT. Note that within the same prompt, it is totally OK to have many other $(i',j')$ pairs and many chains of varying lengths.
%In other words, use same subskill
\end{itemize}

\noindent\textbf{Remark:} I consider the above dataset to be \emph{clean} in the sense that a skill $i$ uses the same subskill throughout so there is no \emph{noise} when learning which subskill to call. This will be helpful for our CoT to work smoothly. Our next goal is creating a clean dataset for skill prediction.
%$f_j^i$ where $i$ is the skill ID and $j$ is the subskill ID. We create

\smallskip\smallskip
\noindent\textbf{Dataset 2: Predicting skills.} The previous dataset aimed to answer $(x,s_i,?)$. This dataset aims to answer $(s_{i-1},x,?)$. The idea is learning the transition purely based on the previous skill $s_{i-1}$. We generate arbitrary admissable prompts with the following rules
\begin{itemize}
\item Suppose $(i,j)$ are all feasible skill pairs where $j$ can follow $i$. More generally, we can assume skill pairs is a graph (perhaps some skills can't follow another). In that case $j$ is a neighbor of $i$. All feasible $(i,j)$ pairs should appear in the training data.
\item First $n/2$ tokens in the prompt can be arbitrary (which will lie within the prefix demonstrations for the CoT). However, in the second $n/2$ half of the prompt, the skill that follows $i$ should always be based on majority rule. For instance if first half contains $(i,1),(i,2),(i,1)$ pairs, then for the rest of the prompt $1$ is the skill that follows $i$. 
\item Note that prompt can contain many skills besides $i$. Also it is OK to make the data noiseless in the sense that $i$ is always followed by the same skill. However this would make our prompts less realistic.
\item \textbf{(To discuss)} We need to decide whether $s_{stop}$ skill uses the majority rule as well. Because if it does, then after $n/2$ all chains will have to be same making the prompt model less realistic.
\end{itemize}

\smallskip\smallskip
\noindent\textbf{Test Dataset for CoT:} We would like CoT to work without showing the exact skill sequence and for arbitrarily many skills. We engineer the CoT prompt backwards.

Suppose we would like the following CoT chain to succeed:
\[
(x_1,s_1,x_2,\dots, s_n,x_{n+1},s_{\text{stop}})
\]
after only seeing $(x_1)$.
%\footnote{In general we only need to see $(x_1)$ as long as $x_1$ the input distribution is always followed by the prompt $s_1$ during training.} 
Here is how:
\begin{enumerate}
\item The model moves to the correct skill $s_1$ because in the prefix $s_1$ follows $s_{stop}$ majority of the times $s_{stop}$ appears. Similarly correct $s_2$ will follow $s_1$ based on the prefix appearances of $s_1$.
\item The model outputs $f^{s_1}_{j_1}(x_1)$ correctly because prefix prompt always uses subskill $j_1$ for $s_1$.
\item Repeat this argument until seeing $s_{stop}$.
\item \textbf{(To discuss)} If $s_{stop}$ does not follow the majority rule described above, then we have 2 options: We either have to specify $(x_1,s_1)$ to start the CoT or we have to infer $s_1$ from distribution of $x$. The latter can be done by partitioning the input space so that each starter skill $s_1$ can be uniquely distinguished from its input.
\end{enumerate}

\noindent\textbf{Remark:} Note that in order to create a chain of length $10$, we only need 10 short chains of size $2$. We just need to show instances of $s_i\rightarrow s_{i+1}$ but those instances can be different input features.

==> backup/sec/filtering.tex <==
As we mentioned in Subsection \ref{subsec cot}, we would expect \AG{Add here that we want to see why ICL-IO performs better and evaluate our intuition and observation of previous setting. To do so we extend it to deep NN and observe again }

\paragraph{Dataset. }

\paragraph{Filtering. }We speculated that this behavior is due to a filtering step. RESULTS and figures.


\paragraph{Construction of the filtering process. }To demonstrate that it is indeed possible for a transformer to perform a filtering process we explicitly construct..

==> backup/sec/functions.tex <==

In this section, we demonstrate how to implement a variety of nonlinear functions and basic linear algebra operations using transformers. These techniques will be crucial in the construction of iterative algorithms in the following sections. %We will show how to use transformer function blocks to implement non-linear sigmoid based functions, and basic matrix operations. 
Each transformer-based function block in this section fits in our unified template in terms of input/output parameters' locations. We note here that each transformer-based function block might have its own positional encodings used to transfer the output in the correct place or perform some \texttt{read/write} operations and they are part of the design of the block.


\subsection{Encoding Non-linear Functions within the Attention Mechanism}%\label{ss:sigmoids}
One key ingredient of our constructions %demonstrate how to emulate 
is encoding various functions within the attention mechanism. We do this by forcing the softmax to act as a sigmoid function and by storing multiple coefficients in the query and value weight matrices. As far as we know, this is the first work that shows how general non-linear functions can be emulated by attention layers. This allows us to create linear combinations of sigmoids that can be accessed by an indicator vector in the input. Our analysis is based on the result of \cite{Barron93} which we present below. 

\begin{definition} Let $\Gamma_{C,B}$ be the set of functions defined in a bounded domain $B$, $f:B\to \mathbb{R}, B\subseteq \R^d$ with a proper extension to $\R^d$ such that they have $C$ bounded Fourier integral, \ie \\$\int \sup_{x \in B} | w \cdot x | \ F(dw) \le C$ holds where $F(dw)$ is the magnitude of the Fourier distribution.
%\jnote{is bounded fourier integral clear? It's like the $\| \hat f\|_1$?}
\end{definition}
\begin{definition} Given $\tau >0, C>0$ and a bounded set $B$, 
    let 
    \begin{equation}
        G_{\sigmoid,\tau} = \braces{\gamma\sigmoid(\tau(\rva^T\rvx + b)): \abs{\gamma}\leq 2C,\norm{\rva}_B \leq 1, \abs{b} \leq 1} \nonumber
    \end{equation}
    where $\norm{\rva}_B = \sup_{\rvx\in B} \braces{\rvx^T\rva}$ and $\sigmoid$ is the sigmoid function, \ie $\sigmoid(x) =\frac{1}{1+e^{-x}}$.
\end{definition}
\begin{theorem}[Theorem 3 in \cite{Barron93}]\label{th:Barron}
Every function $f\in\Gamma_{C,B}$ with $f(0) =0 $ and  can be approximated by a linear  combination of sigmoids $f_i\in G_{\sigmoid,\tau}$, $i=1,\hdots m$. If $\tau \geq m^{1/2}\ln m$  the  error scales as
\begin{equation}
    \abs*{f(\rvx) - \sum_{i=1}^m f_i(\rvx)}\leq O\parens*{\dfrac{1}{m^{{1/2}}}} , \; \rvx\in B \nonumber
\end{equation}
\end{theorem}

To encode $N$ different functions, we use the index $j\in[N]$ and write $c_{ji},\rva_{ji}$ for the coefficients of the sigmoids that approximate them or 

\begin{equation}
    f_j(\rvx) = \sum_{i=1}^m c_{ji} \sigmoid( \rvx^T\rva_{ji}) \text{ for }j = 1,\hdots,N \nonumber
\end{equation}
We here note that the terms $\tau, b$ can be incorporated in the term $\rva_{ij}$ by adding an extra coefficient of $1$ in $\rvx$ and multiplying everything with $\tau$.

We are now able to present the lemma on approximating functions using transformer blocks, in a format that is consistent with the FLEQ design outlined in the previous section.

\begin{lemma}\label{lem:sigmoids}
Fix $\epsilon>0$ and consider an input of the form 
\begin{equation}
    \Input = \bracks*{ \begin{array}{cc|cc|cc}
        \ve & \zero&\rvx&\zero &\zero &\zero \\%&\zero\\
        \zero  &\zero & \zero& \zero &\zero&\zero\\
        \zero &\zero &\emb_{2d+1} &\zero &\zero &\zero\\
        \emb_1&\emb_{2:d}&\zero&\emb_{d+2:2d} &\emb_{2d+1} &\emb_{2d+2:3d}\\
        0 & 0_{2:d} & 1 & 0_{d+2:2d} & 0 & 0_{2d+2:3d}
    \end{array}} . \nonumber
\end{equation}
where $d$ is chosen according to the \texttt{FLEQ} construction from the previous section and $N$ is the number of functions we encode . $\ve = \rve_j\in\R^N$ is an indicator vector signifying the function we wish to execute.  Then there  exists a   transformer-based function block with 3 layers, $m$ heads and dimensionality $r = 2\log(d) +d+1 = O(d)$ such that  \begin{equation}
    f(\Input) =  \bracks*{ \begin{array}{cc|cc|cc}
        *&*&*&*&\sum_{i=1}^m c_{ji}\sigmoid(\rvx^T\rva_{ji}) +\epsilon & *\\
        \zero  &\zero & \rvx& \zero &\zero&\zero\\
         \zero &\zero &\emb_{2d+1} &\zero &\zero &\zero\\
       \emb_1&\emb_{2:d}&\zero&\emb_{d+2:2d} &\emb_{2d+1} &\emb_{2d+2:3d}\\
        0 & 0_{2:d} & 1 & 0_{d+2:2d} & 0 & 0_{2d+2:3d}
    \end{array} }\nonumber
\end{equation}
where $*$ denoted inconsequential values that will be ignored downstream. This implies that arbitrary function $g \in \Gamma_{C,B}$ can be well approximated by attention layers. 
\end{lemma}
\begin{remark}
Notice that in this case we don't use any extra scratchpad space and thus $s=3d$; however if this function block was to be used with another one that needs $s>3d$ scratchpad space, we would simply zero pad the input of \cref{lem:sigmoids} and ignore these columns. The same holds for the rest of the transformer-based function blocks and we will not mention it from now on. 
\end{remark}

In the expression $\sum_{i=1}^m c_{ji}\sigmoid(\rvx^T\rva_{ji})$, the number head is equal to the number of terms we need.%is equal to the number of heads $m$. 
We show in the appendix that we can actually encode these $m$ terms in the dimension of the transformer architecture with just one head (See \cref{cor:lem_5_alt}). %the number of terms can also scale proportional to the dimension $d$ in \cref{cor:lem_5_alt}. 
The choice of which result to use can depend on the specific design and can affect both accuracy and efficiency of the implemented transformer network.

The proof of this Lemma is given in \cref{app:functions}.
% %We note that the first layer will create the value $\sum_{i=1}^m c_{ji}\sigmoid(\rvx^T\rva_{ji})$ similarly to the proof of \cref{lem:sigmoids}, while the second layer will use the \cref{lem:write} to place the value in the desired position.
% %; a formal proof is given in \cref{app:functions}.
% %\cref{app:functions}.
% \begin{proof} 
% The first thing we do is to move the $\rvx$ to the second row block, as follows:
% \begin{equation*}
%     \Input = \begin{bmatrix}
%         \ve & \zero&\rvx &\zero &\zero &\zero\\
%         \zero  &\zero & \zero& \zero &\zero&\zero\\
%         \zero &\zero &\emb_{2d+1} &\zero &\zero &\zero\\
%         \emb_1&\emb_{2:d}&\zero&\emb_{d+2:2d} &\emb_{2d+1} &\emb_{2d+2:3d}\\
%         0 & 0_{2:d} & 1 & 0_{d+2:2d} & 0 & 0_{2d+2:3d}
%     \end{bmatrix} \to \begin{bmatrix}
%         \ve & \zero&\zero &\zero &\zero &\zero\\
%         \zero  &\zero & \rvx & \zero &\zero&\zero\\
%         \zero &\zero &\emb_{2d+1} &\zero &\zero &\zero\\
%         \emb_1&\emb_{2:d}&\zero&\emb_{d+2:2d} &\emb_{2d+1} &\emb_{2d+2:3d}\\
%         0 & 0_{2:d} & 1 & 0_{d+2:2d} & 0 & 0_{2d+2:3d}
%     \end{bmatrix}
% \end{equation*}
% This can be done using a ReLU feedforward layer that performs this using the last row of the input as the indicator bit for the column containing $\dpoint$.

% Then we want to create the following transformation
% \begin{equation*}
%     \begin{bmatrix}
%         \ve & \zero&\zero &\zero &\zero &\zero\\
%         \zero  &\zero & \rvx& \zero &\zero&\zero\\
%         \zero &\zero &\emb_{2d+1} &\zero &\zero &\zero\\
%         \emb_1&\emb_{2:d}&\zero&\emb_{d+2:2d} &\emb_{2d+1} &\emb_{2d+2:3d}\\
%          0 & 0_{2:d} & 1 & 0_{d+2:2d} & 0 & 0_{2d+2:3d}
%     \end{bmatrix} \xrightarrow[]{} \begin{bmatrix}
%         *&*&*&*&\sum_{i=1}^m c_{ji}\sigmoid(\rvx^T\rva_{ji}) & *\\
%         \zero  &\zero & \rvx& \zero &\zero&\zero\\
%          \zero &\zero &\emb_{2d+1} &\zero &\zero &\zero\\
%       \emb_1&\emb_{2:d}&\zero&\emb_{d+2:2d} &\emb_{2d+1} &\emb_{2d+2:3d}\\
%         0 & 0_{2:d} & 1 & 0_{d+2:2d} & 0 & 0_{2d+2:3d}
%     \end{bmatrix}
% \end{equation*}
% The proof follows that of \cref{lem:sigmoids}. We again ignore the last three rows by setting the corresponding rows in the key, query and values weight matrices to be zero. Let 
% \begin{equation}
%          \query^{i} = \begin{bmatrix}
%          \zero &\id_d\\
%          \zero &\zero 
%      \end{bmatrix}, \key^i = \begin{bmatrix}
%          [\rva_{1i} \; \hdots \; \rva_{Ni}] & \zero\\
%          \zero &\zero
%      \end{bmatrix} , \val^i = \begin{bmatrix}
%         [c_{1i} \;\hdots \; c_{Ni}] &\zero \\
%         \zero  &\zero
%      \end{bmatrix} \nonumber
% \end{equation}
% We note that for the purpose of this proof, each $\rva_i$ has one extra element at the end equal to $-\log(3d-1)$, while the vectors $\rvx$ will have the last element equal to one. Then we will have
% \begin{align*}
%     \softmax((\key^i\Input)^T(\query^i\Input)) &= \begin{bmatrix}
% \rva_{ji}^\top & \zero \\ 
% \zero  & \zero  \\ 
% \zero  & \zero  \\ 
% \zero  & \zero  \\ 
% \zero  & \zero  \\ 
% \zero  & \zero  \\ 
% \end{bmatrix}\begin{bmatrix}
% \zero &\zero &\rvx &\zero &\zero &\zero\\
% \zero &\zero &\zero &\zero &\zero &\zero\\
% \end{bmatrix}\\
% &= \begin{bmatrix}
%     \zero &\zero &\rva_{ji}^\top\rvx&\zero &\zero &\zero\\
%     \zero &\zero &\zero &\zero &\zero &\zero\\
%     \zero &\zero &\zero &\zero &\zero &\zero\\
%     \zero &\zero &\zero &\zero &\zero &\zero\\
%     \zero &\zero &\zero &\zero &\zero &\zero\\
%     \zero &\zero &\zero &\zero &\zero &\zero\\
% \end{bmatrix}\\
%     &=\begin{bmatrix}
% * & * &\sigmoid(\rvx^T\rva_{ji}) & * & *   &*\\ 
% * & * &*  & * & * &*\\ 
% * & * &*  & * & * &*\\ 
% * & * &*  & * & * &*\\ 
% * & * &*  & * & * &*\\ 
% * & * &*  & * & * &*\\ 
% \end{bmatrix}
% \end{align*}
% since $\rva_{ji}^\top\rvx = \rva_{ji}^\top\rvx -\log{3d-1}$ and thus $\exp^{\rva_{ji}^\top\rvx}/(3d-1 + \exp^{\rva_{ji}^\top\rvx}) = \sigmoid(\rva_{ji}^\top\rvx)$ with a slight abuse of notation over the inner product $\rva_{ji}^\top\rvx$ to account for the extra corrections bias term. Thus, 
% \begin{equation}
%  \val\Input\softmax( (\key\Input)^T(\query\Input) ) = \begin{bmatrix}
%  * & * &c_{ji}\sigmoid(\rvx^T\rva_{ji}) & * & *   &*\\
%   \zero &\zero &\zero &\zero &\zero &\zero\\
%     \zero &\zero &\zero &\zero &\zero &\zero\\
%     \zero &\zero &\zero &\zero &\zero &\zero\\
%     \zero &\zero &\zero &\zero &\zero &\zero\\
%  \end{bmatrix} \nonumber
% \end{equation}
% By summing over all heads and adding the residual we get
% \begin{equation}
%     \begin{bmatrix}
%         *&*&\sum_{i=1}^m c_{ji}\sigmoid(\rvx^T\rva_{ji})&*&* & *\\
%         \zero  &\zero & \rvx& \zero &\zero&\zero\\
%          \zero &\zero &\emb_{2d+1} &\zero &\zero &\zero\\
%       \emb_1&\emb_{2:d}&\zero&\emb_{d+2:2d} &\emb_{2d+1} &\emb_{2d+2:3d}\\
%         0 & 0_{2:d} & 1 & 0_{d+2:2d} & 0 & 0_{2d+2:3d}
%     \end{bmatrix} \nonumber
% \end{equation}
% Finally, we use an extra layer similarly to \cref{lem:write} to write the result in the desired output. Hence, we get
% \begin{equation}
%     \begin{bmatrix}
%         *&*&*&*&\sum_{i=1}^m c_{ji}\sigmoid(\rvx^T\rva_{ji}) & *\\
%         \zero  &\zero & \rvx& \zero &\zero&\zero\\
%          \zero &\zero &\emb_{2d+1} &\zero &\zero &\zero\\
%       \emb_1&\emb_{2:d}&\zero&\emb_{d+2:2d} &\emb_{2d+1} &\emb_{2d+2:3d}\\
%         0 & 0_{2:d} & 1 & 0_{d+2:2d} & 0 & 0_{2d+2:3d}
%     \end{bmatrix} \nonumber
% \end{equation} 
% \end{proof}



\subsection{Matrix Transposition and Multiplication by Linearizing the Softmax}
We assume that a $d\times d$ matrix $\rmA$ in the input $\Input$ is represented by a sequence of length $d$, and each of these $d$ columns  has $d$ rows. %of $\Input$ contains one column of $\rmA$. 
While this representation has the advantage that it is well suited for the matrix multiplication operation (as we will see in the next sub-section), a vectorized form of the matrix is more suited to create transpose. This is how we implement the transpose; we first vectorize the matrix $\rmA$, then with a fixed permutation of the columns we create its vectorized version of a transpose.

% Two important components of linear algebra are matrix multiplication and transposition. We now show that a matrix can be stored in two forms in the transformer input, and each has an advantage for one of these operations.
\begin{lemma}\label{lem:transpose}
Fix $\epsilon >0$ and consider an input of the following form
\begin{equation}
    \Input = \left[\begin{array}{c|c|c|cc}
        \rmA  &\zero&\zero &\dots & \zero \\
 \zero&      \zero&\zero &\dots & \zero\\
         \emb_{1:d}&\emb_{1:d}&\emb_{1:d}& \dots  &\emb_{1:d}\\
         \rmP_1'&\rmP_{2}'&\rmP_{3}'& \dots  &\rmP_{d}'
    \end{array}\right]. \nonumber
\end{equation}
where $\rmA\in\R^{d\times d}$; then there exists transformer-based function block with 4 layers, 1 head and dimensionality $r = 2d+2\log d = O(d)$ that outputs the following matrix
\begin{equation}
    \Input = \left[\begin{array}{c|c|c|cc}
\rmA' &\rmA'&\rmA'&\dots &\rmA' \\
        \zero&\zero&\zero &\dots &\zero \\
         \emb_{1:d}& \emb_{1:d}& \emb_{1:d}& \dots &\emb_{1:d} \\
        \rmP_1'&\rmP_{2}'&\rmP_{3}'& \dots  &\rmP_{d}'
    \end{array}\right]. \nonumber
\end{equation}
where $\rmA' = \rmA^\top +\epsilon\rmM$, for some $\norm{\rmM}\leq 1$. The error $\epsilon$ depends on the choice of the temperature $\lambda$, as it is  a consequence of the \texttt{read/write} operations.
\end{lemma}
% \begin{lemma}\label{lem:transpose}
% Let the input of the transformer-based function block to be
% \begin{equation}
%     \Input = \left[\begin{array}{cccc|c|c}
%         \rmA  &\zero&\dots & \zero &\zero  \\
%  \zero&      \zero&\dots & \zero \\
%          \emb_{1:m}&\emb_{1:m}& \dots  &\emb_{1:m}\\
%          \rmP_1'&\rmP_{2}'& \dots  &\rmP_{m}'\\
%          \zero &\rvOne^\top &\dots&\rvOne^\top 
%     \end{array}\right]. \nonumber
% \end{equation}
% where $\rmA\in\R^{k\times m}, m\geq k$, the total number of columns is $m^2$ and $\embed_i^{'} = [\emb_i \dots \emb_i] $ for all $i=1,\dots,m$. Then,
% there  exists a transformer-based function block with 4 layers, 1 head and dimensionality $O(k+\log m)$ that has as output the following matrix
% \begin{equation}
%     \Input = \left[\begin{array}{cc|c}
% \rmA^\top &\dots &\rmA^\top \\
%         \zero &\dots &\zero \\
%          \emb_{1:m}& \dots &\emb_{1:m} \\
%          \embed_1'& \dots &\embed_{m}' 
%     \end{array}\right]. \nonumber
% \end{equation}
% \end{lemma}
% Notice that this form fits in our unified template, with the first $d = \dfrac{m^2-m}{2} $
% \proof
% We can vectorize the matrix $\rmA$ into a $d^2$ dimensional vector using the attention mechanism, as shown in Eq. \eqref{eq:vectorized_matrix}. 
% Notice that once we have the matrix in this form we can implement its transpose with a fixed permutation of the columns of the matrix to get the vectorized form of $\rmA^\top$. Once we have the transpose in vector form, we matricize it back to get the matrix transform using the attention mechanism. We explain the details of this process below:

% \emph{Vectorization: } We assume that the input is of the following form, where $\rmA$ is the matrix to be vectorized.
% % \begin{equation}
% %     \Input = \left[\begin{array}{ccc|c}
% % \zero &\dots &\zero &\zero\\
% %         \zero &\dots &\zero & \rmA\\
% %          \emb_{1:d}& \dots &\emb_{1:d} &\emb_{1:d}\\
% %          \emb_1'& \dots &\emb_{d}' &\emb_{d+1}'
% %     \end{array}\right].
% % \end{equation}
% \begin{equation}
%     \Input = \left[\begin{array}{cccc}
%         \rmA  &\zero&\dots & \zero\\
%  \zero&      \zero&\dots & \zero\\
%          \emb_{1:d}&\emb_{1:d}& \dots  &\emb_{1:d}\\
%          \rmP_1'&\rmP_{2}'& \dots  &\rmP_{d}'
%     \end{array}\right]. \nonumber
% \end{equation}
% Here, $\rmP_i'$ represents a matrix of $d$ columns, where each column is $\emb_i$.

% % \begin{equation}
% %     \Input = \left[\begin{array}{c|c}
% %          \rmS & \zero \\
% %         \zero & \rmA\\
% %         \zero &\emb_{d^2+1:d^2+d}\\
% %          \emb_{1:d} &\zero\\
% %          \emb_{1:d^2} &\emb_{d^2+1:d^2+d}
% %     \end{array}\right]
% % \end{equation}
% %The attention mechanism 
% The first layer uses the $\emb_{1:d}$ encodings to make $d$ copies of the matrix $\rmA$, as follows:
% \begin{equation}
%     \Input = \left[\begin{array}{cccc}
% \rmA&\zero &\dots &\zero \\
%  \rmA &\rmA&\dots & \rmA\\
%          \emb_{1:d}&\emb_{1:d}& \dots &\emb_{1:d} \\
%          \emb_1'&\emb_2'& \dots &\emb_{d}' 
%     \end{array}\right]. \nonumber
% \end{equation}


% The feed forward part of the second layer then uses the encodings $\emb_i'$ to vectorize the matrix in the second row block as follows:

% \begin{equation}
%     \Input = \left[\begin{array}{ccc}
%     \rmA&\dots&\zero\\
% \begin{bmatrix}
%     A_{(1,1)}&\dots &A_{(1,d)}\\
%     \zero&\dots&\zero\\
% \end{bmatrix} &\dots &\begin{bmatrix}
%     A_{(d,1)}&\dots &A_{(d,d)}\\
%     \zero&\dots&\zero\\
% \end{bmatrix} \\
%          \emb_{1:d}& \dots &\emb_{1:d} \\
%          \emb_1'& \dots &\emb_{d}' 
%     \end{array}\right].\label{eq:vectorized_matrix} 
% \end{equation}

% \emph{Transposition in the vector form:}
% Once we have the matrix vectorized as the second row block of the scratchpad, the following key and query matrices 
% \begin{align*}
%     \key = \begin{bmatrix}
%         \zero &\zero & \id& \zero\\
%         \zero &\zero & \zero& \id
%     \end{bmatrix}, \query = \begin{bmatrix}
%         \zero &\zero & \zero& \id\\
%         \zero &\zero & \id&\zero
%     \end{bmatrix},  
% \end{align*}
% results in the head outputting the following, which is the vectorized form of $\rmA^\top$ (in the second row block)
% \begin{align*}
%     \Input \softmax((\key \Input)^\top (\query \Input)) = \left[\begin{array}{ccc}
%      *&\dots&*\\
% \begin{bmatrix}
%     A_{(1,1)}&\dots &A_{(d,1)}\\
%     \zero&\dots&\zero\\
% \end{bmatrix} &\dots &\begin{bmatrix}
%     A_{(1,d)}&\dots &A_{(d,d)}\\
%     \zero&\dots&\zero\\
% \end{bmatrix} \\
%          \emb_1'& \dots & \emb_{d}'\\
%          \emb_{1:d}& \dots &\emb_{1:d} 
%     \end{array}\right].
% \end{align*} Then, using the following value matrix gives
% \begin{align*}
%     \val = \begin{bmatrix}
%     \zero&\zero & \zero& \zero\\
%         \zero&\id & \zero& \zero\\
%         \zero&\zero & \zero& \zero\\
%         \zero&\zero & \zero& \zero
%     \end{bmatrix},
% \end{align*}
% \begin{align*}
%   \val \Input \softmax((\key \Input)^\top (\query \Input)) = \left[\begin{array}{ccc}
%   \zero&\dots&\zero\\
% \begin{bmatrix}
%     A_{(1,1)}&\dots &A_{(d,1)}\\
%     \zero&\dots&\zero\\
% \end{bmatrix} &\dots &\begin{bmatrix}
%     A_{(1,d)}&\dots &A_{(d,d)}\\
%     \zero&\dots&\zero\\
% \end{bmatrix} \\
%          \zero& \dots & \zero\\
%          \zero& \dots &\zero 
%     \end{array}\right],
% \end{align*}
% Adding back the $\Input$ (see \eqref{eq:TF}), results in 
% \begin{equation}
%     \Input + \val \Input \softmax((\key \Input)^\top (\query \Input)) = \left[\begin{array}{ccc}
%     \rmA&\dots&\zero\\
% \begin{bmatrix}
%     A_{(1,1)}&\dots &A_{(d,1)}\\
%     \zero&\dots&\zero\\
% \end{bmatrix} &\dots &\begin{bmatrix}
%     A_{(1,d)}&\dots &A_{(d,d)}\\
%     \zero&\dots&\zero\\
% \end{bmatrix} \\
%          \emb_{1:d}& \dots &\emb_{1:d} \\
%          \emb_1'& \dots &\emb_{d}' 
%     \end{array}\right]. \nonumber
% \end{equation}

% Using the feedforward layers and the encodings $\emb_i'$, we get
% \begin{equation}
%     \Input = \left[\begin{array}{ccc}
%     \rmA&\dots&\zero\\
% \begin{bmatrix}
%     A_{(1,1)}&\dots &A_{(d,1)}\\
%     \zero&\dots&\zero
% \end{bmatrix} &\dots &\begin{bmatrix}
%     \zero&\dots&\zero\\
%      A_{(1,d)}&\dots &A_{(d,d)}
% \end{bmatrix}\\
%          \emb_{1:d}& \dots &\emb_{1:d} \\
%          \emb_1'& \dots &\emb_{d}' 
%     \end{array}\right]. \nonumber
% \end{equation}

% Using an attention layer, we get 
% \begin{equation}
%     \Input = \left[\begin{array}{ccc}
% \rmA^\top &\dots &\rmA^\top \\
%         \zero &\dots &\zero \\
%          \emb_{1:d}& \dots &\emb_{1:d} \\
%          \emb_1'& \dots &\emb_{d}' 
%     \end{array}\right]. \nonumber
% \end{equation}
% %  We set $\emb'_{1:d^2}$ to be the encodings $\emb_{d^2+1:d^2+d}$ copied $d$ times. For $\emb^{''}_{1:d^2}$ we use the encodings to do the necessary copy of the column such that in the first $d$ rows we will Now by using the general form of the copy operation we can create 
% % \begin{equation}
% %     \Input = \left[\begin{array}{ccc|c}
% % \rmA &\dots &\rmA &\zero\\
% %         \zero &\dots &\zero & \rmA\\
% %         \zero &\dots & \zero &\emb_{d^2+1:d^2+d}\\
% %          \emb'_{1:d}& \dots &\emb'_{d^-d:d^2} &\zero\\
% %          \emb_{1:d}& \dots &\emb_{d^-d:d^2} &\emb_{d^2+1:d^2+d}
% %     \end{array}\right]
% % \end{equation}



%paragraph{Matrix Multiplication by Linearizing the Softmax.}

In order for matrix multiplication to fit in our unified template, we need to show for example for the result of $\rmA^\top\rmB$ , where $\rmA\in\R^{k\times m}$ and $\rmB\in\R^{k\times n}$ with $k,m,n <d$ we can achieve the following:
\begin{equation}
   \bracks*{  \begin{array}{cc|cc|cc}
        \rmA & \zero &\rmB &\zero &\zero&\zero\\
        \zero& \zero &\zero&\zero&\zero &\zero
    \end{array}}\xrightarrow[]{}\bracks*{ \begin{array}{cc|cc|cc}
        *& *&*&* &\rmA^\top\rmB &*\\
        \zero& \zero &\zero&\zero&\zero &\zero 
    \end{array} }\nonumber
\end{equation}
The idea we leverage is the linearization of the softmax, \ie for a column vector $\vz = [\vx\;, C]$ for some large constant $C$ we have that $$\softmax(\vz)  = [\vx + \eps \;, *]$$
The error $\eps$ is controlled by the constant $C$.
% \begin{equation}
%     \begin{bmatrix}
%         \rmA & \zero%_{(k,d-m)} &\rmB &\zero_{(k,d-n)} &\zero_{(k,d)}\\
%         \zero_{(d-k,m)} & \zero_{(d-k,d-m)} &\zero_{(d-k,n)}&\zero_{(d-k,d-n)}&\zero_{(d-k,d)}
%     \end{bmatrix}\xrightarrow[]{}\begin{bmatrix}
%         \rmA & \zero_{(k,d-m)} &\rmB &\zero_{(k,d-n)} &\zero_{(k,d)}\\
%         \zero_{(d-k,m)} & \zero_{(d-k,d-m)} &\zero_{(d-k,n)}&\zero_{(d-k,d-n)}&\zero_{(d-k,d)}
%     \end{bmatrix}
% \end{equation}
\begin{lemma}\label{lem:matrixmul}
Let $\rmA\in \R^{k\times m}$ and $\rmB \in \R^{k\times n}$; then for any $\epsilon >0$ there exists a transformer-based function block with  2 layers, 1 head and dimensionality $r = O(d)$ that  outputs the multiplication $\rmA^\top\rmB +\eps\rmM$, for some $\norm{\rmM}\leq 1$ .
\end{lemma}
The implementation of $\rmB^\top\rmA$, $\rmA^\top\rmA$ and $\rmB^\top\rmB$ are simple corollaries of the lemma presented above and we will freely use them in the subsequent sections.
In \cref{app:functions}, we provide the exact form of the input $\Input$ for implementing matrix transposition/multiplication,
%(with the encodings needed), 
as well as the proof of the corresponding Lemmas. 
%this and the previous two lemmas can be found in \cref{app:functions}. 


% \begin{corollary}
% Let $\rmA\in k\times m$ and $\rmB \in k\times n$; then there exists a transformer-based function block with 2 layers, 1 head and dimensionality $O(d)$ %two layer transformer-based function block 
% that approximately implements the multiplication $\rmB^T\rmA^T$.
% \end{corollary}
% \begin{corollary}
% Let $\rmA\in k\times m$ and $\rmB \in k\times n$; then there exists a  transformer-based function block  with 2 layers, 1 head and dimensionality $O(d)$, that approximately implements the multiplication $\rmA^T\rmA$.
% \end{corollary}
% \begin{corollary}
% Let $\rmA\in k\times m$ and $\rmB \in k\times n$; then there exists a  transformer-based function block  with 2 layers, 1 head and dimensionality $O(d)$, that approximately implements the multiplication $\rmB^T\rmB$.
% \end{corollary}


% We will prove just the first of these results and the rest are a simple corollary of it.
% \begin{proof}
% Let $\rmM\in \R^{2d\times 2d}$, $\rmA\in\R^{k\times m}$ and $\rmB\in\R^{k\times n}$ be the following matrices:
% \begin{align*}
%     \rmM = \begin{bmatrix}
%         \rmA &\zero&\rmB  &\zero \\
%         \zero&\zero &\zero &\zero
%     \end{bmatrix}.
% \end{align*}
% The zeros pad the rows and columns to ensure that the matrix $M$ is $2d\times 2d$.
% Then, consider the input matrix to be of the following form:
% \begin{equation}
%     \Input = \begin{bmatrix}
%         \rmM& \zero &\zero \\
%         \zero & \rvOne\rvOne^\top &\zero\\
%         \id&\zero &\zero\\ 
%         &\emb^{(1)}&\\
%         &\emb^{(2)}&\\
%         \zero &\rvOne^T &\zero 
%     \end{bmatrix}  \nonumber
% \end{equation} 
%  where $\rvOne\in\R^{2d}$ is the all ones vector. The identity matrix $\id$ and the all ones matrix $\rvOne\rvOne^\top$ are part of the design of the input and they are always fixed. For now we ignore the  encodings and the last row, by setting the corresponding rows of the key,query and value weight matrices to be zero. These rows will be used to copy the output to the  place that we want. %Assuming that we want to output $\rmA^\top\rmA$ these encodings would be 
% % \begin{align}
% % \embed_1&= \begin{bmatrix}
% %     \emb_1 &\cdots &\emb_d & \zero& \cdots &\zero &\zero &\cdots &\zero 
% % \end{bmatrix}\\
% % \embed_2 &= \begin{bmatrix}
% %     \zero &\cdots & \zero &\zero &\cdots&\zero &\emb_{1} &\cdots &\emb_d
% % \end{bmatrix}
% % \end{align}

% Focusing on the rest of the rows, we set the key  and query weight matrices to be 
% \begin{equation}
% \key = \id, \query = \begin{bmatrix}
%      c\id & \zero &\zero\\
%     \zero &\zero &C\id\\
%      \zero & \id &\zero
% \end{bmatrix}, \val = \begin{bmatrix}
% \zero & \zero &\zero\\
% \zero & \zero &ne^C\cD_d\\
% \zero &\zero &\zero
% \end{bmatrix} \nonumber
% \end{equation}
% where $\cD_d\in \R^{2d\times 2d}$ is the diagonal matrix with the first $d$ diagonal elements $1$, and the rest 0.
% %as in \cref{ss:matrixmul} and by repeating the same steps and considering the same transformation $\ell$ we have
% Thus we have
% \begin{align}
%     (\key\Input)^\top\query\Input &= \begin{bmatrix}
%         \rmM& \zero &\zero \\
%         \zero & \rvOne\rvOne^\top &\zero\\
%         \id&\zero &\zero\\
%     \end{bmatrix}^\top \begin{bmatrix}
%         c\rmM & \zero &\zero\\
%         C\id &\zero &\zero\\
%         \zero &\rvOne\rvOne^\top &\zero 
%     \end{bmatrix}\\
%     &= \begin{bmatrix}
%         c\rmM^\top\rmM &\rvOne\rvOne^\top &\zero\\
%         C\rvOne\rvOne^\top &\zero &\zero\\
%         &\zero &\zero &\zero 
%     \end{bmatrix}
% \end{align}
% Each of the first $2d$ columns above looks as follows
% \begin{equation}
%     \begin{bmatrix}
%       cz_{1i} &cz_{2i} &\dots &cz_{ni} & C\rvOne^\top &\zero
%     \end{bmatrix} \nonumber
% \end{equation}
%  After we apply the softmax $\sigma_s$ per column, we get 
%  \begin{equation}
%   \sigma_s(cz_{ij}) = \dfrac{e^{cz_{ij}}}{\sum_{j=1}^n e^{cz_{ij}} + n(e^{C}+1) } \nonumber
% \end{equation}
% where $n=2d$, $z_{ij}$  is the $(i,j)$ element of the matrix $\rmM^\top\rmM$. Let $\ell(\cdot)$ be the transformation above then we have

% \begin{align*} \val\Input\softmax((\key\Input)^\top\query\Input) &= \begin{bmatrix}
%     \zero &\zero &\zero\\
%     ne^C\cD_d &\zero &\zero\\
%     \zero &\zero &\zero 
%     \end{bmatrix}\begin{bmatrix}
%         \ell(c\rmM^\top\rmM) &* &*\\
%         * &* &*\\
%         *&*&*
%     \end{bmatrix}\\
%     &=\begin{bmatrix}
%         \zero &\zero &\zero\\
%         ne^C\cD_d\ell(c\rmM^\top\rmM) &* &*\\
%         \zero &\zero &\zero
%     \end{bmatrix}\\
%     &\approx \begin{bmatrix}
%         \zero &\zero &\zero\\
%         \rvOne\rvOne^\top + c\rmM^\top\rmM &* &*\\
%         \zero &\zero &\zero 
%     \end{bmatrix}
% \end{align*}
% and by adding back the residual we have
% \begin{equation}
%     \Input = \begin{bmatrix}
%         \rmM &\zero &\zero\\
%         \rvOne\rvOne^\top + c\rmM^\top\rmM &* &*\\
%         \id&\zero &\zero 
%     \end{bmatrix} \nonumber
% \end{equation}
% for small enough $c$ and large enough $C$. This is because 
% \begin{align*}
%     ne^C\dfrac{e^{cx_{ij}}}{\sum_{j=1}^n e^{cx_{ij}} + n(e^{C} +1)}  &= e^{cx_{ij}}\dfrac{1}{1+ \sum_{j=1}^ne^{cx_{ij}-C-\log n}+n}  \\
%     &= (1 + cx_{ij} + O((cx_{ij})^2))( 1 - e^{cx_{ij}-C-\log n} + O( e^{2(cx_{ij}-C-\log n)}))\\
%     &= (1 + cx_{ij} + O((cx_{ij})^2))( 1 - e^{cx_{ij}-C-\log n} )\\
%     &\approx (1 + cx_{ij})
% \end{align*}
% We now use the feedforward layers to perform the following transform 
% \begin{align*}
% \Input &= \begin{bmatrix}
% * & * & * \\
%  \rmM^\top\rmM&*&*\\
% * &*  &*
% \end{bmatrix} \\ 
% &= \begin{bmatrix}
%     * & * & *  &* &* \\
%     \rmA^\top \rmA &\zero &\rmA^\top\rmB &\zero & *\\
%     \zero &\zero &\zero &\zero &*\\
%     \rmB^\top\rmA &\zero &\rmB^\top\rmB &\zero&*\\
%     \zero &\zero &\zero &\zero &*\\
%     *&*&*&*&*
% \end{bmatrix}
% \end{align*}
% Now if $\emb^{(1)} = \begin{bmatrix} \zero &\zero & \emb_{2d+1:2d+n}& \zero &\zero  \end{bmatrix}$ and  $\emb^{(2)} = \begin{bmatrix}
% \emb_{1:n} &\emb_{n+1:d} &\zero &\emb_{d+n+1:2d} &\emb_{2d:3d}
% \end{bmatrix}$ we can copy $\rmA^\top\rmB$ to the desired place using \cref{lem:read}.
% % where $\cD_d\in \R^{2d\times 2d}$ is the diagonal matrix with the first $d$ diagonal elements $1$, and the rest 0.
% % Using $*$ to denote inconsequential values, we have:
% % \begin{align}
% % \val\Input\softmax((\key\Input)^\top\query\Input) &= \begin{bmatrix}
% % \zero & \zero &\zero\\
% % \zero & \zero &ne^C\cD_d\\
% % \zero &\zero &\zero
% % \end{bmatrix}\begin{bmatrix}
% %         \rmM& \zero\\
% %         \zero & \rvOne\rvOne^\top\\
% %         \id&\zero
% %     \end{bmatrix}\begin{bmatrix}
% %     \ell(c\rmM^\top\rmM) & *\\
% %        *& *
% %     \end{bmatrix}\\
% %     &= \begin{bmatrix}
% %        \zero & \zero &\zero\\
% % \zero & \zero &ne^C\cD_d\\
% % \zero &\zero &\zero
% %     \end{bmatrix}\begin{bmatrix}
% %         * & *\\
% %        * & *\\
% %        \ell(c\rmA^\top\rmA) &*
% %     \end{bmatrix}\\
% %     &= \begin{bmatrix}
% % \zero & \zero \\
% %  ne^C \cD_d\ell(c\rmA^\top\rmA)&*\\
% % \zero &\zero 
% % \end{bmatrix}\\
% % &\approx 
% % \begin{equation}
% % \begin{bmatrix}
% % \zero & \zero & \zero \\
% % \rvOne\rvOne^\top + c\rmA^\top\rmA&\rvOne\rvOne^\top + c\rmA^\top\rmB&*\\
% % \zero &\zero  &\zero 
% % \end{bmatrix},
% % \end{equation}
% %As we already mentioned we will get
% %Finally, by setting the layernorm parameters to be the diagonal matrix $\mscale$ to have the values $1/c$ in all of the elements, while the bias vector $\bias$ to have the value $-1/c$ everywhere, we get the following output.
% %Finally, the feed forward layers can subtract 1 and scale by $1/c$ to produce the following output:\AG{I used the Layer norm, we need to discuss the open the Relu technique. We should choose one.}
% %\begin{align}
% %\begin{bmatrix}
% %-\rvOne\rvOne^\top/c & -\rvOne\rvOne^\top/c & -\rvOne\rvOne^\top/c \\
% % \rmA^\top\rmA&\rmA^\top\rmB&*\\
% %-\rvOne\rvOne^\top/c &-\rvOne\rvOne^\top/c  &-\rvOne\rvOne^\top/c 
% %\end{bmatrix}
% %\end{align}
% %Then by using the encodings $\embed_1, \embed_2$ and the last line we can get 
% %\begin{equation}
% %    \begin{bmatrix}
% %-\rvOne\rvOne^\top/c & -\rvOne\rvOne^\top/c & -\rvOne\rvOne^\top/c \\
% % \rmA^\top\rmA&\rmA^\top\rmB&*\\
% %-\rvOne\rvOne^\top/c &-\rvOne\rvOne^\top/c  &\rmA^\top\rmA
% %\end{bmatrix}
% %\end{equation}

% % To output $\rmA^\top\rmB$ we will use a different set of encodings as to move in the output position the value $\rmA^\top\rmB$.
% \end{proof}




==> backup/sec/instruction_selection.tex <==
\subsection{Instruction Selection via Attention}


Consider a prompt $\pmt$ where instruction $\s_i$ follows features $\x_i$
\[
\pmt=(\x_i,\s_i)_{i=1}^{n}
\]
Let $\ins$ be an instruction. Define the filtered prompt $\pmt_{\ins}=\flt(\pmt,\ins)$ where 
% \[

% \]
Within this prompt, consider all instances where instruction $\ins$ is used, namely all tuples $(\x_i,\s_i=\ins,\x_{i+1})$. There exists a transformer which admits

==> backup/sec/intro.tex <==
\vspace{-10pt}
\section{Introduction}
\vspace{-5pt}
%, such as machine translation, sentiment analysis, and question-answering systems
The advent of transformers~\citep{vaswani2017attention} has revolutionized natural language processing, paving the way for remarkable performance in a wide array of tasks. LLMs, such as~GPTs~\citep{brown2020language}, have demonstrated an unparalleled ability to capture and leverage vast amounts of data, thereby facilitating near human-level performance across a variety of language generation tasks. Despite this success, a deep understanding of their underlying mechanisms remains elusive.

Chain-of-thought prompting \citep{wei2022chain} is an emergent ability of transformers where the model solves a complex problem~\citep{wei2022emergent}, by decomposing it into intermediate steps. Intuitively, such this underlies the ability of general-purpose language models to accomplish previously-unseen complex tasks by leveraging more basic skills acquired during the pretraining phase.

Compositional learning and CoT has enjoyed significant recent success in practical language modeling tasks spanning question answering, code generation, and mathematical reasoning \citep{perez2021automatic, imani2023mathprompter, yuan2023well}. In this work, we attempt to demystify some of the mechanics underlying this success and the benefits of CoT in terms of sample complexity and approximation ability. To do this we explore the role of CoT in learning in-context multi-layer perceptrons (MLP), that we believe can lead to a first set of insightful observations. Throughout, we ask:
% To do this we explore the role of CoT in learning in-context multi-layer perceptrons (MLP),a universal approximation to arbitrary composition functions, that we believe can lead to a first set of insightful observations. Throughout, we ask: 
\vspace{-2pt}

\begin{center}
\emph{Does CoT improve in-context learning of MLPs, and what are the underlying mechanics?}
    
\end{center}

%``heterogeneous'' ``homogeneous'' 
\noindent\textbf{Contributions:} As our central contribution, we establish a rigorous and experimentally-supported abstraction that decouples CoT prompting into a \emph{filtering phase} and an \emph{in-context learning (ICL) phase}. In the \emph{filtering phase}, the model attends to the relevant tokens within the prompt based on an instruction, and suppresses those irrelevant. In the \emph{ICL phase}, the model runs inference on the filtered prompt to output a \emph{step}. The model then moves to the next \emph{step} in the chain. How a transformer architecture can actually realize this process is formalized in Theorem \ref{thm:MLP} for MLPs. 

Building on this, we identify and thoroughly compare three schemes as illustrated in Figure~\ref{fig:intro}. (a) ICL: In-context learning from input-output pairs provided in the prompt, (b) CoT-I: Examples in the prompt are augmented with intermediate steps, (c) CoT-I/O: The model also outputs intermediate steps during prediction. Our main contributions are:

\input{fig_sec/fig_intro}


\begin{myitemize}
\item \textbf{Approximation and sample complexity:} Through experiments and theory, we establish that intermediate steps in CoT-I improves the sample complexity of learning whereas step-by-step output improves the approximation ability through looping. Specifically, CoT-I/O can learn an MLP with input dimension $d$ and $k$ neurons using ${\cal{O}}(\max(k,d))$ in-context samples by filtering individual layers and solving them via linear regression -- in contrast to the $\Omega(kd)$ lower bound without step-augmented prompt. In line with theory, our experiments (e.g.~Figs.~\ref{fig:smallk}\&\ref{fig:largek}) identify a striking universality phenomenon (as $k$ varies) and also demonstrate clear approximation benefits of CoT compared to vanilla ICL.
%reveal that CoT accuracy is remarkably agnostic to $k$ whenever $k\leq d$ in support of our theory. In contrast, transformer can fail to learn a two-layer MLP with ICL or CoT-I even with large sample size  demonstrating the approximation benefits of CoT. 
% \item CoT increases model expressivity; in-context sample efficiency
%Learning shallow MLPs

\item \textbf{Accelerated pretraining via learning shortcuts:} We construct deep linear MLPs where each layer is chosen from a discrete set of matrices. This is in contrast to above where MLP weights can be arbitrary. We show that CoT can dramatically accelerate pretraining by memorizing these discrete matrices and can infer all layers correctly from a \emph{single} demonstration. Notably the pretraining loss goes to zero step-by-step where each step \emph{``learns to filter a layer''}. Together, these showcase how CoT identifies composable shortcuts to avoid the need for solving linear regression. In contrast, we show that, ICL (without CoT) collapses to the linear regression performance as it fails to memorize exponentially many candidates (due to lack of composition).

%(ii) Pretraining loss goes to zero step-by-step where each step \emph{``learns to filter a layer''}. (iii) As the chain gets shorter, there are more matrices (as combinations of the initial ones) to memorize and convergence substantially slows down. (iv) Without CoT, the model fails to learn shortcuts and its performance collapses to linear regression.

%learning shortcuts: Specifically, rather than learning linear regression, CoT can memorize

%with deep linear MLPs reveal that transformer indeed \emph{learns to filter} during pretraining which leads to sudden drops in the test risk and accelerated convergence via CoT. It also evidences the emergent ability of CoT: learning each step function separately and then composing them. In addition to these benefits during inference time, we highlight how CoT accelerates pretraining by learning shortcuts to representing complex functions and how filtering plays a visible role.

% \item Finally, through linear MLPs, we demonstrate that a transformer pretrained with only the short chains can compose long previously-unseen chains during test-time by acquiring skills (e.g.~memorizing MLP weights), and \emph{learning to filter and compose them}.
\end{myitemize}
The paper is organized as follows. In Section \ref{sec prelim}, we introduce the problem setup and preliminaries. Section \ref{sec:main} provides an empirical investigation of CoT with 2-layer MLPs and states our main theoretical results. Section~\ref{sec:exp} presents holistic experiments on the sample complexity and approximation benefits of CoT. Finally, we elucidate the benefits of CoT during pretraining via experiments on deep linear MLPs in Section \ref{sec:deep nn}. Related work and discussion  are provided in Section~\ref{sec:related} and \ref{sec:discuss}.
% elucidating how CoT accelerates pretraining and enables the composition of long novel chains

%These contributions not only deepen our understanding of the inner workings of transformer models but also serve as a foundation for future research and optimization efforts. 


==> backup/sec/linear_nn.tex <==
\subsection{Deep Linear MLPs}\label{sec:deep nn}


% \subsection{Deep Linear Neural Networks}
In Sections~\ref{sec:emp} and \ref{sec:2nn}, we have discussed the approximation benefits of $\COT$ and how it in-context learns 2-layer random  MLPs by parallel learning of $k$ $d$-dimensional ReLU and 1 $k$-dimensional linear regression. In this section, we investigate the capability of $\COT$ in learning longer compositions. For brevity, we will use CoT to refer to $\COT$ in the rest of the discussion.

\textbf{Dataset. } Consider $L$-layer linear MLPs with input $\x\in\R^d\sim\Nc(0,\Iden_d)$, and output generated by $\y=\W_L\W_{L-1}\cdots\W_1\x$, where the $\ell$th layer is parameterized by $\W_\ell\in\R^{d\times d}$, $\ell\in[L]$. In this work, to better understand the emerging ability of CoT, we assume that each layer draws from the same discrete sub-function set $\bar\Fc=\{\bar\W_k:\bar\W_k^\top\bar\W_k=\Iden,k\in[K]\}$\footnote{This assumption ensures that the norm of the feature remains constant across layers ( $\|\x\|=\|\y\|=\|\tb^\ell\|$), enabling fair evaluation across different layers.}. Therefore, to learn the $L$-layer neural net, CoT only needs to learn $\bar\Fc$ with $|\bar\Fc|=K$, whereas $\ICL$ needs to learn the function set $\bar\Fc^{L}$, which contains $K^L$ random matrices. 

\textbf{Composition ability of CoT (Figures~\ref{fig:long chain}). } Set $d=5$, $L=6$ and $K=4$. At each round, we randomly select $L$ matrices $\W_\ell$, $\ell\in[L]$ from $\bar\Fc$ so that for any input $\x$, we can form a chain
\[
\x\to\tb^{1}\to\tb^{2}\dots\to\tb^{6}:=\y,
\]
where $\tb^{\ell}=\W_\ell\tb^{\ell-1}$, $\ell\in[L]$ and $\tb^{0}:=\x$. Let CoT-$X$ denote $X$-step $\COT$ method. For example, the in-context sample of CoT-6 has form of $(\x,\tb^{1},\tb^{2},\dots\tb^{5},\y)$, which contains all the intermediate outputs from each layer; while CoT-3, CoT-2 have prompt samples formed as $(\x,\tb^{2},\tb^{4},\y)$ and $(\x,\tb^{3},\y)$ respectively. In this setting, ICL is also termed as CoT-1, as its prompt contains only $(\x,\y)$ pairs. To solve the length-6 chain, CoT-$X$ needs to learn a model that can remember $4^{6/X}$ matrices. Therefore, ICL is face a significantly challenge sincd it needs to remember $4^6=4,096$ matrices (all combinations of the 4 matrices used for training and testing) compared to just $4$ for CoT-6. 

We train small GPT-2 models using the CoT-2/-3/-6 and ICL methods, and present the results in Fig.~\ref{fig:d5}. As evident from the figure, the performance curves of CoT-2 (orange), CoT-3 (green) and CoT-6 (red)  overlap, and they can all make precise predictions in one shot (given an in-context example $n=1$). It seems that $\TF$ has effectively learned to remember up to $64$ matrices (for CoT-2) and compose up to $6$ layers (for CoT-6). However, ICL (blue) struggles to learn the 6-layer MLPs in one shot. The black dashed curve shows the solution for linear regression $y=\bbeta^\top\x$ computed directly via least squares given $n$ random training samples, where $\x$ is the input and $y$ is from the output of the 6-layer MLPs (e.g., $\y[0]$). The test risks for $n=1,\hdots 10$ are plotted (in Fig.~\ref{fig:d5}), which show that the ICL curve aligns with the least squares performance. This implies that, instead of remembering all $4,096$ matrices, ICL solves the problem from the linear regression phase. 

In addition to the meta-learning results which highlight the approximation benefits of multi-step CoT, we also investigate the convergence rate of CoT-2/-3/-6 and ICL, with results displayed in Fig.~\ref{fig:one shot}. We test the one-shot performance during training and find that CoT-6 converges fastest. This is because it has the smallest sub-function set, and given the same tasks (e.g., deep neural nets), shortening the chain leads to slower convergence. This supports the evidence that taking more steps facilitates faster and more effective learning of complex problems.

% the more steps we have, the less complex each subfunction set is and 

 % given different function complexities, and results are shown in Fig.~\ref{fig:one shot}  are  results, we also 

% Then given different training sample size $n$, test risks when trained with 


\input{fig_sec/fig_50k_it}

\textbf{Evidence of Filtering (Figure~\ref{fig:long chain 50k}). } {As per Theorem~\ref{thm:MLP} and the appendix, transformers can perform filtering over CoT prompts, and the results from 2-layer MLPs align with our theoretical findings. However, can we explicitly observe filtering behaviors?} In Fig.~\ref{fig:composed 50k}, we display the results of the first 50k iterations from Fig.~\ref{fig:one shot}, and observe risk drops in CoT-6 (red) at the 15k and 25k iteration (shown as grey dotted and dashed lines). Subsequently, in Fig.~\ref{fig:each layer 50k}, we plot the test risk of each layer prediction (by feeding the model with correct intermediate features not the predicted ones), where CoT-6 (red) predicts the outputs from all 6 layers ($\tb^1,\cdots,\tb^L$). From these figures, we can identify risk drops when predicting different layers, which appear at either 15k (for layer 2, 3, 4, 5, 6) or 25k (for layer 1) iteration. This implies that the model learns to predict each step/layer function independently. Further, we test the filtering evidence of the $\ell$th layer by filling irrelevant positions with random features. Specifically, an in-context example is formed by
\[
(\z^0,\cdots,\tb^{\ell-1},\tb^{\ell},\z^{\ell+1},\dots\z^{L}),~~\text{where}~~\tb^{\ell}=\W_\ell(\tb^{\ell-1})~~\text{and}~~\z\sim\Nc(0,\Iden_d).
\]
 The test risks are represented by black dotted curves in Fig.~\ref{fig:each layer 50k}, which aligned precisely with the CoT-6 curves (red). %It means that 
This signifies that each layer's prediction concentrate solely on the corresponding intermediate steps in the prefix, while disregarding irrelevant features. This observation provides evidence that the process of filtering is indeed performed.

% and then padding the irrelevat positions do not harm the prediction performance. 

% \subsection{Unordered CoT Prompting}

% The CoT prompt defined in \eqref{cot pmt} is homogeneous, since step messages ($\tb^1,\cdots,\tb^{L-1}$) are given fully and ordered. However, in real world applications, prompt as a hint will not provide the whole and precise messages, and therefore we are expecting that even the whole chain is not provided in the prompt, $\TF$ can still complete the chain automatically by identifying the token space. Recall that $\tb^0=\x$ and $\tb^L=\y$, then an heterogeneous CoT example is no longer as \eqref{cot pmt} with $L+1$ tokens but can be any example from length $2$ to $L+1$, that is
% \begin{align}
% \text{homogeneous: }(\tb^0,\tb^1,\cdots\tb^{L-1},\tb^L)\longrightarrow\text{heterogeneous: }(\tb^{\ell_{\text{start}}}\cdots\tb^{\ell_{\text{end}}}).\label{heter cot pmt}
% \end{align}
% where $0\leq\ell_{\text{start}}<\ell_{\text{end}}\leq L$. We emphasize that $\ell_{\text{start}}$ and $\ell_{\text{end}}$ are arbitrary for any example within any prompt, and then if given a new input $\x$, same $L$-step procedure is applied. 

==> backup/sec/main.tex <==
\section{Empirical and Theoretical Perspectives on CoT}\label{sec:main}
\vspace{-5pt}
In this section, we begin by examining the performance of $\COT$ when learning 2-layer MLPs with input dimension of $d$ and hidden dimension of $k$. Our experimentation indicates that $\COT$ necessitates only $O(\max(d,k))$ in-context samples. Subsequently, in Section~\ref{sec:theory}, we present our theoretical findings that demonstrate how $\COT$ can execute filtering over the CoT prompt, thereby learning a 2-layer MLP, akin to resolving $k$ $d$-dimensional ReLU problems and $1$ $k$-dimensional linear regression problem.
% \vspace{-5pt}
\subsection{Empirical Exploration of 2-layer MLPs}\label{sec:emp}
% \vspace{-5pt}
To investigate how MLP architecture impacts $\COT$ performance, we train 2-layer MLPs with varying input dimensions ($d$) and hidden layer sizes ($k$). The results are presented in Figures~\ref{fig:smallk} and \ref{fig:largek}. Here, $\x,\tb,y$ represent input, hidden state, and output respectively. Detailed information on the implementation is deferred to Section~\ref{sec:2nn}. All experiments utilize a small GPT-2 model for training\footnote{Our code is available at \url{https://github.com/yingcong-li/Dissecting-CoT}.}.

\textbf{$\COT$ performance is agnostic to $k$ when $k\leq d$ (Figure~\ref{fig:smallk}). } In Fig.~\ref{fig:cot_d10_vs_d20}, we train MLPs with $d=10,20$ and $k=4,8,16$. Solid and dashed curves represent the $\COT$ test risk of $d=10$ and $20$ respectively for varying in-context samples. The results indicate that an increase in $d$ will amplifies the number of samples needed for in in-context learning, while the performance remains unaffected by changes in $k\in\{4,8,16\}$. To further scrutinize the impact of $d$ on $\COT$ accuracy, in Fig.~\ref{fig:cot_d10_vs_d20_align}, we adjust the horizontal axis by dividing it by the input dimension $d$, and superimpose both $d=10,k=16$ (blue solid) and $d=20,k=16$ (orange dashed) results. This alignment of the two curves implies that the in-context sample complexity of $\COT$ is linearly dependent on $d$. 

% $\bullet$ \textbf{$\COT$ requires $\mathbf{N=O(\max(d,k))}$ to learn 2-layer MLPs (Figures~\ref{fig:smallk}\&\ref{fig:largek}). } \red{As stated in Theorem~\ref{?}, to solve 2-layer MLPs with input dimension $d$ and hidden size $k$, $\COT$ requires $O(\max(d,k))$ in-context samples.} 
% Then the $\COT$ averaged test risks keeping the same in Fig.~\ref{fig:avg risk k} may be from the fact that under the given MLP setting, the input dimension $d$ dominates the in-context sample complexity, and since we fix $d$ to be $10$, the performance keeps unchangeable. To further investigate how $d$ and $k$ affect the $\COT$ performance, we either enlarge input dimension $d$ or hidden dimension $k$, and results are respectively displayed in Figure~\ref{fig:smallk} and Figure~\ref{fig:largek}. In Fig.~\ref{fig:cot_d10_vs_d20}, except the $\COT$ results already presented in Figure~\ref{fig:diff k}, we train the same small GPT-2 but with input dimension $d=20$. Solid and dashed curves represent the point-to-point $\COT$ test risk of $d=10$ and $20$ respectively. Results show that enlarging $d$ will increase the samples needed in in-context learning, and varying $k$ will not influence the test performance. In Fig.~\ref{fig:cot_d10_vs_d20_align}, we rescale the horizontal axis by dividing with input dimension $d$, and put both $d=10$ (blue solid) and $20$ (orange dashed) results on it. The two curves are aligned, which verifies the linear dependence of in-context sample complexity on $d$. 

\textbf{Large $k$ dominates $\COT$ performance (Figure~\ref{fig:largek}). } We further investigate the circumstances under which $k$ begins to govern the $\COT$ performance. In Figure~\ref{fig:largek compose}, we replicate the same experiments with $d=10$, but train with wider MLPs ($k=64$). Blue, orange and green curves represent results for $k=4,16,64$ respectively. Since the hidden dimension $k=64$ is larger, learning the second layer requires more hidden features ($\tb$), thus $N=100$ in-context samples (providing $100$ $\tb$s) are insufficient to fully restore the second layer, leading to performance gaps between $k=4,16$ and $k=64$. 
% hidden dimension $k$ turns to dominate the $\COT$ performance and there is performance gap between $k=4,16$ and $k=64$. 
To quantify the existing gaps, we conduct single-step evaluations for both the first and the second layers, with the results shown in Figures~\ref{fig:largek first} and \ref{fig:largek second}. Specifically, let $\pmt_n(\tilde f)$ be a test prompt containing $n$ in-context samples where $\tilde f$ represents any arbitrary 2-layer MLP. Given a test sample $(\xtest,\tb_{\text{\tiny{test}}},y_{\text{\tiny{test}}})$, the layer predictions are performed as follows.
\begin{align}
\text{1st layer prediction: } &\TF(\pmt_n(\tilde f),\xtest):=\hat\tb,\nn\\
\text{2nd layer prediction: } &\TF(\pmt_n(\tilde f),\xtest,\tb_{\text{\tiny{test}}}):=\hat y.\nn
\end{align}
The test risks are calculated by $\|\hat\tb-\tb_{\text{\tiny{test}}}\|^2$ and $(\hat y-y_{\text{\tiny{test}}})^2$. The risks illustrated in the figures are normalized for comparability (refer to Section~\ref{sec:2nn} and appendix for more details). Evidence from Fig.~\ref{fig:largek first} and \ref{fig:largek second} shows that while increasing $k$ does not affect the first layer's prediction, it does augment the number of samples required to learn the second layer. Moreover, by plotting the first layer risks of $k=4,16$  (blue/orange dotted) and second layer risk of $k=64$ (green dashed) in Fig.~\ref{fig:largek compose}, we can see that they align with the $\COT$ composed risks. This substantiates the hypothesis that $\COT$ learns 2-layer MLP through compositional learning of separate layers.
% , and its performance is determined by aggregate risks over all layers. 

% The interpretation is that, $\COT$ treats the 2-layer MLP as $k$ $d$-dimensional $\texttt{ReLU}$ and $1$ $k$-dimensional linear regression problems and solves them in parallel. Therefore, the function complexities of first and second layers are $O(d)$ and $O(k)$ separately, and then it answers why only $N=O(\max(d,k))$ samples are required for $\COT$ to learn 2-layer MLPs.   

==> backup/sec/outline.tex <==
% \paragraph{Outline}
% \begin{itemize}
%     \item \textbf{Setup:}
%     \begin{itemize}
%         \item \textbf{Vanilla CoT}
%         \item \textbf{Skill-based CoT}
%     \end{itemize}
%     \item \textbf{Part 1 (vanilla CoT):}
%     \begin{itemize}
%         \item \textbf{Experiments:} 5-layer neural nets experiments. 
%     \end{itemize}
%     \item \textbf{Part 2 (skill-based CoT):}
%     \begin{itemize}
%         \item \textbf{Experiments:}
%     \end{itemize}
% \end{itemize}
\paragraph{Outline of the paper (tentative)}
\begin{myitemize}
\item \textbf{Section 1:} Experiments and theory on deep neural nets (no instruction ID needed and we can reuse existing experiments since test and training is same)
\begin{myitemize}
\item \textbf{Statistical benefits of CoT: Experiment.} $(x,P_{d'}(g(x)),f(g(x)))$. $d'$ is the dimensionality of features after projection. This interpolates from vanilla ICL to full CoT ICL. Mathematical intuition: Thanks to $d'$ additional equations CoT learns faster by a factor of $O(d')$ (which is clear when $d'=d$).

\item \textbf{Approximation benefits of CoT: Experiment.} In ICL, provide the full DNN features $x1,x2,...,y=xD$. During prediction, train to predict $x1,x2,...xk,xD$ for $k=1$ to $k=D$. At $k=1$ it is regular CoT, at $k=D$ it is one shot prediction.
\begin{myitemize}
    \item We may use approximation aspect to explain distillation power of CoT where we teach a small model recurrence by using chains of a big model.% (needs thinking)
\end{myitemize}
\item \textbf{GSM8K experiments (instead arithmetic, more structured).} On GPT3 or ChatGPT show that more reasoning steps help for CoT to support approximation benefit.
\begin{myitemize}
\item https://paperswithcode.com/dataset/gsm8k
\item https://arxiv.org/abs/2210.00720
\end{myitemize}
\end{myitemize}
\item \textbf{Section 2:} Instruction-based CoT: Main emphasis: Long previously-unseen chains.
\begin{myitemize}
    \item Training involves only basic skills and skill transitions
    \item Test-time prompt can substantially differ from training (i.e.~previously unseen chains)
    \item \textbf{Blackbox reduction:} Show that TF can filter instructions to do ICL learning and TF can deduce next instruction. Combine this to show TF can learn previously-unseen chains.
    \item \textbf{GSM8K experiments.} Select problems whose solution require division operator `/' (or '*'). Contrast 
    \begin{myitemize}
    \item Case 1: In ICL randomly sample examples whose solutions don't contain `/'
    \item Case 2: In ICL randomly sample examples whose solutions do contain `/'
    \item Intuition: In Case 2, the model gets to see `/' operator as well as its transitions. Even if the chain of the problem differs, ICL examples remind it the instruction `/'. Case 2 is similar to active learning.
    \end{myitemize}
\end{myitemize}
\end{myitemize}

==> backup/sec/prlim.tex <==
\vspace{-5pt}\section{Preliminaries and Setup}\vspace{-5pt}\label{sec prelim}
We denote the set $\{1,2,\ldots,n\}$ as $[n]$. Vectors and matrices are represented in bold text (e.g., $\vx, \mA$), while scalars are denoted in plain text (e.g., $y$). 
The input and output domains are symbolized as $\Xc$ and $\Yc$ respectively (unless specified otherwise), and $\x\in\Xc$, $\y\in\Yc$ denote the input and output. 
% \subsection{The transformer architecture}



\subsection{In-context Learning}\label{subsec icl}
Following the study by \citet{garg2022can}, the fundamental problem of vanilla in-context learning (ICL) involves constructing a prompt with input-output pairs in the following manner: 
% considers a prompt with input-output pairs of the following form:
\begin{align}
\pmt_n(f)=(\x_i,\y_i)_{i=1}^n~~~~\text{where}~~~~\y_i=f(\x_i),\tag{P-ICL}\label{icl pmt}
\end{align}
where the transition function $f\in\Fc:\Xc\to\Yc$ remains constant within a single prompt but can vary across prompts, and the subscript $n$ signifies the number of in-context samples contained in the prompt. Considering language translation as an example, $f$ is identified as the target language, and the prompt can be defined as  $\pmt(\texttt{Spanish})$ = ((\emph{apple, manzana}), (\emph{ball, pelota}), $\ldots$) or $\pmt(\texttt{French})$=((\emph{cat, chat}), (\emph{flower, fleur}), $\ldots$). Let $\TF$ denote any auto-regressive model (e.g., Decoder-only Transformer). The aim of in-context learning is to learn a model that can accurately predict the output, given a prompt $\pmt$ and the test input $\xtest$, as shown in the following equation:
\begin{equation}\label{icl out}
\TF(\pmt_n(\tilde f),\xtest) \approx \tilde f(\xtest)
\end{equation}
where $\tilde f\in\Fc$ is the test function which may differ from the functions used during training. Previous work \citep{zhou2022teaching, li2023transformers} has demonstrated that longer prompts (containing more examples $n$) typically enhance the performance of the model.
% \AG{Unnecessary-- For the rest of the paper, we will denote vanilla in-context-learning as ICL.}

\subsection{Chain-of-thought Prompt and Prediction}\label{subsec cot}
\vspace{-5pt}

{As defined in \eqref{icl pmt}, the prompt in vanilla ICL only contains input-output pairs of the target function. This} 
%As defined in \eqref{icl pmt}, vanilla ICL prompting contains input-output pairs only, which 
demands that the model learns the function $f\in\Fc$ in one go, which becomes more challenging as $\Fc$ grows more complex, since larger models and increased prompt length ($n$) are needed to make correct predictions (as depicted by the green curves in Figures~\ref{fig:diff gpt} and \ref{fig:diff k}). {Existing studies on chain-of-thought methods \citep{wei2022chain} observed that prompts containing step-by-step instructions assist }%Existing chain-of-thought research \citep{wei2022chain} has observed that prompt containing step-by-step \emph{thoughts} helps 
the model in decomposing the function and making better predictions. 
%% The main benefit is that, instead of predicting the final output ($\y$) directly, CoT takes intermediate outputs (referred to as \emph{thought}) into consideration. 
Specifically, consider a function composed of $L$ subfunctions, represented as $f:=f_L\circ f_{L-1}\circ\dots f_1$. Each intermediate output 
{can be viewed as a step, enabling us to define a }%is a thought and we can define 
length-$n$ CoT prompt related to $f$ with $L$ steps (expressed with $\tb^\ell,\ell\in[L]$) as follows:
% For clear notation, let $\tb_i^0=\x_i$, $\tb_i^L=\y_i$ and $\f:=(f_1,f_2,\cdots,f_L)$.
\begin{align}
\pmt_n(f)=(\x_i,\tb_i^1,\cdots\tb_i^{L-1},\tb_i^L)_{i=1}^n~~~~\text{where}~~~~\tb_i^{\ell}=f_\ell(\tb_i^{\ell-1}),~\ell\in[L].\tag{P-CoT}\label{cot pmt}
\end{align}
Here $\x_i=\tb_i^0$, $\y_i=\tb_i^L$ {and $f_\ell\in\Fc_\ell$, which implies that $f\in\Fc_L\times\cdots\Fc_1:=\Fc$.}
%Here let $f_\ell\in\Fc_\ell$ and then $f\in\Fc_1\times\cdots\Fc_L:=\Fc$. 
%% Let $\f(\x):=f_L(f_{L-1}(\cdots f_1(\x))$. 

% \AG{Not sure what these want to say: ***In addition to admitting CoT prompts, we are asking how the $\TF$ preforms with or without predicting thoughts.  
% Then given a test input $\x$ and prompt from \eqref{cot pmt} corresponding to test function $\tilde f\in\Fc$, we define the model prediction in two ways: ***}

Next we introduce two methodologies for making predictions within the CoT framework:
% different ways that predictions can be made in the context of CoT:

\textbf{CoT over input only ($\EXP$). }Contrasted with ICL, $\EXP$ considers step-by-step instructions as inputs, 
% breaking down the computation of the final value into a collection of simpler tasks.
nonetheless, the prediction for the last token is performed as a single entity. 
% Compared to ICL, $\EXP$ takes in step-by-step instructions as inputs, which {fragments the calculation of the target value into a set of simpler ones. However, the prediction over the last token is performed all together in one shot}. %help in `explaining' the problem better. 
    % can be thought as explanations. Here, the intermediate thoughts are provided within the input prompts. It can also be seen as explanations of the input function target ($\tilde\f$). 
 Our experiments indicate that this approach lowers the sample complexity for $\TF$ to comprehend the function $\tilde f$ being learned (refer to the orange curves in Figures~\ref{fig:diff gpt}\&\ref{fig:diff k}). The $\EXP$ prediction aligns with Eq. \eqref{icl out}, but the prompt is determined by \eqref{cot pmt}.
    \begin{align}
    &\text{One-shot prediction: }\TF(\pmt_n(\tilde f),\xtest)\approx \tilde  f(\xtest).\label{exp out}
    \end{align}
%$\TF$ still needs to be able to express any function set $\Fc$, which will be very challenging (e.g., if assuming $\Fc_\ell=\tilde \Fc,\ell\in[L]$, then $\Fc=\tilde\Fc^L$ whose complexity is exponential to the thought step size $L$.).
\textbf{CoT over both input and output ($\COT$). } Despite the fact that $\EXP$  improves the sample complexity of learning $\tilde f$,  the $\TF$ must still possess the capacity to approximate functions from the function class $\Fc$, given that the prediction is made in one shot. To mitigate this challenge, we consider a scenario where in addition to implementing a CoT prompt, we also carry out CoT predictions. Specifically, for a composed problem with inputs formed via \eqref{cot pmt}, the model recurrently makes $L$-step predictions as outlined below:
    \begin{align}
    &\text{Step 1: }\TF(\pmt_n(\tilde f),\xtest):=\hat\tb^1\nn\\
    &\text{Step 2: }\TF(\pmt_n(\tilde f),\xtest,\hat\tb^1):=\hat \tb^2\nn\\
    &~~~~\vdots\nn\\
    &\text{Setp $L$: }\TF(\pmt_n(\tilde f),\xtest,\hat\tb^1\cdots,\hat\tb^{L-1})\approx \tilde 
 f(\xtest),\label{cot out}
    \end{align}
where at each step, the model outputs an intermediate step ($\hat\tb^\ell$) which is then fed back to the input sequence %to help 
 to facilitate the next-step prediction ($\hat\tb^{\ell+1}$). 
% \YL{[MIGHT NOT NEEDED!]As depicted in Figure~\ref{fig:intro}, (\emph{blue, orange, yellow}) blocks represent ($\x$, $\tb$, $\y$) respectively, and thought output $\hat\tb$ (the toppest orange block) is feed back to the input which completes the recurrent prediction.} 
Following this strategy, the model only needs to learn the union of the sub-function sets, $\bigcup_{\ell=1}^L\Fc_\ell$, whose complexity scales linearly with the number of steps $L$. Empirical evidence of the benefits of $\COT$ over $\ICL$ and $\EXP$ in enhancing sample efficiency and model expressivity is reflected in the blue curves shown in Figures~\ref{fig:diff gpt} and \ref{fig:diff k}. 




==> backup/sec/related.tex <==
\section{Related Work}\label{sec:related}
% \ks{breaking it up into paragraphs for simplicity. But it wastes a lot of space. Can remove that later if we need.}

% \textbf{In-context learning:} 
With the success of LLMs and prompt structure \citep{lester2021power}, there is growing interest in in-context learning (ICL) from both theoretical and experimental lens~\citep{garg2022can,brown2020language, von2022transformers, dai2022can, min2022rethinking, lyu2022z,li2023transformers, xie2021explanation,min2021metaicl, wei2023larger}. 
% \citet{garg2022can} analyze the question of expressivity by training TFs to learn simple function classes from in-context examples without the issues of tokenization and language.
As an extension, chain-of-thought (CoT) prompts have made impressive improvements in performing complex reasoning by decomposing it into step-by-step intermediate solutions \citep{wei2022chain, narang2020wt5, lampinen2022can, wei2022emergent,zhou2022teaching, nye2021show, velivckovic2021neural, lanchantin2023learning}, which in general, shows the ability of transformer in solving compositional functions, and the idea of learning how to compose skills has been well studied in other literatures~\citep{sahni2017learning, livska2018memorize}. More specifically, for the problem of learning shallow networks, there are several well known hardness results~\citet{goel2017reliably, goel2020tight, zhang2019learning}. In particular, \citet{hahn2023theory} shows a formal learnability bound which implies that compositional structure can benefit ICL. However, most of the work focuses on investigating empirical benefits and algorithmic designing of CoT, and there exists little effort studying the underlying mechanisms of  CoT. 

%There is also literature showing expressivity of transformer. 
Considering the expressivity of the transformer architecture itself, \citet{yun2019transformers} showed that TFs are universal sequence to sequence approximators. More recently, \citet{giannou2023looped} use an explicit construction to show that shallow $\TF$s can be used to run general purpose programs as long as we loop them. Other works have also shown the turing-completeness of the $\TF$ architecture but these typically require infinite/high precision and recursion around attention layers~\citep{wei2022statistically, perez2019turing, perez2021attention, liu2022transformers}. Closer to our work, \citet{akyurek2022learning} prove that a transformer with constant number of layers can implement gradient descent in solving linear regression, and \citet{giannou2023looped} introduce similar results by looping outputs back into inputs. In this work, we prove CoT can be treated as: first apply filtering on the CoT prompts using special construction, and then in-context learn the filtered prompt. 

% \textbf{Chain-of-thought:} TFs also display a property commonly known as chain-of-thought~\citep{wei2022chain, narang2020wt5, lampinen2022can, wei2022emergent}, showing improved performance when prompted to go \emph{step-by-step}~\citep{zhou2022teaching, nye2021show, kaiser2015neural, velivckovic2021neural, lanchantin2023learning}. \citet{hahn2023theory} in particular, show a formal learnability bound using that implies that compositional structure can benefit ICL.




% \textbf{Emergent Properties:} ICL and CoT are just few of the remarkable properties seem to ``emerge'' from LLMs with scale~\citep{chowdhery2022palm, ganguli2022predictability, srivastava2022beyond, radford2019language}. \citet{wei2022emergent} define \emph{emergent properties} as those that appear in models only beyond a certain amount of scale. These may include the ability to do arithmetic, program execution, instruction following, etc.
% More recently, \citet{schaeffer2023emergent} claim that scale may not be the only factor in deciding if a property is emergent and that the evaluation metric may also play a significant role.



==> backup/sec/setup__backup_.tex <==
\section{Problem Setup}
\noindent\textbf{Notation:} Let $\x$ denote the input, $\y$ denote the output, and $\tb=(\tb_1,\dots,\tb_L)$ denote the chain of intermediate thoughts output by \ct. 

\noindent$\bullet$ \textbf{Vanilla \ct with \icl:} Define the $i^{th}$ tuple $\z\n{i}=(\x\n{i},\tb\n{i},\y\n{i})$. ICL admits prompts of the form
\[
\pb=[\z\n{1}~\dots~\z\n{n-1}~\x\n{n}].
\]
Above, the goal is to learn a function sequence $\FF=(f_i)_{i=1}^L$ where each function $f_i$ belongs to a fixed hypothesis set $\Fc_i$. TF will know when to apply which function by index of its current input.\smallskip

% that skill's ID number during \ct
\noindent$\bullet$ \textbf{Skill-based \ct:} Rather than artificially requiring a specific function order, a more realistic setting is \underline{teaching transformer a set of skills} and explicitly instructing TF to apply that skill during \ct demonstrations. This is akin to what happens when an LLM is provided with a math/commonsense reasoning problem and \ct demonstrations reminds the LLM which skills to use.

In this setting, each skill $i$ is associated with a hypothesis set $\Fc_i$ and a distribution $\Dc_i$ over $\Fc_i$. Suppose there are $M$ skills in total. During \icl, we draw $L$ skills denoted by the $L$-dimensional skill indices $\s\in [M]^L$. We also draw $f_i\sim\Dc_i$ for $i\in \Sc$. Declare \ct explanations
\[
\tb=(\s_1,\tb_1,\s_2,\tb_2,\dots,\s_L,\tb_L)
\]
where $\tb_i$ corresponds to the output after applying skill $\s_i$ on $\tb_{i-1}$. The tuples $\z\n{i}$ and \icl prompt is constructed same as before.
%$=(\x\n{i},\tb\n{i},\y\n{i})$. ICL admits prompts of the form

\noindent\textbf{Why skills:} In a nutshell, skill-based setting is more realistic as TF and versatile. Skill-based setting also interpolates between \emph{pure-learning} and \emph{pure-instruction} settings. By this, we mean:
%Perhaps more importantly, s

 \noindent\emph{Pure-learning:} If $\Dc_i$ is a rich continuous distribution, during test time, we need a lot of \icl demonstrations to learn $f_i\in\Fc_i$ associated with the test task. TF can learn a good algorithm from source tasks but it is not enough to identify the rich test function.

 \noindent\emph{Pure-instruction:} Imagine $\Dc_i$ is a singleton! This means all tasks share the exact same function during training or test-time of the TF. Thus, during \icl time, TF can infer the $f_i$ from a single demonstration as it only needs the skill ID to perfectly identify the associated function. In this scenario, the learning cost is only during training time and \icl can one-shot during test-time.

\iffalse
and $\s\in\Sc$ denote skill, where $\Xc,\Sc$ correspond to feature (including input/output) and skill space respectively. Let $\p:=(\x,\s)$ denote an ICL example.



\noindent\textbf{Notation:} Let $\x\in\Xc$ denote the input, $\y\in\Yc$ denote the output, and $\tb=(\tb\n{0},\dots,\tb\n{L})$ denote the chain of intermediate thoughts output by \ct, where $\tb\n{0}=\x,\tb\n{L}=\y$. Let $[n]=\{1,\cdots,n\}$.



Consider a composition function $\y=f_1\circ f_2\dots \circ f_L(\x)$ where $f_\ell\in\Fc_\ell,~\ell\in[L]$. Then we can generate \emph{thought} by $\tb\n{\ell}=f_\ell(\tb\n{\ell-1}),~\ell\in[L]$.

\noindent$\bullet$ \textbf{Vanilla \ct with \icl:} Define the $i$th tuple $\tb_i=(\tb\n{0}_i,\cdots,\tb\n{L}_i)$. ICL admits prompts of the form
\[
\p_i\n{\ell}=[\tb_{1}~\dots~\tb_{i-1}~;\tb_{i}\n{0}~\dots\tb_{i}\n{\ell}].
\]
Above, the goal is to learn a function sequence $\f=(f_\ell)_{\ell=1}^L\in\bFc$ where $\bFc:=\Fc_1\times\dots\Fc_L$. TF will know when to apply which function by index of its current input. Now assume we are given $T$ sequences each containing $n$ chains. Then the objective function is defined as follows.
\begin{align}
    &\widehat\TF=\arg\min\frac{1}{nT}\sum_{t=1}^T\sum_{i=1}^n\Lch_{ti}(\TF)\\
    \text{where}\quad&\Lch_{ti}(\TF)=\frac{1}{L}\sum_{\ell=1}^L\ell\left(\tb_{ti}\n{\ell},\TF(\p_{ti}\n{\ell-1})\right).\nn
\end{align}
% \begin{align}
%     \widehat\TF=\arg\min\frac{1}{nLT}\sum_{t=1}^T\sum_{i=1}^n\sum_{\ell=1}^L\ell\left(\tb_{ti}\n{\ell},\TF(\p_{ti}\n{\ell-1};\tb_{ti}\n{\ell-1})\right).
% \end{align}
\YL{Should the loss function be the same or different for different $\ell\in[L]$}
\begin{align}
    \Rc(\widehat\TF)=\frac{1}{n}\sum_{i=1}^n\E\left[\ell\left(\y,\TF^{\otimes L}(\x)\right)\right],\\
    \text{where}\quad\TF^{\otimes L}(\x):=\underset{\text{Composition of $L$ $\TF$'s.}}{\underbrace{\TF\circ\dots\circ\TF(\x)}}.\nn
\end{align}

\smallskip

% that skill's ID number during \ct
\noindent$\bullet$ \textbf{Skill-based \ct:} Rather than artificially requiring a specific function order, a more realistic setting is \underline{teaching transformer a set of skills} and explicitly instructing TF to apply that skill during \ct demonstrations. This is akin to what happens when an LLM is provided with a math/commonsense reasoning problem and \ct demonstrations reminds the LLM which skills to use.

In this setting, each skill $i$ is associated with a hypothesis set $\Fc_i$ and a distribution $\Dc_i$ over $\Fc_i$. Suppose there are $M$ skills in total. During \icl, we draw $L$ skills denoted by the $L$-dimensional skill indices $\s\in [M]^L$. We also draw $f_i\sim\Dc_i$ for $i\in \Sc$. Declare \ct explanations
\[
\tb=(\tb\n{0},\s\n{1},\tb\n{1},\s\n{2},\tb\n{2},\dots,\s\n{L},\tb\n{L})
\]
where $\tb_i$ corresponds to the output after applying skill $\s_i$ on $\tb_{i-1}$. The tuples $\z\n{i}$ and \icl prompt is constructed same as before.
%$=(\x\n{i},\tb\n{i},\y\n{i})$. ICL admits prompts of the form

\noindent\textbf{Why skills:} In a nutshell, skill-based setting is more realistic as TF and versatile. Skill-based setting also interpolates between \emph{pure-learning} and \emph{pure-instruction} settings. By this, we mean:
%Perhaps more importantly, s

 \noindent\emph{Pure-learning:} If $\Dc_i$ is a rich continuous distribution, during test time, we need a lot of \icl demonstrations to learn $f_i\in\Fc_i$ associated with the test task. TF can learn a good algorithm from source tasks but it is not enough to identify the rich test function.

 \noindent\emph{Pure-instruction:} Imagine $\Dc_i$ is a singleton! This means all tasks share the exact same function during training or test-time of the TF. Thus, during \icl time, TF can infer the $f_i$ from a single demonstration as it only needs the skill ID to perfectly identify the associated function. In this scenario, the learning cost is only during training time and \icl can one-shot during test-time.
 \fi

==> backup/sec/statements_construction.tex <==
\subsection{Provable Approximation of MLPs via Chain-of-Thought}\label{sec:theory}
The observations we made in Section~\ref{sec:emp} are indicative of the model processing each one of the two layers sequentially. Now in this section, we state our main contribution of
% ; an observation we also verify empirically in the subsequent sections. 
% Our main contribution is 
establishing a result that decouples CoT-based in-context learning ($\COT$) into two phases: (1) \emph{Filtering Phase:} Given a prompt that contains features of multiple MLP layers, retrieve only the features related to a target layer to create a \emph{homogeneous} prompt. (2) \emph{ICL Phase:} Given filtered prompt, learn the target layer weights through gradient descent. Combining these two phases, and looping over all layers, we will show that there exists a transformer architecture such that $\COT$ can provably approximate a multilayer MLP up to a given resolution. To state our result, we assume access to an oracle that performs linear regression and consider the consider the condition number of the data matrix.%make the following assumption on the MLP features provided within the prompt.
%\begin{assumption} \end{assumption}
\begin{definition}[MLP and condition number]\label{MLP assump} Consider a multilayer MLP defined by the recursion $\tb_i^{\ell}=\phi(\W_\ell \tb_i^{\ell-1})$ for $\ell\in[L]$, $i\in[n]$ and $\tb_i^0=\x_i$. Here $\phi(x)=\max(\alpha x,x)$ is a Leaky-ReLU activation with $1\geq \alpha>0$. Define the feature matrix $\Tb_\ell=[\tb_1^\ell~\dots~\tb_n^\ell]^\top$ and  
% where $\tb_{\ell,k}=\tb_{\ell}(\x_k)$ is the $k$'th chain element of the example $\x_k$. 
define its condition number $\kappa_\ell=\sigma_{\max}(\Tb_\ell)/\sigma_{\min}(\Tb_\ell)$ (with $\sigma_{\min}:=0$ for fat matrices) and $\kappa_{\max}=\max_{0\leq\ell< L}\kappa_\ell$.
%efine the condition number associated with layer $\ell$ as
\end{definition}
\begin{assumption}[Oracle Model]\label{assume oracle} We assume access to a transformer $\TFLR$ which can run $T$ steps of gradient descent on the quadratic loss $\Lc(\w)=\sum_{i=1}^n(y_i-\w^\top \x_i)^2$ given a prompt of the form $(\x_1,y_1,\dots, \x_n,y_n)$.
\end{assumption}
We remark that this assumption is realistic and has been formally established by earlier work \citep{giannou2023looped,akyurek2022learning}. Our CoT abstraction builds on these to demonstrate that $\COT$ can call a blackbox \TF model to implement a compositional function when combined with filtering.

The following result summarizes our main theoretical contribution. The precise statement is deferred to the supplementary material. 
\begin{theorem}[Decoupling CoT]\label{thm:MLP} Consider a prompt $\pmt_n(f)$ generated from an $L$-layer MLP $f(\cdot)$ as described in Definition \ref{MLP assump}, and assume given test example $(\xtest,\tb^1_{\text{\tiny test}}, \dots\tb^L_{\text{\tiny test}})$. 
% , containing $n$ examples and ends with $\x^{\texttt{test}}$. 
For any resolution $\eps>0$, there exists $\delta=\delta(\eps)$, iteration choice $T={\cal{O}}(\kappa_{\max}^2\log(1/\eps))$, and a backend transformer construction $\TFBE$ such that the concatenated transformer $\TF=\TFLR \circ \TFBE$ implements the following: Let $(\tht^{i})_{i=1}^{\ell-1}$ denote the first $\ell-1$ $\COT$ outputs of $\TF$ and set $\pb[\ell]=(\pb_n(f),\xtest,\tht^{1}\dots\tht^{\ell-1})$. At step $\ell$, $\TF$ implements
\begin{enumerate}
\item \textbf{Filtering.} Define the filtered prompt with input/output features of layer $\ell$,
\[
\arraycolsep = 1pt
\pbf_n=\left(\begin{array}{*{10}c}
\hdots \zero,&\tb^{\ell-1}_{1},&\zero&\hdots&\zero,&\tb^{\ell-1}_n, &\zero&\hdots&\zero,&\tht^{\ell-1}\\
\hdots\zero,&\zero,& \tb^{\ell}_{1}&\dots&\zero,&\zero,& \tb^{\ell}_n&\dots&\zero,&\zero\end{array}\right).
\]
There exists a fixed projection matrix $\bPi$ that applies individually on tokens such that the backend output obeys $\tn{\bPi(\TFBE(\pb[\ell]))-\pbf_n}\leq \delta$. %The more precise statement is provided in Lemma \ref{lem:filtering}. % up to $\eps$ accuracy via a fixed linear projection. 
\item \textbf{Gradient descent.} The combined model obeys $\tn{\TF(\pb[\ell])-\tb_{\text{\tiny test}}^{\ell}}\leq {\ell\cdot \eps}/{L}$.
\end{enumerate}
$\TFBE$ has constant number of layers independent of $T$ and $n$. Consequently, after $L$ rounds of $\COT$, \TF outputs $f(\xtest)$ up to $\eps$ accuracy.
\end{theorem}
% (more generally we expect
{\begin{remark}
Note that, this result effectively shows that, with a sufficiently good blackbox transformer $\TFLR$ (per Assumption \ref{assume oracle}), $\COT$ can learn an $L$-layer MLP using in-context sample size $n>\max_{\ell\in[L]}d_\ell$ where $d_\ell$ is the input dimension of $\ell$th layer. This is assuming condition number $\kappa_{\max}$ of the problem is finite as soon as all layers become over-determined. Consequently, $\COT$ needs $\max(k,d)$ sample complexity to learn a two layer MLP. This provides a formal justification for the observation that empirical $\COT$ performance is agnostic to $k$ as long as $k\leq d$.
%(so that following Def.~\ref{MLP assump}, $\Tb_\ell, \ell\in[L]$ are tall matrices and $\kappa_{\max}\to\infty$). It proves that to learn a 2-layer MLP with input dimension $d$ and hidden dimension $k$, $\COT$ needs ${\cal{O}}(\max(k,d))$ in-context samples, and when $k<d$, varying $k$ will not influence the performance (Fig.~\ref{fig:smallk} and Section~\ref{sec:emp}).
\end{remark}}
We provide the filtering statements in the Appendix, and the key components of our construction are the following: (i) Inputs are projected through the embedding layer in which a set of encodings, an enumeration of the tokens ($1,2,\dots, N$), an enumeration of the layers ($1,2,\dots,L$) and an identifier for each layer already predicted are all attached. Notice that this ``modification'' to the input only depends on the sequence length and is agnostic to the token to-be-predicted. This allows for an automated looping over $L$ predictions. (ii) We use this information to extract the sequence length $N$ and the current layer $\ell$ to-be-predicted. (iii) With these at hand we construct an `if - then' type of function using the ReLU layers to filter out the samples that are not needed for the prediction.

% We now demonstrate how a transformer model, can perform a processing of the data depending on the current prediction to be made. Specifically, assuming that the CoT is performed for $L$ layers and that the model has already made $\ell-1$ predictions we provide the following lemma
% \begin{lemma}[Filtering (Informal)]\label{lem:filtering}
%     Assume that the input to a transformer model is of the following form
%     \renewcommand{\arraystretch}{1.5}
%     % \begin{equation}
%     %     \arraycolsep=2pt
%     %     \X = \left[\begin{array}{cccc|ccccc|ccc}
%     %         \x_1 & \tb_1^1 &\dots&\tb^{\ell}_L &\hdots &\tb^{\ell-1}_n &\tb^{\ell}_n &\hdots &\tb_n^{L} &\xtest &\hdots &f^{\ell-1}(\xtest)\\
%     %         &&&&&&\zero&&&&&\\
%     %        \hline
%     %        0 & \hdots &\ell &\ell+1 &\hdots &\ell &\ell+1&\hdots &L &1 &\hdots &\ell\\
%     %        1 & \hdots &\ell &\ell+1 &\hdots &\ell &\ell+1&\hdots &L &1 &\hdots &\ell\\
%     %         0 & \hdots &0 &0&\hdots &0&0  &\hdots &0&1 &\hdots &1\\
%     %         % 1& \hdots &\ell &\hdots &L+\ell+1 &\hdots &n &n+1 &\hdots &N\\
%     %         % \ln(1)& \hdots &\ln(\ell) &\hdots &\ln(L+\ell+1) &\hdots &\ln(n) &\ln(n+1) &\hdots &\ln(N)\\
%     %        \emb_1 & \hdots &\emb_\ell &\emb_{\ell+1} &\hdots &\emb_{\ell+L+1}& \emb_{\ell+L+2} &\hdots &\emb_n &\emb_{n+1} &\hdots &\emb_{N}
%     %     \end{array}\right]
%     % \end{equation}
%     \begin{equation}
%         \arraycolsep=2pt
%         \X = \left[\begin{array}{*{12}c}
%             \x_1 & \hdots &\tb^{\ell-1}_1&\tb^{\ell}_1 &\hdots &\tb^{\ell-1}_2 &\tb^{\ell}_2 &\hdots &\tb_n^{L} &\x_{\text{\tiny test}} &\hdots &\tb^\ell_{\text{\tiny test}}\\
%            \zero &\hdots &\zero &\zero  &\hdots &\zero &\zero&\hdots &\zero &\zero &\hdots &\zero\\
%            \hline
%            1 & \hdots &\ell &\ell+1 &\hdots &\ell &\ell+1&\hdots &L &1 &\hdots &\ell\\
%            1 & \hdots &\ell &\ell+1 &\hdots &\ell &\ell+1&\hdots &L &1 &\hdots &\ell\\
%             0 & \hdots &0 &0&\hdots &0&0  &\hdots &0&1 &\hdots &1\\
%             % 1& \hdots &\ell &\hdots &L+\ell+1 &\hdots &n &n+1 &\hdots &N\\
%             % \ln(1)& \hdots &\ln(\ell) &\hdots &\ln(L+\ell+1) &\hdots &\ln(n) &\ln(n+1) &\hdots &\ln(N)\\
%            \emb_0 & \hdots &\emb_{\ell-1} &\emb_{\ell} &\hdots &\emb_{\ell+L}& \emb_{\ell+L+1} &\hdots &\emb_{nL+n-1} &\emb_{nL+n} &\hdots &\emb_{nL+n+\ell}
%         \end{array}\right]
%     \end{equation}
%     where $\X\in\R^{d\times N}$ and $\emb_i$, $i=1,\hdots, N$ are the positional encodings\footnote{The exact form of these encodings is provided to the appendix for ease of exposition. We would like to note however that the follow an oblivious to the ``token-to-be-generated'' pattern.}. 
%     Then there exists a transformer $\TF:\R^{d\times N} \to \R^{d\times N}$ consisting of  seven layers with output
%     \begin{equation}
%     \arraycolsep=2pt
%         \TF(\X) = \left[\begin{array}{*{12}c}
%            \zero  & \hdots &\tb_1^{\ell}  &\zero  &\hdots &\tb_2^{\ell} &\zero  &\hdots &\zero &\zero &\hdots &\tb^\ell_{\text{\tiny test}}\\
%            \zero  & \hdots &\zero &\tb_1^{\ell+1}  &\hdots &\zero &\tb_2^{\ell+1}  &\hdots &\zero &\zero &\hdots &\zero \\
%            \hline
% * & \hdots &* &* &\hdots &* &*&\hdots &* &* &\hdots &*\\
%         \end{array}\right] 
%     \end{equation}
%     where $*$ denotes inconsequential values. 
% \end{lemma}

% Some observations are in order.
%\begin{remark} 
%    The process of filtering can be performed by designing the positional encoding as to be able to extract the information of which token is to be predicted automatically for any token. In other words, the encodings follow a pattern that is oblivious to the ``token-to-be-generated''. 
%    Notice that one the current data points and their corresponding labels have been extracted, we can apply previous results on in-context learning gradient descent to perform linear regression (see \cite{giannou2023looped, akyurek2022learning}). For the update of the neural network, assuming that the activation functions are invertible we can use the result of \cite{giannou2023looped} to first invert the labels, then perform the linear regression and finally apply again the activation function. We provide the steps required for such a construction in the appendix.
%\end{remark}
%\begin{remark}
%    When the filtering is performed, there is an $\pm\varepsilon >0$ error at left and right point of the non-zero positions. This error is controlled and can be arbitrarily small. The analysis of the error is given in the Appendix \ref{app:filtering}
%\end{remark}
% The operation performed is in essence the operation of filtering. Each one of the five layers performs one of the following steps 
% \begin{enumerate}
%     \item The first layer uses the third line of the input, and created a weighted sum of it. The result would be equal to $k/N$, since there are $k$ ones and the total tokens are $N$.
%     \item The second layer calculates the number of tokens $N$. Notice that this information cannot be directly provided to the input, since for the prediction of the next token we can just append one extra column. Thus, it is not clear how this information can be isolated without the input size being proportional to the number $L$.
%     \item The third layer implements the multiplication and extracts the information regarding the current prediction, \textit{i.e., }$k$.
%     \item In the next layer the number $k$ is subtracted from each one of the elements of the second row presented in the input. 
%     \item The ReLUs of the next layer output one in the second row if the point is zero, and zero otherwise.
%     \item Finally this information is used, to filter the data points through another set of ReLus.
%     \end{enumerate}
% \begin{theorem}
%     In the setting of Lemma \ref{lem:filtering}
% \end{theorem}

==> backup/sec/todo.tex <==
\section*{Organization}
\subsection{Introduction}
\subsection{Problem description}
\subsection{Neural nets experiments}
ICL vs Explanation vs CoT
\subsection{ICL with heterogeneous prompts}

\section*{TODO}

\noindent\textbf{Experiments:} 

\textbf{What to test:} 
\begin{itemize}
    \item Sample benefit (more/less ICL), 
    \item Expessivity (small/large GPT), 
    \item How to predict (direct vs multi-step) 
\end{itemize}
\begin{enumerate}
    \item Expressivity (direct vs multi-step): 2-layer neural net: DONE?
    \item \textbf{Priority:} $>2$-layer neural net: Identify a setting with gap btwn 2 vs 3 layer
    \begin{itemize}
        \item Dimensions like 5-5-10-1
        \item diffable act
        \item pretrained subnets
        \item small vs large
    \end{itemize}
    \item Sample benefit: $y=v^Tphi(Wx)$, ICL=> $x, \text{dim-reduce}(phi(Wx)), y$
    \item Unseen chain length (DONE)
    \item Impact of number of subskill
    \begin{itemize}
        \item Make subskill difficult (e.g. noise)
    \end{itemize}
    \item Wrong features in prefix does not impact negative
\end{enumerate}


\noindent\textbf{Theory:} 
\begin{enumerate}
    \item Framing: Learn basic skills and chain them in darkness
    \item Reducing a skill sequence to pure ICL
    \item \textbf{Feature predictions:} A transformer can pick out the skill-specific features and give it to a pure ICL downstream layers
    \item \textbf{Skill predictions:} => If chain is noiseless, SATT can output the correct majority rule
\end{enumerate}

==> backup/sec/zz_statements_construction.tex <==
\subsection{The process of filtering}
The observations made so far are indicative of the model processing each one of the two layers sequentially; an observation we also verify empirically in the subsequent sections. We now demonstrate how a transformer model, can perform a subselection of the data depending on the current prediction to be made. Specifically, assuming that the CoT is performed for $L$ layers and that the model has already made $\ell-1$ predictions we provide the following lemma
\begin{lemma}[Filtering (Informal)]\label{lem:filtering}
    Assume that the input to a transformer model is of the following form
    \renewcommand{\arraystretch}{1.5}
    % \begin{equation}
    %     \arraycolsep=2pt
    %     \X = \left[\begin{array}{cccc|ccccc|ccc}
    %         \x_1 & \tb_1^1 &\dots&\tb^{\ell}_L &\hdots &\tb^{\ell-1}_n &\tb^{\ell}_n &\hdots &\tb_n^{L} &\xtest &\hdots &f^{\ell-1}(\xtest)\\
    %         &&&&&&\zero&&&&&\\
    %        \hline
    %        0 & \hdots &\ell &\ell+1 &\hdots &\ell &\ell+1&\hdots &L &1 &\hdots &\ell\\
    %        1 & \hdots &\ell &\ell+1 &\hdots &\ell &\ell+1&\hdots &L &1 &\hdots &\ell\\
    %         0 & \hdots &0 &0&\hdots &0&0  &\hdots &0&1 &\hdots &1\\
    %         % 1& \hdots &\ell &\hdots &L+\ell+1 &\hdots &n &n+1 &\hdots &N\\
    %         % \ln(1)& \hdots &\ln(\ell) &\hdots &\ln(L+\ell+1) &\hdots &\ln(n) &\ln(n+1) &\hdots &\ln(N)\\
    %        \emb_1 & \hdots &\emb_\ell &\emb_{\ell+1} &\hdots &\emb_{\ell+L+1}& \emb_{\ell+L+2} &\hdots &\emb_n &\emb_{n+1} &\hdots &\emb_{N}
    %     \end{array}\right]
    % \end{equation}
    \begin{equation}
        \arraycolsep=2pt
        \X = \left[\begin{array}{*{12}c}
            \x_1 & \hdots &\tb^{\ell-1}_1&\tb^{\ell}_1 &\hdots &\tb^{\ell-1}_2 &\tb^{\ell}_2 &\hdots &\tb_n^{L} &\x_{\text{\tiny test}} &\hdots &\tb^\ell_{\text{\tiny test}}\\
           \zero &\hdots &\zero &\zero  &\hdots &\zero &\zero&\hdots &\zero &\zero &\hdots &\zero\\
           \hline
           1 & \hdots &\ell &\ell+1 &\hdots &\ell &\ell+1&\hdots &L &1 &\hdots &\ell\\
           1 & \hdots &\ell &\ell+1 &\hdots &\ell &\ell+1&\hdots &L &1 &\hdots &\ell\\
            0 & \hdots &0 &0&\hdots &0&0  &\hdots &0&1 &\hdots &1\\
            % 1& \hdots &\ell &\hdots &L+\ell+1 &\hdots &n &n+1 &\hdots &N\\
            % \ln(1)& \hdots &\ln(\ell) &\hdots &\ln(L+\ell+1) &\hdots &\ln(n) &\ln(n+1) &\hdots &\ln(N)\\
           \emb_0 & \hdots &\emb_{\ell-1} &\emb_{\ell} &\hdots &\emb_{\ell+L}& \emb_{\ell+L+1} &\hdots &\emb_{nL+n-1} &\emb_{nL+n} &\hdots &\emb_{nL+n+\ell}
        \end{array}\right]
    \end{equation}
    where $\X\in\R^{d\times N}$ and $\emb_i$, $i=1,\hdots, N$ are the positional encodings\footnote{The exact form of these encodings is provided to the appendix for ease of exposition. We would like to note however that the follow an oblivious to the ``token-to-be-generated'' pattern.}. 
    Then there exists a transformer $\TF:\R^{d\times N} \to \R^{d\times N}$ consisting of  seven layers with output
    \begin{equation}
    \arraycolsep=2pt
        \TF(\X) = \left[\begin{array}{*{12}c}
           \zero  & \hdots &\tb_1^{\ell}  &\zero  &\hdots &\tb_2^{\ell} &\zero  &\hdots &\zero &\zero &\hdots &\tb^\ell_{\text{\tiny test}}\\
           \zero  & \hdots &\zero &\tb_1^{\ell+1}  &\hdots &\zero &\tb_2^{\ell+1}  &\hdots &\zero &\zero &\hdots &\zero \\
           \hline
* & \hdots &* &* &\hdots &* &*&\hdots &* &* &\hdots &*\\
        \end{array}\right] 
    \end{equation}
    where $*$ denotes inconsequential values. 
\end{lemma}

Some observations are in order.
\begin{remark} 
    The process of filtering can be performed by designing the positional encoding as to be able to extract the information of which token is to be predicted automatically for any token. In other words, the encodings follow a pattern that is oblivious to the ``token-to-be-generated''. 
    Notice that one the current data points and their corresponding labels have been extracted, we can apply previous results on in-context learning gradient descent to perform linear regression (see \cite{giannou2023looped, akyurek2022learning}). For the update of the neural network, assuming that the activation functions are invertible we can use the result of \cite{giannou2023looped} to first invert the labels, then perform the linear regression and finally apply again the activation function. We provide the steps required for such a construction in the appendix.
\end{remark}
\begin{remark}
    When the filtering is performed, there is an $\pm\varepsilon >0$ error at left and right point of the non-zero positions. This error is controlled and can be arbitrarily small. The analysis of the error is given in the Appendix \ref{app:filtering}
\end{remark}
% The operation performed is in essence the operation of filtering. Each one of the five layers performs one of the following steps 
% \begin{enumerate}
%     \item The first layer uses the third line of the input, and created a weighted sum of it. The result would be equal to $k/N$, since there are $k$ ones and the total tokens are $N$.
%     \item The second layer calculates the number of tokens $N$. Notice that this information cannot be directly provided to the input, since for the prediction of the next token we can just append one extra column. Thus, it is not clear how this information can be isolated without the input size being proportional to the number $L$.
%     \item The third layer implements the multiplication and extracts the information regarding the current prediction, \textit{i.e., }$k$.
%     \item In the next layer the number $k$ is subtracted from each one of the elements of the second row presented in the input. 
%     \item The ReLUs of the next layer output one in the second row if the point is zero, and zero otherwise.
%     \item Finally this information is used, to filter the data points through another set of ReLus.
%     \end{enumerate}
% \begin{theorem}
%     In the setting of Lemma \ref{lem:filtering}
% \end{theorem}

==> fig_sec/fig_largek.tex <==
\begin{figure}[!t]
\centering
\subfigure[Composed risk]{
    \includegraphics[width=.315\columnwidth]{fig_sec/figs/cot_d10_largek.pdf}
    \label{fig:largek compose}
    % \hspace{-1mm}
}
\subfigure[Risk of first layer]{
    \includegraphics[width=.315\columnwidth]{fig_sec/figs/cot_d10_largek_first_layer.pdf}
    \label{fig:largek first}
    % \hspace{1mm}
}
\subfigure[Risk of second layer]{
    \includegraphics[width=.315\columnwidth]{fig_sec/figs/cot_d10_largek_second_layer.pdf}
    \label{fig:largek second}
    % \hspace{1mm}
}
\vspace{-2mm}
\caption{Decouple the composed risk into risks of first and second layers. }

\label{fig:largek}
\end{figure}

==> fig_sec/fig_main.tex <==
% \begin{figure}
% \centering
% \begin{minipage}{0.325\textwidth}
% 	\centering
% 	\includegraphics[scale=0.22]{fig_sec/figs/k16.pdf}
% % \caption{}
% \end{minipage}
% \begin{minipage}{0.325\textwidth}
% 	\centering
% 	\includegraphics[scale=0.22]{fig_sec/figs/cot_d10_vs_d20.pdf}
% % \caption{}
% \end{minipage}
% \begin{minipage}{0.325\textwidth}
% 	\centering
% 	\includegraphics[scale=0.22]{fig_sec/figs/cotk16_d10_vs_d20.pdf}
% % \caption{}
% \end{minipage}
% \caption{Comparing the }
% \end{figure}

\begin{figure}[!t]
\centering
\subfigure[$\COT~vs~\EXP~vs~\ICL$]{
    \includegraphics[width=.315\columnwidth]{fig_sec/figs/k16.pdf}
    \label{fig:k16}
    % \hspace{-1mm}
}
\subfigure[$\COT$: $d=10~vs~20$]{
    \includegraphics[width=.315\columnwidth]{fig_sec/figs/cot_d10_vs_d20.pdf}
    \label{fig:cot_d10_vs_d20}
    % \hspace{1mm}
}
\subfigure[Alignment in Fig.~\ref{fig:cot_d10_vs_d20}]{
    \includegraphics[width=.315\columnwidth]{fig_sec/figs/cotk16_d10_vs_d20.pdf}
    \label{fig:cot_d10_vs_d20_align}
    % \hspace{1mm}
}
\vspace{-2mm}
\caption{(a) Comparing the performance of the three algorithms CoT-I/O, CoT-I and ICL. \ks{I think all the plots should be CoT vs ICL vs CoT-I. So fig1: algo comparison with fixed model, fixed d, varying k. fig2: algo comparison with varying model, fixed d, fixed k and so on.. Like our older plots? What do you think @yc?}}

\label{fig:main_fig1}
\end{figure}

==> fig_sec/fig_method.tex <==
% \setlength{\arrayrulewidth}{.5pt}
% \begin{equation}
% \arraycolsep=2pt
% \def\arraystretch{1}
% \begin{array}{lc|ccccccccccc|ccc}
% \cline{3-13}
% \ICL&&\cellcolg\x_1 &\cellcolg&\cellcolg\y_1 & \cellcolr\x_2 &\cellcolr&\cellcolr\y_2 & \cellcolb\x_3 &\cellcolb&\cellcolb\y_3 & \cdots & \x_n \\
% \cline{3-13}
% \\
% \cline{3-13}
% \EXP&&\cellcolg\x_1 &\cellcolg\tb_1 &\cellcolg\y_1 & \cellcolr\x_2 & \cellcolr\tb_2 &\cellcolr\y_2 & \cellcolb\x_3 & \cellcolb\tb_3 & \cellcolb\y_3 & \cdots & \x_n & \hat\tb\\
% \cline{3-13}\\
% \cline{3-13}
% \COT&&\cellcolg\x_1 & \cellcolg\tb_1 &\cellcolg\y_1 & \cellcolr\x_2 & \cellcolr\tb_2 &\cellcolr\y_2 & \cellcolb\x_3 & \cellcolb\tb_3 & \cellcolb\y_3 & \cdots & \x_n & \hat\tb & \hat\y\\
% \cline{3-13}
% \end{array}
% \end{equation}


\setlength{\arrayrulewidth}{.5pt}
\begin{equation}
\arraycolsep=2pt
\def\arraystretch{1}
\begin{array}{ccc}
    \begin{array}{l}
    \begin{array}{ccccccccccccc|ccc}
    % \cline{3-13}
    \cellcolg\hat\y_1 && \cellcolr\hat\y_2 && \cellcolb\hat\y_3 && \cdots & \x_n \\
    % \cline{3-13}
    \\
    % \cline{3-13}
    \end{array}\\
    \begin{array}{ccccccccccccc|ccc}
    \cellcolg\x_1 &\cellcolg\y_1 & \cellcolr\x_2 &\cellcolr\y_2 & \cellcolb\x_3 & \cellcolb\y_3 & \cdots & \x_n & \hat\tb\\
    \end{array}\\
    \begin{array}{ccccccccccccc|ccc}
    \cellcolg\x_1 &\cellcolg\y_1 & \cellcolr\x_2 &\cellcolr\y_2 & \cellcolb\x_3 & \cellcolb\y_3 & \cdots & \x_n & \hat\tb & \hat\y    \end{array}
    \end{array}
    &
    \begin{array}{cc}
         &  \\
         & 
    \end{array}
    &
    \begin{array}{cc}
         &  \\
         & 
    \end{array}\\
    \ICL & \EXP & \COT
\end{array}
\end{equation}

==> fig_sec/fig_skill.tex <==
\begin{figure}[t]
\centering
\begin{minipage}[t]{0.45\linewidth}
    \centering
    \includegraphics[width=\linewidth]{fig_sec/figs/diff_clen}
    \caption{}
    \label{fig:diff_clen}
\end{minipage}
\hspace{30pt}
\begin{minipage}[t]{0.45\linewidth}
    \centering
    \includegraphics[width=\linewidth]{fig_sec/figs/diff_nfunc.pdf}
    \caption{}
    \label{fig:diff_func}
\end{minipage}
\end{figure}

% \begin{minipage}[b]{0.5\textwidth}
% \centering
% \setlength{\arrayrulewidth}{0.5mm}
% \setlength{\tabcolsep}{2pt}
\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.2}
{\small{
    \begin{tabular}{|c|cccc|c|}
        \hline
        Chain length & $3$ & $5$ & $7$ & $9$ & Unique\\
        \hline
         Zero-shot risk ($\times10^{-4}$)  & - & - & - & - & $9.7$\\
         One-shot risk ($\times10^{-4}$)  & $0.21$ & $0.57$ & $0.95$ & $1.29$ & $0.16$\\
        \hline
    \end{tabular}}}
    \captionof{table}{Your caption here}
    \label{tab:skill}
\end{table}
% \end{minipage}

==> rebuttal/fig_filter.tex <==
\begin{figure}[H]
% \vspace{-20pt}
\centering
\begin{tikzpicture}
    \node at (0,0){\includegraphics[scale=0.35]{figs/filter_v2.pdf}};


    \node at (-4.2,.0) {\textbf{\small CoT}};
    \node at (4.5,1.5) {\textbf{\small Step-1 ICL}};
    \node at (4.5,.0) {\textbf{\small Step-2 ICL}};
    \node at (4.5,-1.55) {\textbf{\small Step-3 ICL}};
    
    \node at (0,.5) {\textbf{\small Filtering}};
    \node at (2.3,2.7) {{\small 1st sample}};
    \node at (4.2,2.7) {{\small 2nd sample}};
    \node at (6.3,2.7) {{\small Test sample}};
    \node at (6.6,-2.7) {{\small Prediction}};
    \node at (4.2,3.3) {\textbf{{ICL with Filtered Prompts}}};
    \node at (4.2,2) {{}};
    
    % \node at (-5.05,0.5) {{\small $\x$}};
    % \node at (-4.7,0.5) {{\small $\s_1$}};
    % \node at (-4.35,0.5) {{\small $\s_2$}};
    % \node at (-4.,0.5) {{\small $\y$}};
    % \node at (-3.65,0.5) {{\small $\x$}};
    % \node at (-3.3,0.5) {{\small $\s_1$}};
    % \node at (-2.95,0.5) {{\small $\s_2$}};
    % \node at (-2.6,0.5) {{\small $\y$}};
    % \node at (-2.3,0.5) {{\small ...}};
    % \node at (-2.3,0.5) {{\small ...}};

    % \node at (-0.2,-0.9) {\textbf{\small $\EXP$}};
    % \node at (-1.4,-1.4) {{\tiny $\x_1$}};
    % \node at (-1.1,-1.39) {{\tiny $\tb^1_1$}};
    % \node at (-0.8,-1.39) {{\tiny $\tb^2_1$}};
    % \node at (-0.5,-1.4) {{\tiny $\y_1$}};
    % \node at (-0.2,-1.4) {{\tiny $\x_2$}};
    % \node at (0.1,-1.39) {{\tiny $\tb_2^1$}};
    % \node at (0.6,-1.4) {{\tiny\dots}};
    % \node at (1.1,-1.4) {{\tiny$\xtest$}};
    % \node at (1,-2.35) {{\tiny $\hat\y$}};


    % \node at (4,2.) {\textbf{\small $\COT$}};
    % \node at (2.7,1.5) {{\tiny $\x_1$}};
    % \node at (3,1.55) {{\tiny $\tb^1_1$}};
    % \node at (3.3,1.55) {{\tiny $\tb^2_1$}};
    % \node at (3.6,1.5) {{\tiny $\y_1$}};
    % \node at (3.9,1.5) {{\tiny $\x_2$}};
    % \node at (4.35,1.5) {{\tiny\dots}};
    % \node at (4.8,1.5) {{\tiny$\xtest$}};
    % \node at (4.8,0.55) {{\tiny $\hat\tb^1$}};

    % \node at (4.35,0.1) {{\tiny\dots}};
    % \node at (4.75,0.1) {{\tiny$\xtest$}};
    % \node at (5.15,0.15) {{\tiny$\hat\tb^1$}};
    % \node at (5.1,-0.9) {{\tiny$\hat\tb^2$}};

    % \node at (4.35,-1.35) {{\tiny\dots}};
    % \node at (4.75,-1.35) {{\tiny$\xtest$}};
    % \node at (5.15,-1.3) {{\tiny$\hat\tb^1$}};
    % \node at (5.5,-1.3) {{\tiny$\hat\tb^2$}};
    % \node at (5.4,-2.35) {{\tiny$\hat\y$}};

\end{tikzpicture}
\vspace{-5pt}
\caption{\textbf{An illustration of our theory: $\text{CoT}=\text{filtering}+\ICL$.} Here, (Yellow, Green, Orange, Blue) circles represent in-context sample ($\x,\s^1,\s^2,\y$). }
\vspace{-10pt}
\end{figure}

==> rebuttal/icl_padding.tex <==
\begin{figure}[H]
\centering
% \begin{minipage}{12cm}
% \begin{minipage}{6cm}
%  % \vspace{-.5cm} 
%     \centering
%    % \subfigure[small GPT-2, $d=10$, $k=4$]{
%         \begin{tikzpicture}
%         \node at (0,0) {\includegraphics[scale=.3]{figs/noise_rebuttal.pdf}};
%         \node at (0.4, -2.5) {(a) Test with noisy data};
%         \end{tikzpicture}
% \end{minipage}
% \begin{minipage}{6cm}
%  % \vspace{-.5cm}
%     % \centering
%    % \subfigure[small GPT-2, $d=10$, $k=4$]{
%         \begin{tikzpicture}
%         \node at (0,0) {\includegraphics[scale=.3]{figs/diff_k_rebuttal.pdf}};
%         \node at (0.4, -2.5) {(b) Test with different $k$};
%         \end{tikzpicture}
% \end{minipage}
% \caption{}
% \end{minipage}
\begin{minipage}{8cm}
 % \vspace{-.5cm} 
    \centering
   % \subfigure[small GPT-2, $d=10$, $k=4$]{
        \begin{tikzpicture}
        \node at (0,0) {\includegraphics[scale=.3]{figs/5-layer_MLP_rebuttal.pdf}};
        % \node at (0.4, -2.5) {(a) Train ICL with sample formed by $(\x,[?],\y)$};
        \end{tikzpicture}
        \caption{\textbf{Investigation of deep MLPs.}}
\end{minipage}
\hspace{10pt}
\begin{minipage}{8cm}
 % \vspace{-.5cm} 
    \centering
   % \subfigure[small GPT-2, $d=10$, $k=4$]{
        \begin{tikzpicture}
        % \node at (0,0) {\includegraphics[scale=.3]{figs/icl_random_rebuttal.pdf}};
        \node at (0,0) {\includegraphics[scale=.3]{figs/icl_random_-1_rebuttal.pdf}};
        % \node at (0.4, -2.5) {(a) Train ICL with sample formed by $(\x,[?],\y)$};
        \end{tikzpicture}
        \caption{\textbf{Train ICL with input $(\x,[?],\y)$.}}
\end{minipage}

\end{figure}

==> rebuttal/n200.tex <==
\begin{figure}[H]
\centering
%\begin{minipage}{15cm}
 \vspace{-.5cm} 
    \centering
   % \subfigure[small GPT-2, $d=10$, $k=4$]{
        \begin{tikzpicture}
        \node at (0,0) {\includegraphics[scale=.3]{figs/small_d10k4_n200_rebuttal.pdf}};
        \node at (0.4, -2.5) {(a) Small GPT-2, $d=10$, $k=4$};
        \end{tikzpicture}
   % }
    \hspace{10pt}
   % \subfigure[standard GPT-2, $d=10$, $k=4$]{
        \begin{tikzpicture}
        \node at (0,0) {\includegraphics[scale=.3]{figs/standard_d10k4_n200_rebuttal.pdf}};
        \node at (0.4, -2.5) {(b) Standard GPT-2, $d=10$, $k=4$};
        \end{tikzpicture}
   % }
    % \vspace{-10pt}
    \caption{\textbf{Train ICL with more in-context samples.} }
   % \end{minipage}
\end{figure}

==> rebuttal/robust.tex <==

\begin{figure}[H]
\centering
\begin{minipage}{19cm}
% \begin{minipage}{6cm}
 % \vspace{-.5cm} 
    \centering
   % \subfigure[small GPT-2, $d=10$, $k=4$]{
 \hspace{-.5cm}
        \begin{tikzpicture}
        \node at (0,0) {\includegraphics[scale=.3]{figs/noise_rebuttal.pdf}};
        \node at (0.4, -2.5) {(a) Test with noisy data};
        \end{tikzpicture}
% \end{minipage}
% \begin{minipage}{6cm}
 \hspace{-.5cm}
    % \centering
   % \subfigure[small GPT-2, $d=10$, $k=4$]{
        \begin{tikzpicture}
        \node at (0,0) {\includegraphics[scale=.3]{figs/diff_k_rebuttal.pdf}};
        \node at (0.4, -2.5) {(b) Test with different $k$};
        \end{tikzpicture}
% \end{minipage}
% \caption{}
% \end{minipage}
% \begin{minipage}{6cm}
 \hspace{-.5cm} 
    \centering
   % \subfigure[small GPT-2, $d=10$, $k=4$]{
        \begin{tikzpicture}
        \node at (0,0) {\includegraphics[scale=.3]{figs/diff_d_rebuttal.pdf}};
        \node at (0.4, -2.5) {(c) Test with different $d$};
        \end{tikzpicture}
        \caption{\textbf{Out-of-distribution experiments.}}
\end{minipage}

\end{figure}



==> sec/backup/main.tex <==
\section{How can Transformer Deal with the CoT Prompts?}\label{sec main theory}
\YL{Show the main results: filtering+composition}
\begin{theorem}[Filtering]

\end{theorem}

\begin{theorem}[Composition]

\end{theorem}

\begin{assumption}
    Assume the model $\TF$ is $\Gamma$-Lipschitz with respect to the last input, that is
    \[
    \|\TF(\pmt,\x)-\TF(\pmt,\x')\|\leq\Gamma\|\x-\x'\|.
    \]
\end{assumption}

\begin{assumption}[Approximation to ERM]
Assume there exists model $\tTF$ such that for any $f\in\Fc_\ell$,
\[
\E_{(\x_i)_{i=1}^n,\x}\left[\|\tTF(\pmt_n,\x)- \hat f_n(\x)\|\right]\leq\eps
\]
\[
\text{where}~~~~\pmt_n=(\x_i,f(\x_i))_{i=1}^n,~~\text{and}~~
\hat f_n =\arg\min_{f_n\in\Fc_\ell}\frac{1}{n}\sum_{i=1}^n\ell(f_n(\x_i),f(\x_i))
\]
and $\x\sim\Dc_{\Fc_{\ell-1}}\times\dots\Dc_{\Fc_1}\times\Dc_{\x}$. 
% Here $r(n)$ is a non-increasing function capturing the ability of transformer of learning function $f\in\Fc_\ell$ with randomly distributed $n$ samples.
\end{assumption}

% Here, if treating $\TF$ as a learning algorithm that admits a dataset as input, $r(n)$ can be treated as the approximation error $\TF$ achieves

\begin{theorem}
\begin{align}
    \lesssim\sum_{\ell=1}^L\Gamma^{\ell+1}(\eps+\Rc_n(\Fc_\ell))
\end{align}    
\end{theorem}

\input{sec/nn}


==> sec/backup/nn.tex <==
\subsection{Deep Neural Networks as Compositional Functions}
\YL{Introduce the results when functions are linear}\\
% \YL{Also introduce neural nets experiments}


==> sec/backup/setup__backup_v2_.tex <==
\section{Problem Setup}
\noindent\textbf{Notation:} Let $[n]=\{1,2,\cdots,n\}$. Let $\Xc$ denote token/input space, $\Yc$ denote output space and $\Zcid{k}$, $k\in[K]$ denote the intermediate feature space, where $\x\in\Xc,\y\in\Yc$ and $\zid{k}\in\Zcid{k}$. We can define an ICL example of CoT by 
\[
\p=(\x,\zid{1},\zid{2},\cdots,\zid{K},\y).
\]
Then ICL admits length-$t$ prompt as form $\pmt=(\p_1,\p_2,\cdots,\p_t,\x)$.

Consider an in-context-learning (ICL) problem, and assume we are given $n$ training sequences, and each contains $T$ samples. Specifically, define training dataset $\Sc=((\p_{it})_{t=1}^T)_{i=1}^n$ where $\p_{it}=(\x_{it},\zid{1}_{it},\cdots\zid{K}_{it},\y_{it})$, and assume the input-output pairs follow the distribution $\y_{it}=f_{it}(\x_{it})$ where $f_{it}=\fid{K}_{it}\circ\cdots\fid{1}_{it}\circ\fid{0}_{it}$ where $f_{it}\in\Fc:\Xc\to\Yc$, $\fid{k}_{it}\in\Fcid{k} (0\leq k\leq K)$, and $\Fc=\Fcid{K}\times\cdots\Fcid{0}$. Let $\TF$ denote any auto-regressive model (e.g., Transformer) which admits sequences of data as inputs, and $\ell_0:\Yc\times\Yc\to\R$, $\ell_k:\Zcid{k}\times\Zcid{k}\to\R$ be loss functions. Then ICL aims to solve the empirical risk minimization problem over training dataset $\Sc$ as follows.
\begin{align}
% \hat\bt=&\arg\min_{\bt}\frac{1}{nT}\sum_{i=1}^n\sum_{t=1}^T\ell(\TF(\pmtid{K}_{it}),\y_{it})\label{erm}\\
\hat\bt=\arg\min_{\bt}\frac{1}{nT}&\sum_{i=1}^n\sum_{t=1}^T\left(\ell_0(\TF(\pmtid{K}_{it}),\y_{it})+\sum_{k=1}^K\ell_k(\TF(\pmtid{k-1}_{it}),\zid{k}_{it})\right)\label{erm}\\
\text{where}~~~~&\pmtid{0}_{it}=(\p_{i1},\p_{i2},\cdot,\p_{i,t-1},\x_{it})\nn\\
&\pmtid{k}_{it}=(\p_{i1},\p_{i2},\cdot,\p_{i,t-1},\x_{it},\zid{1}_{it},\cdots,\zid{k}_{it}).\nn
\end{align}
where model $\TF$ is parameterized by $\bt$ and let $\widehat\TF$ be the trained model weighted by $\hat\bt$ from \eqref{erm}. Then the CoT test risk can be defined as 
\begin{align}
    \Lc(\hat\bt)=&\E\left[\frac{1}{T}\sum_{t=1}^T\ell_0(\widehat\TF(\pmtid{K}_t),\y)\right]\\
    \text{where}~~~~&\pmtid{0}_t=(\p_1,\cdots,\p_{t-1},\x),\nn\\
    &\pmtid{k}_t=(\p_1,\cdots,\p_{t-1},\x,\hzid{1}_t,\cdots,\hzid{k}_t),\nn\\
    &\hzid{k}_t=\widehat\TF(\pmtid{k-1}_t).\nn
\end{align}


\section{Problem Setup}
\noindent\textbf{Notation:} Let $\Xc$ denote token/input space and $\Yc$ denote output space where $\x\in\Xc$ and $\y\in\Yc$. Assume there are $K$ types of tokens and  denote the set of $k$th type as $\Xcid{k}$, then we have $\Xc=\bigcup_{k=1}^K\Xcid{k}$. For an example, in natural language processing, words can be categorized into verbs, nouns, adjectives etc. Denote $\Xc^{\otimes t}$ as $t$-times Cartesian product of $\Xc$. 

Consider an in-context-learning (ICL) problem, and assume we are given $n$ training sequences, and each contains $T$ samples. Specifically, define training dataset $\Sc=((\X_{it},\y_{it})_{t=1}^T)_{i=1}^n$ where $\X_{it}=(\x_{i1},\x_{i2},\cdots\x_{it})\in\Xc^{\otimes t}$ and $\y_{it}\in\Yc$, and assume the input-output pairs follow the distribution $\y_{it}=f_{it}(\x_{it})$ where $f_{it}\in\Fc=\bigcup_{k=1}^K\Fc^k$. We say that $\x_{it}\in\Xcid{k}$ if $f_{it}\in\Fc^k$. Let $\TF$ denote any auto-regressive model (e.g., Transformer) which admits sequences of data as inputs, and $\ell:\Yc\times\Yc\to\R$ be loss function. Then ICL aims to solve the empirical risk minimization problem over $\Sc$ as follows.
\begin{align}
\hat\bt=\arg\min_{\bt}\frac{1}{nT}\sum_{i=1}^n\sum_{t=1}^T\ell(\TF(\X_{ti}),\y_{it})\label{erm}
\end{align}
where model $\TF$ is parameterized by $\bt$ and let $\widehat\TF$ be the trained model weighted by $\hat\bt$ from \eqref{erm}.

Consider any input sequence $\X=(\x_1,\x_2,\cdots,\x_t)$, and its corresponding output $\Y=(f_!(\x_1),f_2(\x_2),\cdots,f_t(\x_t))$. Then we say that $\x_\tau$ is relevant to $\x_t$ if they are from the same token space. Without loss of generality, let us assume $\x_t\in\Xcid{1}$, and then we can build relevant set of $\x_t$ by $\X_R=\{\x_\tau:\tau\leq t,\x_\tau\in\Xcid{1}\}$.

\noindent $\bullet$ \textbf{Transformer can handle heterogeneous prompts.} Given a prompt containing tokens from multiple feature spaces, the $\TF$ is able to filter out irrelevant tokens and focus on the relevant ones. That is 
\[
\TF(\X)\approx\TF(\X_R).
\]
Here, $\X_R$ is defined by the sequence $\X$ and the feature space its last token belongs to. Then instead of taking $T$-length sequence as input, the $\TF$ performs almost the same as treating $\X_R$ as input with $|\X_R|<T$. It implies that the irrelevant tokens are helpless in predicting the input at hand. This allows the model to effectively handle prompts with heterogeneous features, and the resulting performance is almost as good as if the prompt was constructed using only the relevant tokens.

\noindent $\bullet$ \textbf{Implicit chain-of-thought property.} The property arises from the Transformer's ability to focus on different relevant sets of tokens. Generally, we have $\Yc\subseteq\Xc$. When the Transformer generates an output based on a given input, the relevant set of tokens for the output is different from the relevant set for the input. Let $\hat\y_t=\TF(\X)$ and without loss of generality, assume $\y_t\in\Xcid{2}$. Feeding $\hat\y$ back to the model as the next token results in different relevant set, that is $\X'_R=\{\x_\tau:\tau\leq t+1,\x_\tau\in\Xcid{2}\}$ where $\X'=(\X,\hat\y)$ and $\x_{t+1}=\hat\y$. By repeating this process, the Transformer generates a sequence of outputs that reflect a "chain-of-thought" behavior, where each output is generated based on a different set of relevant tokens.
% \noindent\textbf{Notation:} Let $\Xc$ denote the token/feature space where $\x\in\Xc$, and assume there are $D$ types of tokens. Denote the $i$th type as $\Xcid{i}$, then we have $\Xc=\bigcup_{i=1}^D\Xcid{i}$. For an example, in natural language processing, words can be categorized into verbs, nouns, adjectives etc.

% Now define the input sequence (as prompt) by 
% \[
% \pmt=(\x_1,f_1(\x_1),\x_2,f_2(\x_2),\cdots,\x_t,f_t(\x_t);\x_\new).
% \]
% The goal of ICL is to predict current input $\x_\new$ based on the given prefix and the training stage. Let $\TF$ define any auto-regressive model admits the prompt as input and outputs $\hat f(\x_\new)=\TF(\pmt)$. 
% % For cleaner notations, let $\y_{i}=f_i(\x_i)$ and $\hat\y=\hat f(\x_\new)$. 
% Assume we are given training dataset $\Sc=((\x_{it},f_{it})_{t=1}^T)_{i=1}^n$ where $\pmt_{it}:=(\x_{i1},f_{i1}(\x_{i1}),\cdots,\x_{i,t-1},f_{i,t-1}(\x_{i,t-1});\x_t)$. What's more, assume for each $(\x,f)$ pair, if $\x\in\Xc^1$ then $f\in\Fc^1$, and within a sequence, function is fixed for $\x$ from the same feature space. Then the objective function is written by
% \[
% \arg\min_{\bt}\frac{1}{nT}\sum_{i=1}^n\sum_{t=1}^T\ell(\TF(\pmt_{it}),f_{it}(\x_{it}))
% \]
% where model $\TF$ is parameterized by $\bt$.
% There are two main observations contributing this work.

% \noindent $\bullet$ \textbf{Transformer can handle heterogeneous prompts.} Without loss of generality, let us assume $\x_\new\in\Xcid{1}$ and define $\pmtid{1}=(\texttt{FILTERED},\x_i,f_i(\x_i)\cdots;\x_\new)$ where $\pmtid{1}$ filters out the irrelevant tokens and the relevant ones remain, that is $\x_i\in\Xc^1$. Then instead $\pmt^1$ turns to be a homogeneous prompt. We observe that  $\TF(\pmt)\approx\TF(\pmt^1)$. In a nutshell, transformers can filter the prompt and automatically pick the most relevant tokens (from the same feature space in our case) as inference. 

% \noindent $\bullet$ \textbf{ICL as a function learning.} Consider a filtered homogeneous prompt $\pmt^1=(\x'_1,f(\x'_1),\cdots,\x'_\tau,f(\x'_\tau);\x_\new)$, and we observe that ICL outputs $\hat f(\x_\new)$ where 

% Combining both properties results in the chain-of-thought behavior of transformers, that is, given a few in-context examples, the model can automatically generate the next prediction sequentially, and the generation is based on 1) Which feature follows the input more frequently; and 2) How generating function is learned based on the given identified examples.



==> sec/construction_v2.tex <==
\section{Construction}
\subsection{The transformer architecture. }\label{ss:transformer}
For the purpose of this proof, we consider encoder-based transformer architectures; we assume that the positional encodings are appended to the input\footnote{We note here that in terms of our construction adding the encodings or appending them to the input can be viewed in a similar manner. Specifically, we can consider that the up-projection step projects the input to  zero padded vectors, while the encodings are orthogonal to that projection in the sense that the have zero in the non-zero coordinates of the input. In that case adding the positional encodings  corresponds to appending them to the input. }. We also consider that the heds are added and each one has each own key, query and value weight matrices. Formally, we have 
\begin{align}\label{eq:transformer}
    \attn(\X) &= \X + \sum_{h=1}^H\weights^h_\val\X\sfm((\weights^h_\key\X)^\top\weights^h_\query\X)\\
    \TF(\X) &= \attn(\X) + \weights_2(\weights_1\attn(\X) +\vb_1\one_n)_{+} +\vb_2\one_n
\end{align}
where $\X\in\R^{d\times n}$, $H$ is the number of heads used and $f(x) = (x)_{+}$ is the ReLU function. We also make use of the temperature $\lambda$, which is a parameter of the softmax. Specifically, $\sfm(\x) = \{\e^{\lambda x_i}/\sum_j\e^{\lambda x_j}\}_{i}$. Notice that as $\lambda\to\infty$ we have $\sfm(\x)\to \max_i x_i$. We also assume that the inputs are bounded; we denote with $N_{max}$ the maximum sequence length of the model.
\begin{assumption}Each entry is bounded by some constant $c$, which implies that  $\|\X\|\leq c'$, for some large $c'$ that depends on the maximum sequence length and the width of the transformer.
\end{assumption}
\subsection{The positional encodings}\label{ss:pencodings} In the constructions below we use a combination of the binary representation of each position as well as some more information mentioned in the sections to follow. The binary representations, as well the encodings we construct,  require only logarithmic space with respect to the sequence length. Notice that binary representation of the positions satisfy the following two conditions:
\begin{enumerate}
    \item Let $\emb_i$ be the binary representation of the $i$-th position, then there exists $\varepsilon > 0$ such that $\emb_i^\top\emb_i > \emb_i^\top\emb_j +\varepsilon$ for all $j\neq i$.
    \item There exists a one layer transformer that can implement the addition of two pointers (see Lemma \ref{lem:addition} ).
\end{enumerate}%We note here that any choice of encodings could be made that satisfy the following two conditions: 
% \begin{assumption}\label{asm:distinct}
%     Let $\emb_i$ be the encoding of the $i$-th position, then there exists $\varepsilon > 0$ such that $\emb_i^\top\emb_i > \emb_i^\top\emb_j +\varepsilon$ for all $j\neq i$. 
% \end{assumption} 
% \begin{assumption}\label{asm:increasing}
%     There exists an operator $*$ that the transformer can implement in one layer (or constant layers) such that $\emb_i *\emb_j  =\emb_{i+j}$.
% \end{assumption}
% We note here that multiple choices of positional encodings satisfy these two assumptions. For example, \cite{..} have used binary positional encodings

One useful fact about the encodings is that as 
\subsection{``Black-box'' functions}
We follow the construction of \cite{giannou2023looped}  and we use the following individual implementations as they are. We repeat the statements here for convenience.
\begin{lemma}\label{lem:copy}
A transformer with one layer, one head, and width of $O(\log n +d)$, where $d$ is the dimension of the data vectors and $n$ is the length of the input, can read data/command vectors from the input to the scratchpad from the location pointed to by the position embedding vector in the scratchpad.
\end{lemma}
\begin{remark} For the idea on how this is possible we illustrate a simple example. Assume that $\seqlen=5$ and we want to copy and element from position (1,2) where the first element signifies the row and the second the column to position (3,5). The first step is to copy the second column to the fifth one; to do so we force the softmax matrix to acts as a permutation matrix, \emph{i.e.,} $[\ve_1\;\ve_2\;\ve_3\;\ve_4\;\ve_2]$ where $\ve_i$ is the one hot vector for the $i$-th row. This is achieved by the bianary representations by using as $\weights_\key\X = [\emb_1\;\hdots\;\emb_5]$, $\weights_\query\X = [\emb_1\;\hdots\;\emb_2]$ and by using $\lambda$ large enough the result follows. Then, we use a value matrix that only keeps the row $1$ and permutes it to the row 3. Finally, to account for the residual, we use an extra head, which softmax is approximately the identity and the value weight matrix is zero expect for the first row which is again permuted to the third one. This description follows the construction of \cite{akyurek2022learning}.
\end{remark}
\begin{lemma}\label{lem:addition}
   There exists a 1-hidden layer feedforward, ReLU network, with $8d$ activations in the hidden layer and $d$ neurons in the output layer that when given two $d$-dimensional binary vectors representing two non-negative integers, can output the binary vector representation of their sum, as long as the sum is less than $2^{d+1}$. 
   % Further, there is a special bit indicator that is 1 for the scratchpad and 0 for the rest of the input. If this bit is 1 then the operation above is performed, otherwise 0 is returned.
\end{lemma}
\begin{lemma}\label{lem:transpose}
Fix $\epsilon >0$ and consider an input of the following form
\begin{equation}
    \X = \left[\begin{array}{c|c|c|cc}
        \rmA  &\zero&\zero &\dots & \zero \\
 \zero&      \zero&\zero &\dots & \zero\\
         \emb_{1:d}&\emb_{1:d}&\emb_{1:d}& \dots  &\emb_{1:d}\\
         \rmP_1'&\rmP_{2}'&\rmP_{3}'& \dots  &\rmP_{d}'
    \end{array}\right]. \nonumber
\end{equation}
where $\rmA\in\R^{d\times d}$; then there exists transformer-based function block with 4 layers, 1 head and dimensionality $r = 2d+2\log d = O(d)$ that outputs the following matrix
\begin{equation}
    \X = \left[\begin{array}{c|c|c|cc}
\rmA' &\rmA'&\rmA'&\dots &\rmA' \\
        \zero&\zero&\zero &\dots &\zero \\
         \emb_{1:d}& \emb_{1:d}& \emb_{1:d}& \dots &\emb_{1:d} \\
        \rmP_1'&\rmP_{2}'&\rmP_{3}'& \dots  &\rmP_{d}'
    \end{array}\right]. \nonumber
\end{equation}
where $\rmA' = \rmA^\top +\epsilon\rmM$, for some $\|\rmM\|\leq 1$. The error $\epsilon$ depends on the choice of the temperature $\lambda$, as it is  a consequence of the \texttt{read/write} operations.
\end{lemma}
\begin{lemma}\label{lem:matrixmul_app}
Let $\rmA\in \R^{k\times m}$ and $\rmB \in \R^{k\times n}$; then for any $\epsilon >0$ there exists a transformer-based function block with  2 layers, 1 head and dimensionality $r = O(d)$ that  outputs the multiplication $\rmA^T\rmB^T +\eps\rmM$, for some $\|\rmM\|\leq 1$ .
\end{lemma}
\begin{remark}
    Notice that based on the proof of this lemma, the matrices/scalars/vectors need to be in the same rows, \emph{i.e.},
$\begin{bmatrix}
          \rmQ =  \rmA &\rmB 
        \end{bmatrix}
$. By also appending the appropriate binary encodings we can move the output in any specific place we choose as in Lemma \ref{lem:copy}. Also, following the proof of the paper the input matrix is actually 
\begin{equation*}
    \X = \begin{bmatrix}
        \rmQ& \zero &\zero \\
        \zero & \one\one^{\top} &\zero\\
        \Iden&\zero &\zero\\ 
        &\emb^{(1)}&\\
        &\emb^{(2)}&\\
        %\zero &\one^{\top} &\zero 
    \end{bmatrix}  
\end{equation*} 
where $\emb^{(1)}, \emb^{(2)}$ are chosen as in Lemma \ref{lem:copy} to specify the position of the result.
\end{remark}
\subsection{Filtering}\label{ss filtering}
\begin{lemma}\label{lem:zeroout-app}
    Assume that the input to a transformer layer is of the following form
    \begin{equation}
        \X = \begin{bmatrix}
            \x_1 &\x_2 &\hdots&\x_{n-1} &\x_n\\
            \zero &\zero &\hdots &\zero &\zero\\
        b_1 & b_2 & \hdots &b_{n-1} &b_n\\
        b_1' &b_2' &\hdots &b_{n-1}' &b_n
        \end{bmatrix}
    \end{equation}
    where $b_i,b_i'\in\{0,1\}$, with zero indicating that the corresponding point should be ignored. Then there exists a transformer $\TF$ consisting only of a ReLU layer that performs this filtering, \textit{i.e.}, 
    \begin{equation}
        \TF(\X) = \begin{bmatrix}
           \one\{b_1\neq 0\}\x_1&\one\{b_2\neq 0\}\x_2 &\hdots &\one\{b_{n-1}\neq 0\}\x_{n-1} &\one\{b_n\neq 0\}\x_n\\
            \one\{b_1'\neq 0\}\x_1&\one\{b_2'\neq 0\}\x_2 &\hdots &\one\{b_{n-1}'\neq 0\}\x_{n-1} &\one\{b_n'\neq 0\}\x_n\\
            b_1 & b_2 & \hdots &b_{n-1} &b_n\\
            b_1' &b_2' &\hdots &b_{n-1}' &b_n
        \end{bmatrix}
    \end{equation}
\end{lemma}
\begin{proof}
    The layer is the following:
    \begin{equation}
       \TF(\x_i) = x_i + (-Cb_i - \x_i)_+ - (-Cb_i + \x_i)_+
    \end{equation}
    for some large constant $C$. Notice that if $b_i =1$ the output is just $\x_i$. But if $b_i = 0$ then the output is zero. For the second set instead of using the bits $b_i$,  we use the $b_i'$.
\end{proof}
\begin{remark}\label{rem:error-app} Notice that if some $b_i$ is instead of $1$, $1\pm \varepsilon$, $\varepsilon < c/C$. Then the output of the above layer would be \begin{align}
\TF(\x_i) &= \x_i + (-C \pm C\varepsilon - \x_i) -( -C \pm C\varepsilon +\x_i)\\
& = \x_i
\end{align}
while if some $b_i =\pm \varepsilon$ instead of zero, and assuming that $\x_i > c>0$ or $\x_i < -c< 0$ the output would be 
\begin{align}
    \TF(\x_i) &= \x_i  +(-C\varepsilon - \x_i)_+ - (-Cb_i +\x_i)_+\\
    &= \x_i \pm C\varepsilon - \x_i \\
    &\leq c
\end{align}
If $\abs{\x_i} \leq c$ again the output would be less or equal than $c$, where $c$ can be arbitrarily small.
\end{remark}
But how we can create these bits for each different token we want to produce?  We now describe for clarity how next word prediction is performed. An $d\times N$-dimensional input is given to the transformer architecture, which is up-projected using the embedding layer; afterwards the positional encodings are added/appended to the it. At the last layer, the last token predicted is appended to the input, while the rest of the tokens remain unchanged. The same holds for the actual input to the transformer after appending the encodings. The only difference of the new input is the $n+1$-th token. We consider encoder-based architectures in all of our lemmas below. 

In the subsequent lemma we will try to construct and automated process that works along those guidelines.
To do so we assume that the input to the transformer contains the following information:
\begin{enumerate}
    \item An enumeration of the tokens from $1$ to $N$. 
    \item The $\ln$ of the above enumeration.
    \item Zeros for the tokens that correspond to the data points, $1$ for each token that is the $\x_{\text{test}}$ or it is a prediction based on this.
    \item An enumeration $1$ to $L$ for each one of the data points provided. For example, if we are given three sets of data we would have : $1\hdots L \; 1\hdots L\; 1\hdots L$.
    \item Some extra information that is needed to implement a multiplication step as described in Lemma \ref{lem:matrixmul_app} and to move things to the correct place.
\end{enumerate}
The above information can be viewed as part of the encodings that are appended to the transformer. Formally, we have
\begin{lemma}\label{lem:binary-app}
Consider that the $\ell-1$-th prediction has been made and the transformer is to  make the $\ell$-th one. The input to the transformer is:
\renewcommand{\arraystretch}{1.5}
\begin{equation*}
\arraycolsep=1.5pt
\X = \left[\begin{array}{*{12}c}
    \x_1 & \hdots &\x_{\ell}& \x_{\ell+1}&\hdots & \x_{L+\ell+1} &\x_{L+\ell+2} &\hdots & \x_{n} &\x &\hdots &f_{\ell-1}(\x)\\
    \zero &\hdots &\zero  &\zero &\hdots &\zero &\zero &\hdots &\zero &\zero &\hdots &\zero\\
        \hline
     1 & \hdots & \ell & \ell+1& \hdots &\ell &\ell+1 &\hdots &L &1&\hdots & \ell\\
     1 & \hdots & \ell &\ell+1 &\hdots &\ell &\ell+1&\hdots &L &1&\hdots & \ell\\
     \hline
     1 & \hdots & \ell &\ell+1 &\hdots &L+\ell+1 &L+\ell+2 &\hdots &n &n+1 &\hdots & N\\
    \ln(1) & \hdots & \ln(\ell) &\ln(\ell+1) &\hdots &\ln(L+\ell+1) &\ln(L+\ell+2) &\hdots &\ln(n) &\ln(n+1) &\hdots & \ln(N)\\
 0 & \hdots & 0 &0&\hdots &0  &0 &\hdots &0 &1 &\hdots & 1\\
1 & \hdots & 1 &1 &\hdots &1&1 &\hdots &1 &1 &\hdots & 1\\ 
\m_1 & \hdots & \m_\ell &\m_{\ell+1} &\hdots &\m_{L+\ell+1} &\m_{L+\ell+2} &\hdots &\m_{n} &\m_{n+1} &\hdots & \m_{N}\\
 \end{array}\right]
\end{equation*}
Then there exists a transformer $\TF$ consisting of 4 layers that has as output
\renewcommand{\arraystretch}{1.3}
\begin{equation*}
\arraycolsep=1.2pt
  \TF(\X)  =  \left[\begin{array}{*{12}c}
      \x_1  &\hdots &\x_{\ell}& \x_{\ell+1}&\hdots & \x_{L+\ell+1} &\x_{L+\ell+2} &\hdots & \x_{n} &\x &\hdots &f_{\ell-1}(\x)\\
      \x_1  &\hdots &\x_{\ell}& \x_{\ell+1}&\hdots  & \x_{L+\ell+1} &\x_{L+\ell+2} &\hdots & \x_{n} &\x &\hdots &f_{\ell-1}(\x)\\
      \hline
     0 & \hdots & 1 &0 &\hdots &1 &0 &\hdots &0&0 &\hdots & 1\\
     0 & \hdots & 0 &1 &\hdots &0 &1 &\hdots &0 &0 &\hdots &0 \\
     \hline
     1 & \hdots & \ell &\ell+1 &\hdots &L+\ell+1 &L+\ell+2 &\hdots &n &n+1 &\hdots & N\\
       \ln(1) & \hdots & \ln(\ell) &\ln(\ell+1) &\hdots &\ln(L+\ell+1) &\ln(L+\ell+2) &\hdots &\ln(n) &\ln(n+1) &\hdots & \ln(N)\\
 0 & \hdots & 0 &0&\hdots &0  &0 &\hdots &0 &1 &\hdots & 1\\
1 & \hdots & 1 &1 &\hdots &1&1 &\hdots &1 &1 &\hdots & 1\\ 
\m_1 & \hdots & \m_\ell &\m_{\ell+1} &\hdots &\m_{L+\ell+1} &\m_{L+\ell+2} &\hdots &\m_{n} &\m_{n+1} &\hdots & \m_{N}\\
  \end{array}\right] 
\end{equation*}
with error up to $\varepsilon\rmM$, where $\|{\rmM}\|\leq 1$ and $\varepsilon$ is a constant that is controlled and can be arbitrarily small.
\end{lemma}
\begin{proof}
\noindent\textbf{Step 1: Extract the sequence length (1 layer).} Let 
\begin{align}
\weights_{\query} =  \begin{bmatrix}
    \zero &\zero &0 &0 &0 &0 &0 &0 &1 &\zero 
\end{bmatrix}
 \;\;\; 
\weights_{\key}= \begin{bmatrix}
    \zero &\zero &0 &0 &0&1 &0 &0 &\zero
\end{bmatrix} 
\end{align}
and thus 
\begin{equation}
    (\weights_{\query}\X)^\top(\weights_{\key}\X) = \begin{bmatrix}
        \ln(1) &\ln(2) &\hdots &\ln(\seqlen)\\
        \ln(1) &\ln(2) &\hdots &\ln(\seqlen)\\
        \vdots &\vdots &\ddots &\vdots\\
        \ln(1) &\ln(2) &\hdots &\ln(\seqlen)\\
    \end{bmatrix}.
\end{equation}
So after the softmax is applied we have
\begin{equation} \sfm((\weights_{\query}\X)^\top(\weights_{\key}\X)) = \begin{bmatrix}
        \dfrac{1}{\sum_{i=1}^\seqlen i} &\dfrac{2}{\sum_{i=1}^\seqlen i}&\hdots &\dfrac{\seqlen}{\sum_{i=1}^\seqlen i}\\
        \dfrac{1}{\sum_{i=1}^\seqlen i} &\dfrac{2}{\sum_{i=1}^\seqlen i}&\hdots &\dfrac{\seqlen}{\sum_{i=1}^\seqlen i}\\
        \vdots &\vdots &\ddots &\vdots\\
        \dfrac{1}{\sum_{i=1}^\seqlen i} &\dfrac{2}{\sum_{i=1}^\seqlen i}&\hdots &\dfrac{\seqlen}{\sum_{i=1}^\seqlen i}\\
    \end{bmatrix}.
\end{equation}
We then set the weight value matrix as to zero-out all lines except for one line as follows
\begin{equation}
   \weights_{\val}\X =\begin{bmatrix}
   \zero &\zero & \hdots &\zero \\
    1 & 2 &\hdots &\seqlen\\
 \zero &\zero &\hdots &\zero 
   \end{bmatrix}
\end{equation}
% \begin{equation}
%    \weights_{\val}\rmI =\begin{bmatrix}
%    \zero &\zero & \hdots &\zero \\
%   \zero &\zero & \hdots &\zero \\
%     \zero &\zero & \hdots &\zero \\
%     \zero &\zero & \hdots &\zero \\
%     1 & 2 &\hdots &\seqlen\\
%     0 &0 &\hdots &0\\
%      0 &0 &\hdots &0\\
%        0 &0 &\hdots &0
%    \end{bmatrix}
% \end{equation}
After adding the residual and using an extra head whose softmax returns identity matrix and the value weight matrix is minus the identity, we get 
\renewcommand{\arraystretch}{1.5}
\begin{equation*}
\arraycolsep = 1.5pt
    \X = \left[\begin{array}{*{12}c}
    \x_1 & \hdots &\x_{\ell}& \x_{\ell+1}&\hdots & \x_{L+\ell+1} &\x_{L+\ell+2} &\hdots & \x_{n} &\x &\hdots &f_{\ell-1}(\x)\\
    \zero &\hdots &\zero  &\zero &\hdots &\zero &\zero &\hdots &\zero &\zero &\hdots &\zero\\
        \hline
     1 & \hdots & \ell & \ell+1& \hdots &\ell &\ell+1 &\hdots &L &1&\hdots & \ell\\
     1 & \hdots & \ell &\ell+1 &\hdots &\ell &\ell+1&\hdots &L &1&\hdots & \ell\\
     \hline
     \dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i} & \hdots & \dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i} &\dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i} &\hdots &\dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i}&\dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i} &\hdots &\dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i} &\dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i} &\hdots & \dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i}\\
    \ln(1) & \hdots & \ln(\ell) &\ln(\ell+1) &\hdots &\ln(L+\ell+1) &\ln(L+\ell+2) &\hdots &\ln(n) &\ln(n+1) &\hdots & \ln(N)\\
 0 & \hdots & 0 &0&\hdots &0  &0 &\hdots &0 &1 &\hdots & 1\\
1 & \hdots & 1 &1 &\hdots &1&1 &\hdots &1 &1 &\hdots & 1\\ 
\m_1 & \hdots & \m_\ell &\m_{\ell+1} &\hdots &\m_{L+\ell+1} &\m_{L+\ell+2} &\hdots &\m_{n} &\m_{n+1} &\hdots & \m_{N}\\
 \end{array}\right]
\end{equation*}
Notice that $\dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i} = \dfrac{2\seqlen(\seqlen+1)(2\seqlen+1)}{6\seqlen(\seqlen+1)} = \dfrac{2\seqlen+1}{3}$. We then use the ReLU layer as to multiply with $3/2$ and subtract $1/3$ from this column. This results to 
\begin{equation*}
\arraycolsep = 1.5pt
    \X = \left[\begin{array}{*{12}c}
    \x_1 & \hdots &\x_{\ell}& \x_{\ell+1}&\hdots & \x_{L+\ell+1} &\x_{L+\ell+2} &\hdots & \x_{n} &\x &\hdots &f_{\ell-1}(\x)\\
    \zero &\hdots &\zero  &\zero &\hdots &\zero &\zero &\hdots &\zero &\zero &\hdots &\zero\\
        \hline
     1 & \hdots & \ell & \ell+1& \hdots &\ell &\ell+1 &\hdots &L &1&\hdots & \ell\\
     1 & \hdots & \ell &\ell+1 &\hdots &\ell &\ell+1&\hdots &L &1&\hdots & \ell\\
     \hline
     N & \hdots & N &N&\hdots &N&N &\hdots &N&N&\hdots & N\\
    \ln(1) & \hdots & \ln(\ell) &\ln(\ell+1) &\hdots &\ln(L+\ell+1) &\ln(L+\ell+2) &\hdots &\ln(n) &\ln(n+1) &\hdots & \ln(N)\\
 0 & \hdots & 0 &0&\hdots &0  &0 &\hdots &0 &1 &\hdots & 1\\
1 & \hdots & 1 &1 &\hdots &1&1 &\hdots &1 &1 &\hdots & 1\\ 
\m_1 & \hdots & \m_\ell &\m_{\ell+1} &\hdots &\m_{L+\ell+1} &\m_{L+\ell+2} &\hdots &\m_{n} &\m_{n+1} &\hdots & \m_{N}\\
 \end{array}\right]
\end{equation*}

\textbf{Step 2: Extract the number of the prediction to be made $\ell$ (3 layers). }Now, by setting the key and query weight matrices of the attention as  to just keep the all ones row, we get a matrix that attends equally  to all tokens. Then the value weight matrix keeps the row that contains $\ell$ ones and thus we get the number $\dfrac{\ell}{N}$, propagated in all the sequence length. 
\begin{equation}
    \arraycolsep = 1.5pt
    \X = \left[\begin{array}{*{12}c}
    \x_1 & \hdots &\x_{\ell}& \x_{\ell+1}&\hdots & \x_{L+\ell+1} &\x_{L+\ell+2} &\hdots & \x_{n} &\x &\hdots &f_{\ell-1}(\x)\\
    \zero &\hdots &\zero  &\zero &\hdots &\zero &\zero &\hdots &\zero &\zero &\hdots &\zero\\
        \hline
     1 & \hdots & \ell & \ell+1& \hdots &\ell &\ell+1 &\hdots &L &1&\hdots & \ell\\
     1 & \hdots & \ell &\ell+1 &\hdots &\ell &\ell+1&\hdots &L &1&\hdots & \ell\\
     \hline
     N & \hdots & N &N&\hdots &N&N &\hdots &N&N&\hdots & N\\
    \dfrac{\ell}{N} & \hdots & \dfrac{\ell}{N} &\dfrac{\ell}{N} &\hdots &\dfrac{\ell}{N} &\dfrac{\ell}{N} &\hdots &\dfrac{\ell}{N} &\dfrac{\ell}{N} &\hdots &\dfrac{\ell}{N}\\
 0 & \hdots & 0 &0&\hdots &0  &0 &\hdots &0 &1 &\hdots & 1\\
1 & \hdots & 1 &1 &\hdots &1&1 &\hdots &1 &1 &\hdots & 1\\ 
\m_1 & \hdots & \m_\ell &\m_{\ell+1} &\hdots &\m_{L+\ell+1} &\m_{L+\ell+2} &\hdots &\m_{n} &\m_{n+1} &\hdots & \m_{N}\\
 \end{array}\right]
\end{equation}
As described in Lemma \ref{lem:matrixmul_app} to implement multiplication of two values up to any error $\eps$, we need 1) have the two numbers to be multiplied next to each other and an extra structure (some constants, which we consider that are encoded in the last rows of the matrix $\m_i$) and 2) the corresponding structure presented in Lemma \ref{lem:matrixmul_app} . So we need to make the following transformation in the rows containing $N$ and $\dfrac{\ell}{N}$
\begin{align}
    \begin{bmatrix}
        N & N &\hdots &N\\
        \dfrac{\ell}{N} &\dfrac{\ell}{N} &\hdots &\dfrac{\ell}{N}
    \end{bmatrix} &\to \begin{bmatrix}
        N & \dfrac{\ell}{N} &\hdots &N\\
        \dfrac{\ell}{N} &\dfrac{\ell}{N} &\hdots &\dfrac{\ell}{N}
    \end{bmatrix}\\
    &\to 
    \begin{bmatrix}
         \ell& *&\hdots &*\\
        * &* &\hdots &*
    \end{bmatrix}\\
    &\to \begin{bmatrix}
        \ell& \ell&\hdots &\ell\\
         * &* &\hdots &*
    \end{bmatrix}
\end{align}
where $*$ denotes inconsequential values.
For the first step we assume that we have the necessary binary representations \footnote{the size that we need will be $2\log N_{\text{max}}+1$, where $N_{\text{max}}$ is the maximum sequence length} and then we use Lemma \ref{lem:copy} which shows how we can perform the operation of copy/paste. For the second step now we use Lemma \ref{lem:matrixmul_app} to perform the multiplication, this will affect some of the other values. Then for the last step consider the follow (sub-)rows of the matrix $\X$
\begin{equation}
    \begin{bmatrix}
        \ell & * &* &\hdots &*\\
        \emb_1 &\emb_1 &\emb_1 &\hdots &\emb_1\\
        \emb_1 &\emb_2 &\emb_3 &\hdots &\emb_N
    \end{bmatrix}
\end{equation}
where $\emb_i$ is the binary representation of position $i$. By choosing $\weights_\key,\weights_\query$ as to
\begin{equation}
    \weights_\key\X = \begin{bmatrix}
        \emb_1 &\emb_2 &\hdots &\emb_N
    \end{bmatrix}, \;\;\;\weights_\query\X = \begin{bmatrix}
        \emb_1 &\emb_1 &\hdots &\emb_1 
    \end{bmatrix} 
\end{equation}
and consider $\weights_\val\X = \begin{bmatrix}
        \ell & * & \hdots &*\\
        \zero &\zero &\hdots &\zero 
    \end{bmatrix}$ we have that 
    \begin{align*}
       \attn(\X) &= \X+ \weights_\val\X \sfm((\weights_\key\X)^\top\weights_\query)\\
       &= \X + \begin{bmatrix}
        \ell & * & \hdots &*\\
        \zero &\zero &\hdots &\zero 
    \end{bmatrix} \sfm(\begin{bmatrix}
        \emb_1^\top\emb_1 &\emb_1^\top\emb_1 &\hdots &\emb_1^\top\emb_1\\
         \emb_1^\top\emb_2 &\emb_1^\top\emb_2 & \hdots &\emb_1^\top\emb_2 \\
         \vdots &\vdots &\ddots &\vdots\\
         \emb_1^\top\emb_N &\emb_1^\top\emb_N &\hdots &\emb_1^\top\emb_N
    \end{bmatrix})\\
    &= \X+ \begin{bmatrix}
        \ell & * & \hdots &*\\
        \zero &\zero &\hdots &\zero 
    \end{bmatrix}   \begin{bmatrix}
        1 & 1 &\hdots &1 \\
        0 & 0 &\hdots &0\\
        \vdots &\vdots &\hdots &\vdots\\
        0 & 0 &\hdots & 0
    \end{bmatrix} +\varepsilon \rmM
    \end{align*}
    By subtracting one identity head for the first that we focus on as described in Lemma \ref{lem:copy} we have that $\attn(\X)$ results in the desired matrix. We output this result and overwrite $\ell/N$, thus we have
    \begin{equation}
    \arraycolsep = 1.5pt
    \X = \left[\begin{array}{*{12}c}
    \x_1 & \hdots &\x_{\ell}& \x_{\ell+1}&\hdots & \x_{L+\ell+1} &\x_{L+\ell+2} &\hdots & \x_{n} &\x &\hdots &f_{\ell-1}(\x)\\
    \zero &\hdots &\zero  &\zero &\hdots &\zero &\zero &\hdots &\zero &\zero &\hdots &\zero\\
        \hline
     1 & \hdots & \ell & \ell+1& \hdots &\ell &\ell+1 &\hdots &L &1&\hdots & \ell\\
     1 & \hdots & \ell &\ell+1 &\hdots &\ell &\ell+1&\hdots &L &1&\hdots & \ell\\
     \hline
     N & \hdots & N &N&\hdots &N&N &\hdots &N&N&\hdots & N\\
   \ell & \hdots & \ell &\ell &\hdots &\ell &\ell &\hdots &\ell &\ell &\hdots &\ell\\
 0 & \hdots & 0 &0&\hdots &0  &0 &\hdots &0 &1 &\hdots & 1\\
1 & \hdots & 1 &1 &\hdots &1&1 &\hdots &1 &1 &\hdots & 1\\ 
\m_1 & \hdots & \m_\ell &\m_{\ell+1} &\hdots &\m_{L+\ell+1} &\m_{L+\ell+2} &\hdots &\m_{n} &\m_{n+1} &\hdots & \m_{N}\\
 \end{array}\right]
\end{equation}
    \paragraph{Step 3: Create $\ell+1$ (0 layer). } We first copy the row with $\ell$ to the row with $N$, this can trivially be done with a ReLU layer that outputs zero everywhere else except for the row of $N$s that output $(\ell)_{+} - (N)_{+}$ to account also for the residual. We now use one of the bias terms (notice that $\ell$ is always positive) and set to one in one of the two rows that contain the $\ell$, again we account for the residual as before; everything else remains unchanged. Thus, we have
    \begin{equation}
    \arraycolsep = 1.5pt
    \X = \left[\begin{array}{*{12}c}
    \x_1 & \hdots &\x_{\ell}& \x_{\ell+1}&\hdots & \x_{L+\ell+1} &\x_{L+\ell+2} &\hdots & \x_{n} &\x &\hdots &f_{\ell-1}(\x)\\
    \zero &\hdots &\zero  &\zero &\hdots &\zero &\zero &\hdots &\zero &\zero &\hdots &\zero\\
        \hline
     1 & \hdots & \ell & \ell+1& \hdots &\ell &\ell+1 &\hdots &L &1&\hdots & \ell\\
     1 & \hdots & \ell &\ell+1 &\hdots &\ell &\ell+1&\hdots &L &1&\hdots & \ell\\
     \hline
     \ell+1 & \hdots & \ell+1 &\ell+1&\hdots &\ell+1 &\ell+1 &\hdots &\ell+1 &\ell+1 &\hdots &\ell+1\\
    \ell & \hdots & \ell &\ell &\hdots &\ell &\ell &\hdots &\ell &\ell &\hdots &\ell\\
 0 & \hdots & 0 &0&\hdots &0  &0 &\hdots &0 &1 &\hdots & 1\\
1 & \hdots & 1 &1 &\hdots &1&1 &\hdots &1 &1 &\hdots & 1\\ 
\m_1 & \hdots & \m_\ell &\m_{\ell+1} &\hdots &\m_{L+\ell+1} &\m_{L+\ell+2} &\hdots &\m_{n} &\m_{n+1} &\hdots & \m_{N}\\
 \end{array}\right]
\end{equation}
This operation can collectively be implemented (add the bias + copy the row) in the ReLU layer of the previous transformer layer that was not used in the previous step.
    \paragraph{Step 4: Create the binary bits (1 layer). }We will now use the information extracted in the previous steps, to create the binary indicators/bit to identify which tokens we want to filter. This can be easily implemented with one layer of transformer and especially the  ReLU part of it. Notice that if we subtract the row that contains the tokens that have already been predicted, \emph{i.e.,} $[\ell\ell\hdots \ell]$ from the row that contains $[12\hdots L  12\hdots L \hdots L]$ we will get zero only in the positions that we want to filter out and some non-zero quantity in the rest. So, we need to implement an if..then type of operation. Basically, if the quantity at hand is zero we want to set the bit to one, while if it non-zero to set it to be zero. This can be implemented with the following ReLU layer
    \AG{Add the expression}

    \textbf{Step 5: Implement the filtering (1 layer).}  We now apply Lemma \ref{lem:binary-app} and our proof is completed.
\end{proof}

\begin{theorem}[Decoupling CoT]\label{thm:MLP} Consider a prompt $\pmt_n(f)$ generated from an $L$-layer MLP $f(\cdot)$ as described in Definition \ref{MLP assump}, and assume given test example $(\xtest,\tb^1_{\text{\tiny test}}, \dots\tb^L_{\text{\tiny test}})$. 
% , containing $n$ examples and ends with $\x^{\texttt{test}}$. 
For any resolution $\eps>0$, there exists $\delta=\delta(\eps)$, iteration choice $T={\cal{O}}(\kappa_{\max}^2\log(1/\eps))$, and a backend transformer construction $\TFBE$ such that the concatenated transformer $\TF=\TFLR \circ \TFBE$ implements the following: Let $(\tht^{i})_{i=1}^{\ell-1}$ denote the first $\ell-1$ $\COT$ outputs of $\TF$ and set $\pb[\ell]=(\pb_n(f),\xtest,\tht^{1}\dots\tht^{\ell-1})$. At step $\ell$, $\TF$ implements
\begin{enumerate}
\item \textbf{Filtering.} Define the filtered prompt with input/output features of layer $\ell$,
\[
\arraycolsep = 1pt
\pbf_n=\left(\begin{array}{*{10}c}
\hdots \zero,&\tb^{\ell-1}_{1},&\zero&\hdots&\zero,&\tb^{\ell-1}_n, &\zero&\hdots&\zero,&\tht^{\ell-1}\\
\hdots\zero,&\zero,& \tb^{\ell}_{1}&\dots&\zero,&\zero,& \tb^{\ell}_n&\dots&\zero,&\zero\end{array}\right).
\]
There exists a fixed projection matrix $\bPi$ that applies individually on tokens such that the backend output obeys $\tn{\bPi(\TFBE(\pb[\ell]))-\pbf_n}\leq \delta$. %The more precise statement is provided in Lemma \ref{lem:filtering}. % up to $\eps$ accuracy via a fixed linear projection. 
\item \textbf{Gradient descent.} The combined model obeys $\tn{\TF(\pb[\ell])-\tb_{\text{\tiny test}}^{\ell}}\leq {\ell\cdot \eps}/{L}$.
\end{enumerate}
$\TFBE$ has constant number of layers independent of $T$ and $n$. Consequently, after $L$ rounds of $\COT$, \TF outputs $f(\xtest)$ up to $\eps$ accuracy.
\end{theorem}
% \begin{lemma}[Filtering]\label{lem:filtering-app}
    
% \end{lemma}
% \begin{lemma}[Skills] Consider an input of the form
% \begin{equation}
%     \X = \begin{bmatrix}
%         \x_1 &\x_2 &\hdots &\x_n &\x\\
%         \s_{f_1} &\s_{f_2} &\hdots &\s_{f_n} &\s_k\\
%         \emb_1 &\emb_2 &\hdots &\emb_n &\emb_{n+1}
%     \end{bmatrix}
% \end{equation}
%  Then there exists a transformer $\TF$ with  five layers with output
%  \begin{equation}
%      \TF(\X) = \begin{bmatrix}
%          \one_{\{\s_{f_1} = \s_k\}}\x_1 &\one_{\{\s_{f_2} = \s_k\}}\x_2 &\hdots &\one_{\{\s_{f_n} = \s_k\}}\x_n &\x\\
%         \s_{f_1} &\s_{f_2} &\hdots &\s_{f_n} &\s_k\\
%         \emb_1 &\emb_2 &\hdots &\emb_n &\emb_{n+1}
%      \end{bmatrix}
%  \end{equation}
% \end{lemma}
% \begin{proof}
%     \begin{enumerate}
%         \item Use $\emb_i$ create one line that has everywhere $n+1$ like in lemma 1. 
%         \item Create the $\emb_{n+1}$ everywhere. 
%         \item Use this and the classic embeddings and copy everyehre the skill $\s_k$. 
%         \item Subtract the skill 
%     \end{enumerate}
%\end{proof}
% Our implementation of filtering is divided in two parts. In the first part we show how the filtering can be performed, given the appropriate encodings. In the second part we will show how we can perform some preprocessing to generalize this operation to any iteration, given always encodings of a specific form. The second part is to demonstrate that as it holds in practice we don't require to change the encodings to perform the filtering at each one of the iterations \AG{I will rephrase this}. 

% For the first lemma, we consider the more general setting in which the data are given in a possibly random order attached with an indicator vector that defines which is their actual position as explained in \AG{Mention the section in which we explain this setting.}
% \begin{lemma}
%     Assume that the input to a transformer after the embedding layer is of the following form 
%     \begin{equation}
%         \X = \begin{bmatrix}
%             \x_1&\x_2&\hdots &\x_{n-1}&\x_n\\
%             \emb_1 &\emb_2 &\hdots&\emb_{n-1} &\emb_n\\
%             \emb_{f_1}&\emb_{f_2}&\hdots &\zero &\zero\\
%             1 & 1 &\hdots & 0 & 0\\
%             \zero &\zero &\hdots &\zero &\zero\\
%             \zero &\zero &\hdots &\zero &\zero
%         \end{bmatrix}
%     \end{equation}
%     where $\x_i\in\R^{d'}$ $\emb_i$, $i=1,\hdots,n$ is the positional encoding as described in subsection \ref{sub:pencodings} for the $i$-th position and $\emb_{f_i}$, $i=1,\hdots, k$ is the encoding of the position we want to filter. If $k\leq n$ then we are given zeroes afterwards. Then there exists one layer of transformer $\TF$ such that 
%     \begin{equation}
%         \TF(\X) = \begin{bmatrix}
%             \x_1&\x_2&\hdots &\x_{n-1}&\x_n\\
%             \emb_1 &\emb_2 &\hdots&\emb_{n-1} &\emb_n\\
%             \emb_{f_1}&\emb_{f_2}&\hdots &\zero &\zero\\
%                         1 & 1 &\hdots & 0 & 0\\
%                         \zero &\zero &\hdots &\zero &\zero\\
%             \x_{f_1}&\x_{f_2}&\hdots &\zero &\zero
%         \end{bmatrix}
%     \end{equation}
% \end{lemma}
% \begin{proof}
% Notice that the dimension of the input is $d = 3d' + 2e $, where $e$ is the dimension of the positional encodings that the model has chosen. Let
%     \begin{equation}
%         \W_\key = \begin{bmatrix}
%             \zero_{d'} &
%             \Iden_{e} & \zero_{2d'+e}            
%         \end{bmatrix}, \W_\query = \begin{bmatrix}
%             \zero_{d'+e} &
%             \Iden_{e} & \zero_{2d'}            
%         \end{bmatrix}
%     \end{equation}
%     we have that 
%    \renewcommand{\arraystretch}{1.5}
%     \begin{align}
%     \arraycolsep=0.1pt
%         \sfm((\W_\key\X)^\top(\W_\query\X)) &= \sfm(\begin{bmatrix}
%             \emb_1^\top\emb_{f_1} &\emb_1^\top\emb_{f_2}&\hdots &\zero\\
%            \emb_2^\top\emb_{f_1} &\emb_2^\top\emb_{f_2}&\hdots &\zero\\
%            \vdots &\vdots &\ddots &\vdots\\
%            \emb_n^\top\emb_{f_1} &\emb_n^\top\emb_{f_2}&\hdots &\zero\\
%         \end{bmatrix})\\
%         &= \begin{bmatrix}
%             \dfrac{ \exp(\lambda\emb_1^\top\emb_{f_1})} {\sum_{i=1}^n\exp( \lambda\emb_i^\top\emb_{f_1})}&\hdots &\dfrac{1}{n}\\
%             \vdots &\hdots &\vdots \\
%              \dfrac{ \exp(\lambda\emb_n^\top\emb_{f_1})} {\sum_{i=1}^n\exp(\lambda \emb_i^\top\emb_{f_1})}&\hdots &\dfrac{1}{n}
%         \end{bmatrix}
%     \end{align}
%     Notice that for the columns that we had non-zeros the above matrix becomes a permutation matrix (as $\lambda\to\infty$ ) with $1$ at the $f_i$-th position of each column $i$. For example, for the first column we will have one in the $f_1$-th row. After this permutation of the identity matrix ( plus some error matrix, which can have arbitrarily small norm by tuning the temperature) is multiplied with $\X$ and by letting 
%     \begin{equation}
%         \W_\val = \begin{bmatrix}
%         \zero & \zero &\zero &\zero &\zero \\
%         \zero & \zero &\zero &\zero &\zero \\
%         \zero & \zero &\zero &\zero &\zero \\
%        \zero & \zero &\zero &\zero &\zero \\
%         \Iden_{d'} & \zero &\zero &\zero &\zero\\
%         \zero & \zero &\zero &\zero &\zero 
%     \end{bmatrix}
%     \end{equation}
%    Thus, the output of the attention becomes
%     \begin{align}
%         \attn(\X) &=  \begin{bmatrix}
%             \x_1&\x_2&\hdots &\x_{n-1}&\x_n\\
%             \emb_1 &\emb_2 &\hdots&\emb_{n-1} &\emb_n\\
%             \emb_{f_1}&\emb_{f_2}&\hdots &\zero &\zero\\
%                         1 & 1 &\hdots & 0 & 0\\
%             \x_{f_1}&\x_{f_2}&\hdots &* &*\\
%             \zero &\zero &\hdots &\zero &\zero 
%         \end{bmatrix}
%         \end{align}
%     where * denotes inconsequential values. We then use the ReLU layers to move the result in the last rows and substitute * with zeros. To do so we follow the construction of \cite{}; specifically we use the fourth row of ones and zeros, which indicates which columns should be updated and which not. For this we have that 
%     \begin{equation}
%         \TF(\X) = \X + \W_2\relu{\W_1\X}
%     \end{equation}
%     Then we set $\W_1, \W_2$ as to output zero in the first four set of rows. For the last set of rows we have \AG{Will add here the relu construction. But this proof is completed}... Thus,
%     \begin{equation}
%         \TF(\X) = \begin{bmatrix}
%             \x_1&\x_2&\hdots &\x_{n-1}&\x_n\\
%             \emb_1 &\emb_2 &\hdots&\emb_{n-1} &\emb_n\\
%             \emb_{f_1}&\emb_{f_2}&\hdots &\zero &\zero\\
%                         1 & 1 &\hdots & 0 & 0\\
%                         \zero &\zero &\hdots &\zero &\zero\\
%             \x_{f_1}&\x_{f_2}&\hdots &\zero &\zero
%         \end{bmatrix}
%     \end{equation}
%     and the proof is completed.
% \end{proof}







% We now continue to show how a transformer can predict 
% The following lemma states that transformers can implement the step of filtering. For simplicity we consider that we have just two intermediate steps and that  the model will predict the second step. It would be easy then to see that this construction can be generalized to multiple intermediate steps and implement a specific step each time depending on the given input.
% \begin{lemma} 

% \end{lemma}
% \begin{proof}
% We consider the following set-up: 
% The user gives an input of the form $\rmI = \begin{bmatrix}
%         \dpoint_1 &\prompt{1}{1} &\prompt{1}{2} \hdots &  \prompt{1}{\layer} &\hdots &\dpoint_n &\prompt{n}{1} &\hdots &\prompt{n}{\layer} &\dpoint_{\text{test}}
% \end{bmatrix}$.

% After the embedding layer the input is transformed as follows: 
%  \renewcommand{\arraystretch}{1.7}
% \begin{equation*}
% \arraycolsep=1.5pt
%    \rmI = \left[\begin{array}{*{11}c}
%     \dpoint_1 &\prompt{1}{1} &\prompt{1}{2}& \hdots &  \prompt{1}{\layer} &\hdots &\dpoint_n &\prompt{n}{1} &\hdots &\prompt{n}{\layer} &\dpoint_{\text{test}}\\
%     \zero &\zero &\zero&\hdots &\zero &\hdots &\zero &\zero &\hdots &\zero &\zero \\
%     \emb_0 &\emb_{L+1} &\emb_2 &\hdots &\emb_{\layer} &\hdots& \emb_{(n-1)(\layer + 1)+1} &\emb_{(n-1)(\layer+1)+ 2} &\hdots &\emb_{\seqlen-2}&\emb_{\seqlen-1}\\
%     \emb_0 & \emb_{\layer+1} &\emb_{2\layer+1} &\hdots & \emb_{f(\layer)}&\hdots& \emb_{f((n-1)(\layer + 1)+1)} & \emb_{f((n-1)(\layer+1)+ 2)}&\hdots &\emb_{f(\seqlen-1)}&\emb_{f(\seqlen)}\\
%      \text{!!!!} & \emb_{\layer+1} &\emb_{2\layer+1} &\hdots & \emb_{f(\layer)}&\hdots& \emb_{f((n-1)(\layer + 1)+1)} & \emb_{f((n-1)(\layer+1)+ 2)}&\hdots &\emb_{f(\seqlen-1)}&\emb_{f(\seqlen)}\\
%     1 & 2 &3&\hdots &\layer+1 &\hdots& (n-1)\layer + n &(n-1)\layer + n+1 &\hdots &\seqlen-1 &\seqlen\\ 
%      \ln(1) & \ln(2) & \ln(3)&\hdots &\ln(\layer+1) &\hdots& \ln((n-1)\layer + n) &\ln((n-1)\layer + n+1 )&\hdots &\ln(\seqlen-1) &\ln(\seqlen)\\ 
%      1 & 1 &1 &\hdots &1 &\hdots &1 &1 &\hdots &1 &1 \\ 
%      0 & 0&0&\hdots &0 &\hdots &0 &0 &\hdots &0 &0
%     \end{array} 
%     \right]
% \end{equation*}
% where $\seqlen$ is the sequence length, (write the function***)$f(x) =...$. Also, the second row is a block of rows set to zero, which will be used for storing necessary intermediate results.

% \noindent\textbf{Step 1: Extract the number of tokens.} Let 
% \begin{align}
% \weights_{\key}= \begin{bmatrix}
%     \zero &\zero &\zero &\zero &\zero &0 &1 &0 &0 
% \end{bmatrix} 
%  \;\;\; \weights_{\query} =  \begin{bmatrix}
%     \zero &\zero &\zero &\zero &\zero &0 &0 &1 &0 
% \end{bmatrix}
% \end{align}
% and thus 
% \begin{equation}
%     (\weights_{\key}\rmI)^\top(\weights_{\query}\rmI) = \begin{bmatrix}
%         \ln(1) &\ln(1) &\hdots &\ln(1)\\
%         \ln(2) &\ln(2) &\hdots &\ln(2)\\
%         \vdots &\vdots &\ddots &\vdots\\
%         \ln(\seqlen) &\ln(\seqlen) &\hdots &\ln(\seqlen)\\
%     \end{bmatrix}
% \end{equation}
% So after the softmax is applied we have
% \begin{equation}
%     \softmax((\weights_{\key}\rmI)^\top(\weights_{\query}\rmI)) = \begin{bmatrix}
%         \dfrac{1}{\sum_{i=1}^\seqlen i} &\dfrac{1}{\sum_{i=1}^\seqlen i}&\hdots &\dfrac{1}{\sum_{i=1}^\seqlen i}\\
%         \dfrac{2}{\sum_{i=1}^\seqlen i} &\dfrac{2}{\sum_{i=1}^\seqlen i} &\hdots &\dfrac{2}{\sum_{i=1}^\seqlen i}\\
%         \vdots &\vdots &\ddots &\vdots\\
%         \dfrac{\seqlen}{\sum_{i=1}^\seqlen i} &\dfrac{\seqlen}{\sum_{i=1}^\seqlen i}  &\hdots &\dfrac{\seqlen}{\sum_{i=1}^\seqlen i} \\
%     \end{bmatrix}
% \end{equation}
% We then set the weight value matrix as to zero-out all lines except for one line as follows
% \begin{equation}
%    \weights_{\val}\rmI =\begin{bmatrix}
%    \zero &\zero & \hdots &\zero \\
%     1 & 2 &\hdots &\seqlen\\
%  \zero &\zero &\hdots &\zero 
%    \end{bmatrix}
% \end{equation}
% % \begin{equation}
% %    \weights_{\val}\rmI =\begin{bmatrix}
% %    \zero &\zero & \hdots &\zero \\
% %   \zero &\zero & \hdots &\zero \\
% %     \zero &\zero & \hdots &\zero \\
% %     \zero &\zero & \hdots &\zero \\
% %     1 & 2 &\hdots &\seqlen\\
% %     0 &0 &\hdots &0\\
% %      0 &0 &\hdots &0\\
% %        0 &0 &\hdots &0
% %    \end{bmatrix}
% % \end{equation}
% After adding the residual this results to 
% \begin{equation*}
%     \arraycolsep=1.5pt
%    \rmI = \left[\begin{array}{*{11}c}
%     \dpoint_1 &\prompt{1}{1} &\prompt{1}{2}& \hdots &  \prompt{1}{\layer} &\hdots &\dpoint_n &\prompt{n}{1} &\hdots &\prompt{n}{\layer} &\dpoint_{\text{test}}\\
%     \zero &\zero &\zero&\hdots &\zero &\hdots &\zero &\zero &\hdots &\zero &\zero \\
%     \emb_0 &\emb_{1} &\emb_2 &\hdots &\emb_{\layer} &\hdots& \emb_{(n-1)(\layer + 1)+1} &\emb_{(n-1)(\layer+1)+ 2} &\hdots &\emb_{\seqlen-2}&\emb_{\seqlen-1}\\
%     \emb_0 & \emb_{\layer+1} &\emb_{2\layer+1} &\hdots & \emb_{f(\layer)}&\hdots& \emb_{f((n-1)(\layer + 1)+1)} & \emb_{f((n-1)(\layer+1)+ 2)}&\hdots &\emb_{f(\seqlen-1)}&\emb_{f(\seqlen)}\\
%      \text{!!!!} & \emb_{\layer+1} &\emb_{2\layer+1} &\hdots & \emb_{f(\layer)}&\hdots& \emb_{f((n-1)(\layer + 1)+1)} & \emb_{f((n-1)(\layer+1)+ 2)}&\hdots &\emb_{f(\seqlen-1)}&\emb_{f(\seqlen)}\\
%     \dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i} & \dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i} &\dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i}&\hdots &\dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i}&\hdots& \dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i}&\dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i} &\hdots &\dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i} &\dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i}\\ 
%      \ln(1) & \ln(2) & \ln(3)&\hdots &\ln(\layer+1) &\hdots& \ln((n-1)\layer + n) &\ln((n-1)\layer + n+1 )&\hdots &\ln(\seqlen-1) &\ln(\seqlen)\\ 
%      1 & 1 &1 &\hdots &1 &\hdots &1 &1 &\hdots &1 &1 \\ 
%      0 & 0&0&\hdots &0 &\hdots &0 &0 &\hdots &0 &0
%     \end{array} 
%     \right]
% \end{equation*}
% However, notice that $\dfrac{\sum_{i=1}^\seqlen i^2}{\sum_{i=1}^\seqlen i} = \dfrac{2\seqlen(\seqlen+1)(2\seqlen+1)}{6\seqlen(\seqlen+1)} = \dfrac{2\seqlen+1}{3}$. We then use the ReLU layer as to multiply with $3/2$ and subtract $1/3$ from this column. This results to 
% \begin{equation*}
%     \arraycolsep=1.5pt
%    \rmI = \left[\begin{array}{*{11}c}
%     \dpoint_1 &\prompt{1}{1} &\prompt{1}{2}& \hdots &  \prompt{1}{\layer} &\hdots &\dpoint_n &\prompt{n}{1} &\hdots &\prompt{n}{\layer} &\dpoint_{\text{test}}\\
%     \zero &\zero &\zero&\hdots &\zero &\hdots &\zero &\zero &\hdots &\zero &\zero \\
%     \emb_0 &\emb_{1} &\emb_2 &\hdots &\emb_{\layer} &\hdots& \emb_{(n-1)(\layer + 1)+1} &\emb_{(n-1)(\layer+1)+ 2} &\hdots &\emb_{\seqlen-2}&\emb_{\seqlen-1}\\
%     \emb_0 & \emb_{\layer+1} &\emb_{2\layer+1} &\hdots & \emb_{f(\layer)}&\hdots& \emb_{f((n-1)(\layer + 1)+1)} & \emb_{f((n-1)(\layer+1)+ 2)}&\hdots &\emb_{f(\seqlen-1)}&\emb_{f(\seqlen)}\\
%      \text{!!!!} & \emb_{\layer+1} &\emb_{2\layer+1} &\hdots & \emb_{f(\layer)}&\hdots& \emb_{f((n-1)(\layer + 1)+1)} & \emb_{f((n-1)(\layer+1)+ 2)}&\hdots &\emb_{f(\seqlen-1)}&\emb_{f(\seqlen)}\\
%     \seqlen&  \seqlen& \seqlen&\hdots & \seqlen&\hdots&  \seqlen& \seqlen &\hdots & \seqlen & \seqlen\\ 
%      \ln(1) & \ln(2) & \ln(3)&\hdots &\ln(\layer+1) &\hdots& \ln((n-1)\layer + n) &\ln((n-1)\layer + n+1 )&\hdots &\ln(\seqlen-1) &\ln(\seqlen)\\ 
%      1 & 1 &1 &\hdots &1 &\hdots &1 &1 &\hdots &1 &1 \\ 
%      0 & 0&0&\hdots &0 &\hdots &0 &0 &\hdots &0 &0
%     \end{array} 
%     \right]
% \end{equation*}
% \noindent\textbf{Step 2: Create the positional encodings for $\seqlen$.}
% This step is implemented by \textcolor{orange}{Lemma}. Now output is
% \begin{equation*}
%     \arraycolsep=1.5pt
%    \rmI = \left[\begin{array}{*{11}c}
%     \dpoint_1 &\prompt{1}{1} &\prompt{1}{2}& \hdots &  \prompt{1}{\layer} &\hdots &\dpoint_n &\prompt{n}{1} &\hdots &\prompt{n}{\layer} &\dpoint_{\text{test}}\\
%     \zero &\zero &\zero&\hdots &\zero &\hdots &\zero &\zero &\hdots &\zero &\zero \\
%     \emb_{\seqlen} &\emb_{\seqlen} &\emb_{\seqlen}&\hdots &\emb_{\seqlen} &\hdots &\emb_{\seqlen} &\emb_{\seqlen} &\hdots &\emb_{\seqlen} &\emb_{\seqlen} \\
%     \emb_0 &\emb_{1} &\emb_2 &\hdots &\emb_{\layer} &\hdots& \emb_{(n-1)(\layer + 1)+1} &\emb_{(n-1)(\layer+1)+ 2} &\hdots &\emb_{\seqlen-2}&\emb_{\seqlen-1}\\
%     \emb_0 & \emb_{\layer+1} &\emb_{2\layer+1} &\hdots & \emb_{f(\layer)}&\hdots& \emb_{f((n-1)(\layer + 1)+1)} & \emb_{f((n-1)(\layer+1)+ 2)}&\hdots &\emb_{f(\seqlen-1)}&\emb_{f(\seqlen)}\\
%      \text{!!!!} & \emb_{\layer+1} &\emb_{2\layer+1} &\hdots & \emb_{f(\layer)}&\hdots& \emb_{f((n-1)(\layer + 1)+1)} & \emb_{f((n-1)(\layer+1)+ 2)}&\hdots &\emb_{f(\seqlen-1)}&\emb_{f(\seqlen)}\\
%     \seqlen&  \seqlen& \seqlen&\hdots & \seqlen&\hdots&  \seqlen& \seqlen &\hdots & \seqlen & \seqlen\\ 
%      \ln(1) & \ln(2) & \ln(3)&\hdots &\ln(\layer+1) &\hdots& \ln((n-1)\layer + n) &\ln((n-1)\layer + n+1 )&\hdots &\ln(\seqlen-1) &\ln(\seqlen)\\ 
%      1 & 1 &1 &\hdots &1 &\hdots &1 &1 &\hdots &1 &1 \\ 
%      0 & 0&0&\hdots &0 &\hdots &0 &0 &\hdots &0 &0
%     \end{array} 
%     \right]
% \end{equation*}
% \textcolor{orange}{We need to create the encodings of max length.}
% \end{proof}

==> sec/exp.tex <==
\section{Experiments}
% \subsection{Experimental Setup}
In this section, we present our experiments to evaluate the expressiveness and effectiveness of ICL as compositional learning. Our main results are trained with GPT-2 models.

%Our main results are trained with GPT-2 models with different model sizes.: Small GPT-2, consisting of $6$ layers, $4$ attention heads, and $128$-dimensional embeddings; Tiny GPT-2, with half the layer, attention head, and embedding size; and Standard GPT-2, with double the number of those components. 

% \input{fig_sec/fig_largek}

\subsection{Compositional Learning of 2-layer ReLU Neural Networks}\label{sec:2nn}
To first evaluate the statistical benefit of ICL, we introduce 2-layer neural network experiments by comparing three different methods: $\ICL$, $\EXP$ and $\COT$. Here $\ICL$ follows the same setting as in \cite{garg2022can}, where prompts are given by input-output pairs (also see \eqref{icl pmt}). While $\EXP$ and $\COT$ admit chain-of-thought prompting and $\COT$ does chain-of-thought predictions as well (see \eqref{exp pmt} for $\EXP$ and \eqref{cot pmt} for $\COT$). 


% While the difference between  and Vanilla is that, Explanation has prompt formed by input-instruction-output. Therefore, Transformer can learn more by following the step-by-step messages. In addition to taking all step-messages as input, CoT also trains to predict each step so that the model performs as expected. 

\textbf{Dataset.} Consider 2-layer neural nets with input $\x\in\R^d$, hidden feature (1-step thought) $\tb\in\R^k$, and output $y\in\R$, where $\tb=(\W\x)_+$ and $y=\vv^\top\tb$. Here $\W\in\R^{k\times d}$, $\vv\in\R^{k}$, and $(\cdot)_+$ is the \texttt{ReLU} activation. Hence, the function is composed as $y=\vv^\top(\W\x)_+$ where $\W$, $\vv$ are the respective function parameters following i.i.d. Gaussian distribution, specifically, each entry of $\W$ is sampled via $\W_{ij}\sim\Nc(0,\frac{2}{k})$, and $\vv\sim\Nc(0,\Iden_k)$. Within each prompt, we also randomly sample inputs through $\x\sim\Nc(0,\Iden_d)$. To avoid the implicit bias due to distribution shift, both training and test datasets are generated following the same strategy.

In Figure~\ref{fig:diff gpt}, we train the same dataset with $d=10$ and $k=8$ over three different GPT-2 models: standard, small and tiny GPT-2. The small GPT-2 has $6$ layers, $4$ attention heads per layer and $128$ dimensional embeddings. While, standard GPT-2 contains twice of the layer number, attention heads and embedding dimension of small GPT-2 and tiny only contains half of each. Results show that small model is enough to solve the problem for $\COT$ (Fig.~\ref{fig:diff gpt cot}), while $\EXP$ requires standard GPT-2 model (Fig.~\ref{fig:diff gpt exp}), and $\ICL$ is not able to learn the model recovering the neural networks. It is because that to learn the problem in one shot, the model should be enough to represent all possible 2-layer neural networks and additionally, needs at least $O(dk+d)$ samples.

We then evaluate the three methods based on different neural net architectures (by varying neuron size $k$) and results are shown in Figure~\ref{fig:diff k}. All experiments are trained using small GPT-2, which contains $6$ layers, $4$ attention heads per layer and $128$ dimensional embedding, and blue, orange and green curves correspond to the hidden layer size $4$, $8$, and $16$ respectively. Fix $d=10$ and change neuron number $k\in\{4,8,16\}$. Results show that $\COT$ can learn the neural net using around $60$ samples for $k$ up to $16$ (Fig.~\ref{fig:diff k cot}), $\EXP$ can only learn the narrow neural network with $k=4$ (Fig.~\ref{fig:diff k exp}), and $\ICL$ is not able to learn the networks given $100$ samples (Fig.~\ref{fig:diff k icl}). Following the same setting, Figure~\ref{fig:k16} shows the result when $k=16$. This validates the approximation benefits of CoT prompts and predictions. 

We also observe that there exist alignments in Figure~\ref{fig:diff k cot}, which means $\COT$ needs the same number of sample to learn the given three neural width. The interpretation is that, $\COT$ treats the problem as $k$ $d$-dimensional and $1$ $k$-dimensional linear regression problems and solves them in parallel. Therefore, solving the problem requires $O(\max{(k,d)})$ samples. The evidence in Fig.~\ref{fig:diff k cot} dues from the fact that the data dimension $d$ dominates the problem. To further verify our explanation, in Figure~\ref{fig:cot_d10_vs_d20}, we repeat the $\COT$ experiments but with $d=20$. Dashed curves are showing $d=20$ results with the same $k$ choices. Fig.~\ref{fig:cot_d10_vs_d20_align} shows the alignment in Fig.~\ref{fig:cot_d10_vs_d20}, where $x$-axis is valued by $n/d$ where $n$ is the sample size, which shows that for $d=20$, $\COT$ needs exact two times more samples to learn the neural network compared to $d=10$. What's more in Fig.~\ref{fig:largek}, we tried with larger $k$ so that hidden dimension size $k$ turns to dominate the problem. Fig.~\ref{fig:largek compose} shows the composed CoT risk where $\TF$ first generates \emph{thought} prediction $\hat\tb$, and feeding it back to the model results in the final prediction $\hat y$. While in Fig.~\ref{fig:largek first}, losses are calculated by $\|\tb-\hat\tb\|^2$, and to get the second layer risk in Fig.~\ref{fig:largek second}, we feed toe model with the oracle \emph{thought} $\tb$ and the model only needs to learn the last linear function. To clearer compare their performance, we plot the first risks of $k=4,16$ (dotted) and second layer risk of $k=64$ (dashed) in Fig.~\ref{fig:largek second}. The alignments again verifies our statement that to learn a 2-layer neural network with $d$ input dimension and $k$ neurons, CoT needs exact $O(\max(k,d))$ samples. 

\red{MORE EXPERIMENTS TO DISCUSS:
\begin{itemize}
    \item feed the output of second with zeros/random, and test the filtering observation of first-layer prediction
    \item separately first/second layer predictions are aligned with linear regression problem
\end{itemize}
}

% ----------------------------------

% Comparing $\EXP$ with $\ICL$ shows that, CoT prompt helps in reducing sample size needed in learning the neural network, and $\COT$ achieves the best performance verifies the benefit of step-by-step predictions.


% We evaluate our results based on different neural net architectures (by varying neuron size $k$) and transformer models. 
% ---------------------------

% $\bullet$ \textbf{Vanilla:} $\X_{it}=(\x_{i1},y_{i1},\x_{i2},y_{i2},\cdots,\x_{it})$ and $\y_{it}=y_{it}$.\\
% $\bullet$ \textbf{Explanation: }$\X_{it}=(\x_{i1},\eb_{i1},y_{i1},\x_{i2},\eb_{i2},y_{i2},\cdots,\x_{it},\eb_{it})$ and $\y_{it}=y_{it}$.\\
% $\bullet$ \textbf{CoT: }Different to Vanilla and Explanation, CoT needs to predict both $\eb$ and $y$. Therefore its dataset has two forms: $\X_{it}=(\x_{i1},\eb_{i1},y_{i1},\x_{i2},\eb_{i2},y_{i2},\cdots,\x_{it})$ and $\y_{it}=\eb_{it}$; while $\X'_{it}= (\X_{it},\eb_{it})$ and $\y'_{it}=y_{it}$.

% Treat each sequence as a task, that it, $\W_1,\W_2$ are the same within a sequence, and we randomly sample $n$ tasks as $\W_1,\W_2\sim\Nc(0,1)$.



% the raw input and final prediction in prompt contains all the step message (in neural network, the step messages are the intermediate features). Comparing Explanation with Vanilla shows that ...

% What's more, as for CoT, in addition to feeding all the step messages as prompt, the model also outputs each step following the instruction. The comparison of the three methods are given in Figure~\ref{}.

% % \input{fig_sec/fig_skill}

\subsection{Deep Linear Neural Networks}
In Section~\ref{sec:2nn}, we have discussed the approximation benefit of CoT and how it in-context learns 2-layer ReLU neural network as compositional learns two linear regression problems. In the section, we investigate the ability of CoT in compositional learning long novel chains. In the following, for cleaner notation, we use CoT to refer to $\COT$. 

\textbf{Dataset. } Consider a $L$-layer linear neural nets with input $\x\in\R^d\sim\Nc(0,\Iden_d)$, and output is generated by $\y=\W_L(\W_{L-1}\cdots\W_1(\x))$, where $\W_\ell\in\R^{d\times d}$, $\ell\in[L]$. In this work, we assume each layer is parameterized from the same function set $\Wc=\{\bar\W_k:\bar\W_k^\top\bar\W_k=\Iden,k\in[K]\}$. Therefore to learn the $L$-layer neural net, CoT only needs to learn $\Wc$ whereas $\ICL$ needs to learn function set $\Wc^{L}$, which contains $K^L$ random matrices. 



\subsection{Heterogeneous CoT Prompting}


----------------------------------------------

 and let $\widehat\TF$ be the trained model weighted by $\hat\bt$ from \eqref{erm}. Then the CoT test risk can be defined as 
\begin{align}
    \Lc^{\text{CoT-I}}(\hat\bt,n)=&\E_{\{\x_i\}_{i=1}^n,\f}\left[\ell(\hat\y_n,\y_n)\right]~~~~\text{where}~~~~\hat\y_n=\widehat\TF(\pmt_n(\f),\x_n)
\end{align}
\begin{align}
    \Lc^{\text{CoT-I/O}}(\hat\bt,n)=&\E_{\{\x_i\}_{i=1}^n,\f}\left[\ell(\hat\y_n,\y_n)\right]\\
    \text{where}~~~~&\hat\tb_n^1=\widehat\TF(\pmt_n(\f),\x_n)\\
    &\hat\tb_n^\ell=\widehat\TF(\pmt_n(\f),\x_n,\hat\tb_n^1\cdots,\hat\tb_n^{\ell-1}),~\ell\in[L]
\end{align}

==> sec/experiment_setup.tex <==
\subsection{Experimental setting}


% (we might want to call this a \emph{session} instead?)
\noindent\textbf{Prompt structure:} Each prompt pmt is obtained by concatenating chains i.e.~$pmt=(chn1~chn2~\dots)$. Each chain $chn$ has the following form:
\[
chn=(x_1,s_1,x_2,s_2,\dots,x_{n+1},s_{\text{stop}}).
\]
Here $x_i$ are the features and $s_i$ are the skills. The only requirement is that a chain has to end with $s_{\text{stop}}$.

%distribution $D_i$ over a 
\noindent\textbf{What skills do:} Each skill $s_i$ is associated to a function class $F_i$: Skill $s_i$ means we will apply some $f\in F_i$ on the input. Thus, during training, all triples $(x_i,s_i,x_{i+1})$ satisfy $x_{i+1}=f(x_i)$ where $f\in F_i$. We can call these functions \emph{skill repertoire} (or subskill?). We will later learn these functions in-context because, given $s_i$, it is not clear which function to apply. So training chains have the form
\[
chn=(x,s_1,f^{s_1}(x),f^{s_{1:2}}(x),\dots,f^{s_{1:n}}(x),s_{\text{stop}}).
\]

\noindent\textbf{Example skills to kickstart experiments:} I think each skill $s_i$ can do a matrix multiplication and ReLU nonlinearity (honestly we can even avoid ReLU initially). So imagine for each $F_i$, we generate $1\leq k\leq 10$ random matrices $(W_{ij})_{j=1}^k$ of size $d\times d$ (with $d\leq 5$?) with proper normalization. Then $f_i=(W_{ij}x)_+$.

Important thing here is that each skill has access to their own unique matrices. So it is not simply learning matmul. It is learning exact weights so skill ID matters. Also for skills with $k=1$, skill ID uniquely determines the function so no function learning is needed during ICL time.\footnote{On the other hand, when $k=\infty$, then we have to select from a rich set of functions by learning a continuous ERM algorithm.}
%linear regression (or more generally 

Training involves two datasets. The main goal is to make it so that training process only involves basic learning elements but that basic stuff should suffice to do complex compositional learning.\\

\noindent\textbf{Dataset 1: Learning skills:} Consider all $(i,j)$ pairs where $i$ is the skill ID and $j$ is the subskill ID. We create many prompts with the following rules:
\begin{itemize}
\item All $(i,j)$ pairs should appear in the training data (e.g.~equally likely).
\item Throughout the same prompt, skill $i$ always uses the same subskill/function $f_j^i$. This way transformer will learn $f_j^i$ functions and get to call them in-context.
\item \textbf{Input distribution:} We want to train skill $i$ always with the same input distribution we will use in CoT. This is not difficult for the neural net model above because with He-initialization all other layers except the input should have the same distribution. So we can as well train the skill for both distributions?
\item \textbf{(To discuss)} $(x,i,f_j^i(x))$ tuples should ideally be randomly located throughout the prompt. This way transformer will be less likely to get confused during test-time CoT. Note that within the same prompt, it is totally OK to have many other $(i',j')$ pairs and many chains of varying lengths.
%In other words, use same subskill
\end{itemize}

\noindent\textbf{Remark:} I consider the above dataset to be \emph{clean} in the sense that a skill $i$ uses the same subskill throughout so there is no \emph{noise} when learning which subskill to call. This will be helpful for our CoT to work smoothly. Our next goal is creating a clean dataset for skill prediction.
%$f_j^i$ where $i$ is the skill ID and $j$ is the subskill ID. We create

\smallskip\smallskip
\noindent\textbf{Dataset 2: Predicting skills.} The previous dataset aimed to answer $(x,s_i,?)$. This dataset aims to answer $(s_{i-1},x,?)$. The idea is learning the transition purely based on the previous skill $s_{i-1}$. We generate arbitrary admissable prompts with the following rules
\begin{itemize}
\item Suppose $(i,j)$ are all feasible skill pairs where $j$ can follow $i$. More generally, we can assume skill pairs is a graph (perhaps some skills can't follow another). In that case $j$ is a neighbor of $i$. All feasible $(i,j)$ pairs should appear in the training data.
\item First $n/2$ tokens in the prompt can be arbitrary (which will lie within the prefix demonstrations for the CoT). However, in the second $n/2$ half of the prompt, the skill that follows $i$ should always be based on majority rule. For instance if first half contains $(i,1),(i,2),(i,1)$ pairs, then for the rest of the prompt $1$ is the skill that follows $i$. 
\item Note that prompt can contain many skills besides $i$. Also it is OK to make the data noiseless in the sense that $i$ is always followed by the same skill. However this would make our prompts less realistic.
\item \textbf{(To discuss)} We need to decide whether $s_{stop}$ skill uses the majority rule as well. Because if it does, then after $n/2$ all chains will have to be same making the prompt model less realistic.
\end{itemize}

\smallskip\smallskip
\noindent\textbf{Test Dataset for CoT:} We would like CoT to work without showing the exact skill sequence and for arbitrarily many skills. We engineer the CoT prompt backwards.

Suppose we would like the following CoT chain to succeed:
\[
(x_1,s_1,x_2,\dots, s_n,x_{n+1},s_{\text{stop}})
\]
after only seeing $(x_1)$.
%\footnote{In general we only need to see $(x_1)$ as long as $x_1$ the input distribution is always followed by the prompt $s_1$ during training.} 
Here is how:
\begin{enumerate}
\item The model moves to the correct skill $s_1$ because in the prefix $s_1$ follows $s_{stop}$ majority of the times $s_{stop}$ appears. Similarly correct $s_2$ will follow $s_1$ based on the prefix appearances of $s_1$.
\item The model outputs $f^{s_1}_{j_1}(x_1)$ correctly because prefix prompt always uses subskill $j_1$ for $s_1$.
\item Repeat this argument until seeing $s_{stop}$.
\item \textbf{(To discuss)} If $s_{stop}$ does not follow the majority rule described above, then we have 2 options: We either have to specify $(x_1,s_1)$ to start the CoT or we have to infer $s_1$ from distribution of $x$. The latter can be done by partitioning the input space so that each starter skill $s_1$ can be uniquely distinguished from its input.
\end{enumerate}

\noindent\textbf{Remark:} Note that in order to create a chain of length $10$, we only need 10 short chains of size $2$. We just need to show instances of $s_i\rightarrow s_{i+1}$ but those instances can be different input features.

==> sec/filtering.tex <==
As we mentioned in Subsection \ref{subsec cot}, we would expect \AG{Add here that we want to see why ICL-IO performs better and evaluate our intuition and observation of previous setting. To do so we extend it to deep NN and observe again }

\paragraph{Dataset. }

\paragraph{Filtering. }We speculated that this behavior is due to a filtering step. RESULTS and figures.


\paragraph{Construction of the filtering process. }To demonstrate that it is indeed possible for a transformer to perform a filtering process we explicitly construct..

==> sec/functions.tex <==

In this section, we demonstrate how to implement a variety of nonlinear functions and basic linear algebra operations using transformers. These techniques will be crucial in the construction of iterative algorithms in the following sections. %We will show how to use transformer function blocks to implement non-linear sigmoid based functions, and basic matrix operations. 
Each transformer-based function block in this section fits in our unified template in terms of input/output parameters' locations. We note here that each transformer-based function block might have its own positional encodings used to transfer the output in the correct place or perform some \texttt{read/write} operations and they are part of the design of the block.


\subsection{Encoding Non-linear Functions within the Attention Mechanism}%\label{ss:sigmoids}
One key ingredient of our constructions %demonstrate how to emulate 
is encoding various functions within the attention mechanism. We do this by forcing the softmax to act as a sigmoid function and by storing multiple coefficients in the query and value weight matrices. As far as we know, this is the first work that shows how general non-linear functions can be emulated by attention layers. This allows us to create linear combinations of sigmoids that can be accessed by an indicator vector in the input. Our analysis is based on the result of \cite{Barron93} which we present below. 

\begin{definition} Let $\Gamma_{C,B}$ be the set of functions defined in a bounded domain $B$, $f:B\to \mathbb{R}, B\subseteq \R^d$ with a proper extension to $\R^d$ such that they have $C$ bounded Fourier integral, \ie \\$\int \sup_{x \in B} | w \cdot x | \ F(dw) \le C$ holds where $F(dw)$ is the magnitude of the Fourier distribution.
%\jnote{is bounded fourier integral clear? It's like the $\| \hat f\|_1$?}
\end{definition}
\begin{definition} Given $\tau >0, C>0$ and a bounded set $B$, 
    let 
    \begin{equation}
        G_{\sigmoid,\tau} = \braces{\gamma\sigmoid(\tau(\rva^T\rvx + b)): \abs{\gamma}\leq 2C,\norm{\rva}_B \leq 1, \abs{b} \leq 1} \nonumber
    \end{equation}
    where $\norm{\rva}_B = \sup_{\rvx\in B} \braces{\rvx^T\rva}$ and $\sigmoid$ is the sigmoid function, \ie $\sigmoid(x) =\frac{1}{1+e^{-x}}$.
\end{definition}
\begin{theorem}[Theorem 3 in \cite{Barron93}]\label{th:Barron}
Every function $f\in\Gamma_{C,B}$ with $f(0) =0 $ and  can be approximated by a linear  combination of sigmoids $f_i\in G_{\sigmoid,\tau}$, $i=1,\hdots m$. If $\tau \geq m^{1/2}\ln m$  the  error scales as
\begin{equation}
    \abs*{f(\rvx) - \sum_{i=1}^m f_i(\rvx)}\leq O\parens*{\dfrac{1}{m^{{1/2}}}} , \; \rvx\in B \nonumber
\end{equation}
\end{theorem}

To encode $N$ different functions, we use the index $j\in[N]$ and write $c_{ji},\rva_{ji}$ for the coefficients of the sigmoids that approximate them or 

\begin{equation}
    f_j(\rvx) = \sum_{i=1}^m c_{ji} \sigmoid( \rvx^T\rva_{ji}) \text{ for }j = 1,\hdots,N \nonumber
\end{equation}
We here note that the terms $\tau, b$ can be incorporated in the term $\rva_{ij}$ by adding an extra coefficient of $1$ in $\rvx$ and multiplying everything with $\tau$.

We are now able to present the lemma on approximating functions using transformer blocks, in a format that is consistent with the FLEQ design outlined in the previous section.

\begin{lemma}\label{lem:sigmoids}
Fix $\epsilon>0$ and consider an input of the form 
\begin{equation}
    \Input = \bracks*{ \begin{array}{cc|cc|cc}
        \ve & \zero&\rvx&\zero &\zero &\zero \\%&\zero\\
        \zero  &\zero & \zero& \zero &\zero&\zero\\
        \zero &\zero &\emb_{2d+1} &\zero &\zero &\zero\\
        \emb_1&\emb_{2:d}&\zero&\emb_{d+2:2d} &\emb_{2d+1} &\emb_{2d+2:3d}\\
        0 & 0_{2:d} & 1 & 0_{d+2:2d} & 0 & 0_{2d+2:3d}
    \end{array}} . \nonumber
\end{equation}
where $d$ is chosen according to the \texttt{FLEQ} construction from the previous section and $N$ is the number of functions we encode . $\ve = \rve_j\in\R^N$ is an indicator vector signifying the function we wish to execute.  Then there  exists a   transformer-based function block with 3 layers, $m$ heads and dimensionality $r = 2\log(d) +d+1 = O(d)$ such that  \begin{equation}
    f(\Input) =  \bracks*{ \begin{array}{cc|cc|cc}
        *&*&*&*&\sum_{i=1}^m c_{ji}\sigmoid(\rvx^T\rva_{ji}) +\epsilon & *\\
        \zero  &\zero & \rvx& \zero &\zero&\zero\\
         \zero &\zero &\emb_{2d+1} &\zero &\zero &\zero\\
       \emb_1&\emb_{2:d}&\zero&\emb_{d+2:2d} &\emb_{2d+1} &\emb_{2d+2:3d}\\
        0 & 0_{2:d} & 1 & 0_{d+2:2d} & 0 & 0_{2d+2:3d}
    \end{array} }\nonumber
\end{equation}
where $*$ denoted inconsequential values that will be ignored downstream. This implies that arbitrary function $g \in \Gamma_{C,B}$ can be well approximated by attention layers. 
\end{lemma}
\begin{remark}
Notice that in this case we don't use any extra scratchpad space and thus $s=3d$; however if this function block was to be used with another one that needs $s>3d$ scratchpad space, we would simply zero pad the input of \cref{lem:sigmoids} and ignore these columns. The same holds for the rest of the transformer-based function blocks and we will not mention it from now on. 
\end{remark}

In the expression $\sum_{i=1}^m c_{ji}\sigmoid(\rvx^T\rva_{ji})$, the number head is equal to the number of terms we need.%is equal to the number of heads $m$. 
We show in the appendix that we can actually encode these $m$ terms in the dimension of the transformer architecture with just one head (See \cref{cor:lem_5_alt}). %the number of terms can also scale proportional to the dimension $d$ in \cref{cor:lem_5_alt}. 
The choice of which result to use can depend on the specific design and can affect both accuracy and efficiency of the implemented transformer network.

The proof of this Lemma is given in \cref{app:functions}.
% %We note that the first layer will create the value $\sum_{i=1}^m c_{ji}\sigmoid(\rvx^T\rva_{ji})$ similarly to the proof of \cref{lem:sigmoids}, while the second layer will use the \cref{lem:write} to place the value in the desired position.
% %; a formal proof is given in \cref{app:functions}.
% %\cref{app:functions}.
% \begin{proof} 
% The first thing we do is to move the $\rvx$ to the second row block, as follows:
% \begin{equation*}
%     \Input = \begin{bmatrix}
%         \ve & \zero&\rvx &\zero &\zero &\zero\\
%         \zero  &\zero & \zero& \zero &\zero&\zero\\
%         \zero &\zero &\emb_{2d+1} &\zero &\zero &\zero\\
%         \emb_1&\emb_{2:d}&\zero&\emb_{d+2:2d} &\emb_{2d+1} &\emb_{2d+2:3d}\\
%         0 & 0_{2:d} & 1 & 0_{d+2:2d} & 0 & 0_{2d+2:3d}
%     \end{bmatrix} \to \begin{bmatrix}
%         \ve & \zero&\zero &\zero &\zero &\zero\\
%         \zero  &\zero & \rvx & \zero &\zero&\zero\\
%         \zero &\zero &\emb_{2d+1} &\zero &\zero &\zero\\
%         \emb_1&\emb_{2:d}&\zero&\emb_{d+2:2d} &\emb_{2d+1} &\emb_{2d+2:3d}\\
%         0 & 0_{2:d} & 1 & 0_{d+2:2d} & 0 & 0_{2d+2:3d}
%     \end{bmatrix}
% \end{equation*}
% This can be done using a ReLU feedforward layer that performs this using the last row of the input as the indicator bit for the column containing $\dpoint$.

% Then we want to create the following transformation
% \begin{equation*}
%     \begin{bmatrix}
%         \ve & \zero&\zero &\zero &\zero &\zero\\
%         \zero  &\zero & \rvx& \zero &\zero&\zero\\
%         \zero &\zero &\emb_{2d+1} &\zero &\zero &\zero\\
%         \emb_1&\emb_{2:d}&\zero&\emb_{d+2:2d} &\emb_{2d+1} &\emb_{2d+2:3d}\\
%          0 & 0_{2:d} & 1 & 0_{d+2:2d} & 0 & 0_{2d+2:3d}
%     \end{bmatrix} \xrightarrow[]{} \begin{bmatrix}
%         *&*&*&*&\sum_{i=1}^m c_{ji}\sigmoid(\rvx^T\rva_{ji}) & *\\
%         \zero  &\zero & \rvx& \zero &\zero&\zero\\
%          \zero &\zero &\emb_{2d+1} &\zero &\zero &\zero\\
%       \emb_1&\emb_{2:d}&\zero&\emb_{d+2:2d} &\emb_{2d+1} &\emb_{2d+2:3d}\\
%         0 & 0_{2:d} & 1 & 0_{d+2:2d} & 0 & 0_{2d+2:3d}
%     \end{bmatrix}
% \end{equation*}
% The proof follows that of \cref{lem:sigmoids}. We again ignore the last three rows by setting the corresponding rows in the key, query and values weight matrices to be zero. Let 
% \begin{equation}
%          \query^{i} = \begin{bmatrix}
%          \zero &\id_d\\
%          \zero &\zero 
%      \end{bmatrix}, \key^i = \begin{bmatrix}
%          [\rva_{1i} \; \hdots \; \rva_{Ni}] & \zero\\
%          \zero &\zero
%      \end{bmatrix} , \val^i = \begin{bmatrix}
%         [c_{1i} \;\hdots \; c_{Ni}] &\zero \\
%         \zero  &\zero
%      \end{bmatrix} \nonumber
% \end{equation}
% We note that for the purpose of this proof, each $\rva_i$ has one extra element at the end equal to $-\log(3d-1)$, while the vectors $\rvx$ will have the last element equal to one. Then we will have
% \begin{align*}
%     \softmax((\key^i\Input)^T(\query^i\Input)) &= \begin{bmatrix}
% \rva_{ji}^\top & \zero \\ 
% \zero  & \zero  \\ 
% \zero  & \zero  \\ 
% \zero  & \zero  \\ 
% \zero  & \zero  \\ 
% \zero  & \zero  \\ 
% \end{bmatrix}\begin{bmatrix}
% \zero &\zero &\rvx &\zero &\zero &\zero\\
% \zero &\zero &\zero &\zero &\zero &\zero\\
% \end{bmatrix}\\
% &= \begin{bmatrix}
%     \zero &\zero &\rva_{ji}^\top\rvx&\zero &\zero &\zero\\
%     \zero &\zero &\zero &\zero &\zero &\zero\\
%     \zero &\zero &\zero &\zero &\zero &\zero\\
%     \zero &\zero &\zero &\zero &\zero &\zero\\
%     \zero &\zero &\zero &\zero &\zero &\zero\\
%     \zero &\zero &\zero &\zero &\zero &\zero\\
% \end{bmatrix}\\
%     &=\begin{bmatrix}
% * & * &\sigmoid(\rvx^T\rva_{ji}) & * & *   &*\\ 
% * & * &*  & * & * &*\\ 
% * & * &*  & * & * &*\\ 
% * & * &*  & * & * &*\\ 
% * & * &*  & * & * &*\\ 
% * & * &*  & * & * &*\\ 
% \end{bmatrix}
% \end{align*}
% since $\rva_{ji}^\top\rvx = \rva_{ji}^\top\rvx -\log{3d-1}$ and thus $\exp^{\rva_{ji}^\top\rvx}/(3d-1 + \exp^{\rva_{ji}^\top\rvx}) = \sigmoid(\rva_{ji}^\top\rvx)$ with a slight abuse of notation over the inner product $\rva_{ji}^\top\rvx$ to account for the extra corrections bias term. Thus, 
% \begin{equation}
%  \val\Input\softmax( (\key\Input)^T(\query\Input) ) = \begin{bmatrix}
%  * & * &c_{ji}\sigmoid(\rvx^T\rva_{ji}) & * & *   &*\\
%   \zero &\zero &\zero &\zero &\zero &\zero\\
%     \zero &\zero &\zero &\zero &\zero &\zero\\
%     \zero &\zero &\zero &\zero &\zero &\zero\\
%     \zero &\zero &\zero &\zero &\zero &\zero\\
%  \end{bmatrix} \nonumber
% \end{equation}
% By summing over all heads and adding the residual we get
% \begin{equation}
%     \begin{bmatrix}
%         *&*&\sum_{i=1}^m c_{ji}\sigmoid(\rvx^T\rva_{ji})&*&* & *\\
%         \zero  &\zero & \rvx& \zero &\zero&\zero\\
%          \zero &\zero &\emb_{2d+1} &\zero &\zero &\zero\\
%       \emb_1&\emb_{2:d}&\zero&\emb_{d+2:2d} &\emb_{2d+1} &\emb_{2d+2:3d}\\
%         0 & 0_{2:d} & 1 & 0_{d+2:2d} & 0 & 0_{2d+2:3d}
%     \end{bmatrix} \nonumber
% \end{equation}
% Finally, we use an extra layer similarly to \cref{lem:write} to write the result in the desired output. Hence, we get
% \begin{equation}
%     \begin{bmatrix}
%         *&*&*&*&\sum_{i=1}^m c_{ji}\sigmoid(\rvx^T\rva_{ji}) & *\\
%         \zero  &\zero & \rvx& \zero &\zero&\zero\\
%          \zero &\zero &\emb_{2d+1} &\zero &\zero &\zero\\
%       \emb_1&\emb_{2:d}&\zero&\emb_{d+2:2d} &\emb_{2d+1} &\emb_{2d+2:3d}\\
%         0 & 0_{2:d} & 1 & 0_{d+2:2d} & 0 & 0_{2d+2:3d}
%     \end{bmatrix} \nonumber
% \end{equation} 
% \end{proof}



\subsection{Matrix Transposition and Multiplication by Linearizing the Softmax}
We assume that a $d\times d$ matrix $\rmA$ in the input $\Input$ is represented by a sequence of length $d$, and each of these $d$ columns  has $d$ rows. %of $\Input$ contains one column of $\rmA$. 
While this representation has the advantage that it is well suited for the matrix multiplication operation (as we will see in the next sub-section), a vectorized form of the matrix is more suited to create transpose. This is how we implement the transpose; we first vectorize the matrix $\rmA$, then with a fixed permutation of the columns we create its vectorized version of a transpose.

% Two important components of linear algebra are matrix multiplication and transposition. We now show that a matrix can be stored in two forms in the transformer input, and each has an advantage for one of these operations.
\begin{lemma}\label{lem:transpose}
Fix $\epsilon >0$ and consider an input of the following form
\begin{equation}
    \Input = \left[\begin{array}{c|c|c|cc}
        \rmA  &\zero&\zero &\dots & \zero \\
 \zero&      \zero&\zero &\dots & \zero\\
         \emb_{1:d}&\emb_{1:d}&\emb_{1:d}& \dots  &\emb_{1:d}\\
         \rmP_1'&\rmP_{2}'&\rmP_{3}'& \dots  &\rmP_{d}'
    \end{array}\right]. \nonumber
\end{equation}
where $\rmA\in\R^{d\times d}$; then there exists transformer-based function block with 4 layers, 1 head and dimensionality $r = 2d+2\log d = O(d)$ that outputs the following matrix
\begin{equation}
    \Input = \left[\begin{array}{c|c|c|cc}
\rmA' &\rmA'&\rmA'&\dots &\rmA' \\
        \zero&\zero&\zero &\dots &\zero \\
         \emb_{1:d}& \emb_{1:d}& \emb_{1:d}& \dots &\emb_{1:d} \\
        \rmP_1'&\rmP_{2}'&\rmP_{3}'& \dots  &\rmP_{d}'
    \end{array}\right]. \nonumber
\end{equation}
where $\rmA' = \rmA^\top +\epsilon\rmM$, for some $\norm{\rmM}\leq 1$. The error $\epsilon$ depends on the choice of the temperature $\lambda$, as it is  a consequence of the \texttt{read/write} operations.
\end{lemma}
% \begin{lemma}\label{lem:transpose}
% Let the input of the transformer-based function block to be
% \begin{equation}
%     \Input = \left[\begin{array}{cccc|c|c}
%         \rmA  &\zero&\dots & \zero &\zero  \\
%  \zero&      \zero&\dots & \zero \\
%          \emb_{1:m}&\emb_{1:m}& \dots  &\emb_{1:m}\\
%          \rmP_1'&\rmP_{2}'& \dots  &\rmP_{m}'\\
%          \zero &\rvOne^\top &\dots&\rvOne^\top 
%     \end{array}\right]. \nonumber
% \end{equation}
% where $\rmA\in\R^{k\times m}, m\geq k$, the total number of columns is $m^2$ and $\embed_i^{'} = [\emb_i \dots \emb_i] $ for all $i=1,\dots,m$. Then,
% there  exists a transformer-based function block with 4 layers, 1 head and dimensionality $O(k+\log m)$ that has as output the following matrix
% \begin{equation}
%     \Input = \left[\begin{array}{cc|c}
% \rmA^\top &\dots &\rmA^\top \\
%         \zero &\dots &\zero \\
%          \emb_{1:m}& \dots &\emb_{1:m} \\
%          \embed_1'& \dots &\embed_{m}' 
%     \end{array}\right]. \nonumber
% \end{equation}
% \end{lemma}
% Notice that this form fits in our unified template, with the first $d = \dfrac{m^2-m}{2} $
% \proof
% We can vectorize the matrix $\rmA$ into a $d^2$ dimensional vector using the attention mechanism, as shown in Eq. \eqref{eq:vectorized_matrix}. 
% Notice that once we have the matrix in this form we can implement its transpose with a fixed permutation of the columns of the matrix to get the vectorized form of $\rmA^\top$. Once we have the transpose in vector form, we matricize it back to get the matrix transform using the attention mechanism. We explain the details of this process below:

% \emph{Vectorization: } We assume that the input is of the following form, where $\rmA$ is the matrix to be vectorized.
% % \begin{equation}
% %     \Input = \left[\begin{array}{ccc|c}
% % \zero &\dots &\zero &\zero\\
% %         \zero &\dots &\zero & \rmA\\
% %          \emb_{1:d}& \dots &\emb_{1:d} &\emb_{1:d}\\
% %          \emb_1'& \dots &\emb_{d}' &\emb_{d+1}'
% %     \end{array}\right].
% % \end{equation}
% \begin{equation}
%     \Input = \left[\begin{array}{cccc}
%         \rmA  &\zero&\dots & \zero\\
%  \zero&      \zero&\dots & \zero\\
%          \emb_{1:d}&\emb_{1:d}& \dots  &\emb_{1:d}\\
%          \rmP_1'&\rmP_{2}'& \dots  &\rmP_{d}'
%     \end{array}\right]. \nonumber
% \end{equation}
% Here, $\rmP_i'$ represents a matrix of $d$ columns, where each column is $\emb_i$.

% % \begin{equation}
% %     \Input = \left[\begin{array}{c|c}
% %          \rmS & \zero \\
% %         \zero & \rmA\\
% %         \zero &\emb_{d^2+1:d^2+d}\\
% %          \emb_{1:d} &\zero\\
% %          \emb_{1:d^2} &\emb_{d^2+1:d^2+d}
% %     \end{array}\right]
% % \end{equation}
% %The attention mechanism 
% The first layer uses the $\emb_{1:d}$ encodings to make $d$ copies of the matrix $\rmA$, as follows:
% \begin{equation}
%     \Input = \left[\begin{array}{cccc}
% \rmA&\zero &\dots &\zero \\
%  \rmA &\rmA&\dots & \rmA\\
%          \emb_{1:d}&\emb_{1:d}& \dots &\emb_{1:d} \\
%          \emb_1'&\emb_2'& \dots &\emb_{d}' 
%     \end{array}\right]. \nonumber
% \end{equation}


% The feed forward part of the second layer then uses the encodings $\emb_i'$ to vectorize the matrix in the second row block as follows:

% \begin{equation}
%     \Input = \left[\begin{array}{ccc}
%     \rmA&\dots&\zero\\
% \begin{bmatrix}
%     A_{(1,1)}&\dots &A_{(1,d)}\\
%     \zero&\dots&\zero\\
% \end{bmatrix} &\dots &\begin{bmatrix}
%     A_{(d,1)}&\dots &A_{(d,d)}\\
%     \zero&\dots&\zero\\
% \end{bmatrix} \\
%          \emb_{1:d}& \dots &\emb_{1:d} \\
%          \emb_1'& \dots &\emb_{d}' 
%     \end{array}\right].\label{eq:vectorized_matrix} 
% \end{equation}

% \emph{Transposition in the vector form:}
% Once we have the matrix vectorized as the second row block of the scratchpad, the following key and query matrices 
% \begin{align*}
%     \key = \begin{bmatrix}
%         \zero &\zero & \id& \zero\\
%         \zero &\zero & \zero& \id
%     \end{bmatrix}, \query = \begin{bmatrix}
%         \zero &\zero & \zero& \id\\
%         \zero &\zero & \id&\zero
%     \end{bmatrix},  
% \end{align*}
% results in the head outputting the following, which is the vectorized form of $\rmA^\top$ (in the second row block)
% \begin{align*}
%     \Input \softmax((\key \Input)^\top (\query \Input)) = \left[\begin{array}{ccc}
%      *&\dots&*\\
% \begin{bmatrix}
%     A_{(1,1)}&\dots &A_{(d,1)}\\
%     \zero&\dots&\zero\\
% \end{bmatrix} &\dots &\begin{bmatrix}
%     A_{(1,d)}&\dots &A_{(d,d)}\\
%     \zero&\dots&\zero\\
% \end{bmatrix} \\
%          \emb_1'& \dots & \emb_{d}'\\
%          \emb_{1:d}& \dots &\emb_{1:d} 
%     \end{array}\right].
% \end{align*} Then, using the following value matrix gives
% \begin{align*}
%     \val = \begin{bmatrix}
%     \zero&\zero & \zero& \zero\\
%         \zero&\id & \zero& \zero\\
%         \zero&\zero & \zero& \zero\\
%         \zero&\zero & \zero& \zero
%     \end{bmatrix},
% \end{align*}
% \begin{align*}
%   \val \Input \softmax((\key \Input)^\top (\query \Input)) = \left[\begin{array}{ccc}
%   \zero&\dots&\zero\\
% \begin{bmatrix}
%     A_{(1,1)}&\dots &A_{(d,1)}\\
%     \zero&\dots&\zero\\
% \end{bmatrix} &\dots &\begin{bmatrix}
%     A_{(1,d)}&\dots &A_{(d,d)}\\
%     \zero&\dots&\zero\\
% \end{bmatrix} \\
%          \zero& \dots & \zero\\
%          \zero& \dots &\zero 
%     \end{array}\right],
% \end{align*}
% Adding back the $\Input$ (see \eqref{eq:TF}), results in 
% \begin{equation}
%     \Input + \val \Input \softmax((\key \Input)^\top (\query \Input)) = \left[\begin{array}{ccc}
%     \rmA&\dots&\zero\\
% \begin{bmatrix}
%     A_{(1,1)}&\dots &A_{(d,1)}\\
%     \zero&\dots&\zero\\
% \end{bmatrix} &\dots &\begin{bmatrix}
%     A_{(1,d)}&\dots &A_{(d,d)}\\
%     \zero&\dots&\zero\\
% \end{bmatrix} \\
%          \emb_{1:d}& \dots &\emb_{1:d} \\
%          \emb_1'& \dots &\emb_{d}' 
%     \end{array}\right]. \nonumber
% \end{equation}

% Using the feedforward layers and the encodings $\emb_i'$, we get
% \begin{equation}
%     \Input = \left[\begin{array}{ccc}
%     \rmA&\dots&\zero\\
% \begin{bmatrix}
%     A_{(1,1)}&\dots &A_{(d,1)}\\
%     \zero&\dots&\zero
% \end{bmatrix} &\dots &\begin{bmatrix}
%     \zero&\dots&\zero\\
%      A_{(1,d)}&\dots &A_{(d,d)}
% \end{bmatrix}\\
%          \emb_{1:d}& \dots &\emb_{1:d} \\
%          \emb_1'& \dots &\emb_{d}' 
%     \end{array}\right]. \nonumber
% \end{equation}

% Using an attention layer, we get 
% \begin{equation}
%     \Input = \left[\begin{array}{ccc}
% \rmA^\top &\dots &\rmA^\top \\
%         \zero &\dots &\zero \\
%          \emb_{1:d}& \dots &\emb_{1:d} \\
%          \emb_1'& \dots &\emb_{d}' 
%     \end{array}\right]. \nonumber
% \end{equation}
% %  We set $\emb'_{1:d^2}$ to be the encodings $\emb_{d^2+1:d^2+d}$ copied $d$ times. For $\emb^{''}_{1:d^2}$ we use the encodings to do the necessary copy of the column such that in the first $d$ rows we will Now by using the general form of the copy operation we can create 
% % \begin{equation}
% %     \Input = \left[\begin{array}{ccc|c}
% % \rmA &\dots &\rmA &\zero\\
% %         \zero &\dots &\zero & \rmA\\
% %         \zero &\dots & \zero &\emb_{d^2+1:d^2+d}\\
% %          \emb'_{1:d}& \dots &\emb'_{d^-d:d^2} &\zero\\
% %          \emb_{1:d}& \dots &\emb_{d^-d:d^2} &\emb_{d^2+1:d^2+d}
% %     \end{array}\right]
% % \end{equation}



%paragraph{Matrix Multiplication by Linearizing the Softmax.}

In order for matrix multiplication to fit in our unified template, we need to show for example for the result of $\rmA^\top\rmB$ , where $\rmA\in\R^{k\times m}$ and $\rmB\in\R^{k\times n}$ with $k,m,n <d$ we can achieve the following:
\begin{equation}
   \bracks*{  \begin{array}{cc|cc|cc}
        \rmA & \zero &\rmB &\zero &\zero&\zero\\
        \zero& \zero &\zero&\zero&\zero &\zero
    \end{array}}\xrightarrow[]{}\bracks*{ \begin{array}{cc|cc|cc}
        *& *&*&* &\rmA^\top\rmB &*\\
        \zero& \zero &\zero&\zero&\zero &\zero 
    \end{array} }\nonumber
\end{equation}
The idea we leverage is the linearization of the softmax, \ie for a column vector $\vz = [\vx\;, C]$ for some large constant $C$ we have that $$\softmax(\vz)  = [\vx + \eps \;, *]$$
The error $\eps$ is controlled by the constant $C$.
% \begin{equation}
%     \begin{bmatrix}
%         \rmA & \zero%_{(k,d-m)} &\rmB &\zero_{(k,d-n)} &\zero_{(k,d)}\\
%         \zero_{(d-k,m)} & \zero_{(d-k,d-m)} &\zero_{(d-k,n)}&\zero_{(d-k,d-n)}&\zero_{(d-k,d)}
%     \end{bmatrix}\xrightarrow[]{}\begin{bmatrix}
%         \rmA & \zero_{(k,d-m)} &\rmB &\zero_{(k,d-n)} &\zero_{(k,d)}\\
%         \zero_{(d-k,m)} & \zero_{(d-k,d-m)} &\zero_{(d-k,n)}&\zero_{(d-k,d-n)}&\zero_{(d-k,d)}
%     \end{bmatrix}
% \end{equation}
\begin{lemma}\label{lem:matrixmul}
Let $\rmA\in \R^{k\times m}$ and $\rmB \in \R^{k\times n}$; then for any $\epsilon >0$ there exists a transformer-based function block with  2 layers, 1 head and dimensionality $r = O(d)$ that  outputs the multiplication $\rmA^\top\rmB +\eps\rmM$, for some $\norm{\rmM}\leq 1$ .
\end{lemma}
The implementation of $\rmB^\top\rmA$, $\rmA^\top\rmA$ and $\rmB^\top\rmB$ are simple corollaries of the lemma presented above and we will freely use them in the subsequent sections.
In \cref{app:functions}, we provide the exact form of the input $\Input$ for implementing matrix transposition/multiplication,
%(with the encodings needed), 
as well as the proof of the corresponding Lemmas. 
%this and the previous two lemmas can be found in \cref{app:functions}. 


% \begin{corollary}
% Let $\rmA\in k\times m$ and $\rmB \in k\times n$; then there exists a transformer-based function block with 2 layers, 1 head and dimensionality $O(d)$ %two layer transformer-based function block 
% that approximately implements the multiplication $\rmB^T\rmA^T$.
% \end{corollary}
% \begin{corollary}
% Let $\rmA\in k\times m$ and $\rmB \in k\times n$; then there exists a  transformer-based function block  with 2 layers, 1 head and dimensionality $O(d)$, that approximately implements the multiplication $\rmA^T\rmA$.
% \end{corollary}
% \begin{corollary}
% Let $\rmA\in k\times m$ and $\rmB \in k\times n$; then there exists a  transformer-based function block  with 2 layers, 1 head and dimensionality $O(d)$, that approximately implements the multiplication $\rmB^T\rmB$.
% \end{corollary}


% We will prove just the first of these results and the rest are a simple corollary of it.
% \begin{proof}
% Let $\rmM\in \R^{2d\times 2d}$, $\rmA\in\R^{k\times m}$ and $\rmB\in\R^{k\times n}$ be the following matrices:
% \begin{align*}
%     \rmM = \begin{bmatrix}
%         \rmA &\zero&\rmB  &\zero \\
%         \zero&\zero &\zero &\zero
%     \end{bmatrix}.
% \end{align*}
% The zeros pad the rows and columns to ensure that the matrix $M$ is $2d\times 2d$.
% Then, consider the input matrix to be of the following form:
% \begin{equation}
%     \Input = \begin{bmatrix}
%         \rmM& \zero &\zero \\
%         \zero & \rvOne\rvOne^\top &\zero\\
%         \id&\zero &\zero\\ 
%         &\emb^{(1)}&\\
%         &\emb^{(2)}&\\
%         \zero &\rvOne^T &\zero 
%     \end{bmatrix}  \nonumber
% \end{equation} 
%  where $\rvOne\in\R^{2d}$ is the all ones vector. The identity matrix $\id$ and the all ones matrix $\rvOne\rvOne^\top$ are part of the design of the input and they are always fixed. For now we ignore the  encodings and the last row, by setting the corresponding rows of the key,query and value weight matrices to be zero. These rows will be used to copy the output to the  place that we want. %Assuming that we want to output $\rmA^\top\rmA$ these encodings would be 
% % \begin{align}
% % \embed_1&= \begin{bmatrix}
% %     \emb_1 &\cdots &\emb_d & \zero& \cdots &\zero &\zero &\cdots &\zero 
% % \end{bmatrix}\\
% % \embed_2 &= \begin{bmatrix}
% %     \zero &\cdots & \zero &\zero &\cdots&\zero &\emb_{1} &\cdots &\emb_d
% % \end{bmatrix}
% % \end{align}

% Focusing on the rest of the rows, we set the key  and query weight matrices to be 
% \begin{equation}
% \key = \id, \query = \begin{bmatrix}
%      c\id & \zero &\zero\\
%     \zero &\zero &C\id\\
%      \zero & \id &\zero
% \end{bmatrix}, \val = \begin{bmatrix}
% \zero & \zero &\zero\\
% \zero & \zero &ne^C\cD_d\\
% \zero &\zero &\zero
% \end{bmatrix} \nonumber
% \end{equation}
% where $\cD_d\in \R^{2d\times 2d}$ is the diagonal matrix with the first $d$ diagonal elements $1$, and the rest 0.
% %as in \cref{ss:matrixmul} and by repeating the same steps and considering the same transformation $\ell$ we have
% Thus we have
% \begin{align}
%     (\key\Input)^\top\query\Input &= \begin{bmatrix}
%         \rmM& \zero &\zero \\
%         \zero & \rvOne\rvOne^\top &\zero\\
%         \id&\zero &\zero\\
%     \end{bmatrix}^\top \begin{bmatrix}
%         c\rmM & \zero &\zero\\
%         C\id &\zero &\zero\\
%         \zero &\rvOne\rvOne^\top &\zero 
%     \end{bmatrix}\\
%     &= \begin{bmatrix}
%         c\rmM^\top\rmM &\rvOne\rvOne^\top &\zero\\
%         C\rvOne\rvOne^\top &\zero &\zero\\
%         &\zero &\zero &\zero 
%     \end{bmatrix}
% \end{align}
% Each of the first $2d$ columns above looks as follows
% \begin{equation}
%     \begin{bmatrix}
%       cz_{1i} &cz_{2i} &\dots &cz_{ni} & C\rvOne^\top &\zero
%     \end{bmatrix} \nonumber
% \end{equation}
%  After we apply the softmax $\sigma_s$ per column, we get 
%  \begin{equation}
%   \sigma_s(cz_{ij}) = \dfrac{e^{cz_{ij}}}{\sum_{j=1}^n e^{cz_{ij}} + n(e^{C}+1) } \nonumber
% \end{equation}
% where $n=2d$, $z_{ij}$  is the $(i,j)$ element of the matrix $\rmM^\top\rmM$. Let $\ell(\cdot)$ be the transformation above then we have

% \begin{align*} \val\Input\softmax((\key\Input)^\top\query\Input) &= \begin{bmatrix}
%     \zero &\zero &\zero\\
%     ne^C\cD_d &\zero &\zero\\
%     \zero &\zero &\zero 
%     \end{bmatrix}\begin{bmatrix}
%         \ell(c\rmM^\top\rmM) &* &*\\
%         * &* &*\\
%         *&*&*
%     \end{bmatrix}\\
%     &=\begin{bmatrix}
%         \zero &\zero &\zero\\
%         ne^C\cD_d\ell(c\rmM^\top\rmM) &* &*\\
%         \zero &\zero &\zero
%     \end{bmatrix}\\
%     &\approx \begin{bmatrix}
%         \zero &\zero &\zero\\
%         \rvOne\rvOne^\top + c\rmM^\top\rmM &* &*\\
%         \zero &\zero &\zero 
%     \end{bmatrix}
% \end{align*}
% and by adding back the residual we have
% \begin{equation}
%     \Input = \begin{bmatrix}
%         \rmM &\zero &\zero\\
%         \rvOne\rvOne^\top + c\rmM^\top\rmM &* &*\\
%         \id&\zero &\zero 
%     \end{bmatrix} \nonumber
% \end{equation}
% for small enough $c$ and large enough $C$. This is because 
% \begin{align*}
%     ne^C\dfrac{e^{cx_{ij}}}{\sum_{j=1}^n e^{cx_{ij}} + n(e^{C} +1)}  &= e^{cx_{ij}}\dfrac{1}{1+ \sum_{j=1}^ne^{cx_{ij}-C-\log n}+n}  \\
%     &= (1 + cx_{ij} + O((cx_{ij})^2))( 1 - e^{cx_{ij}-C-\log n} + O( e^{2(cx_{ij}-C-\log n)}))\\
%     &= (1 + cx_{ij} + O((cx_{ij})^2))( 1 - e^{cx_{ij}-C-\log n} )\\
%     &\approx (1 + cx_{ij})
% \end{align*}
% We now use the feedforward layers to perform the following transform 
% \begin{align*}
% \Input &= \begin{bmatrix}
% * & * & * \\
%  \rmM^\top\rmM&*&*\\
% * &*  &*
% \end{bmatrix} \\ 
% &= \begin{bmatrix}
%     * & * & *  &* &* \\
%     \rmA^\top \rmA &\zero &\rmA^\top\rmB &\zero & *\\
%     \zero &\zero &\zero &\zero &*\\
%     \rmB^\top\rmA &\zero &\rmB^\top\rmB &\zero&*\\
%     \zero &\zero &\zero &\zero &*\\
%     *&*&*&*&*
% \end{bmatrix}
% \end{align*}
% Now if $\emb^{(1)} = \begin{bmatrix} \zero &\zero & \emb_{2d+1:2d+n}& \zero &\zero  \end{bmatrix}$ and  $\emb^{(2)} = \begin{bmatrix}
% \emb_{1:n} &\emb_{n+1:d} &\zero &\emb_{d+n+1:2d} &\emb_{2d:3d}
% \end{bmatrix}$ we can copy $\rmA^\top\rmB$ to the desired place using \cref{lem:read}.
% % where $\cD_d\in \R^{2d\times 2d}$ is the diagonal matrix with the first $d$ diagonal elements $1$, and the rest 0.
% % Using $*$ to denote inconsequential values, we have:
% % \begin{align}
% % \val\Input\softmax((\key\Input)^\top\query\Input) &= \begin{bmatrix}
% % \zero & \zero &\zero\\
% % \zero & \zero &ne^C\cD_d\\
% % \zero &\zero &\zero
% % \end{bmatrix}\begin{bmatrix}
% %         \rmM& \zero\\
% %         \zero & \rvOne\rvOne^\top\\
% %         \id&\zero
% %     \end{bmatrix}\begin{bmatrix}
% %     \ell(c\rmM^\top\rmM) & *\\
% %        *& *
% %     \end{bmatrix}\\
% %     &= \begin{bmatrix}
% %        \zero & \zero &\zero\\
% % \zero & \zero &ne^C\cD_d\\
% % \zero &\zero &\zero
% %     \end{bmatrix}\begin{bmatrix}
% %         * & *\\
% %        * & *\\
% %        \ell(c\rmA^\top\rmA) &*
% %     \end{bmatrix}\\
% %     &= \begin{bmatrix}
% % \zero & \zero \\
% %  ne^C \cD_d\ell(c\rmA^\top\rmA)&*\\
% % \zero &\zero 
% % \end{bmatrix}\\
% % &\approx 
% % \begin{equation}
% % \begin{bmatrix}
% % \zero & \zero & \zero \\
% % \rvOne\rvOne^\top + c\rmA^\top\rmA&\rvOne\rvOne^\top + c\rmA^\top\rmB&*\\
% % \zero &\zero  &\zero 
% % \end{bmatrix},
% % \end{equation}
% %As we already mentioned we will get
% %Finally, by setting the layernorm parameters to be the diagonal matrix $\mscale$ to have the values $1/c$ in all of the elements, while the bias vector $\bias$ to have the value $-1/c$ everywhere, we get the following output.
% %Finally, the feed forward layers can subtract 1 and scale by $1/c$ to produce the following output:\AG{I used the Layer norm, we need to discuss the open the Relu technique. We should choose one.}
% %\begin{align}
% %\begin{bmatrix}
% %-\rvOne\rvOne^\top/c & -\rvOne\rvOne^\top/c & -\rvOne\rvOne^\top/c \\
% % \rmA^\top\rmA&\rmA^\top\rmB&*\\
% %-\rvOne\rvOne^\top/c &-\rvOne\rvOne^\top/c  &-\rvOne\rvOne^\top/c 
% %\end{bmatrix}
% %\end{align}
% %Then by using the encodings $\embed_1, \embed_2$ and the last line we can get 
% %\begin{equation}
% %    \begin{bmatrix}
% %-\rvOne\rvOne^\top/c & -\rvOne\rvOne^\top/c & -\rvOne\rvOne^\top/c \\
% % \rmA^\top\rmA&\rmA^\top\rmB&*\\
% %-\rvOne\rvOne^\top/c &-\rvOne\rvOne^\top/c  &\rmA^\top\rmA
% %\end{bmatrix}
% %\end{equation}

% % To output $\rmA^\top\rmB$ we will use a different set of encodings as to move in the output position the value $\rmA^\top\rmB$.
% \end{proof}




==> sec/instruction_selection.tex <==
\subsection{Instruction Selection via Attention}


Consider a prompt $\pmt$ where instruction $\s_i$ follows features $\x_i$
\[
\pmt=(\x_i,\s_i)_{i=1}^{n}
\]
Let $\ins$ be an instruction. Define the filtered prompt $\pmt_{\ins}=\flt(\pmt,\ins)$ where 
% \[

% \]
Within this prompt, consider all instances where instruction $\ins$ is used, namely all tuples $(\x_i,\s_i=\ins,\x_{i+1})$. There exists a transformer which admits

==> sec/outline.tex <==
% \paragraph{Outline}
% \begin{itemize}
%     \item \textbf{Setup:}
%     \begin{itemize}
%         \item \textbf{Vanilla CoT}
%         \item \textbf{Skill-based CoT}
%     \end{itemize}
%     \item \textbf{Part 1 (vanilla CoT):}
%     \begin{itemize}
%         \item \textbf{Experiments:} 5-layer neural nets experiments. 
%     \end{itemize}
%     \item \textbf{Part 2 (skill-based CoT):}
%     \begin{itemize}
%         \item \textbf{Experiments:}
%     \end{itemize}
% \end{itemize}
\paragraph{Outline of the paper (tentative)}
\begin{myitemize}
\item \textbf{Section 1:} Experiments and theory on deep neural nets (no instruction ID needed and we can reuse existing experiments since test and training is same)
\begin{myitemize}
\item \textbf{Statistical benefits of CoT: Experiment.} $(x,P_{d'}(g(x)),f(g(x)))$. $d'$ is the dimensionality of features after projection. This interpolates from vanilla ICL to full CoT ICL. Mathematical intuition: Thanks to $d'$ additional equations CoT learns faster by a factor of $O(d')$ (which is clear when $d'=d$).

\item \textbf{Approximation benefits of CoT: Experiment.} In ICL, provide the full DNN features $x1,x2,...,y=xD$. During prediction, train to predict $x1,x2,...xk,xD$ for $k=1$ to $k=D$. At $k=1$ it is regular CoT, at $k=D$ it is one shot prediction.
\begin{myitemize}
    \item We may use approximation aspect to explain distillation power of CoT where we teach a small model recurrence by using chains of a big model.% (needs thinking)
\end{myitemize}
\item \textbf{GSM8K experiments (instead arithmetic, more structured).} On GPT3 or ChatGPT show that more reasoning steps help for CoT to support approximation benefit.
\begin{myitemize}
\item https://paperswithcode.com/dataset/gsm8k
\item https://arxiv.org/abs/2210.00720
\end{myitemize}
\end{myitemize}
\item \textbf{Section 2:} Instruction-based CoT: Main emphasis: Long previously-unseen chains.
\begin{myitemize}
    \item Training involves only basic skills and skill transitions
    \item Test-time prompt can substantially differ from training (i.e.~previously unseen chains)
    \item \textbf{Blackbox reduction:} Show that TF can filter instructions to do ICL learning and TF can deduce next instruction. Combine this to show TF can learn previously-unseen chains.
    \item \textbf{GSM8K experiments.} Select problems whose solution require division operator `/' (or '*'). Contrast 
    \begin{myitemize}
    \item Case 1: In ICL randomly sample examples whose solutions don't contain `/'
    \item Case 2: In ICL randomly sample examples whose solutions do contain `/'
    \item Intuition: In Case 2, the model gets to see `/' operator as well as its transitions. Even if the chain of the problem differs, ICL examples remind it the instruction `/'. Case 2 is similar to active learning.
    \end{myitemize}
\end{myitemize}
\end{myitemize}

==> sec/setup__backup_.tex <==
\section{Problem Setup}
\noindent\textbf{Notation:} Let $\x$ denote the input, $\y$ denote the output, and $\tb=(\tb_1,\dots,\tb_L)$ denote the chain of intermediate thoughts output by \ct. 

\noindent$\bullet$ \textbf{Vanilla \ct with \icl:} Define the $i^{th}$ tuple $\z\n{i}=(\x\n{i},\tb\n{i},\y\n{i})$. ICL admits prompts of the form
\[
\pb=[\z\n{1}~\dots~\z\n{n-1}~\x\n{n}].
\]
Above, the goal is to learn a function sequence $\FF=(f_i)_{i=1}^L$ where each function $f_i$ belongs to a fixed hypothesis set $\Fc_i$. TF will know when to apply which function by index of its current input.\smallskip

% that skill's ID number during \ct
\noindent$\bullet$ \textbf{Skill-based \ct:} Rather than artificially requiring a specific function order, a more realistic setting is \underline{teaching transformer a set of skills} and explicitly instructing TF to apply that skill during \ct demonstrations. This is akin to what happens when an LLM is provided with a math/commonsense reasoning problem and \ct demonstrations reminds the LLM which skills to use.

In this setting, each skill $i$ is associated with a hypothesis set $\Fc_i$ and a distribution $\Dc_i$ over $\Fc_i$. Suppose there are $M$ skills in total. During \icl, we draw $L$ skills denoted by the $L$-dimensional skill indices $\s\in [M]^L$. We also draw $f_i\sim\Dc_i$ for $i\in \Sc$. Declare \ct explanations
\[
\tb=(\s_1,\tb_1,\s_2,\tb_2,\dots,\s_L,\tb_L)
\]
where $\tb_i$ corresponds to the output after applying skill $\s_i$ on $\tb_{i-1}$. The tuples $\z\n{i}$ and \icl prompt is constructed same as before.
%$=(\x\n{i},\tb\n{i},\y\n{i})$. ICL admits prompts of the form

\noindent\textbf{Why skills:} In a nutshell, skill-based setting is more realistic as TF and versatile. Skill-based setting also interpolates between \emph{pure-learning} and \emph{pure-instruction} settings. By this, we mean:
%Perhaps more importantly, s

 \noindent\emph{Pure-learning:} If $\Dc_i$ is a rich continuous distribution, during test time, we need a lot of \icl demonstrations to learn $f_i\in\Fc_i$ associated with the test task. TF can learn a good algorithm from source tasks but it is not enough to identify the rich test function.

 \noindent\emph{Pure-instruction:} Imagine $\Dc_i$ is a singleton! This means all tasks share the exact same function during training or test-time of the TF. Thus, during \icl time, TF can infer the $f_i$ from a single demonstration as it only needs the skill ID to perfectly identify the associated function. In this scenario, the learning cost is only during training time and \icl can one-shot during test-time.

\iffalse
and $\s\in\Sc$ denote skill, where $\Xc,\Sc$ correspond to feature (including input/output) and skill space respectively. Let $\p:=(\x,\s)$ denote an ICL example.



\noindent\textbf{Notation:} Let $\x\in\Xc$ denote the input, $\y\in\Yc$ denote the output, and $\tb=(\tb\n{0},\dots,\tb\n{L})$ denote the chain of intermediate thoughts output by \ct, where $\tb\n{0}=\x,\tb\n{L}=\y$. Let $[n]=\{1,\cdots,n\}$.



Consider a composition function $\y=f_1\circ f_2\dots \circ f_L(\x)$ where $f_\ell\in\Fc_\ell,~\ell\in[L]$. Then we can generate \emph{thought} by $\tb\n{\ell}=f_\ell(\tb\n{\ell-1}),~\ell\in[L]$.

\noindent$\bullet$ \textbf{Vanilla \ct with \icl:} Define the $i$th tuple $\tb_i=(\tb\n{0}_i,\cdots,\tb\n{L}_i)$. ICL admits prompts of the form
\[
\p_i\n{\ell}=[\tb_{1}~\dots~\tb_{i-1}~;\tb_{i}\n{0}~\dots\tb_{i}\n{\ell}].
\]
Above, the goal is to learn a function sequence $\f=(f_\ell)_{\ell=1}^L\in\bFc$ where $\bFc:=\Fc_1\times\dots\Fc_L$. TF will know when to apply which function by index of its current input. Now assume we are given $T$ sequences each containing $n$ chains. Then the objective function is defined as follows.
\begin{align}
    &\widehat\TF=\arg\min\frac{1}{nT}\sum_{t=1}^T\sum_{i=1}^n\Lch_{ti}(\TF)\\
    \text{where}\quad&\Lch_{ti}(\TF)=\frac{1}{L}\sum_{\ell=1}^L\ell\left(\tb_{ti}\n{\ell},\TF(\p_{ti}\n{\ell-1})\right).\nn
\end{align}
% \begin{align}
%     \widehat\TF=\arg\min\frac{1}{nLT}\sum_{t=1}^T\sum_{i=1}^n\sum_{\ell=1}^L\ell\left(\tb_{ti}\n{\ell},\TF(\p_{ti}\n{\ell-1};\tb_{ti}\n{\ell-1})\right).
% \end{align}
\YL{Should the loss function be the same or different for different $\ell\in[L]$}
\begin{align}
    \Rc(\widehat\TF)=\frac{1}{n}\sum_{i=1}^n\E\left[\ell\left(\y,\TF^{\otimes L}(\x)\right)\right],\\
    \text{where}\quad\TF^{\otimes L}(\x):=\underset{\text{Composition of $L$ $\TF$'s.}}{\underbrace{\TF\circ\dots\circ\TF(\x)}}.\nn
\end{align}

\smallskip

% that skill's ID number during \ct
\noindent$\bullet$ \textbf{Skill-based \ct:} Rather than artificially requiring a specific function order, a more realistic setting is \underline{teaching transformer a set of skills} and explicitly instructing TF to apply that skill during \ct demonstrations. This is akin to what happens when an LLM is provided with a math/commonsense reasoning problem and \ct demonstrations reminds the LLM which skills to use.

In this setting, each skill $i$ is associated with a hypothesis set $\Fc_i$ and a distribution $\Dc_i$ over $\Fc_i$. Suppose there are $M$ skills in total. During \icl, we draw $L$ skills denoted by the $L$-dimensional skill indices $\s\in [M]^L$. We also draw $f_i\sim\Dc_i$ for $i\in \Sc$. Declare \ct explanations
\[
\tb=(\tb\n{0},\s\n{1},\tb\n{1},\s\n{2},\tb\n{2},\dots,\s\n{L},\tb\n{L})
\]
where $\tb_i$ corresponds to the output after applying skill $\s_i$ on $\tb_{i-1}$. The tuples $\z\n{i}$ and \icl prompt is constructed same as before.
%$=(\x\n{i},\tb\n{i},\y\n{i})$. ICL admits prompts of the form

\noindent\textbf{Why skills:} In a nutshell, skill-based setting is more realistic as TF and versatile. Skill-based setting also interpolates between \emph{pure-learning} and \emph{pure-instruction} settings. By this, we mean:
%Perhaps more importantly, s

 \noindent\emph{Pure-learning:} If $\Dc_i$ is a rich continuous distribution, during test time, we need a lot of \icl demonstrations to learn $f_i\in\Fc_i$ associated with the test task. TF can learn a good algorithm from source tasks but it is not enough to identify the rich test function.

 \noindent\emph{Pure-instruction:} Imagine $\Dc_i$ is a singleton! This means all tasks share the exact same function during training or test-time of the TF. Thus, during \icl time, TF can infer the $f_i$ from a single demonstration as it only needs the skill ID to perfectly identify the associated function. In this scenario, the learning cost is only during training time and \icl can one-shot during test-time.
 \fi

==> sec/todo.tex <==
\section*{Organization}
\subsection{Introduction}
\subsection{Problem description}
\subsection{Neural nets experiments}
ICL vs Explanation vs CoT
\subsection{ICL with heterogeneous prompts}

\section*{TODO}

\noindent\textbf{Experiments:} 

\textbf{What to test:} 
\begin{itemize}
    \item Sample benefit (more/less ICL), 
    \item Expessivity (small/large GPT), 
    \item How to predict (direct vs multi-step) 
\end{itemize}
\begin{enumerate}
    \item Expressivity (direct vs multi-step): 2-layer neural net: DONE?
    \item \textbf{Priority:} $>2$-layer neural net: Identify a setting with gap btwn 2 vs 3 layer
    \begin{itemize}
        \item Dimensions like 5-5-10-1
        \item diffable act
        \item pretrained subnets
        \item small vs large
    \end{itemize}
    \item Sample benefit: $y=v^Tphi(Wx)$, ICL=> $x, \text{dim-reduce}(phi(Wx)), y$
    \item Unseen chain length (DONE)
    \item Impact of number of subskill
    \begin{itemize}
        \item Make subskill difficult (e.g. noise)
    \end{itemize}
    \item Wrong features in prefix does not impact negative
\end{enumerate}


\noindent\textbf{Theory:} 
\begin{enumerate}
    \item Framing: Learn basic skills and chain them in darkness
    \item Reducing a skill sequence to pure ICL
    \item \textbf{Feature predictions:} A transformer can pick out the skill-specific features and give it to a pure ICL downstream layers
    \item \textbf{Skill predictions:} => If chain is noiseless, SATT can output the correct majority rule
\end{enumerate}

==> sec/zz_statements_construction.tex <==
\subsection{The process of filtering}
The observations made so far are indicative of the model processing each one of the two layers sequentially; an observation we also verify empirically in the subsequent sections. We now demonstrate how a transformer model, can perform a subselection of the data depending on the current prediction to be made. Specifically, assuming that the CoT is performed for $L$ layers and that the model has already made $\ell-1$ predictions we provide the following lemma
\begin{lemma}[Filtering (Informal)]\label{lem:filtering}
    Assume that the input to a transformer model is of the following form
    \renewcommand{\arraystretch}{1.5}
    % \begin{equation}
    %     \arraycolsep=2pt
    %     \X = \left[\begin{array}{cccc|ccccc|ccc}
    %         \x_1 & \tb_1^1 &\dots&\tb^{\ell}_L &\hdots &\tb^{\ell-1}_n &\tb^{\ell}_n &\hdots &\tb_n^{L} &\xtest &\hdots &f^{\ell-1}(\xtest)\\
    %         &&&&&&\zero&&&&&\\
    %        \hline
    %        0 & \hdots &\ell &\ell+1 &\hdots &\ell &\ell+1&\hdots &L &1 &\hdots &\ell\\
    %        1 & \hdots &\ell &\ell+1 &\hdots &\ell &\ell+1&\hdots &L &1 &\hdots &\ell\\
    %         0 & \hdots &0 &0&\hdots &0&0  &\hdots &0&1 &\hdots &1\\
    %         % 1& \hdots &\ell &\hdots &L+\ell+1 &\hdots &n &n+1 &\hdots &N\\
    %         % \ln(1)& \hdots &\ln(\ell) &\hdots &\ln(L+\ell+1) &\hdots &\ln(n) &\ln(n+1) &\hdots &\ln(N)\\
    %        \emb_1 & \hdots &\emb_\ell &\emb_{\ell+1} &\hdots &\emb_{\ell+L+1}& \emb_{\ell+L+2} &\hdots &\emb_n &\emb_{n+1} &\hdots &\emb_{N}
    %     \end{array}\right]
    % \end{equation}
    \begin{equation}
        \arraycolsep=2pt
        \X = \left[\begin{array}{*{12}c}
            \x_1 & \hdots &\tb^{\ell-1}_1&\tb^{\ell}_1 &\hdots &\tb^{\ell-1}_2 &\tb^{\ell}_2 &\hdots &\tb_n^{L} &\x_{\text{\tiny test}} &\hdots &\tb^\ell_{\text{\tiny test}}\\
           \zero &\hdots &\zero &\zero  &\hdots &\zero &\zero&\hdots &\zero &\zero &\hdots &\zero\\
           \hline
           1 & \hdots &\ell &\ell+1 &\hdots &\ell &\ell+1&\hdots &L &1 &\hdots &\ell\\
           1 & \hdots &\ell &\ell+1 &\hdots &\ell &\ell+1&\hdots &L &1 &\hdots &\ell\\
            0 & \hdots &0 &0&\hdots &0&0  &\hdots &0&1 &\hdots &1\\
            % 1& \hdots &\ell &\hdots &L+\ell+1 &\hdots &n &n+1 &\hdots &N\\
            % \ln(1)& \hdots &\ln(\ell) &\hdots &\ln(L+\ell+1) &\hdots &\ln(n) &\ln(n+1) &\hdots &\ln(N)\\
           \emb_0 & \hdots &\emb_{\ell-1} &\emb_{\ell} &\hdots &\emb_{\ell+L}& \emb_{\ell+L+1} &\hdots &\emb_{nL+n-1} &\emb_{nL+n} &\hdots &\emb_{nL+n+\ell}
        \end{array}\right]
    \end{equation}
    where $\X\in\R^{d\times N}$ and $\emb_i$, $i=1,\hdots, N$ are the positional encodings\footnote{The exact form of these encodings is provided to the appendix for ease of exposition. We would like to note however that the follow an oblivious to the ``token-to-be-generated'' pattern.}. 
    Then there exists a transformer $\TF:\R^{d\times N} \to \R^{d\times N}$ consisting of  seven layers with output
    \begin{equation}
    \arraycolsep=2pt
        \TF(\X) = \left[\begin{array}{*{12}c}
           \zero  & \hdots &\tb_1^{\ell}  &\zero  &\hdots &\tb_2^{\ell} &\zero  &\hdots &\zero &\zero &\hdots &\tb^\ell_{\text{\tiny test}}\\
           \zero  & \hdots &\zero &\tb_1^{\ell+1}  &\hdots &\zero &\tb_2^{\ell+1}  &\hdots &\zero &\zero &\hdots &\zero \\
           \hline
* & \hdots &* &* &\hdots &* &*&\hdots &* &* &\hdots &*\\
        \end{array}\right] 
    \end{equation}
    where $*$ denotes inconsequential values. 
\end{lemma}

Some observations are in order.
\begin{remark} 
    The process of filtering can be performed by designing the positional encoding as to be able to extract the information of which token is to be predicted automatically for any token. In other words, the encodings follow a pattern that is oblivious to the ``token-to-be-generated''. 
    Notice that one the current data points and their corresponding labels have been extracted, we can apply previous results on in-context learning gradient descent to perform linear regression (see \cite{giannou2023looped, akyurek2022learning}). For the update of the neural network, assuming that the activation functions are invertible we can use the result of \cite{giannou2023looped} to first invert the labels, then perform the linear regression and finally apply again the activation function. We provide the steps required for such a construction in the appendix.
\end{remark}
\begin{remark}
    When the filtering is performed, there is an $\pm\varepsilon >0$ error at left and right point of the non-zero positions. This error is controlled and can be arbitrarily small. The analysis of the error is given in the Appendix \ref{app:filtering}
\end{remark}
% The operation performed is in essence the operation of filtering. Each one of the five layers performs one of the following steps 
% \begin{enumerate}
%     \item The first layer uses the third line of the input, and created a weighted sum of it. The result would be equal to $k/N$, since there are $k$ ones and the total tokens are $N$.
%     \item The second layer calculates the number of tokens $N$. Notice that this information cannot be directly provided to the input, since for the prediction of the next token we can just append one extra column. Thus, it is not clear how this information can be isolated without the input size being proportional to the number $L$.
%     \item The third layer implements the multiplication and extracts the information regarding the current prediction, \textit{i.e., }$k$.
%     \item In the next layer the number $k$ is subtracted from each one of the elements of the second row presented in the input. 
%     \item The ReLUs of the next layer output one in the second row if the point is zero, and zero otherwise.
%     \item Finally this information is used, to filter the data points through another set of ReLus.
%     \end{enumerate}
% \begin{theorem}
%     In the setting of Lemma \ref{lem:filtering}
% \end{theorem}
